Introduction into Noncommutative Algebra, Volume 1

I dedicated the volume $1$ of monograph 'Introduction into Noncommutative Algebra' to studying of algebra over commutative ring. The main topics that I covered in this volume: definition of module and algebra over commutative ring; linear map of algebra over commutative ring; vector space over associative division algebra; system of linear equations over associative division algebra; homomorphism of vector space over associative division algebra and covariance theory; eigenvalue and eigenvector over associative division algebra.

==> Abelian.Group.Russian.tex <==
%auto-ignore

\input{Abelian.Group.Eq}

\chapter{Абелевая группа}

\section{Группа}

\ShowText{monoid}

Определения мультипликативного и аддитивного моноида
отличаются только формой записи операции.
Поэтому, если выбор операции ясен из контекста,
мы будем соответсвующую алгебру называть моноидом.
Аналогичное замечание верно для групп.
Определения мультипликативной и аддитивной групп
отличаются только формой записи операции.
Поэтому, если выбор операции ясен из контекста,
мы будем соответсвующую алгебру называть группой.
Если не оговоренно противное,
обычно аддитивная группа предполагается абелевой.

\ShowText{inverse in group}

\ShowText{coset in group}

\section{Кольцо}

\begin{\DefinitionStyle}
\labelDefinition{ring}
Пусть на множестве $A$ определены
две бинарные операции\,\footnotemark
\begin{itemize}
\item
сумма
\ShowEq{a,b in A->ab in A (+)}
\item
произведение
\ShowEq{a,b in A->ab in A ()}
\end{itemize}
\StartLabelItem
\begin{enumerate}
\item
\labelItem{A is Abelian additive group}
Множество $A$ является абелевой аддитивной группой
относительно суммы и $0$ - нулевой элемент.
\item
\labelItem{A is multiplicative monoid}
Множество $A$ является мультипликативным моноидом
относительно произведения.
\item
Произведение
\AddIndex{дистрибутивно}{distributive law}
относительно сложения
\ShowEq{a(b+c)=distributive}
\ShowEq{(a+b)c=distributive}
\labelItem{Product is distributive over sum}
\end{enumerate}
Если умножение коммутативно, то кольцо называется коммутативным.
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определения
кольца на странице
\citeBib{Serge Lang}\Hyph 73.
}

\begin{\DefinitionStyle}
Если мультипликативный моноид кольца $D$
содержит единичный элемент $1$,
то кольцо $D$ называется
\AddIndex{унитальным кольцом}{unital ring}.\,\footnotemark
\end{\DefinitionStyle}
\footnotetext{\,
Смотри аналогичное определение на странице
\citeBib{McCrimmon: Jordan Algebras}-52.
}

\begin{\TheoremStyle}
\labelTheorem{0a=0}
Пусть $A$ - кольцо. Тогда
\ShowEq{0a=0}
для любого $A$\Hyph числа $a$.
\end{\TheoremStyle}

\begin{proof}
Равенство
\ShowEq{0a=0 1}
является следствием утверждений
%\RefItem{product has unit element},
\RefItem{A is multiplicative monoid},
\RefItem{Product is distributive over sum}.
Теорема является следствием равенства
\EqRef{0a=0 1},
теоремы
\refTheorem{Unit element of monoid is unique}{+}
и утверждения
\RefItem{unit element (+)}.
\end{proof}

\begin{\TheoremStyle}
Пусть $A$ - кольцо. Тогда
\ShowEq{(-a)b=-ab}
\ShowEq{a(-b)=-ab}
\ShowEq{(-a)(-b)=ab}
для любого $A$\Hyph чисел $a$, $b$.
Если кольцо имеет единичный элемент, то
\ShowEq{(-1)a=-a}
для любого $A$\Hyph числа $a$.
\end{\TheoremStyle}

\begin{proof}
Равенства
\ShowEq{ab+(-a)b=}
\ShowEq{ab+a(-b)=}
являются следствием утверждений
\RefItem{A is Abelian additive group},
\RefItem{Product is distributive over sum}
и равенств
\EqRef{a(a-)=e (+)},
\EqRef{0a=0}.
Равенство
\EqRef{(-a)b=-ab}
является следствием теоремы
\refTheorem{inverse in group is unique}{+}
и равенства
\EqRef{ab+(-a)b=}.
Равенство
\EqRef{a(-b)=-ab}
является следствием теоремы
\refTheorem{inverse in group is unique}{+}
и равенства
\EqRef{ab+a(-b)=}.

Равенство
\ShowEq{(-a)(-b)=}
является следствием равенств
\EqRef{(-a)b=-ab},
\EqRef{a(-b)=-ab}.
Равенство
\EqRef{(-a)(-b)=ab}
является следствием равенств
\EqRef{-(-a)=a (+)},
\EqRef{(-a)(-b)=}.

Если кольцо имеет единичный элемент, то
равенство
\ShowEq{b+(-1)b=}
является следствием утверждений
\RefItem{A is Abelian additive group},
\RefItem{A is multiplicative monoid},
\RefItem{Product is distributive over sum}
и равенств
\EqRef{a(a-)=e (+)},
\EqRef{0a=0}.
\end{proof}

\ShowText{Ring ideal}

\begin{\DefinitionStyle}
Пусть $A$ - коммутативное кольцо.
Если множество
\ShowEq{A'=A-0}
является мультипликативной группой
относительно произведения,
то множество $A$ называется полем.
\end{\DefinitionStyle}

\section{Гомоморфизм групп}

\ShowText{monoid-homomorphism}

\begin{\DefinitionStyle}
\labelDefinition{exact sequence}
Пусть $A_1$, ..., $A_n$ - группы.
Последовательность гомоморфизмов
\ShowEq{A->B->C}
называется
\AddIndex{точной}{exact sequence},
если
\ShowEq{Im f=ker g}
\end{\DefinitionStyle}

\ShowText{0->A->B->C->0}

\section{Базис аддитивной абелевой группы}

\ShowEq{def additive}
\ShowText{basis of group}

\ProveTheorem{ring product Z bilinear}

\ProveTheorem{unit of ring and Z}

\section{Базис мультипликативной абелевой группы}

\ShowEq{def multiplicative}
\ShowText{basis of group}

\section{Свободная абелевая группа}

\ShowText{free Abelian group}

\begin{\TheoremStyle}
Пусть $A$ - абелевый аддитивный моноид.
Рассмотрим категорию $\mathcal K(A)$
гомоморфизмов моноида $A$
в абелевые группы.
Если $B$ и $C$ - абелевые группы,
то для гомоморфизмов
\ShowEq{f:A->B}fAB
\ShowEq{f:A->B}gAC
морфизм категории $\mathcal K(A)$
- это гомоморфизм
\ShowEq{f:A->B}hBC
такой, что диаграмма
\ShowEq{mKA fgh}BCfgh
коммутативна.
Существует абелевая группа
\ShowEq{Grothendieck group}
и универсально отталкивающий гомоморфизм
\ShowEq{f:A->B}{\gamma}A{K(A)}
Группа $K(A)$ называется
\AddIndex{группа Гротендика}{Grothendieck group},
а отображение $\gamma$ называется
\AddIndex{каноническим отображением}{canonical map}.
\end{\TheoremStyle}

\begin{remark}
Согласно определению
\RefDefinition{universally repelling object of category},
если $B$ - абелевая группа и
\ShowEq{f:A->B}fAB
гомоморфизм, то существует единственный гомоморфизм
\ShowEq{f:A->B}g{K(A)}B
такой, что диаграмма
\ShowEq{mKA fgh}{K(A)}C{\gamma}fg
коммутативна.
\hfill\(\odot\)
\end{remark}

\begin{proof}
Пусть $F(A)$ - свободная абелевая группа,
порождённая множеством $A$.
Обозначим $[a]$ образующую группы $F(A)$,
порождённую $A$\Hyph числом $a$.
Пусть $B$ - подгруппа, порождённая всеми
$F(A)$\Hyph числами вида
\ShowEq{(a+b)-()-()}
Положим
\ShowEq{KA=FA/B}
Мы определим гомоморфизм $\gamma$ таким образом,
что следующая диаграмма
\ShowEq{diagram gamma}
коммутативна.
\end{proof}

\begin{\DefinitionStyle}
В аддитивном моноиде $A$ выполняется
\AddIndex{закон сокращения}{cancellation law},
если, для любых $A$\Hyph чисел $a$, $b$, $c$,
из равенства $a+c=b+c$ следует $a=b$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
Если в аддитивном моноиде $A$ выполняется
закон сокращения,
то каноническое отображение
\ShowEq{f:A->B}{\gamma}A{K(A)}
инъективно.
\end{\TheoremStyle}

\begin{proof}
Рассмотрим кортежи
\ShowEq{(ab)A}
Кортеж $(a,b)$ эквивалентен кортежу $(a',b')$, если
\[a+b'=a'+b\]
Мы определим сложение равенством
\[(a,b)+(c,d)=(a+c,b+d)\]
Классы эквивалентности кортежей образуют группу,
нулевым элементом которой является класс кортежа $(0,0)$.
Кортеж $(b,a)$ является противоположным для кортежа $(a,b)$.
Из закона сокращения следует, что гомоморфизм
\def\Class{класс кортежа }
\ShowEq{x->(0,x)}
инъективен.
\end{proof}

\begin{\ExampleStyle}
Определим на множестве чисел
\ShowEq{A=0...}
сложение согласно равенству
\ShowEq{a+b=max}

\begin{lemma}
\labelLemma{a+b=max is commutative}
{\it
Сложение
\EqRef{a+b=max}
коммутативно.
}
\end{lemma}

{\sc Доказательство.}
Лемма является следствием определения
\EqRef{a+b=max}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{a+b=max is associative}
{\it
Сложение
\EqRef{a+b=max}
ассоциативно.
}
\end{lemma}

{\sc Доказательство.}
Для доказательства равенства
\ShowEq{a+(b+c)=(a+b)+c}
достаточно рассмотреть следующие соотношения.
\StartLabelItem
\begin{itemize}
\item
Если 
\ShowEq{a<max bc}
то либо $a\le b$, либо $a\le c$.
\begin{itemize}
\item
Пусть $b\le c$. Тогда
\ShowEq{a+(b+c) 1}
\ShowEq{(a+b)+c 1}
Равенство
\EqRef{a+(b+c)=(a+b)+c}
является следствием равенств
\EqRef{a+(b+c) 1},
\EqRef{(a+b)+c 1}.
\item
Пусть $c\le b$. Тогда
\ShowEq{a+(b+c) 2}
\ShowEq{(a+b)+c 2}
Равенство
\EqRef{a+(b+c)=(a+b)+c}
является следствием равенств
\EqRef{a+(b+c) 2},
\EqRef{(a+b)+c 2}.
\end{itemize}
\item
Если 
\ShowEq{a>max bc}
то
\ShowEq{a>max bc 1}
Следовательно
\ShowEq{a+(b+c) 3}
\ShowEq{(a+b)+c 3}
Равенство
\EqRef{a+(b+c)=(a+b)+c}
является следствием равенств
\EqRef{a+(b+c) 3},
\EqRef{(a+b)+c 3}.
\end{itemize}
Лемма является следствием равенства
\EqRef{a+(b+c)=(a+b)+c}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{a+b=max zero element}
{\it
$A$\Hyph число $0$ является нулевым элементом сложения
\EqRef{a+b=max}.
}
\end{lemma}

{\sc Доказательство.}
Так как
\ShowEq{0<a A}
лемма является следствием определения
\EqRef{a+b=max}.
\hfill\(\odot\)

\begin{\TheoremStyle}
Множество $A$, оснащённое сложением
\EqRef{a+b=max},
является абелевым аддитивным моноидом.
\end{\TheoremStyle}

{\sc Доказательство.}
Теорема является следствием лемм
\ShowEq{ref a+b=max}
и определения
\refDefinition{monoid}{\GroupLbl}.
\hfill\(\odot\)

\begin{\TheoremStyle}
В аддитивном моноиде $A$ закон сокращения
не выполняется.
\end{\TheoremStyle}

{\sc Доказательство.}
Для доказательства теоремы достаточно убедиться, что
\ShowEq{2+9 max}
\ShowEq{4+9 max}
Однако, $2\ne 4$.
\hfill\(\odot\)

\end{\ExampleStyle}


==> Abstract.2207.06506.English.tex <==
%auto-ignore
\begin{abstract}
I dedicated the volume $1$ of monograph
'Introduction into Noncommutative Algebra'
to studying of algebra over commutative ring.
The main topics that I covered in this volume:
\begin{itemize}
\item
definition of module and algebra over commutative ring
\item
linear map of algebra over commutative ring
\item
vector space over associative division algebra
\item
system of linear equations over associative division algebra
\item
homomorphism of vector space over associative division algebra
and covariance theory
\item
eigenvalue and eigenvector over associative division algebra
\end{itemize}
\end{abstract}


==> Abstract.2207.06506.Russian.tex <==
%auto-ignore
\begin{abstract}
Том $1$ монографии
"Введение в некоммутативную алгебру"
посвящён изучению алгебры над коммутативным кольцом.
Основные темы, которые я рассмотрел в этом томе:
\begin{itemize}
\item
определение модуля и алгебры над коммутативным кольцом
\item
линейное отображение алгебры над коммутативным кольцом
\item
векторное пространство над ассоциативной алгеброй с делением
\item
система линейных уравнений над ассоциативной алгеброй с делением
\item
гомоморфизм векторного пространства над ассоциативной алгеброй с делением
и теорию ковариантности
\item
собственное значение и собственный вектор над ассоциативной алгеброй с делением
\end{itemize}
\end{abstract}


==> Algebra.Linear.Map.18.Russian.tex <==
%auto-ignore
\input{Algebra.Linear.Map.18.Eq}

\chapter{Линейное отображение алгебры}
\labelChapter{Linear Map of Algebra}

\section{Линейное отображение \texorpdfstring{$D$}{D}-алгебры}
\labelSection{Linear Map of Algebra}

%\ShowEq{def DModule}
%\ePrints{1502.04063}
%\ifx\Semafor\ValueOff
%\ShowEq{=D1D2}
%исправить d1a1->d2a2
%\ShowDefinition{linear map from A1 to A2, algebra}
%\fi

\ShowEq{=DD}
\ShowDefinition{linear map from A1 to A2, algebra}

\ShowDefinition{polylinear map of algebras}

\ShowTheorem{tensor product of D-algebras is D-algebra}
\begin{proof}
Согласно определению
\RefDefinition{algebra over ring}
и теореме
\RefTheorem{there exists tensor product of modules},
тензорное произведение
$\Tensor A$
$D$\Hyph алгебр
$A_1$, ..., $A_n$
является $D$\Hyph модулем.

Рассмотрим отображение
\ShowEq{xA1n*xA1n->oxA1n}
определённое равенством
\ShowEq{xA1n*xA1n->oxA1n=}
Для заданных значений переменных
$b_1$, ..., $b_n$,
отображение
\EqRef{xA1n*xA1n->oxA1n}
полилинейно по переменным
$a_1$, ..., $a_n$.
Согласно теореме
\RefTheorem{tensor product and polylinear map},
существует линейное отображение
\ShowEq{b:oxA1n->oxA1n}
определённое равенством
\ShowEq{b:oxA1n->oxA1n=}
Так как произвольный тензор
\ShowEq{a in oxA1n}
можно представить в виде суммы тензоров вида
$\Tensor a$,
то для заданного тензора
\ShowEq{a in oxA1n}
отображение
\EqRef{b:oxA1n->oxA1n}
является полилинейным отображением переменных $b_1$, ..., $b_n$.
Согласно теореме
\RefTheorem{tensor product and polylinear map},
существует линейное отображение
\ShowEq{a:oxA1n->oxA1n}
определённое равенством
\ShowEq{a:oxA1n->oxA1n=}
Следовательно, равенство
\EqRef{a:oxA1n->oxA1n=}
определяет билинейное отображение
\ShowEq{oxA1n*oxA1n->oxA1n}
Билинейное отображение
\EqRef{oxA1n*oxA1n->oxA1n}
определяет произведение в $D$\Hyph модуле
$\Tensor A$.
\end{proof}

В случае
тензорного произведения $D$\Hyph алгебр
$A_1$, $A_2$
мы будем рассматривать произведение,
определённое равенством
\ShowEq{A12 2->A12 =}

\begin{theorem}
Пусть $\Basis e_i$ - базис алгебры $A_i$ над кольцом $D$.
Пусть $B_{i\cdot}{}^{\gi j}_{\gi{kl}}$ -
структурные константы алгебры $A_i$ относительно базиса $\Basis e_i$.
Структурные константы тензорного произведение $\Tensor A$
относительно базиса $\TensorBasis i$ имеют вид
\ShowEq{structural constants tensor algebra}
\end{theorem}
\begin{proof}
Непосредственное перемножение тензоров
$\TensorBasis i$ имеет вид
\ShowEq{structural constants tensor algebra, proof, 1}
Согласно определению структурных констант
\ShowEq{structural constants tensor algebra, proof, 2}
Равенство
\EqRef{structural constants tensor algebra}
следует из сравнения
\EqRef{structural constants tensor algebra, proof, 1},
\EqRef{structural constants tensor algebra, proof, 2}.

Из цепочки равенств
\ShowEq{structural constants tensor algebra, proof, 3}
следует, что определение произведения
\EqRef{structural constants tensor algebra, proof, 2}
со структурными константами
\EqRef{structural constants tensor algebra}
согласовано с определением произведения
\EqRef{a:oxA1n->oxA1n=}.
\end{proof}

\begin{theorem}
Для тензоров $a$, $b\in\Tensor A$
стандартные компоненты произведения удовлетворяют равенству
\ShowEq{standard components of product, tensor product}
\end{theorem}
\begin{proof}
Согласно определению
\ShowEq{standard components of product, tensor product, 1}
В тоже время
\ShowEq{standard components of product, tensor product, 2}
Равенство
\EqRef{standard components of product, tensor product}
следует из равенств
\EqRef{standard components of product, tensor product, 1},
\EqRef{standard components of product, tensor product, 2}.
\end{proof}

\begin{theorem}
Если алгебра $A_i$, $i=1$, ..., $n$, ассоциативна,
то тензорное произведение $\Tensor A$ - ассоциативная алгебра.
\end{theorem}
\begin{proof}
Поскольку
\ShowEq{tensor product, associative algebra, 1}
то
\ShowEq{tensor product, associative algebra, 2}
\end{proof}

\begin{theorem}
\labelTheorem{tensor product and product in algebra}
Пусть $A$ -
алгебра над коммутативным кольцом $D$.
Существует линейное отображение
\ShowEq{tensor product and product in algebra}
\end{theorem}
\begin{proof}
Теорема является следствием определения
\RefDefinition{algebra over ring}
и теоремы
\RefTheorem{tensor product and polylinear map}.
\end{proof}

\ShowTheorem{linear map times constant, algebra}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{linear map times constant, 1, algebra}
\end{proof}

\Section{Алгебра \texorpdfstring{$\mathcal L(D;A\rightarrow A)$}{L(D;A->A)}}

\begin{theorem}
\labelTheorem{product of linear map, algebra}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g\circ f$, определённое диаграммой
\ShowEq{product of linear map, algebra}
является линейным отображением из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $C$.
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear map, algebra, 1}
\end{proof}

\begin{theorem}
\labelTheorem{product of linear map, algebra, f}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Отображение $f$ порождает линейное отображение
\ShowEq{product of linear map, algebra, f}
\ShowEq{product of linear map, algebra, f diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\,\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear map, algebra, f1}
\end{proof}

\begin{theorem}
\labelTheorem{product of linear map, algebra, g}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g$ порождает линейное отображение
\ShowEq{product of linear map, algebra, g}
\ShowEq{product of linear map, algebra, g diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\,\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear map, algebra, g1}
\end{proof}

\begin{theorem}
\labelTheorem{product of linear map, algebra, gf}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Отображение
\ShowEq{product of linear map, algebra, gf}
является билинейным отображением.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{product of linear map, algebra, f},
\RefTheorem{product of linear map, algebra, g}.
\end{proof}

\begin{theorem}
\labelTheorem{module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA,
оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{theorem}
\begin{proof}
Теорема является следствием определения
\RefDefinition{algebra over ring}
и теоремы
\RefTheorem{product of linear map, algebra, gf}.
\end{proof}

\section{Линейное отображение в ассоциативную алгебру}

\begin{theorem}
\labelTheorem{bilinear map A LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
отображение
\ShowEq{bilinear map A LA}
является билинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{bilinear map A LA, 1}
\end{proof}

\ShowTheorem{linear map AA LAA}
\begin{proof}
Утверждение теоремы является следствием теорем
\RefTheorem{tensor product and polylinear map},
\RefTheorem{bilinear map A LA}.
\end{proof}

\ShowTheorem{algebra A2 representation in LA}
\begin{proof}
Согласно теореме
\RefTheorem{linear map times constant, algebra},
отображение \EqRef{representation A2 in LA, 1}
является преобразованием модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для данного тензора $c\in \ATwo$
преобразование $h(c)$ является линейным преобразованием
модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
так как
\ShowEq{representation A2 in LA, 2}
Согласно теореме
\RefTheorem{linear map AA LAA},
отображение \EqRef{representation A2 in LA, 1}
является линейным отображением.

Пусть
\ShowEq{algebra A2 representation in LA, 1}
Согласно теореме
\RefTheorem{linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 2}
Следовательно, согласно теореме
\RefTheorem{linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 3}
Поскольку произведение в алгебре $A_2$ ассоциативно, то
\ShowEq{algebra A2 representation in LA, 4}
Следовательно, если мы определим произведение в алгебре $\ATwo$
согласно равенству
\eqRef{product in algebra AA}{A2},
то отображение \EqRef{representation A2 in LA}
является морфизмом алгебр.
Согласно определению
\refDefinition[\RefRepresentation]{side representation of group}{left},
отображение \EqRef{representation A2 in LA, 1}
является представлением алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
\end{proof}

\ShowTheorem{representation of algebra A2 in LA}
\begin{proof}
Согласно теореме
\RefTheorem{linear map AA LAA},
отображение
\ShowEq{f in L(A->B)}DAA{}
и тензор $d\in A\otimes A$
порождают отображение
\ShowEq{tensor and map in A, algebra}
Если мы положим $f=\delta$, $d=a\otimes b$,
то равенство \EqRef{tensor and map in A, algebra}
приобретает вид
\ShowEq{tensor and map in A, 1, algebra}
Если мы положим
\ShowEq{tensor and map in A, 2, algebra}
то сравнение равенств
\EqRef{tensor and map in A, 1, algebra} и
\EqRef{tensor and map in A, 2, algebra}
даёт основание отождествить действие тензора
$a\otimes b$ с
преобразованием $(a\otimes b)\circ\delta$.
\end{proof}

Из теоремы \RefTheorem{representation of algebra A2 in LA}
следует, что отображение
\EqRef{representation A2 in LA, 1}
можно рассматривать как произведение отображений
$a\otimes b$ и $f$.
Тензор $a\in \ATwo$
\AddIndex{невырожден}{nonsingular tensor},
если существует
тензор $b\in \ATwo$ такой, что $a\circ b=1\otimes 1$.

\begin{definition}
\begin{sloppypar}
Рассмотрим\,\footnote{
Определение дано по
аналогии с определением
\RefDefinition[\RefRepresentation]{orbit of left-side representation}.
} представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
\AddIndex{Орбитой линейного отображения}{orbit of linear map}
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
называется множество
\ShowEq{orbit of linear map}
\qed
\end{sloppypar}
\end{definition}

\ShowTheorem{h generated by f, associative algebra}
\begin{proof}
Произвольный тензор $a\in\ATwo$ можно представить в виде
\ShowEq{h generated by f 1, associative algebra}
Согласно теореме \RefTheorem{algebra A2 representation in LA},
отображение \EqRef{representation A2 in LA, 1}
линейно.
Это доказывает утверждение теоремы.
\end{proof}

\begin{\DefinitionStyle}
Выражение
\ShowEq{component a of linear map}
в равенстве
\EqRef{h generated by f, associative algebra}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $h$.
\end{\DefinitionStyle}

\begin{theorem}
\labelTheorem{orbit of linear map}
Пусть $A_2$ - алгебра с единицей $e$.
Пусть
\ShowEq{orbit of linear map, 02}
- невырожденный тензор.
Орбиты линейных отображений
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и \ShowEq{orbit of linear map, 01}
совпадают
\ShowEq{orbit of linear map, f = g}
\end{theorem}
\begin{proof}
Если
\ShowEq{orbit of linear map, 1}
то существует
\ShowEq{orbit of linear map, 2}
такое, что
\ShowEq{orbit of linear map, 3}
Тогда
\ShowEq{orbit of linear map, 4}
Следовательно,
\ShowEq{orbit of linear map, 5}
\ShowEq{orbit of linear map, g in f}

Так как $a$ - невырожденный тензор, то
\ShowEq{orbit of linear map, 6}
Если
\ShowEq{orbit of linear map, 5}
то существует
\ShowEq{orbit of linear map, 2}
такое, что
\ShowEq{orbit of linear map, 7}
Из равенств
\EqRef{orbit of linear map, 6},
\EqRef{orbit of linear map, 7},
следует, что
\ShowEq{orbit of linear map, 8}
Следовательно,
\ShowEq{orbit of linear map, 1}
\ShowEq{orbit of linear map, f in g}

\EqRef{orbit of linear map, f = g}
следует из равенств
\EqRef{orbit of linear map, g in f},
\EqRef{orbit of linear map, f in g}.
\end{proof}

Из теоремы
\RefTheorem{orbit of linear map} также следует, что, если
\ShowEq{orbit of linear map, 01}
и \ShowEq{orbit of linear map, 02}
- вырожденный тензор, то
отношение
\EqRef{orbit of linear map, g in f} верно.
Однако основной результат теоремы
\RefTheorem{orbit of linear map}
состоит в том, что представления алгебры
$\ATwo$ в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает отношение эквивалентности в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Если удачно выбрать представители каждого класса эквивалентности,
то полученное множество будет множеством образующих
рассматриваемого представления.\,\footnote{
Множество образующих
представления определено в определении
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\section{Полилинейное отображение в ассоциативную алгебру}

\begin{theorem}
\labelTheorem{polylinear map A 1n A}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Пусть
\ShowEq{set of maps, L(A;A)}
\ShowEq{set of elements A}
Для заданной перестановки $\sigma$ $n$ переменных
отображение
\ShowEq{n linear map A LA}
является $n$\hyph линейным отображением в алгебру $A$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{polylinear map A 1n A, 1}
\end{proof}

В равенстве \EqRef{n linear map A LA},
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.

\begin{theorem}
\labelTheorem{polylinear map A LA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of maps, L(A;A)}
отображение
\ShowEq{n+1 linear map A LA}
определённое равенством
\ShowEq{n+1 linear map A LA 1}
является $n+1$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{n+1 linear map A LA, 1}
\end{proof}

\begin{theorem}
\labelTheorem{linear map An LAAnA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of maps, L(A;A)}
существует линейное отображение
\ShowEq{linear map An LAAnA}
определённое равенством
\ShowEq{linear map An LAAnA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\RefTheorem{tensor product and polylinear map},
\RefTheorem{polylinear map A LA}.
\end{proof}

\begin{theorem}
\labelTheorem{polylinear map A LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
отображение
\ShowEq{n linear map LA LA}
определённое равенством
\ShowEq{n linear map LA LA 1}
является $n$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{representation An in LAAnA, 3}
\end{proof}

\begin{theorem}
\labelTheorem{linear map LA LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
существует линейное отображение
\ShowEq{linear map LA LA}
определённое равенством
\ShowEq{linear map LA LA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\RefTheorem{tensor product and polylinear map},
\RefTheorem{polylinear map A LA, 1}.
\end{proof}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

%22. A.G. Kurosh, Lectures on General Algebra, Chelsea, New York, 1963

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462.
%
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
%
%
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94, М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Richardson 1928}
{
A. R. Richardson. Simultaneous Linear Equations over a Division Algebra.
Proceedings of the London Mathematical Society.
Volume s2-28, Issue 1, 1928, Pages 395-420.
}%

\BiblioItem{Jacobson. Lie algebras}
{
Джекобсон. Алгебры Ли.
Перевод с английского А. Б. Жижченко
под редакцией А. И. Кострикина.
М., Мир, 1964
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3).
Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{https://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{2110.04354}
{
Dimitri Gurevich, Varvara Petrova, Pavel Saponov,
q-Casimir and q-cut-and-join operators related to Reflection Equation Algebras,
eprint \href{https://arxiv.org/abs/2110.04354}{arXiv:gr-qc/2110.04354} (2021)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem{319-09203}
{
Ralf Schiffler,
Quiver Representations.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\BiblioItem{511-34545}
{
Ibrahim Assem, Daniel Simson, Andrzej Skowro\'nski,\\
Elements of the Representation Theory
of Associative Algebras.
\\
Volume 1: Techniques of Representation Theory.
\\
Cambridge University Press, 2006, ISBN-13: 978-0-511-34545-6
}%

\DefBiblioItem{Rashevsky}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\DefBiblioItem{Korn}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Karthika Viji 2021}
{
S. Karthika, M. Viji,
Unit elements in the path algebra of an acyclic quiver,
Indian J Pure Appl Math\\
Published online: 10 June 2021
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\DefBiblioItem{math.QA-0208146}%

\DefBiblioItem{q-alg-9705026}

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer rule over quaternion skew field,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\DefBiblioItem{0812.4763}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\DefBiblioItem{1302.7204}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1412.5425}
{
Александр Клейн,
Деление в ассоциативной $D$-алгебре,\\
eprint \href{http://arxiv.org/abs/1412.5425}{arXiv:1412.5425} (2014)
}%

\DefBiblioItem{1502.04063}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\DefBiblioItem{1601.03259}%

\DefBiblioItem{1801.01628}

\DefBiblioItem{1908.04418}

\BiblioItem{2020.06.01}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.Russian.pdf)}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Александр Клейн,
Математический анализ над алгеброй кватернионов,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2112.00613}
{
Александр Клейн,
Многочлен в некомутативной алгебре,\\
eprint \href{http://arxiv.org/abs/2112.00613}{arXiv:2112.00613} (2021)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{348311191}
{
Александр Клейн,
Дневник поиска, 2021\\
eprint \href{https://www.researchgate.net/publication/348311191}{RG:348311191} (2021)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\DefBiblioItem{2207.06506}

\BiblioItem{2307.09982}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 2, Модуль над алгеброй\\
eprint \href{http://arxiv.org/abs/2307.09982}{arXiv:2307.09982} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{0767-8264}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй: Экспонента,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{5284-0163}
{
Александр Клейн,
Введение в дифференциальные уранения, банаховая алгебра,\\
Kindle Direct Publishing, 2021;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{8428-0408}
{
Александр Клейн,
Введение в некоммутативную алгебру, Том 1: Алгебра с делением,\\
Kindle Direct Publishing, 2022;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\DefBiblioItem{1812.03397}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\DefBiblioItem{1510.02224}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\DefBiblioItem{Cohn: Skew Fields}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\DefBiblioItem{Sudbery Quaternionic Analysis}%

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{R. Serodio 2001}
{
R. Ser\^odio, E. Pereira, J. Vit\'oria,
Computing the zeros of quaternion polynomials,
Computers \& Mathematics with Applications 42(s 8–9), Pages 1229-1237
}

\BiblioItem{Bulletin AMS 1944 246-248}
{
Samuel Eilenberg, Ivan Niven,
The “fundamental theorem of algebra” for quaternions,
Bulletin of the American Mathematical Society, {\bf 50} (1944), 246-248
}

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Biring.Stmt.Russian.tex <==
%auto-ignore
\input{Biring.Stmt.Eq}

\DefTheorem{transpose of identity}
{
Транспозиция единицы есть единица
\DrawEq{transpose of identity}E
}

\DefProof{transpose of identity}
{
Теорема следует из определений
\RefDefinition{transpose of matrix},
\RefDefinition{biring matrix}.
}

\DefDefinition{biring matrix}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество матриц,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу
\ShowEq{delta n=Matrix}
\end{itemize}
}

\DefLabeledTheorem{product of matrices is distributive over addition}{\Product}
{
\ProductType Произведение матриц
{\bf дистрибутивно}
относительно сложения
\DrawEq{a.\Product.(b1+b2)=}1
\DrawEq{(b1+b2).\Product.a=}1
}

\DefProof{product of matrices is distributive over addition}
{
Равенство
\ShowEq{a.\Product.(b1+b2)= 1}
является следствием равенств
\ShowEq{a.Product.(b1+b2)= 2}
Равенство
\eqRef{a.\Product.(b1+b2)=}1
является следствием равенства
\EqRef{a.\Product.(b1+b2)= 1}.
Равенство
\ShowEq{(b1+b2).\Product.a= 1}
является следствием равенств
\ShowEq{(b1+b2).Product.a= 2}
Равенство
\eqRef{(b1+b2).\Product.a=}1
является следствием равенства
\EqRef{(b1+b2).\Product.a= 1}.
}

\DefSummary{power matrix}
{
Для каждой операции произведения мы определим степень
\ShowEq{show power matrix}
а также обратную матрицу
\ShowEq{show inverse matrix}
}

\DefLabeledDefinition{power matrix}{\ProductS}
{
Мы определим \AddIndex{\ProductType степень}{\ProductS power}
\nTimes матрицы $a$,
пользуясь рекурсивным правилом
\ShowEq{\ProductS power}
\DrawEq{\ProductS power, 0}1
\DrawEq{\Product-power, n}1
}

\AddEq{remark: generalized index structure}
{
Я пользуюсь символом $\cdot$ перед
обобщённым индексом, когда мне необходимо описать его структуру.
Я помещаю символ $'-'$ на месте индекса,
позиция которого изменилась.
Например, если исходное выражение было $\aD a{ij}$,
я пользуюсь записью $a_{\gii\cdot}^{}{}^{\gij}_-$ вместо записи $\aUD aji$.
}

\DefText{range of index}
{
Хотя структура обобщённого индекса произвольна, мы будем предполагать,
что существует взаимно однозначное отображение отрезка натуральных чисел
\ShowEq{gi 1...n}
на множество значений индекса. Пусть $\gi I$ - множество
значений индекса $\gii$. Мы будем обозначать мощность этого множества
символом $|\gi I|$ и будем полагать $|\gi I|=\gin$. Если нам надо
перечислить элементы $\aD ai$, мы будем пользоваться обозначением
\ShowEq{a gi 1...n}
}

\DefText{submatrix}
{
Представление координат вектора в форме матрицы позволяет сделать запись
более компактной. Вопрос о представлении вектора
как строка или столбец матрицы является вопросом соглашения.
Мы можем распространить концепцию обобщённого индекса на элементы матрицы.
Матрица - это двумерная таблица, строки и столбцы которой занумерованы
обобщёнными индексами.
Так как мы пользуемся обобщёнными индексами,
мы не можем сказать, нумерует ли индекс $a$ строки
матрицы или столбцы,
до тех пор, пока мы не знаем структуры индекса.
Однако как мы увидим ниже для нас несущественна форма представления
матрицы.
Для того, чтобы обозначения, предлагаемые ниже,
были согласованы с традиционными,
мы будем предполагать, что матрица представлена в виде
\DrawEq[anm]{a=(a11.nm matrix)}{}
Верхний индекс перечисляет
строки, нижний индекс перечисляет столбцы.
}

\DefDefinition{notation for submatrix}
{
Я использую следующие имена и обозначения различных
\AddIndex{подматриц}{submatrix}
матрицы $a$
\begin{itemize}
\item
\AddIndex{столбец матрицы}{column of matrix}
с индексом $\gii$
\ShowEq{column of matrix}
Верхний индекс перечисляет элементы
столбца, нижний индекс перечисляет столбцы.
\begin{description}
\item
[\ShowEq{A from columns T}\ \ ]
подматрица, полученная из матрицы $a$ выбором
столбцов с индексом из множества $\gi T$
\item [\ShowEq{A without column a}\ \ ]
подматрица, полученный из матрицы $a$ удалением
столбца $\aD ai$
\item [\ShowEq{A without columns T}\ \ ]
подматрица, полученный из матрицы $a$ удалением
столбцов с индексом из множества $\gi T$
\end{description}
\item
\AddIndex{строка матрицы}{row of matrix}
с индексом $\gij$
\ShowEq{row of matrix}
Нижний индекс перечисляет элементы
строки, верхний индекс перечисляет строки.
\begin{description}
\item [\ShowEq{A from rows S}\ \ ]
подматрица, полученный из матрицы $a$ выбором строк с индексом
из множества $\gi S$
\item [\ShowEq{A without row b}\ \ ]
подматрица, полученный из матрицы $a$ удалением
строки $\aU aj$
\item [\ShowEq{A without rows S}\ \ ]
подматрица, полученный из матрицы $a$ удалением строк с индексом
из множества $\gi S$
\end{description}
\end{itemize}
}

\DefText{interval [kl]}
{
Пусть $\gik$, $\gil$, $\gik\le\gil$, - целые числа.
Мы будем рассматривать множество
\ShowEq{interval [kl]}
}

\DefText{Kronecker symbol}
{
Пусть
\ShowEq{I,|I|=n}
- множество индексов.
\AddIndex{Символ Кронекера}{Kronecker symbol}
определён равенством
\ShowEq{Kronecker symbol}
\ShowEq{Kronecker symbol=}
}

\DefRemark{combine the notation of indices}
{
Мы будем комбинировать запись индексов. 
Так \ShowEq{A from b a} является \nTimes[1] подматрицей.
Одновременно, это обозначение элемента матрицы.
Это позволяет отождествить \nTimes[1] матрицу и её элемент.
Индекс $a$ является номером
столбца матрицы и
индекс $b$ является номером строки матрицы.
}

\DefLabeledTheorem{singular matrix and quasideterminant}{\Product}
{
Пусть матрица $a$ - \ProductType вырожденная матрица и подматрица $\SA T$
- \ProductType главная подматрица, тогда
\DrawEq{singular matrix and quasideterminant}{}
}

\DefText{proof of singular matrix and quasideterminant}
{
Чтобы понять, почему подматрица
\DrawEq{singular matrix and quasideterminant, 0}{\Product}
не имеет \ProductType обратной матрицы,\,\footnote{Естественно
ожидать связь между \ProductType вырожденностью матрицы
и её \ProductType квазидетерминантом,
подобную связи, известной в коммутативном случае.
Однако \ProductType квазидетерминант определён не всегда.
Например, если \ProductType обратная матрица имеет слишком много элементов,
равных $0$.
Как следует из этой теоремы, не определён \ProductType квазидетерминант
также в случае, когда \ProductType ранг матрицы меньше $n-1$.}
мы предположим, что существует \ProductType обратная матрица
\ShowEq{B rc-1}
Запишем систему линейных уравнений
\newline
\FrameEqRef{row [J] * col J =0}{\Product}
\newline
\FrameEqRef{row J * col J =E}{\Product}
\newline
полагая
\ShowEq{I= J= \Product}
(в этом случае
\ShowEq{[I]= [J]= \Product})
\DrawEq{singular matrix and quasideterminant, 1}{\Product}
\DrawEq{singular matrix and quasideterminant, 2}{\Product}
и попробуем решить эту систему.
Мы умножим
\eqRef{singular matrix and quasideterminant, 1}{\Product}
на
$\Bf$
\DrawEq{singular matrix and quasideterminant, 3}{\Product}
Теперь мы можем подставить
\eqRef{singular matrix and quasideterminant, 3}{\Product}
в
\eqRef{singular matrix and quasideterminant, 2}{\Product}
\DrawEq{singular matrix and quasideterminant, 4}{\Product}
Из
\eqRef{singular matrix and quasideterminant, 4}{\Product}
следует
\DrawEq{singular matrix and quasideterminant, 5}{\Product}
Равенство
\DrawEq{singular matrix and quasideterminant, 6}{\Product}
является следствием равенства
\newline
\FrameEqRef{j i quasideterminant =}{\Product}
\newline
и равенства
\eqRef{singular matrix and quasideterminant, 5}{\Product}.
Тем самым мы доказали, что квазидетерминант $\Bq$
определён и условие его обращения в $0$ необходимое и достаточное условие
вырожденности матрицы $b$.
}

\DefLabeledTheorem{rank of coordinate matrix}{\Product-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsNA.
Пусть
\ShowEq{set of m vectors}
семейство векторов,
линейно независимых слева. Тогда \ProductType ранг их
координатной матрицы равен $\gim$.
}

\DefProof{rank of coordinate matrix}
{
Пусть \(\Basis e\) - базис  \SideRu вого $A$\Hyph векторного пространства $V$.
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
координатная матрица семейства векторов $(\aU {\Vector a}i)$ относительно базиса $\Basis e$
состоит из \ColsNA, являющихся координатными матрицами векторов
$\aU {\Vector a}i$ относительно базиса $\Basis e$. Поэтому \ProductType ранг
этой матрицы не может превышать $\gim$.

Допустим \ProductType ранг
координатной матрицы меньше $\gim$.
Согласно теореме
\refTheorem{columns of matrix are linearly dependent}{\Product-\Cols},
\ColsRu матрицы линейно зависимы с\SideRu ва
\DrawEq[{\lambda}a]{columns of matrix are linearly dependent}{\Product-\Cols}
Положим
\DrawEq[{\lambda}ac]{c=a rc b}-.
Из равенства
\eqRef{columns of matrix are linearly dependent}{\Product-\Cols}
следует, что \SideRu вая линейная комбинация строк
\DrawEq[c{\Vector e}]{columns of matrix are linearly dependent}{}
векторов базиса равна $0$. Это противоречит утверждению, что векторы $\Vector e$ образуют
базис. Утверждение теоремы доказано.
}

\DefLabeledDefinition{Inverse matrix nm}{\Product-\SideNS}
{
Пусть $a$ - \nmTimes nm матрица
\DrawEq[anm]{a=(a11.nm matrix)}{}
и
\ShowEq{gi k=min nm}
%\ShowEq{gi n<=m \SideNS}
Матрица $a$ называется
\ProductType невырожденной с\SideRu ва,
если существует \nmTimes mn матрица $b$
\DrawEq[bmn]{a=(a11.nm matrix)}{}
такая, что
\ProductType произведение
\DrawEq[bac]{c=a rc b}{Inverse \Product-\SideNS}
содержит подматрицу
\ShowEq{cIJ=Ek}
и остальные элементы матрицы $c$ равны $0$.
Матрица $b$ называется
\SideRu вой \ProductType обратной
матрице $a$.
}

\DefLabeledTheorem{Inverse matrix rank}{\Product-\SideNS}
{
Пусть
\ShowEq{gi k=min nm}
Матрица $a$ имеет
\SideRu вую \ProductType обратную матрицу $b$
тогда и только тогда, когда
\DrawEq[k]{rank a=gi n}{k \Product-\SideNS}
}

\DefProof[5]{Inverse matrix rank}
{
Пусть
\ShowEq{I=[1k]}{#3}
\begin{sloppypar}
Пусть $\gi{#2}$ - множество индексов
линейно независимых с\SideRu ва \RowsRWSA матрицы $a$.
Если $|\gi{#2}|<\gik$,
то мы дополним множество $\gi{#2}$
индексами \ \,оставшихся \RowsRWSA матрицы $a$
таким образом, чтобы получить $|\gi{#2}|=\gik$.
Согласно определению
\ShowEq{ref definition product \Product},
равенство
\end{sloppypar}
\DrawEq[{#2}{#3}]{aI rc bJ=cIJ}{\Product-\SideNS}
является следствием равенства
\newline
\FrameEqRef[bac]{c=a rc b}{Inverse \Product-\SideNS}
\newline
Согласно определениям
\ShowEq{ref definition product \Product},
\refDefinition{Inverse matrix nm}{\Product-\SideNS},
для каждого индекса \jJg {#4}{#3},
система линейных уравнений
\DrawEq[{#1}{#5}{#4}]{linear equations rank \SideNS}{\Product}
является следствием равенства
\eqRef{aI rc bJ=cIJ}{\Product-\SideNS}.
Мы положим,
что неизвестные переменные здесь - это
\ShowEq{xj=bij}{#4}{#5}

Если мы рассмотрим все система линейных уравнений
\eqRef{linear equations rank \SideNS}{\Product},
то их расширенная матрица будет иметь вид
\ShowEq{linear equations for Inverse augmented \Cols}{#1}{#5}
Ранг расширенной матрицы
равен $\gik$.
Согласно теореме
\RefTheorem{star rows system of linear equations},
системы линейных уравнений
\eqRef{linear equations rank \SideNS}{\Product}
имеют решение тогда и только тогда,
когда выполнено условие
\eqRef{rank a=gi n}{k \Product-\SideNS}.
В частности, множество \RowsRWSA
\ShowEq{set vi Acols}a{#5}{#2}
линейно независимо с\SideRu ва.
}

\DefLabeledDefinition[1]{Inverse Matrix set}{\Product-\SideNS}
{
Множество
\ShowEq{set of inverse matrices}{#1}
- это множество
\SideRu вых \ProductType обратных матриц
матрице $a$.
}

\DefLabeledTheorem{a in left = b in right}{\Product}
{
\ShowEq{a in left}ab{\SideNS}{}
тогда и только тогда, когда
\ShowEq{a in left}ba{\OtherSideNS}.
}

\DefProof{a in left = b in right}
{
Теорема является следствием определений
\ShowEq{ref for a in left}
}

\DefLabeledDefinition[4]{divisor of matrix}{\Product-\SideNS}
{
Пусть $a$ - \nmTimes nm матрица
\DrawEq[anm]{a=(a11.nm matrix)}{}
и $c$ - \nmTimes {#1}{#2} матрица
\DrawEq[c{#1}{#2}]{a=(a11.nm matrix)}{}
если существует \nmTimes {#3}{#4} матрица $b$
\DrawEq[b{#3}{#4}]{a=(a11.nm matrix)}{}
такая, что
\DrawEq[abc]{c=a rc b}{}
и остальные элементы равны $0$.
}

\DefLabeledTheorem{quasideterminant and inverse}{\Product}
{
Выражение для \ProductType обратной матрицы имеет вид
\DrawEq{quasideterminant and inverse}{\Product}
\ShowEq{quasideterminant definition= H}
}

\DefProof{quasideterminant and inverse}
{
Равенство
\eqRef{quasideterminant and inverse}{\Product}
следует из равенства
\DrawEq{j i quasideterminant H}{\Product}
}

\DefProof{inverse product of matrix over scalar}
{
Мы докажем равенство
\eqRef{inverse product of matrix over scalar, 1}{\Product}
индукцией по размеру матрицы.

Для \nTimes[1] матрицы
утверждение очевидно, так как
\ShowEq{inverse product of matrix over scalar, 10}

Допустим утверждение справедливо для \nTimes[(n-1)] матрицы. Тогда из равенства
\eqRef{inverse minor}{\Product}
следует
\ShowEq{inverse product of matrix over scalar, 1, 2}
\DrawEq{inverse product of matrix over scalar, 1, 1}{\Product}
Из равенства
\eqRef{inverse product of matrix over scalar, 1, 1}{\Product}
следует равенство
\eqRef{inverse product of matrix over scalar, 1}{\Product}.
Аналогично доказывается равенство
\eqRef{inverse product of matrix over scalar, 2}{\Product}.
}

\DefProof{transpose power}
{
Мы проведём доказательство индукцией по $n$.

\begin{sloppypar}
При $n=0$ утверждение непосредственно следует из равенств
\newline
\FrameEqRef{rc power, 0}1
\newline
\FrameEqRef{cr power, 0}1
\newline
\FrameEqRef{transpose of identity}E
\end{sloppypar}

Допустим утверждение справедливо при $n=k-1$
\DrawEq[{k-1}{}]{transpose power}{k-1 \Product}
Из
\newline
\FrameEqRef{\Product-power, n}1
\newline
следует
\DrawEq{transpose power, 1}{\Product}
Из
\eqRef{transpose power, 1}{\Product}
и
\eqRef{transpose power}{k-1 \Product}
следует
\DrawEq{transpose power, 2}{\Product}
Из
\eqRef{transpose power, 2}{\Product}
и
\eqRef{cr transpose}{Theorem}
следует
\DrawEq{transpose power, 3}{\Product}
Из
\eqRef{transpose power, 1}{\Product}
и
\eqRef{\ProductA-power, n}1
следует
\eqRef{transpose power}{\Product}.
}

\DefLabeledTheorem{transpose inverse}{\Product}
{
Предположим, что \nTimes матрица $a$ имеет \ProductType обратную матрицу.
Тогда транспонированная
матрица $a^T$ имеет \ProductTypeA обратную матрицу и эти
матрицы удовлетворяют равенству
\DrawEq{transpose inverse}{\Product}
}

\DefProof{transpose inverse}
{
Если мы возьмём транспонирование обеих частей
\eqRef{\Product-inverse matrix}1
и применим
\newline
\FrameEqRef{transpose of identity}E
\newline
мы получим
\ShowEq{transpose inverse, 0}
Применяя
\newline
\FrameEqRef{\ProductS transpose}{Theorem}
\newline
мы получим
\DrawEq{transpose inverse, 1}{\Product}
\eqRef{transpose inverse}{\Product} следует из сравнения
\eqRef{cr-inverse matrix}1 и
\eqRef{transpose inverse, 1}{\Product}.
}

\DefLabeledTheorem{inverse unit matrix order 2}{\Product}
{
Пусть
\DrawEq{unit matrix order 2}{\Product}
Тогда
\DrawEq{inverse matrix, unit}{\Product}
}

\DefProof{inverse unit matrix order 2}
{
Из
\eqRef{quasideterminant, matrix 2x2 11}{\Product},
и
\eqRef{quasideterminant, matrix 2x2 22}{\Product}
очевидно, что
\ShowEq{inverse matrix, unit 1 1}
и
\ShowEq{inverse matrix, unit 2 2}
Тем не менее выражение для
\ShowEq{inverse matrix, unit 1 2}
и
\ShowEq{inverse matrix, unit 2 1}
не может быть определено из
\eqRef{quasideterminant, matrix 2x2 12}{\Product}
и
\eqRef{quasideterminant, matrix 2x2 21}{\Product}
так как
\ShowEq{inverse matrix, unit 01}
Мы можем преобразовать эти выражения. Например
\ShowEq{inverse matrix, unit 02}
Мы непосредственно видим, что
\ShowEq{inverse matrix, unit 03}
Таким же образом мы можем найти, что
\ShowEq{inverse matrix, unit 04}
Это завершает доказательство
\eqRef{inverse matrix, unit}{\Product}.
}

\DefLabeledTheorem{quasideterminant, expression}{\Product}
{
Выражение для
\QDef\hyph \ProductType квазидетерминанта
имеет вид
\DrawEq{quasideterminant, expression}{\Product}
}

\DefProof{quasideterminant, expression}
{
Равенство
\eqRef{quasideterminant, expression}{\Product}
является  следствием равенств
\eqRef{inverse matrix, Hadamard}{\Product},
\eqRef{j i quasideterminant =}{\Product}.
}

\DefLabeledTheorem{rdet=a--}{\Product}
{
\DrawEq{rdet=a--}{\Product}
\DrawEq{rdet-=a-}{\Product}
}

\DefProof{rdet=a--}
{
Равенство
\eqRef{rdet=a--}{\Product}
является следствием равенства
\eqRef{j i quasideterminant =}{\Product}.
Равенство
\eqRef{rdet-=a-}{\Product}
является следствием равенства
\eqRef{rdet=a--}{\Product}.
}

\DefLabeledTheorem{quasideterminant, matrix 2x2}{\Product}
{
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Тогда
\DrawEq{quasideterminant, matrix 2x2}{\Product}
\DrawEq{inverse matrix 2x2}{\Product}
}

\DefProof{quasideterminant, matrix 2x2}
{
Согласно равенству
\eqRef{j i quasideterminant =}{\Product}
\DrawEq{quasideterminant, matrix 2x2 11}{\Product}
\DrawEq{quasideterminant, matrix 2x2 21}{\Product}
\DrawEq{quasideterminant, matrix 2x2 12}{\Product}
\DrawEq{quasideterminant, matrix 2x2 22}{\Product}
Равенство
\eqRef{quasideterminant, matrix 2x2}{\Product}
является следствием равенств
\ShowEq{ref quasideterminant matrix}
}

\DefLabeledDefinitionNote{quasideterminant}{\Product}
{
\AddIndex{\QDef\hyph \ProductType квазидетерминант}{j i \Product-quasideterminant}
\nTimes матрицы $a$
- это формальное выражение\,\footnotemark
\ShowEq{j i quasideterminant definition}
\DrawEq{j i quasideterminant =}{\Product}
Мы можем рассматривать \QDef\hyph \ProductType квазидетерминант
как элемент матрицы
\ShowEq{quasideterminant definition}
\DrawEq{quasideterminant definition=}{\Product}
которую мы будем называть
\AddIndex{\ProductType квазидетерминантом}{\Product-quasideterminant}.
}
{
В определении
\refDefinition{quasideterminant}{\Product},
я следую определению
\citeBib{math.QA-0208146}-1.2.2
на странице 9.
}

\DefLabeledTheorem{inverse matrix, Hadamard}{\Product}
{
Предположим, что \nTimes матрица $a$
имеет \RC обратную матрицу.
Тогда элементы \RC обратной матрицы удовлетворяют равенству
\DrawEq{inverse matrix}{\Product}
\DrawEq{inverse matrix, Hadamard}{\Product}
}

\DefProof{inverse matrix, Hadamard}
{
Равенство
\eqRef{inverse matrix}{\Product}
является следствием равенства
\eqRef{inverse minor}{\Product},
если мы положим
\ShowEq{I=i J=j}
Равенство
\eqRef{inverse matrix, Hadamard}{\Product}
является следствием равенств
\EqRef{Hadamard inverse of matrix 2 entry},
\eqRef{inverse matrix}{\Product}.
}

\DefLabeledTheoremNote{inverse minor}{\Product}
{
Предположим, что \nTimes матрица $a$
имеет \ProductType обратную матрицу.\,\footnotemark
Тогда \nTimes[k] подматрица \ProductType обратной матрицы 
удовлетворяет равенству
\DrawEq{inverse minor}{\Product}
\ShowEq{|I|=|J|=k}
}
{
Это утверждение и его доказательство основаны
на утверждении 1.2.1 на странице
\citeBib{math.QA-0208146}\Hyph page 8
для матриц над свободным кольцом с делением.
}

\DefProof{inverse minor}
{
Мы можем записать определение
\newline
\FrameEqRef{\Product-inverse matrix}1
\newline
\ProductType обратной матрицы
следующим образом
\ShowEq{a*a- submatrix, \Product}
Равенство
\ShowEq{a[J]*aJ=0 \Product}
\DrawEq{row [J] * col J =0}{\Product}
и равенство
\ShowEq{aJ*aJ=E \Product}
\DrawEq{row J * col J =E}{\Product}
являются следствием равенства
\EqRef{a*a- submatrix, \Product}
Мы умножим равенство
\eqRef{row [J] * col J =0}{\Product}
на
\ShowEq{minor [I][J] inverse}
\DrawEq{row [J] * col J =0 1}{\Product}
Равенство
\DrawEq{row J * col J =E 1}{\Product}
является следствием равенств
\eqRef{row [J] * col J =0 1}{\Product},
\eqRef{row J * col J =E}{\Product}.
Равенство
\eqRef{inverse minor}{\Product} следует из
\eqRef{row J * col J =E 1}{\Product},
если мы обе части равенства
\eqRef{row J * col J =E 1}{\Product}
умножим на
\ShowEq{minor IJ inverse}
}

\DefLabeledDefinition{singular matrix}{\Product}
{
Если $\gin\times\gin$ матрица $a$ имеет \ProductType обратную матрицу,
мы будем называть такую матрицу
\AddIndex{\ProductType невырожденной матрицей}{\Product nonsingular matrix}.
В противном случае, мы будем называть такую матрицу
\AddIndex{\ProductType вырожденной матрицей}{\Product singular matrix}.
}

\DefLabeledDefinition{inverse matrix}{\Product}
{
Пусть $a$ - \nTimes матрица.
Если существует \nTimes матрица $b$
такая, что
\ShowEq{\Product-inverse matrix 1}
то матрица
\ShowEq{\Product-inverse element}
называется
\AddIndex{\ProductType обратной матрицей}{\Product-inverse matrix}
матрицы $a$
\DrawEq{\Product-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Матрица $a$ называется
\RC невырожденной,
если существует \RC обратная матрица.
\fi
}

\AddEq{theorem: two products equal}
{
\begin{ShadedTheorem}
\labelTheorem{two \Product-products equal}
Если матрица $a$ имеет \ProductType обратную матрицу, то для любых матриц
$b$ и $c$ из равенства
\ShowEq{two \Product-products equal, 1}
следует равенство
\DrawEq{two products equal, 2}{\Product}
\end{ShadedTheorem}
}

\DefProof{two products equal}
{
Равенство \eqRef{two products equal, 2}{\Product} следует из
\EqRef{two \Product-products equal, 1}, если обе части равенства
\EqRef{two \Product-products equal, 1} умножить на
\ShowEq{a-\Product}
}

\DefLabeledTheorem{inverse matrix of product}{\Product}
{
Если \nTimes матрицы $a$, $b$ имеют \ProductType обратную матрицу, то
матрица
\ShowEq{a.\Product.b}
также имеет \ProductType обратную матрицу и
\ShowEq{\Product-inverse matrix of product}
}

\DefProof{inverse matrix of product}
{
Равенство
\ShowEq{\Product.ab b-a-}
является следствием равенства
\newline
\FrameEqRef{\Product-inverse matrix}1
\newline
и определения
\RefDefinition{biring matrix}.
Согласно определению
\refDefinition{inverse matrix}{\Product}
и равенству
\EqRef{\Product.ab b-a-},
матрица
\ShowEq{a.\Product.b}
имеет \ProductType обратную матрицу
\ShowEq{\Product.ab ba-}
Равенство
\EqRef{\Product-inverse matrix of product}
является следствием равенств
\EqRef{\Product.ab b-a-},
\EqRef{\Product.ab ba-}.
}


==> Covariance.Russian.tex <==
%auto-ignore
\input{Covariance.Eq}

\chapter{Многообразие базисов \texorpdfstring{$A$}{A}-векторного пространства}

\ShowEq{def left}
\ShowText{Basis Manifold}

\ShowEq{def right}
\ShowText{Basis Manifold}


==> Covariance.Summary.Russian.tex <==
%auto-ignore
\input{Covariance.Summary.Eq}

\chapter{Ковариантность в \texorpdfstring{$A$}{A}\Hyph векторном пространстве}

\ShowEq{def left}
\section{Геометрический объект в \SideRu вом \texorpdfstring{$A$}{A}\Hyph векторном пространстве}
\ShowEq{Geometric Object of Vector Space}

\ShowEq{def right}
\section{Геометрический объект в \SideRu вом \texorpdfstring{$A$}{A}\Hyph векторном пространстве}
\ShowEq{Geometric Object of Vector Space}

\section{Итоги}

Вопрос как велико разнообразие геометрических объектов
хорошо изучен в случае векторных пространств. Однако он
не столь очевиден в случае
левого или правого $A$\Hyph векторных пространств. Как видно из таблицы
\ref{table:Passive and Active Representations}
левое $A$\Hyph векторное пространство столбцов
и правое $A$\Hyph векторное пространство строк
имеют общую группу симметрии $\CRGL nA$. Это позволяет,
рассматривая пассивное представление в левом $A$\Hyph векторном пространстве столбцов,
изучать геометрический объект в правом $A$\Hyph векторном пространстве строк.
Можем ли мы одновременно
изучать геометрический объект в левом $A$\Hyph векторном пространстве строк?
На первый взгляд, в силу теоремы
\RefTheorem{CR RC singular matrix}
ответ отрицательный. Однако, равенство
\eqRef{rc transpose}{Theorem}
устанавливает искомое линейное отображение между $\RCGL nA$ и $\CRGL nA$.

\begin{table}[h]
\caption{Активное и пассивное представления\\в $A$\Hyph векторном пространстве}
\label{table:Passive and Active Representations}
\begin{tabular}{|c|c|c|c|}
\hline
векторное пространство&группа&активное&пассивное\\
&представления&представление&представление\\
\hline
\ShowEq{table, Passive and Active Representations}
\end{tabular}
\end{table}

\begin{theorem}
\labelTheorem{rcd dcr basis, vector space}
Многообразие базисов левого $A$\Hyph векторного пространства $V$
и многообразие базисов правого $A$\Hyph векторного пространства $V$ отличны
\ShowEq{RCGL En ne En CRGL}
\end{theorem}
\begin{proof}
\,

\ShowProof{rcd dcr basis}

Из лемм
\refLemma{rcd dcr basis}{right},
\refLemma{rcd dcr basis}{left}
следует, что
если множество векторов
\ShowEq{set of vectors f}
порождают базис левого $A$\Hyph векторного пространства столбцов
и базис правого $A$\Hyph векторного пространства столбцов,
то их координатная матрица
\ShowEq{set of vectors f 1}
является \RC невырожденной и \CR невырожденной матрицей.
Утверждение теоремы следует из теоремы
\RefTheorem{CR RC singular matrix}.
\end{proof}


==> D.Algebra.17.Russian.tex <==
%auto-ignore
\input{D.Algebra.17.Eq}

\chapter{\texorpdfstring{$D$}{D}-алгебра}

\section{Алгебра над коммутативным кольцом}

\ShowText{algebra over ring}

\section{Тип \texorpdfstring{$D$}{D}-алгебры}

\ShowText{D-Algebra Type}

\ShowText{product in algebra}

\section{Диаграмма представлений}

\ShowTheorem{endomorphism of module from product}

\ShowTheorem{Free Algebra over Ring}
\ShowProof{Free Algebra over Ring}

\section{Гомоморфизм \texorpdfstring{$D$}{D}-алгебры}

\subsection{Общее определение}

\ShowText{homomorphism of D algebra}1122{h(p)}{h(a)}

\subsection{Гомоморфизм, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{homomorphism of D algebra}{}1{}2pa


==> D.Module.17.Russian.tex <==
%auto-ignore
\input{D.Module.17.Eq}

\chapter{\texorpdfstring{$D$}{D}-модуль}

\section{Модуль над коммутативным кольцом}

\ShowText{Module over Commutative Ring}

\section{Тип \texorpdfstring{$D$}{D}-модуля}

\begin{sloppypar}
\subsection{Концепция обобщённого индекса}

Единственное преимущество выражения
\ShowEq{A linear combination() =}
линейной комбинации векторов
\DrawEq[vV]{v(i) V}{}
- это его универсальность.
Однако для того чтобы наглядней видеть операции над векторами,
удобно группировать координаты вектора в таблицу,
называемую матрицей.
Поэтому вместо аргумента, записанного в скобках,
мы будем пользоваться индексами,
которые говорят как координаты вектора организованы в матрице.
\end{sloppypar}

\ShowText{D-module type}

\ShowText{D-module type 1}

Если рассматривать выражение $\gii$ в записи $v(\gii)$ координат вектора
как обобщённый индекс,
то мы увидим, что поведение вектора не зависит от типа $D$\Hyph модуля.
Мы можем расширить определение обобщённого индекса
и рассматривать индекс $\gii$ в выражении $\aU ai$ как обобщённый индекс.
\ShowRemark{generalized index structure}
Это позволяет записать равенство вида
\ShowEq{b'i=. fb}
Равенство
\EqRef{b'i=. fb}
предполагает равенство индексов
\ShowEq{au i=.-ad k}

\ShowText{range of index}

В геометрии существует традиция записывать координаты вектора
с индексом вверху
\ShowEq{v(i)=vi col}v
и перечислять векторы базиса, используя индекс внизу
\ShowEq{v(i)=vi row}e
Мы также будем пользоваться соглашениеи
\RefConvention{av=sum av convention}.

\ShowConvention{av=sum av convention}

Если мы запишем систему линейных уравнений
\ShowEq{aij xj=0}
пользуясь матрицами
\ShowEq{aij xj=0 matrix}
то мы можем отождествить решение системы линейных уравнений
\EqRef{aij xj=0}
и столбец матрицы.
В тоже время, множество решений системы линейных уравнений
\EqRef{aij xj=0}
является $D$\Hyph модулем.

\subsection{Обозначение элементов матрицы}

\ShowText{Notation for Matrix Entry}

\subsection{\texorpdfstring{$D$}{D}-модуль столбцов}

\ShowEq{\DefCol}
\ShowText{Vector Space Type}

\subsection{\texorpdfstring{$D$}{D}-модуль строк}

\ShowEq{\DefRow}
\ShowText{Vector Space Type}

\section{Линейное отображение \texorpdfstring{$D$}{D}-модуля}

\subsection{Общее определение}

\ShowText{linear map of D module}1122{h(p)}{h(a)}

\ProveTheorem{da in DA->da in D1A}

\ShowConvention{da in DA->da in D1A}

\subsection{Линейное отображение, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{linear map of D module}{}1{}2pa

\begin{\TheoremStyle}
\labelTheorem{linear map, 0, D algebra}
Пусть отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{\TheoremStyle}
\begin{proof}
Следствие равенства
\ShowEq{linear map, 0, D algebra, 1}
\end{proof}

\ShowDefinition{D module, endomorphism}

\section{Полилинейное отображение \texorpdfstring{$D$}{D}-модуля}

\ShowText{Polylinear Map of D-Module}

\section{\texorpdfstring{$D$}{D}-модуль \texorpdfstring{$\mathcal L(D;A\rightarrow B)$}{L(D;A->B)}}

\begin{\TheoremStyle}
\labelTheorem{L(p;L(q;B))=L(p+q;B)}
\ShowEq{L(p;L(q;B))=L(p+q;B)}
\end{\TheoremStyle}
\begin{proof}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{basis h in L(A->D)}
Пусть
\ShowEq{basis e, i in I}
базис $D$\Hyph модуля $A$.
Множество
\ShowEq{basis h in L(A->D)}
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DAD.
\end{\TheoremStyle}
\begin{proof}

\begin{lemma}
\labelLemma{maps hi are linear independent}
{\it
Отображения $h^{\gii}$ линейно независимы.
}
\end{lemma}

{\sc Доказательство.}
Пусть существуют $D$\Hyph числа $c_{\gii}$ такие, что
\ShowEq{ci hi =0}
Тогда для любого $A$\Hyph числа $e_{\gij}$
\ShowEq{cj=0}
Лемма является следствием определения
\refDefinition{linearly independent vectors}{\SideNS}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{map f is linear composition of maps hi}
{\it
Отображение
\ShowEq{f in L(A->D)}
является линейной композицией отображений $h^{\gii}$.
}
\end{lemma}

{\sc Доказательство.}
Для любого $A$\Hyph числа $a$,
\ShowEq{a in basis e}
равенство
\ShowEq{hi a =}
является следствием равенств
\EqRef{basis h in L(A->D)},
\EqRef{a in basis e}
и теоремы
\refTheorem{linear map of D module}1.
Равенство
\ShowEq{f(a)=}
является следствием равенства
\EqRef{hi a =}.
Равенство
\ShowEq{f=...hi}
является следствием равенств
\ShowEq{ref proof basis h in L(A->D)}
\hfill\(\odot\)

Теорема является следствием лемм
\RefLemma{maps hi are linear independent},
\RefLemma{map f is linear composition of maps hi}
и определения
\refDefinition{free module over ring}{\SideNS}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{basis of D-module L(xA->B)}
Пусть $D$ - коммутативное кольцо.
Пусть
\ShowEq{basis e in Ai}
базис $D$\Hyph модуля $A_i$, $i=1$, ..., $n$.
Пусть
\ShowEq{basis e in B}
базис $D$\Hyph модуля $B$.
Множество
\ShowEq{basis h, xA->B}
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B.
\end{\TheoremStyle}
\begin{proof}

\begin{lemma}
\labelLemma{maps hij are linear independent}
{\it
Отображения
\EqParm{hij}{=z}
линейно независимы.
}
\end{lemma}

{\sc Доказательство.}
Пусть существуют $D$\Hyph числа
\ShowEq{cij}
такие, что
\ShowEq{cij hij =0}
Тогда для любого набора индексов
\ShowEq{cij ei=0}
Следовательно,
\ShowEq{cij=0}
Лемма является следствием определения
\refDefinition{linearly independent vectors}{\SideNS}.
\hfill\(\odot\)

\begin{lemma}
\labelLemma{map f is linear composition of maps hij}
{\it
Отображение
\ShowEq{f in L(xA->B)}
является линейной композицией отображений
\EqParm{hij}{=.}
}
\end{lemma}

{\sc Доказательство.}
Для любого $A_1$\Hyph числа $a_1$
\ShowEq{a1 in basis e1}
...,
для любого $A_n$\Hyph числа $a_n$
\ShowEq{an in basis en}
равенство
\ShowEq{hij a =}
является следствием равенств
\EqRef{basis h, xA->B},
\EqRef{a1 in basis e1},
\EqRef{an in basis en}
и теоремы
\refTheorem{linear map of D module}1.
Равенство
\ShowEq{f(a1n)=}
является следствием равенств
\EqRef{a1 in basis e1},
\EqRef{an in basis en}.
Так как
\ShowEq{fe1n in B}
то
\ShowEq{fe1n=}
Равенство
\ShowEq{f(a1n)= 1}
является следствием равенств
\EqRef{hij a =},
\EqRef{f(a1n)=},
\EqRef{fe1n=}.
Равенство
\ShowEq{f=...hij}
является следствием равенств
\ShowEq{ref proof basis h, xA->B}
\hfill\(\odot\)

Теорема является следствием лемм
\RefLemma{maps hij are linear independent},
\RefLemma{map f is linear composition of maps hij}
и определения
\refDefinition{free module over ring}{\SideNS}.
\end{proof}

\ShowTheorem{L(An;B) is free D module}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{basis of D-module L(xA->B)}.
\end{proof}

\section{Тензорное произведение \texorpdfstring{$D$}{D}-модулей}
\labelSection{Tensor Product of Modules}

\begin{\TheoremStyle}
\labelTheorem{commutative ring is Abelian multiplicative Omega group}
Коммутативное кольцо $D$ является
абелевой мультипликативной $\Omega$\Hyph группой.
\end{\TheoremStyle}
\begin{proof}
Мы полагаем, что произведение $\circ$ в кольце $D$
определён согласно правилу
\ShowEq{a circ b=ab}
Так как произведение в кольце дистрибутивно относительно сложения,
теорема является следствием определений
\RefDefinition[\RefRepresentation]{multiplicative Omega group},
\RefDefinition[\RefRepresentation]{Abelian multiplicative Omega group}.
\end{proof}

\ShowTheorem{there exists tensor product of modules}
\begin{proof}
Теорема является следствием определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теорем
\RefTheorem[\RefRepresentation]{tensor product of representations},
\RefTheorem{commutative ring is Abelian multiplicative Omega group}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{\TheoremStyle}
\begin{proof}
Равенство
\EqRef{tensors 1, tensor product}
является следствием равенства
\EqRef[\RefRepresentation]{tensors 1, representation, tensor product}.
Равенство
\EqRef{tensors 2, tensor product}
является следствием равенства
\EqRef[\RefRepresentation]{tensors 2, representation, tensor product}.
\end{proof}

\ShowTheorem{tensor product and polylinear map}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem[\RefRepresentation]{tensor product and polymorphism}{}
и определений
\refDefinition{linear map of D module}1,
\RefDefinition{polylinear map of modules}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem[\RefRepresentation]{B times->B otimes}{}
и определения
\RefDefinition{polylinear map of modules}.
\end{proof}

\ShowTheorem{standard component of tensor, module}
\begin{proof}
Вектор $a_i\in A_i$ имеет разложение
\ShowEq{expansion i relative basis}
относительно базиса $\Basis e_i$.
Из равенств
\EqRef{tensors 1, tensor product},
\EqRef{tensors 2, tensor product}
следует
\ShowEq{expansion i relative basis, 1}
Так как множество тензоров $\Tensor a$
является множеством образующих модуля $\Tensor A$,
то тензор
$a\in\Tensor A$
можно записать в виде
\ShowEq{tensor canonical representation 1}
где
\ShowEq{tensor canonical representation 2}
Положим
\ShowEq{tensor canonical representation 3}
Тогда равенство \EqRef{tensor canonical representation 1}
примет вид
\EqRef{tensor canonical representation, algebra}.

Следовательно, множество тензоров $\TensorBasis i$
является множеством образующих модуля $\Tensor A$.
Так как размерность модуля $A_i$, $i=1$, ..., $n$, конечна,
то конечно множество тензоров $\TensorBasis i$.
Следовательно, множество тензоров $\TensorBasis i$
содержит базис модуля $\Tensor A$, и модуль $\Tensor A$
является свободным модулем над кольцом $D$.
\end{proof}

\section{Прямая сумма \texorpdfstring{$D$}{D}-модулей}

\ShowEq{def DModule}
\ShowEq{def ab=ba}
\ShowText{Direct Sum of Modules}

\ShowTheorem{foa=fi ai}
\begin{proof}
Теорема является следствием определения
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
\end{proof}

\ShowTheorem{foa=fi a}
\begin{proof}
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
\end{proof}

\ShowTheorem{map of direct sum of modules}
\begin{proof}
Согласно теореме
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}1
Согласно теореме
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}1
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}1,
\eqRef{fioa=fij aj}1.
\end{proof}

\ShowRemark{map of direct sum of modules}

\ProveTheorem{direct sum of submodules}

\section{Ядро линейного отображения}

\ShowText{Kernel of Linear Map}


==> Homomorphism.A.Module.Russian.tex <==
%auto-ignore
\ifx\HomomorphismAModule\undefined
\input{Homomorphism.A.Module.Eq}%
\fi

\chapter{Гомоморфизм \SideRu вого \texorpdfstring{$A$}{A}-\VectorSetRuBNS}

\ShowText{homomorphism A module}

\section{Сумма гомоморфизмов \texorpdfstring{$A$}{A}-\VectorSetRuBNS}

\ShowEq{sum of homomorphisms, A vector space}

\section{Произведение гомоморфизмов \texorpdfstring{$A$}{A}-\VectorSetRuBNS}

\ShowEq{product of homomorphisms, A vector space}

\Section{Прямая сумма левых \texorpdfstring{$A$}{A}-векторных пространств}

\ShowEq{def AVector}
\ShowText{Direct Sum of Modules}


==> Homomorphism.Vector.Space.English.tex <==
%auto-ignore
\input{Homomorphism.Vector.Space.Eq}

\chapter{Homomorphism of \SideWSC \texorpdfstring{$A$}{A}-Vector Space}

\ShowText{homomorphism A module}

\section{Sum of Homomorphisms of \texorpdfstring{$A$}{A}-Vector Space}

\ShowEq{sum of homomorphisms, A vector space}

\section{Product of Homomorphisms of \texorpdfstring{$A$}{A}-Vector Space}

\ShowEq{product of homomorphisms, A vector space}


==> Homomorphism.Vector.Space.Eq.tex <==
%auto-ignore

\AddEq{sum of homomorphisms, A vector space}
{
\ShowTheorem{sum of homomorphisms is homomorphism, A vector space}

\ShowProof{sum of homomorphisms is homomorphism, A vector space}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{sum of homomorphisms, A vector space}
\begin{sloppypar}
\ShowProof{sum of homomorphisms, A vector space}
\end{sloppypar}
}
{
\ShowEq{\DefRow}
\ShowTheorem{sum of homomorphisms, A vector space}
\begin{sloppypar}
\ShowProof{sum of homomorphisms, A vector space}
\end{sloppypar}
}
}

\AddEq{product of homomorphisms, A vector space}
{
\ShowTheorem{product of homomorphisms is homomorphism, A vector space}
\ShowProof{product of homomorphisms is homomorphism, A vector space}

\TwoColText
{
\ShowEq{\DefCol}
\ShowTheorem{product of homomorphisms, A vector space}gUVhVW
}
{
\ShowEq{\DefRow}
\ShowTheorem{product of homomorphisms, A vector space}hVWgUV
}

\TwoColText
{
\ShowEq{\DefCol}
\begin{sloppypar}
\ShowProof{product of homomorphisms, A vector space}gh
\end{sloppypar}
}
{
\ShowEq{\DefRow}
\begin{sloppypar}
\ShowProof{product of homomorphisms, A vector space}hg
\end{sloppypar}
}
}


==> Homomorphism.Vector.Space.Russian.tex <==
%auto-ignore
\input{Homomorphism.Vector.Space.Eq}

\chapter{Гомоморфизм \SideRu вого \texorpdfstring{$A$}{A}-векторного пространства}

\ShowText{homomorphism A module}

\section{Сумма гомоморфизмов \texorpdfstring{$A$}{A}-векторного пространства}

\ShowEq{sum of homomorphisms, A vector space}

\section{Произведение гомоморфизмов \texorpdfstring{$A$}{A}-векторного пространства}

\ShowEq{product of homomorphisms, A vector space}


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%15%A%A-векторное пространство
   {$A$\hyph векторное пространство}%
   {A vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%705%C%cr вырожденная матрица
   {\CR вырожденная матрица}%
   {cr singular matrix}%
\Index%954%C%cr квазидетерминант
   {\CR квазидетерминант}%
   {cr-quasideterminant}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%956%C%cr невырожденная матрица
   {\CR невырожденная матрица}%
   {cr nonsingular matrix}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%134%C%cr-обратная матрица
   {\CR обратная матрица}%
   {cr-inverse matrix}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i rc-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%rc вырожденная матрица
   {\RC вырожденная матрица}%
   {rc singular matrix}%
\Index%62%R%rc квазидетерминант
   {\RC квазидетерминант}%
   {rc-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%rc невырожденная матрица
   {\RC невырожденная матрица}%
   {r? nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%218%R%rc-обратная матрица
   {\RC обратная матрица}%
   {rc-inverse matrix}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%976%В%векторное подпространство
   {векторное подпространство}%
   {subspace}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%61%Г%главная подматрица
   {главная подматрица}%
   {major submatrix}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%959%Г%гомоморфизм векторного пространства
   {гомоморфизм векторного пространства}%
   {homomorphism of vector space}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%964%З%закон коммутативности
   {закон коммутативности}%
   {commutative law}%
\Index%701%З%закон сокращения
   {закон сокращения}%
   {cancellation law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%971%И%идеал
   {идеал}%
   {ideal}%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%438%И%интегрируемая дифференциальная форма
   {интегрируемая дифференциальная форма}%
   {integrable differential form}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%368%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%913%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%535%К%квазибазис
   {квазибазис}%
   {quasibasis}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%258%К%колинеарные векторы
   {колинеарные векторы}%
   {colinear vectors}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%974%К%координаты гомоморфизма
   {координаты гомоморфизма}%
   {coordinates of homomorphism}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация
   {левая линейная комбинация}%
   {left linear combination}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%975%Л%левый идеал
   {левый идеал}%
   {left ideal}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%973%Л%левый смежный класс
   {левый смежный класс}%
   {left coset}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%136%Л%линейно зависимы слева
   {линейно зависимы слева}%
   {left linear dependent}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%255%М%матрица Вронского
   {матрица Вронского}%
   {Wronskian matrix}%
\Index%958%М%матрица гомоморфизма
   {матрица гомоморфизма}%
   {matrix of homomorphism}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система линейных уравнений
   {невырожденная система линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%219%Н%невырожденная система правых AU* линейных уравнений
   {невырожденная система правых $A^*$\Hyph линейных уравнений}%
   {nonsingular system of right AU* linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%960%Н%непрерывный базис Шаудера
   {непрерывный базис Шаудера}%
   {continuous Schauder basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%702%Н%нормальная подгруппа
   {нормальная подгруппа}%
   {normal subgroup}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%970%О%образ отображения
   {образ отображения}%
   {image of map}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен
   {однородный многочлен}%
   {homogeneous polynomial}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%212%О%определитель Вронского
   {определитель Вронского}%
   {Wronskian determinant}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное G-представление
   {пассивное $G$\Hyph представление}%
   {passive G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation, vector space}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%963%П%первый интеграл
   {первый интеграл}%
   {first integral}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация
   {правая линейная комбинация}%
   {right linear combination}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%912%П%правый идеал
   {правый идеал}%
   {right ideal}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%704%П%правый смежный класс
   {правый смежный класс}%
   {right coset}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%719%П%преобразование подобия
   {преобразование подобия}%
   {similarity transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%384%П%принцип ковариантности
   {принцип ковариантности}%
   {principle of covariance}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%133%П%произведение гомоморфизмов
   {произведение гомоморфизмов}%
   {product of homomorphisms}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%67%Р%ранг матрицы
   {ранг матрицы}%
   {rank of matrix}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица
   {расширенная матрица}%
   {augmented matrix}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%220%С%система левых AD* линейных уравнений
   {система левых $A_*$\Hyph линейных уравнений}%
   {system of left AD* linear equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%721%С%система правых AU* линейных уравнений
   {система правых $A^*$\Hyph линейных уравнений}%
   {system of right AU* linear equations}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%965%С%собственная строка
   {собственная строка}%
   {eigenrow}%
\Index%946%С%собственное значение
   {собственное значение}%
   {eigenvalue}%
\Index%966%С%собственный вектор
   {собственный вектор}%
   {eigenvector}%
\Index%947%С%собственный столбец
   {собственный столбец}%
   {eigencolumn}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%135%Т%тип геометрического объекта
   {тип геометрического объекта}%
   {type of geometric object}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%724%Т%точная последовательность
   {точная последовательность}%
   {exact sequence}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\Index%972%Т%тривиальное ядро гомоморфизма
   {тривиальное ядро гомоморфизма}%
   {trivial kernel}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%132%У%унитальная алгебра
   {унитальная алгебра}%
   {unital algebra}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%369%Ф%факторгруппа
   {факторгруппа}%
   {factor group}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%722%Ц%центр A числа
   {центр $A$\Hyph числа}%
   {center of A number}%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Left.Eigen.Russian.tex <==
%auto-ignore
%\input{Left.Eigen.Eq}

\chapter{Левые и правые собственные значения}

Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.

\section{Левые и правые \texorpdfstring{\RC}{rc-}собственные значения}

\ShowEq{def left}
\def\LeftText{\DefRow}
\ShowEq{def right}
\def\RightText{\DefCol}
\ShowEq{Left and Right Eigenvalues 1}{rc}

\section{Левые и правые \texorpdfstring{\CR}{cr-}собственные значения}

\ShowEq{def left}
\def\LeftText{\DefCol}
\ShowEq{def right}
\def\RightText{\DefRow}
\ShowEq{Left and Right Eigenvalues 1}{cr}

\section{Проблема обратной теоремы}

\begin{\QuestionStyle}
\labelQuestion{Is rc eigenvalue a left rc eigenvalue}
\ShowEq{def right}%
\ShowEq{\DefCol}%
Из теоремы\,\footnotemark
\refTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}
следует, что
любое \SideRu вое \ProductType собственное значение $d(\gi i)$
является \ProductType собственным значением.
Верна ли обратная теорема, а именно,
является ли \ProductType собственное значение
\SideRu вым \ProductType собственным значением?
\end{\QuestionStyle}
\footnotetext{\,
Подобные рассуждения верны для
\OtherSideRu вого \ProductType собственного значения,
\ShowEq{def left}%
\ShowEq{\DefCol}%
а также для левого и правого \ProductType собственного значения.
}

\ShowEq{def right}%
\ShowEq{\DefCol}%
Получить ответ на вопрос
\RefQuestion{Is rc eigenvalue a left rc eigenvalue},
вообще говоря, непросто.
Что произойдёт, если кратность \ProductType собственного значения
будет больше $1$?
Может ли \nTimes матрица иметь меньше чем $\gin$ собственных значений
с учётом кратности?

Может показаться, что, если \nTimes матрица имеет $\gin$ собственных значений
кратности $1$, то это самый простой случай.
Если \nTimes матрица с элементами из коммутативной алгебры имеет $\gin$ собственных значений
кратности $1$, то множество собственных векторов является базисом
векторного пространства размерности $\gin$.
Однако это утверждение неверно, если элементы матрицы
принадлежать некоммутативной алгебре.

Расмотрим теорему
\refTheorem{n eigenvectors}{algebra}.

\ShowEq{prove n eigenvectors}

\ShowEq{Left and Right Eigenvalues not equal}

\section{Собственное значение матрицы линейного отображения}

Пусть
\DrawEq{a=matrix of maps n x n}{}
матрица линейного отображения
\ShowEq{f:A->B}{\Vector a}VV
$A$\Hyph векторного пространства $V$.

\subsection{\texorpdfstring{$\RCcirc$}{rco}-собственное значение матрицы линейного отображения}\,

\def\DefMatrix{\DefCol}
\AddIndex{}{eigencolumn}
\ShowEq{Eigenvalue of Matrix of Linear Map}

\subsection{\texorpdfstring{$\CRcirc$}{cro}-собственное значение матрицы линейного отображения}\,

\def\DefMatrix{\DefRow}
\AddIndex{}{eigenrow}
\ShowEq{Eigenvalue of Matrix of Linear Map}


==> Linear.A.Vector.Space.Russian.tex <==
%auto-ignore
%\ifx\LinearAModule\undefined
%\input{Linear.Vector.Space.Eq}
%\fi

\chapter{Линейное отображение \SideRu вого \texorpdfstring{$A$}{A}-векторного пространства}

\ShowText{Coordinates of Linear Map}

%\section{Ядро линейного отображения}

%\ShowText{Kernel of A Linear Map}


==> Linear.System.Star.Russian.tex <==
%auto-ignore
\input{Linear.System.Star.Eq}

\chapter{Система линейных уравнений в
\texorpdfstring{$A$}{A}-векторном пространстве}

\section{Линейная оболочка в левом
\texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{def left}
\ShowEq{\DefCol}
\ShowText{linear span, vector space}

\ShowEq{\DefRow}
\ShowText{linear span, vector space}

\section{Линейная оболочка в правом
\texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{def right}
\ShowEq{\DefCol}
\ShowText{linear span, vector space}

\ShowEq{\DefRow}
\ShowText{linear span, vector space}

\section{Ранг матрицы}
\labelSection{Rank of Matrix}

Мы делаем следующие предположения в этом разделе
\begin{itemize}
\ShowEq{Rank of Matrix assumption 1}
\ShowEq{Rank of Matrix assumption 2}
- произвольная матрица.
\ShowEq{Rank of Matrix assumption 3 4}
\end{itemize}

Матрица $\SA T$ является \AxA k матрицей.

\ShowText{rank of matrix}

\section{Система линейных уравнений
\ShowEq{a rc x=b pdf}
}

\begin{ShadedDefinition}
Предположим, что
$a$ - матрица системы левых линейных уравнений
\ShowEq{def left}
\ShowEq{\DefRow}
\DrawEq{a*x=b \SideNS}{augmented matrix \Cols}
Мы будем называть матрицу
\ShowEq{augmented matrix, system of drc linear equations}
\AddIndex{расширенной матрицей}{augmented matrix}
системы левых линейных уравнений
\eqRef{a*x=b \SideNS}{augmented matrix \Cols}.
\end{ShadedDefinition}

\begin{ShadedDefinition}
Предположим, что
$a$ - матрица системы правых линейных уравнений
\DrawEq{star rows system of linear equations 2}{2a}
Мы будем называть матрицу
\ShowEq{augmented matrix, system of rcd linear equations}
\AddIndex{расширенной матрицей}{augmented matrix}
системы правых линейных уравнений
\eqRef{star rows system of linear equations 2}{2a}.
\end{ShadedDefinition}

\begin{ShadedTheorem}
\labelTheorem{star rows system of linear equations}
Система правых линейных уравнений
\eqRef{star rows system of linear equations 2}{2a}
имеет решение тогда и только тогда, когда
\ShowEq{star rows system of linear equations, rank}
\end{ShadedTheorem}
\begin{proof}
Пусть $\SA T$ - \RC главная подматрица матрицы $a$.

Пусть система правых линейных уравнений \eqRef{star rows system of linear equations 2}{2a}
имеет решение
\ShowEq{star rows system of linear equations, solution}
Тогда
\DrawEq[d]{nonsingular system of linear equations}d
Уравнение \eqRef{nonsingular system of linear equations}d может быть записано в форме
\ShowEq{star rows system of linear equations, 2}
Подставляя
\EqRef{rank of matrix, rc-cols}
в
\EqRef{star rows system of linear equations, 2}, мы получим
\ShowEq{star rows system of linear equations, 3}
Из \EqRef{star rows system of linear equations, 3} следует, что $A$\Hyph столбец
$b$ является \rcd линейной комбинацией $A$\Hyph столбцов $\aD aT$
\ShowEq{star rows system of linear equations, 4}
Это эквивалентно уравнению \EqRef{star rows system of linear equations, rank}.

Нам осталось доказать, что существование решения системы правых линейных уравнений
\eqRef{star rows system of linear equations 2}{2a} следует из
\EqRef{star rows system of linear equations, rank}.
Истинность \EqRef{star rows system of linear equations, rank} означает, что
$\SA T$ - так же \RC главная подматрица расширенной матрицы.
Из теоремы
\refTheorem{rank of matrix}{rc-cols}
следует, что столбец $b$
является правой линейной композицией столбцов $\aD aT$
\ShowEq{star rows system of linear equations, 5}
Полагая
\ShowEq{star rows system of linear equations, 6},
мы получим
\ShowEq{star rows system of linear equations, 7}
Следовательно, мы нашли, по крайней мере, одно решение системы правых линейных уравнений
\eqRef{star rows system of linear equations 2}{2a}.
\end{proof}

\begin{ShadedTheorem}
\labelTheorem{star rows system of linear equations, solution}
Предположим, что \eqRef{star rows system of linear equations 2}{2a}
- система правых линейных уравнений,
удовлетворяющих \EqRef{star rows system of linear equations, rank}.
Если
\ShowEq{rank=k<m}
то решение системы зависит
от произвольных значений $\gim-\gik$ переменных,
не включённых в \RC главную подматрицу.
\end{ShadedTheorem}
\begin{proof}
Пусть $\SA T$ - \RC главная подматрица матрицы $a$.
Предположим, что
\ShowEq{star rows system of linear equations, reduce, 1}
уравнение с номером $\gi p$.
Применяя теорему
\refTheorem{rank of matrix}{rc-rows}
к расширенной матрице
\EqRef{augmented matrix, system of drc linear equations},
мы получим
\ShowEq{star rows system of linear equations, reduce, 2}
\ShowEq{star rows system of linear equations, reduce, 3}
Подставляя \EqRef{star rows system of linear equations, reduce, 2}
и \EqRef{star rows system of linear equations, reduce, 3}
в \EqRef{star rows system of linear equations, reduce, 1}, мы получим
\ShowEq{star rows system of linear equations, reduce, 4}
\EqRef{star rows system of linear equations, reduce, 4} означает, что
мы можем исключить уравнение \EqRef{star rows system of linear equations, reduce, 1}
из системы \eqRef{star rows system of linear equations 2}{2a}
и новая система эквивалентна старой.
Следовательно, число уравнений может быть уменьшено до $\gik$.

В этом случае
у нас есть два варианта. Если число переменных также равно $\gik$, то
согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols}
система имеет единственное решение
\newline
\FrameEqRef{x=a-*b, quasideterminant \SideNS}{\Cols}
\newline
Если число переменных $\gim>\gik$, то мы можем передвинуть $\gim-\gik$ переменных, которые не
включены в \RC главную подматрицу в правой части.
Присваивая произвольные значения этим переменным, мы определяем значение
правой части и для этого значения мы получим единственное решение
согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols}.
\end{proof}

\begin{ShadedCorollary}
\labelCorollary{ nonsingular rows system of linear equations}
Система правых линейных уравнений \eqRef{star rows system of linear equations 2}{2a}
имеет единственное решение тогда и только тогда, когда
её матрица невырожденная.
\end{ShadedCorollary}

\begin{ShadedTheorem}
\labelTheorem{Solutions homogenous system of linear equations}
Решения однородной системы правых линейных уравнений
\ShowEq{homogenous system of linear equations}
порождают правое $A$\Hyph векторное пространство столбцов.
\end{ShadedTheorem}
\begin{proof}
Пусть $X$ - множество решений системы правых $A$\Hyph линейных уравнений
\EqRef{homogenous system of linear equations}.
Предположим, что
\ShowEq{homogenous system of linear equations x}x
и
\ShowEq{homogenous system of linear equations x}y
Тогда
\ShowEq{aab xa=0}x
\ShowEq{aab xa=0}y
Следовательно,
\ShowEq{homogenous system of linear equations x+y}
Таким же образом мы видим
\ShowEq{homogenous system of linear equations xb}
Согласно определению
\ShowEq{def AVector}%
\ShowEq{def right}%
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS},
$X$ является правым $A$\Hyph векторным пространством столбцов.
\end{proof}

\section{Невырожденная матрица}

Предположим, что нам дана
\nTimes
матрица $a$.
Теоремы
\refTheorem{columns of matrix are linearly dependent}{rc-rows}
и
\refTheorem{columns of matrix are linearly dependent}{rc-cols}
говорят нам, что если
\ShowEq{rc rank<n},
то строки линейно зависимы слева
и столбцы линейно зависимы справа.\,\footnote{Это
утверждение похоже на утверждение
\citeBib{q-alg-9705026}-\href{http://arxiv.org/PS_cache/q-alg/pdf/9705/9705026.pdf\#Page=6}{1.2.5}.}

\begin{ShadedTheorem}
\labelTheorem{rc rank, columns}
Пусть $a$ -
\nTimes
матрица
и столбец $\aD ar$ - левая линейная комбинация других столбцов.
Тогда
\ShowEq{rc rank<n}.
\end{ShadedTheorem}
\begin{proof}
Утверждение, что столбец $\aD ar$ является правой линейной комбинацией других столбцов,
означает, что система линейных уравнений
\ShowEq{rc rank, columns}
имеет, по крайней мере, одно решение.
Согласно теореме
\RefTheorem{star rows system of linear equations}
\ShowEq{rc rank, columns 1}
Так как число столбцов меньше, чем $\gin$, то
\ShowEq{rc rank, columns 2}
\end{proof}

\begin{ShadedTheorem}
\labelTheorem{rc rank, rows}
Пусть $a$ -
\nTimes
матрица
и строка $\aU ap$ - правая линейная комбинация других строк.
Тогда
\ShowEq{rc rank<n}.
\end{ShadedTheorem}
\begin{proof}
Доказательство утверждения похоже на доказательство теоремы
\RefTheorem{rc rank, columns}.
\end{proof}

\begin{ShadedTheorem}
Предположим, что $a$ и $b$ -
\nTimes
матрицы и
\ShowEq{RC product singular, 1}
$c$ - \RC вырожденная матрица тогда и только тогда, когда
либо матрица $a$, либо матрица $b$ - \RC вырожденная матрица.
\end{ShadedTheorem}
\begin{proof}
Предположим, что матрица $b$ - \RC вырожденная.
Согласно теореме
\refTheorem{rank of matrix}{rc-cols}
столбцы матрицы $b$
линейно зависимы справа. Следовательно,
\ShowEq{RC product singular, 2}
где $\lambda\ne 0$. Из
\EqRef{RC product singular, 1}
и \EqRef{RC product singular, 2} следует, что
\ShowEq{RC product singular, 3}
Согласно теореме
\RefTheorem{rc rank, columns}
матрица $c$ является \RC вырожденной.

Предположим, что матрица $b$ - не \RC вырожденная, но матрица $a$ - \RC вырожденная.
Согласно теореме
\refTheorem{rank of matrix}{rc-rows},
столбцы матрицы $a$
линейно зависимы справа. Следовательно,
\ShowEq{RC product singular, 4}
где $\mu\ne 0$. Согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols},
система линейных уравнений
\ShowEq{RC product singular, 5}
имеет единственное решение, где $\lambda\ne 0$.
Следовательно,
\ShowEq{RC product singular, 6}
Согласно теореме
\RefTheorem{rc rank, columns}
матрица $c$ является \RC вырожденной.

Предположим, что матрица $c$ - \RC вырожденная матрица.
Согласно теореме
\refTheorem{rank of matrix}{rc-rows}
столбцы матрицы $c$
линейно зависимы справа. Следовательно,
\ShowEq{RC product singular, 7}
где $\lambda\ne 0$.
Из \EqRef{RC product singular, 1}
и \EqRef{RC product singular, 7} следует, что
\ShowEq{RC product singular, 8}
Если 
\ShowEq{RC product singular, 9}
выполнено, то матрица $b$ - \RC вырожденная. Предположим, что
матрица $b$ не \RC вырожденная. Положим
\ShowEq{RC product singular, 10}
где $\mu\ne 0$. Тогда
\ShowEq{RC product singular, 11}
Из \EqRef{RC product singular, 11} следует, что
матрица $a$ - \RC вырожденная.
\end{proof}

Согласно теореме
\RefTheorem{duality principle, quasideterminants},
мы можем записать подобные утверждения для левой линейной комбинации строк
или правой линейной комбинации столбцов и \CR квазидетерминанта.

\begin{ShadedTheorem}
\labelTheorem{cr rank, rows}
Пусть $a$ -
\nTimes
матрица
и столбец $\aD ar$ - правая линейная комбинация других столбцов.
Тогда
\ShowEq{cr rank<n}.
\qed
\end{ShadedTheorem}

\begin{ShadedTheorem}
\labelTheorem{cr rank, columns}
Пусть $a$ -
\nTimes
матрица
и строка $\aU ap$ - левая линейная комбинация других строк.
Тогда
\ShowEq{cr rank<n}.
\qed
\end{ShadedTheorem}

\begin{ShadedTheorem}
Предположим, что $a$ и $b$ -
\nTimes
матрицы и
\ShowEq{CR product singular, 1}
$c$ - \CR вырожденная матрица тогда и только тогда, когда
либо матрица $a$, либо матрица $b$ - \CR вырожденная матрица.
\qed
\end{ShadedTheorem}

\TwoColText
{
\begin{ShadedDefinition}
\AddIndex{\RC матричная группа}{rc-matrix group}
\ShowEq{rc-matrix group}
- это группа
\RC невырожденных матриц, гле мы определяем
\RC произведение матриц
\EqRef{rc-product of matrices}
и \RC обратную матрица
$a^{\CRInverse}$.
\end{ShadedDefinition}
}
{
\begin{ShadedDefinition}
\AddIndex{\CR матричная группа}{cr-matrix group}
\ShowEq{cr-matrix group}
- это группа
\CR невырожденных матриц
где мы определяем
\CR произведение матриц
\EqRef{cr-product of matrices}
и \CR обратную матрицу
$a^{\CRInverse}$.
\end{ShadedDefinition}
}

\begin{ShadedTheorem}
\labelTheorem{CR RC singular matrix}
\ShowEq{RCGL ne CRGL}
\end{ShadedTheorem}
\begin{remark}
Из теорем
\refTheorem{inverse unit matrix order 2}{rc},
\refTheorem{inverse unit matrix order 2}{cr}
следует, что
существуют матрицы, которые \CR невырожденны и \RC невырожденны.
Теорема \RefTheorem{CR RC singular matrix} означает, что множества
\CR невырожденных матриц и \RC невырожденных матриц
не совпадают. Например,
существует такая \RC невырожденная матрица, которая
\CR вырожденная матрица.
\qed
\end{remark}
\begin{proof}
Это утверждение достаточно доказать для $\gin=\gi 2$.
Предположим, что каждая \CR вырожденная матрица
\ShowEq{RC-singular matrix, 1}
является \RC вырожденной матрицей.
Из теорем
\refTheorem{rank of matrix}{rc-rows},
\refTheorem{rank of matrix}{rc-cols}
следует, что
\RC вырожденная матрица удовлетворяет условию
\ShowEq{RC, row, 2 1, 1 1}
\ShowEq{RC, row, 2 2, 1 2}
\ShowEq{RC, column, 1 2, 1 1}
\ShowEq{RC, column, 2 2, 2 1}
Если мы подставим \EqRef{RC, column, 1 2, 1 1}
в \EqRef{RC, row, 2 2, 1 2}, мы получим
\ShowEq{RC, a22, 2}
$b$ и $c$ - произвольные $A$\Hyph числа и \RC вырожденная матрица
\EqRef{RC-singular matrix, 1} имеет вид ($d=\aUD a11$)
\ShowEq{RC-singular matrix, 2}
Подобным образом мы можем показать, что \CR вырожденная матрица
имеет вид
\ShowEq{CR-singular matrix, 2}
Из предположения следует, что \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2} представляют одну и ту же матрицу.
Сравнивая \EqRef{CR-singular matrix, 2}
и \EqRef{RC-singular matrix, 2}, мы получим, что
для любых $d,c\in D$ существует такое $c'\in D$, которое не зависит от $d$ и
удовлетворяет уравнению
\[d c=c'd\]
Это противоречит утверждению, что $A$ - алгебра с делением.
\end{proof}

\begin{\ExampleStyle}
В случае алгебры кватернионов мы положим $b=1+k$, $c=j$, $d=k$.
Тогда мы имеем
\ShowEq{example rc singular matrix a}
\ShowEq{example rc singular matrix det}

Система линейных уравнений
\ShowEq{example rc singular matrix, rcd}
имеет \RC вырожденную матрицу.
Мы можем записать систему линейных уравнений
\EqRef{example rc singular matrix, rcd} в виде
\ShowEq{example rc singular matrix, rcd 1}

Система линейных уравнений
\ShowEq{example rc singular matrix, crd}
имеет \CR невырожденную матрицу.
Мы можем записать систему линейных уравнений
\EqRef{example rc singular matrix, crd} в виде
\ShowEq{example rc singular matrix, crd 1}

Система линейных уравнений
\ShowEq{example rc singular matrix, drc}
имеет \RC вырожденную матрицу.
Мы можем записать систему линейных уравнений
\EqRef{example rc singular matrix, drc} в виде
\ShowEq{example rc singular matrix, drc 1}

Система линейных уравнений
\ShowEq{example rc singular matrix, dcr}
имеет \CR невырожденную матрицу.
Мы можем записать систему линейных уравнений
\EqRef{example rc singular matrix, dcr} в виде
\ShowEq{example rc singular matrix, dcr 1}
\end{\ExampleStyle}

\section{Обратная матрица}

\ShowText{Inverse Matrix}

Если $\gim=\gin$, то левая \CR обратная матрица
определена однозначно.
Вообще говоря, это неверно, если $\gim\ne\gin$.
Рассмотрим систему линейных уравнений
\eqRef{linear equations rank left}{cr}.
\begin{itemize}
\item
Если $\gim<\gin$, то система линейных уравнений
\eqRef{linear equations rank left}{cr}
содержит неизвестных больше, чем число уравнений.
Решение системы линейных уравнений
\eqRef{linear equations rank left}{cr}
определено однозначно с точностью до выбора значений избыточных переменных.
\item
Если $\gim>\gin$, то система линейных уравнений
\eqRef{linear equations rank left}{cr}
содержит $\gik$ неизвестных и  $\gik$ уравнений.
Следовательно, система линейных уравнений
\eqRef{linear equations rank left}{cr}
имеет единственное решение.
Однако выбор множества $\gi I$ неоднозначен. 
\end{itemize}

\ShowText{Inverse Matrix set}


==> Linear.Vector.Space.Russian.tex <==
%auto-ignore
\input{Linear.Vector.Space.Eq}

\chapter{Линейное отображение \texorpdfstring{$A$}{A}-векторного пространства}

\section{Линейное отображение}

\ShowText{linear map of A vector space}

%Координаты линейного отображения
%не зависят от того,
%рассматриваем ли мы левое или правое
%$A$\Hyph векторное пространство.
%Однако форма записи линейного отображения
%зависит от типа векторного пространства.

\section{Матрица линейного отображения}

\begin{\DefinitionStyle}
Пусть
\ShowEq{Ai, 1n}A -
множество $D$\Hyph алгебр.
Матрица
\ShowEq{matrix f=}
элементы которой являются отображениями
\DrawEq[{f^i_j}{A_i}{A_j}{}]{f: A->B}{}
называется
\AddIndex{матрицей отображений}{matrix of maps}.
\end{\DefinitionStyle}

На множестве матриц отображений определены следующие операции
\begin{itemize}
\item
сложение
\ShowEq{matrix addition}
\item
\RCo произведение
\ShowEq{RCo product}
\item
\CRo произведение
\ShowEq{CRo product}
\end{itemize}


==> Preface.2207.06506.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{About this Book}

I planned to write several different papers
dedicated to linear algebra.
I considered these papers in the following sections in this chapter.
%\ShowEq{list of sections}
However at some point I realized that I am ready to assemble these papers
in one book where I will consider all problems
that I studied in the field of linear algebra.
However, answer to one question raises new questions
that must be answered also.
For instance, since I want to consider Eigenvalue problem,
I must to consider the theory of algebraic equations.

The list of subjects was gradually increasing.
i realized that I want give a broad overview of the theory
of non\Hyph commutative algebra.
I understand that I will not give complete description of the subject. This is wide field.
However list of questions that I want to discuss requires to write few volumes.

\section{Linear Map}
\labelSection{paper Linear Map}

I will start by the following statement.

\begin{\TheoremStyle}
\labelTheorem{L(A->A)=A}
Since division $D$\Hyph algebra $A$
satisfies the following conditions
\StartLabelItem
\begin{enumerate}
\item
$D$\Hyph algebra $A$ is commutative and associative
\labelItem{algebra $A$ is commutative and associative}
\item
the field $D$ is the center of $D$\Hyph algebra $A$
\labelItem{field D is center of D algebra}
\end{enumerate}
then
\ShowEq{L(A->A)=A}
\end{\TheoremStyle}
\ifx\texFuture\Defined
\begin{proof}
If $a\in A$, then from equalities
\ShowEq{linear map a}
it follows that the the map
\ShowEq{x->ax}
is linear map.

Since $A$ is division $D$\Hyph algebra,
then $D$\Hyph algebra $A$ has unit.
Therefore, we may consider $D$\Hyph algebra $A$ as
$A$\Hyph vector space with the basis
\ShowEq{basis e=1}
Therefore, for any linear map
\ShowEq{f in L(A->B)}DAA,
there exists $a\in A$ such that
\ShowEq{fox=ax}
\end{proof}
\fi

We will consider the proof of the theorem
\RefTheorem{L(A->A)=A}
in volume 3.
If at least one condition of the theorem
\RefTheorem{L(A->A)=A}
is not true,
then the the equality
\EqRef{L(A->A)=A}
is imposible.
\begin{itemize}
\item
The set of linear maps
\ShowEq{L(A->B)}RCC{}
of complex field
is $C$\Hyph vector space
of dimension $2$.
This is because the product in real field is commutative
and complex field $C$ is vector space
of dimension $2$
over real field $R$.
\item
The set of linear maps
\ShowEq{L(A->B)}RHH{}
of quaternion algebra
is $H$\Hyph vector space
of dimension $4$.
This is because the product in quaternion algebra is non\Hyph commutative
\end{itemize}
During my research in quaternion algebra,
I considered set of maps with certain symmetry
in papers
\citeBib{1107.1139,1202.6021}.
It was start point of new research.
The desire to find analogues of statements from theory of functions of complex variable
was one of the reasons of this research.

I have made several attempts to find a set of maps
that would allow me to find a structure of the set
\ShowEq{L(A->B)}RHH{}
similar to the structure of the set
\ShowEq{L(A->B)}RCC.
However, I do not consider any of these attempts successful.
However, during this research,
I realized that the set
\ShowEq{L(A->B)}RHH{}
is left or right $H$\Hyph vector space
of dimension $4$.

I concidered the set of linear maps
\ShowEq{L(A->B)}ROO{}
of octonion algebra
the similar way.
However I realized that similar statement is true
for any division $D$\Hyph algebra.

%This is not first time when I do not like the solution of the problem.
%This means that I am ready to move in wrong direction.
%I switch my attention to another problem.
%But, apparently, I keep thinking of the interrupted problem.
%When later I return to the problem,
%I see a solution that I was looking.

It does not mean that consideration of the algebra
\ShowEq{L(A->B)}DAA{}
as $A$\Hyph vector space
can substitute representation of map as tensor.

\section{System of Linear Equations}
\labelSection{paper System of Linear Equations}

%In the process of writing the book, another topic appeared;
%the topic is system of linear equations.

Let $V$ be left vector space
over $D$\Hyph algebra $A$.
Let $\Basis e$ be basis of left $A$\Hyph vector space $V$.
In this case, we can consider two different problems,
whose condition can be written as
system of linear equations.
\begin{itemize}
\item
Let $V$ be
left $A$\Hyph vector space of columns.
Then we write vectors of basis $\Basis e$ as
row of matrix
\DrawEq[en]{a=(a1.n row)}{}
and coordinates of vector $\Vector w$ with respect to basis $\Basis e$ as
column of matrix
\DrawEq[wn]{a=(a1.n col)}{}
We represent the set of vectors
\ShowEq{row set 1n}vm{}
as
row of matrix
\DrawEq[vm]{a=(a1.n row)}{}
We write
coordinates of vector $\aD vi$ with respect to basis $\Basis e$ as
column of matrix
\DrawEq[{\aD vi}n]{a=(a1.n col)}{}
To answer the question whether it is possible to represent the vector $\Vector w$
as linear combination of the set of vectors
\ShowEq{row set 1n}vm,
we must solve the system of linear equations
\DrawEq[cvwmn]{system of linear equations left column row}{}
with respect to the set of unknown scalars
\ShowEq{column set 1n}cm.
\item
Let $A$ be associative division $D$\Hyph algebra.
\ShowText{system of linear equations linear map}
\end{itemize}

\Input{Preface.Eigen}

\section{System of Differential Equations}
\labelSection{System of Differential Equations}

In commutative algebra there is one more problem
to solve which we need to find eigenvalue of matrix.
We are looking for a solution of system of differential equations
\DrawEq{dx/dt=a*x matrix right-cols}{2207.06506}
as
\DrawEq{vec x=vec c eat}{}
In this case, the number $b$ is eigenvalue of the matrix
\DrawEq[ann]{a=(a11.nm matrix)}{}
and the vector
\[
c=\ColMatrix cn
\]
is eigenvector of the matrix $a$
for eigenvalue $b$.

\ShowEq{def a rc x}
In case of non\Hyph commutative $D$\Hyph algebra A,
we can write the system of differential equations
\eqRef{dx/dt=a*x matrix right-cols}{2207.06506}
as follows
\DrawEq[{}{}]{dx/dt=a*x \SideNS-\Cols}{2207.06506}
In such case, the solution of the system of differential equations
\eqRef{dx/dt=a*x \SideNS-\Cols}{2207.06506}
may have one of following representations.
\begin{itemize}
\item
We can write solution as
\DrawEq[{}{}]{x=c*e**bt \SideNS-\Cols}{2207.06506}
where $A$\Hyph number $b$ is \ProductType eigenvalue of the matrix $a$
and \ColWS vector $c$ is
eigen\ColWS for \ProductType eigenvalue $b$.
\item
We can write solution as
\DrawEq[{}{}]{x=c*e**bt \OtherSideNS-\Cols}{2207.06506 1}
where $A$\Hyph number $b$ is \SideWS \ProductType eigenvalue of the matrix $a$
and \ColWS vector $c$ is
eigen\ColWS for \SideWS \ProductType eigenvalue $b$.
\end{itemize}

\DefText[1]{We can write solution as}
{
\ShowEq{\DefCol}
We can write solution as
\ShowEq{x=c ebt c \SideNS-\Cols}
where
\begin{itemize}
\item
$A$\Hyph number $b$ is \SideWS \ProductTypeO eigenvalue of the matrix
\DrawEq{a=matrix of maps n x n}{}
and the \ColWS $c$ is
eigen\ColWS
of the matrix $a$ corresponding to the \SideWS \ProductTypeO eigenvalue $b$.
\item
$A$\Hyph number $b$ and
$A$\Hyph number $C$ satisfy the condition
\DrawEq[b{}{s#1}]{b in AAA[a]}{s#1-\Cols}
\DrawEq[C{}{s#1}]{b in AAA[a]}{Cs#1-\Cols}
\end{itemize}
}

In non\Hyph commutative $D$\Hyph algebra A,
we can consider a more general form
of the system of linear differential equations
\DrawEq{dx/dt=a x a cols}{2207.06506}
We can represent the system of differential equations
\eqRef{dx/dt=a x a cols}{2207.06506}
using product of matrices
\ShowEq{dx/dt=a x a cols.matrix}
The solution of the system of differential equations
\EqRef{dx/dt=a x a cols.matrix}
may have one of following representations.
\begin{itemize}
\item
\ShowEq{def left}
\ShowText{We can write solution as}1
\item
\ShowEq{def right}
\ShowText{We can write solution as}2
\end{itemize}

%Eigenvalue of the matrix
%\DrawEq{a=matrix of maps n x n}{}
%is the definition in non\Hyph commutative algebra
%which does not have an analogue in commutative algebra.

\section{Polynomial}
\labelSection{Polynomial}

%\subsection{Skew right polynomial ring}

In commutative algebra polynomials
have a lot of common with number theory:
divisibility, greatest common factor,
least common multiple, factorization into irreducible factors.
When we study polynomials in non\Hyph commutative algebra,
we want to preserve
statements from commutative algebra as much as possible.

\ShowText{Ore introduced the transformation of monomial}

\begin{\TheoremStyle}
\labelTheorem{ring of polynomials is not Ore ring}
Let $A$ be division $D$\Hyph algebra.
Let
\ShowEq{f in AoA}a.
Let the equation
\ShowEq{aox+b=0}
have infinitely many roots,
but not any $A$\Hyph number is the root of the equation
\EqRef{aox+b=0}.
Then ring of polynomials $A[x]$
is not Ore ring.
\end{\TheoremStyle}

\begin{proof}
Let the transformation
\FrameEqRef{at=taa+ad}1
be defined in $D$ algebra $A$.
Let
\ShowEq{a=as0 ox as1}
The equality
\ShowEq{as0 ox as1+b=0}
follows from equalities
\eqRef{at=taa+ad}1,
\EqRef{aox+b=0},
\EqRef{a=as0 ox as1}.
Let
\ShowEq{A=.. B=..}
The equation
\ShowEq{xA+B=0}
has the same roots as the equation
\EqRef{aox+b=0}.
\begin{itemize}
\item
If $A\ne 0$, then the equation
\EqRef{xA+B=0}
has single root.
\item
If $A=0$, $B\ne 0$, then the equation
\EqRef{xA+B=0}
has no root.
\item
If $A=0$, $B= 0$,
then any $A$\Hyph number is root of the equation
\EqRef{xA+B=0}.
\end{itemize}
All three options contradict the condition of the theorem.
Therefore, the transformation
\FrameEqRef{at=taa+ad}1
is not defined in $D$ algebra $A$.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{ix-xi=k}
General solution of the linear equation
\DrawEq{ix-xi=k}1
in quaternion algebra is
\DrawEq{x=c12+j}P
\end{\TheoremStyle}

\begin{proof}
The tensor
\ShowEq{1 ox i-i ox 1}
corresponds to the matrix
\ShowEq{1 ox i-i ox 1 matrix}
\end{proof}

\begin{\TheoremStyle}
The ring of polynomials $H[x]$
in quaternion algebra
is not Ore ring.
\end{\TheoremStyle}

\begin{proof}
The theorem follows from theorems
\RefTheorem{ring of polynomials is not Ore ring},
\RefTheorem{ix-xi=k}.
\end{proof}

%\subsection{Left-sided Polynomial}

\ShowText{Left-sided Polynomial}

\begin{\ExampleStyle}
Let
\ShowEq{f=1+ix}
\ShowEq{g=k+jx}
Equalities
\ShowEq{f*g=... 1}
\ShowEq{fg=... 1}
follow from the equalities
\EqRef{product of left-sided polynomials f and g},
\EqRef{f=1+ix},
\EqRef{g=k+jx}.
Let $x=k$.
The equality
\ShowEq{f(x)= x=k 1}
follows from the equality
\EqRef{f=1+ix}.
The equality
\ShowEq{g(x)= x=k 1}
follows from the equality
\EqRef{g=k+jx}.
The equality
\ShowEq{f(x)g(x)= x=k 1}
follows from the equalities
\EqRef{f(x)= x=k 1},
\EqRef{g(x)= x=k 1}.
The equality
\ShowEq{f*g(x)= x=k 1}
follows from the equality
\EqRef{f*g=... 1}.
The equality
\ShowEq{fg(x)= x=k 1}
follows from the equality
\EqRef{fg=... 1}.
Therefore,
\ShowEq{fg(k) ne f*g(k)}
\end{\ExampleStyle}

\section{Division in Non-commutative Algebra}

To answer the question about dividing polynomials
in non-commutative algebra, we have to go
beyond algebra of polynomials.

Everything is simple in division algebra.
The equation $ax=b$ has unique solution
as soon as $a\ne 0$.
However, we considered this question
in the proof of the theorem
\RefTheorem{ring of polynomials is not Ore ring}.
Division algebra is small county
in vast kingdom of Algebra.

Consider any $D$\Hyph algebra $A$.
Suppose we claim that $A$\Hyph number $b$
divides $A$\Hyph number $a$.
What does this statement mean?

It would seem that there is simple answer.

\begin{\DefinitionStyle}
\labelDefinition{left divisor of A number}
There exists $A$\Hyph number $c$ such that
\[a=bc\]
In such case, $A$\Hyph number $b$
is called left divisor of $A$\Hyph number $a$.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{right divisor of A number}
There exists $A$\Hyph number $c$ such that
\[a=cb\]
In such case, $A$\Hyph number $b$
is called right divisor of $A$\Hyph number $a$.
\end{\DefinitionStyle}

But should we distinguish between left and right divisors?
According to the definition,
$D$\Hyph algebra $A$ is $D$\Hyph module $A$,
equipped by {\bf bilinear map}
\ShowEq{f:A->B}f{A\times A}A
called {\bf product}.
But if we assume that first argument of the map $f$
is given $A$\Hyph number,
then bilinear map becomes
linear map of second argument.

Therefore, we will say that $A$\Hyph number $b$
divides $A$\Hyph number $a$,
if there exists linear map
\ShowEq{f:A->B}cAA
such that
\[a=c\circ b\]

For instance, we can rewrite definitions
\RefDefinition{left divisor of A number},
\RefDefinition{right divisor of A number}
in the following way:

\begin{\DefinitionStyle}
\labelDefinition{1 ox divisor of A number}
There exists linear map \AoxB 1c such that
\ShowEq{c ox d b=a}1c
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{ox 1 divisor of A number}
There exists linear map \AoxB c1 such that
\ShowEq{c ox d b=a}c1
\end{\DefinitionStyle}

We will also say that $A$\Hyph number $b$
divides $A$\Hyph number $a$ with remainder,
if there exists linear map
\ShowEq{f:A->B}cAA
and $A$\Hyph number $d$ such that
\[a=c\circ b+d\]

Division algorithm, algorithms to search greatest common factor
or least common multiple are standard procedure.

The solution of one question very often raises new questions.
Among the issues that will need to be resolved is
the expansion of $A$\Hyph number using its factors.

For instance, what will be the result of division
of $A$\Hyph number $a$ by $A$\Hyph numbers $b_1$ and $b_2$.
To answer this question, we divide the task
into several steps.\,\footnote{\,
To simplify the reasoning,
we assume that at each stage
we have division without reminder.
We also consider associative $D$\Hyph algebra.
}

The quotient of $A$\Hyph number $a$ divided by $A$\Hyph number $b_1$
has the following form
\ShowEq{a=c1 o b1}
where linear map $c_1$ has the following form
\ShowEq{c1=c10s ox c11s}
We do not have an algorith of dividing a tensor $c_1$ by $A$\Hyph number $b_2$.
However the equality
\ShowEq{a=c10s b1 c11s}
follows from equalities
\EqRef{a=c1 o b1},
\EqRef{c1=c10s ox c11s}.
The equality
\EqRef{a=c10s b1 c11s}
implies that if we want to divide
$A$\Hyph number $a$ by $A$\Hyph numbers $b_1$ and $b_2$,
then we have to divide
every $A$\Hyph number $c_{10s}$, $c_{11s}$ by $A$\Hyph number $b_2$
and substitute the result into equality
\EqRef{a=c10s b1 c11s}
\ShowEq{a=c10s b1 c11s 1}
However, the expression on the right side of the equality
\EqRef{a=c10s b1 c11s 1}
is bilinear map of $A$\Hyph numbers $b_1$ and $b_2$ 
\ShowEq{a=c (a1 a2)}

Gradually increasing the number of factors,
we come to the conclusion that if $A$\Hyph number $a$
is product of $A$\Hyph numbers $b_1$, ..., $b_n$,
then $A$\Hyph number $a$
is polylinear map of $A$\Hyph numbers $b_1$, ..., $b_n$.

Now we can return to polynomials.
In order to find factorization of a polynomial into irreducible factors,
we have to answer some questions.
How to find the set of roots?
How big is the set of factorizations, if the set of roots is infinite?
How we can find factor
if this factor does not have roots?

\DefText{preface rc eigenvalue 1}
{
In such case, the set of eigenvectors
has two equivalent definitions
\newline
\FrameEqRef{U-*A*U=D \Product-\SideNS}1
\newline
and
\newline
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
}

\section{Inverse Matrix}

This topic came up in the process of writing the book.

In this book, I considered definition of left and right
eigenvalues of \nTimes matrix $a_2$
in case when the matrix $a_2$ has $\gi n$
different eigenvalues.
\ShowText{preface rc eigenvalue}
Matrices $u_2$, $a_1$ are also \nTimes matrices.
In such case, sets of left and right
\RC eigenvalues are the same.

However, professor Cohn pointed out that there are cases
when the set of keft
\RC eigenvalues
is different from the set of right
\RC eigenvalues.
To find such matrix, I decided to consider the case
when the matrix $a_2$ has $\gi k$, $\gik<\gin$,
different eigenvalues.
In this case I have to confine myself to the definition
which is similar to the definition
\ShowEq{def left}
\ShowEq{\DefRow}
\newline
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
In such case, the matrix $u_2$
is
\ShowEq{gin x gik \SideNS}
matrix and the matrix $a_1$
is \nTimes[k] matrix.
Trying to answer the question
can I write a definition similar to the definition
\eqRef{U-*A*U=D \Product-\SideNS}1,
I realized that I need to consider the concept of
right \RC inverse matrix.

\section{Non-commutative Sum}

\ShowRemark{Non-commutative Sum}


==> Preface.2207.06506.Eq.tex <==
%auto-ignore

\AddEq{list of sections}
{
\RefSection{paper Linear Map},
\RefSection{paper System of Linear Equations},
\RefSection{paper Eigenvalue of Matrix},
\RefSection{System of Differential Equations},
\RefSection{Polynomial}.
}

\AddEq{fox=ax}
{
$f\circ x=ax$.
}

\AddEq{vec x=vec c eat}
{
\ColMatrix xn
=
\ColMatrix cn
e^{bt}
}

\DefText{preface rc eigenvalue}
{
\TwoColText
{
\ShowEq{def left}
\ShowEq{\DefRow}
\ShowText{preface rc eigenvalue 1}
}
{
\ShowEq{def right}
\ShowEq{\DefCol}
\ShowText{preface rc eigenvalue 1}
}
}

\AddEquation{L(A->A)=A}
{
\LAA DA=A
}

\AddEquation{a=as0 ox as1}
{
a=a_{s0}\otimes a_{s1}
}

\AddEquation{aox+b=0}
{
a\circ x+b=0
}

\AddEq[2]{c ox d b=a}
{
$(\AoxB{#1}{#2})\circ b=a$
}

\AddEquation{c1=c10s ox c11s}
{
c_1=\AoxB{c_{10s}}{c_{11s}}
}

\AddEquation{a=c10s b1 c11s}
{
a=c_{10s}b_1c_{11s}
}

\AddEquation{a=c10s b1 c11s 1}
{
a=(c_{10s2}\circ b_2)b_1c_{11s}+c_{10s}b_1(c_{11s2}\circ b_2)
}

\AddEquation{a=c (a1 a2)}
{
\begin{split}
a&=c\circ(b_1,b_2)
\\
c&=c_{10s20t}\otimes_2c_{10s21t}\otimes_1c_{11s}
+c_{10s}\otimes_1c_{11s20t}\otimes_2c_{11s21t}
\end{split}
}

\AddEquation{a=c1 o b1}
{
a=c_1\circ b_1
}

\AddEquation{as0 ox as1+b=0}
{
\begin{split}
(a_{s0}\otimes a_{s1})\circ x+b
&=a_{s0}xa_{s1}+b
=(xa_{s0}^{\alpha}+a_{s0}^{\delta})a_{s1}+b
\\ &=xa_{s0}^{\alpha}a_{s1}+a_{s0}^{\delta}a_{s1}+b=0
\end{split}
}

\AddEquation{xA+B=0}
{
xA+B=0
}

\AddEq{A=.. B=..}
{
\[
A=a_{s0}^{\alpha}a_{s1}\ \ \ \,B=a_{s0}^{\delta}a_{s1}+b
\]
}

\AddEq{x->ax}
{
\[
a\circ E:x\rightarrow ax
\]
}

\AddEq{linear map a}
{
\begin{align*}
a(b+c)&=ab+ac\\
a(bc)&=(ab)c=(ba)c=b(ac)
\end{align*}
}



==> Preface.2207.06506.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Об этой книге}

Я планировал написать несколько разных статей
по линейной алгебре.
Я рассмотрел эти статьи в последующих разделах этой главы.
%\ShowEq{list of sections}
Но в какой-то момент я понял, что я готов собрать эти статьи
в одну книгу и рассмотреть все задачи,
которыми я занимался в области линейной алгебры.
Однако ответ на один вопрос
порождает новые вопросы, которые тоже должны быть отвечены.
Например, если я хочу рассмотреть задачу о собственных значениях,
я должен рассмотреть теорию алгебраических уравнений.

Список тем постепенно увеличивался.
Мне стало ясно, что я хочу дать широкий обзор теории
некоммутативной алгебры.
Я понимаю что вряд ли дам полное описание, тема обширная.
Но и те вопросы, что я хочу затронуть, займут несколько томов.

\section{Линейное отображение}
\labelSection{paper Linear Map}

Я начну со следуещевого утверждения.

\begin{\TheoremStyle}
\labelTheorem{L(A->A)=A}
Если $D$\Hyph алгебра $A$ с делением
удовлетворяет следующим условиям
\StartLabelItem
\begin{enumerate}
\item
$D$\Hyph алгебра $A$ коммутативна и ассоциативна
\labelItem{algebra $A$ is commutative and associative}
\item
поле $D$ является центром $D$\Hyph алгебры $A$
\labelItem{field D is center of D algebra}
\end{enumerate}
то
\ShowEq{L(A->A)=A}
\end{\TheoremStyle}
\ifx\texFuture\Defined
\begin{proof}
Если $a\in A$, то из равенств
\ShowEq{linear map a}
следует, что отображение
\ShowEq{x->ax}
линейно.

Поскольку $A$ - $D$\Hyph алгебра с деленим,
то $D$\Hyph алгебра $A$ имеет единицу.
Следовательно, мы можем рассматривать $D$\Hyph алгебру $A$ как
$A$\Hyph векторное пространство с базисом
\ShowEq{basis e=1}
Следовательно, для любого линейного отображения
\ShowEq{f in L(A->B)}DAA{}
существует $a\in A$ такое, что
\ShowEq{fox=ax}
\end{proof}
\fi

Мы рассмотрим доказательство теоремы
\RefTheorem{L(A->A)=A}
в томе 3.
Если хотя бы одно условие теоремы
\RefTheorem{L(A->A)=A}
нарушено,
то равенство
\EqRef{L(A->A)=A}
невозможно.
\begin{itemize}
\item
Множество линейных отображений
\ShowEq{L(A->B)}RCC{}
поля комплексных чисел
является $C$\Hyph векторным пространством
размерности $2$.
Это связано с тем, что произведение в поле комплексных чисел коммутативно
и поле комплексных чисел $C$ является векторным пространством
размерности $2$
над полем действительных чисел $R$.
\item
Множество линейных отображений
\ShowEq{L(A->B)}RHH{}
алгебры кватернионов
является $H$\Hyph векторным пространством
размерности $4$.
Это связано с тем, что произведение в алгебре кватернионов не коммутативно
\end{itemize}
Изучая алгебру кватернионов,
в статьях
\citeBib{1107.1139,1202.6021}
я рассмотрел множество отображений, обладающих некоторой симметрией.
Это положило начало нового исследования.
Одним из мотивов этого исследования
было желание найти аналоги утверждениям из теории функции комплексного переменного.

Я сделал несколько попыток найти множество отображений,
которые позволили бы мне найти структуру множества
\ShowEq{L(A->B)}RHH,
подобную структуре множества
\ShowEq{L(A->B)}RCC.
Но не считаю ни одну из этих попыток успешной.
Тем не менее, в процессе этого исследования
я понял, что множество
\ShowEq{L(A->B)}RHH{}
является левым или правым $H$\Hyph векторным пространством
размерности $4$.

Я рассмотрел множество линейных отображений
\ShowEq{L(A->B)}ROO{}
алгебры октонионов
аналогичным образом.
Однако я понял, что подобное утверждение верно
для любой $D$\Hyph алгебры с делением.

%Это не первый раз, когда мне не нравится решение задачи.
%Это говорит о том, что я собираюсь двигаться в неверном направлении.
%Я переключаюсь на другие задачи.
%Но, по\Hyph видимому, я продолжаю думать над прерваной задачей.
%Когда я возвращаюсь к задаче позже,
%я вижу решение, которое искал.

Это не значит, что рассмотрение алгебры
\ShowEq{L(A->B)}DAA{}
как $A$\Hyph векторного пространства
может заменить представление отображения как тензора.

\section{Система линейных уравнений}
\labelSection{paper System of Linear Equations}

%В процессе написания книги появилась ещё одна тема,
%система линейных уравнений.

Пусть $V$ - левое векторное пространство
над $D$\Hyph алгеброй $A$.
Пусть $\Basis e$ - базис левого $A$\Hyph векторного пространства $V$.
В этом случае мы можем рассмотреть две различные задачи,
условие которых можно записать в виде
системы линейных уравнений.
\begin{itemize}
\item
Пусть $V$ -
левое $A$\Hyph векторное пространство столбцов.
Тогда векторы базиса $\Basis e$ мы запишем в виде
строки матрицы
\DrawEq[en]{a=(a1.n row)}{}
и координаты вектора $\Vector w$ относительно базиса $\Basis e$ мы запишем в виде
столбца матрицы
\DrawEq[wn]{a=(a1.n col)}{}
Представим множество векторов
\ShowEq{row set 1n}vm{}
в виде
строки матрицы
\DrawEq[vm]{a=(a1.n row)}{}
Мы запишем
координаты вектора $\aD vi$ относительно базиса $\Basis e$ мы запишем в виде
столбца матрицы
\DrawEq[{\aD vi}n]{a=(a1.n col)}{}
Чтобы ответить на вопрос, можно ли представить вектор $\Vector w$
как линейную комбинацию множества векторов
\ShowEq{row set 1n}vm,
мы должны решить систему линейных уравнений
\DrawEq[cvwmn]{system of linear equations left column row}{}
относительно множества неизвестных скаляров
\ShowEq{column set 1n}cm.
\item
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
\ShowText{system of linear equations linear map}
\end{itemize}

\Input{Preface.Eigen}

\section{Система дифференциальных уравнений}
\labelSection{System of Differential Equations}

В коммутативной алгебре есть ещё одна задача,
для решения которой требуется найти собственное значение матрицы.
Мы ищем решение системы дифференциальных уравнений
\DrawEq{dx/dt=a*x matrix right-cols}{2207.06506}
в виде
\DrawEq{vec x=vec c eat}{}
В этом случае число $b$ является собственным значением матрицы
\DrawEq[ann]{a=(a11.nm matrix)}{}
и вектор
\[
c=\ColMatrix cn
\]
является собственным вектором матрицы $a$,
соответствующим собственному значению $b$.

\ShowEq{def a rc x}
В случае некоммутативной $D$\Hyph алгебры $A$,
мы можем записать систему дифференциальных уравнений
\eqRef{dx/dt=a*x matrix right-cols}{2207.06506}
в виде
\DrawEq[{}{}]{dx/dt=a*x \SideNS-\Cols}{2207.06506}
В этом случае решение системы дифференциальных уравнений
\eqRef{dx/dt=a*x \SideNS-\Cols}{2207.06506}
может иметь одно из следующих представлений.
\begin{itemize}
\item
Мы можем записать решение в виде
\DrawEq[{}{}]{x=c*e**bt \SideNS-\Cols}{2207.06506}
где $A$\Hyph число $b$ является \ProductType собственным значением матрицы $a$
и вектор\Hyph\ColWS $c$ является
собственн\ColBNS, соответствующ\FinB \ProductType собственному числу $b$.
\item
Мы можем записать решение в виде
\DrawEq[{}{}]{x=c*e**bt \OtherSideNS-\Cols}{2207.06506 1}
где $A$\Hyph число $b$ является \SideRu вым \ProductType собственным значением матрицы $a$
и вектор\Hyph\ColWS $c$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному числу $b$.
\end{itemize}

\DefText[1]{We can write solution as}
{
\ShowEq{\DefCol}
Мы можем записать решение в виде
\ShowEq{x=c ebt c \SideNS-\Cols}
где
\begin{itemize}
\item
$A$\Hyph число $b$ является \SideRu вым \ProductTypeO собственным значением матрицы
\DrawEq{a=matrix of maps n x n}{}
и \ColWS $c$ является
собственн\ColB
матрицы $a$, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
\item
$A$\Hyph число $b$ и
$A$\Hyph число $C$ удовлетворяют условию
\DrawEq[b{}{s#1}]{b in AAA[a]}{s#1-\Cols}
\DrawEq[C{}{s#1}]{b in AAA[a]}{Cs#1-\Cols}
\end{itemize}
}

В некоммутативной $D$\Hyph алгебры $A$,
мы можем рассмотреть более общий вид
системы линейных дифференциальных уравнений
\DrawEq{dx/dt=a x a cols}{2207.06506}
Мы можем записать систему дифференциальных уравнений
\eqRef{dx/dt=a x a cols}{2207.06506},
пользуясь произведением матриц
\ShowEq{dx/dt=a x a cols.matrix}
Решение системы дифференциальных уравнений
\EqRef{dx/dt=a x a cols.matrix}
может иметь одно из следующих представлений.
\begin{itemize}
\item
\ShowEq{def left}
\ShowText{We can write solution as}1
\item
\ShowEq{def right}
\ShowText{We can write solution as}2
\end{itemize}

%Собственное значение матрицы
%\DrawEq{a=matrix of maps n x n}{}
%это определение в некоммутативной алгебре,
%которое не имеет аналога в коммутативной алгебре.

\section{Многочлен}
\labelSection{Polynomial}

%\subsection{Кольцо правых косых многочленов}

В коммутативной алгебре теория многочленов имеет
много общего с теорией чисел:
делимость, наибольший общий делитель,
наименьшее общее кратное, разложение на неприводимые множители.
Когда мы изучаем многочлены в некоммутативной алгебре,
мы хотим максимально сохранить
утверждения из коммутативной алгебры.

\ShowText{Ore introduced the transformation of monomial}

\begin{\TheoremStyle}
\labelTheorem{ring of polynomials is not Ore ring}
Пусть $A$ - $D$\Hyph алгебра с делением.
Пусть
\ShowEq{f in AoA}a.
Пусть уравнение
\ShowEq{aox+b=0}
имеет бесконечно много корней,
но не любое $A$\Hyph число является корнем уравнения
\EqRef{aox+b=0}.
Тогда кольцо многочленов $A[x]$
не является кольцом Оре.
\end{\TheoremStyle}

\begin{proof}
Допустим, что в $D$\Hyph алгебре $A$
определено преобразование
\FrameEqRef{at=taa+ad}1.
Пусть
\ShowEq{a=as0 ox as1}
Равенство
\ShowEq{as0 ox as1+b=0}
является следствием равенств
\eqRef{at=taa+ad}1,
\EqRef{aox+b=0},
\EqRef{a=as0 ox as1}.
Положим
\ShowEq{A=.. B=..}
Уравнение
\ShowEq{xA+B=0}
имеет теже корни, что и уравнение
\EqRef{aox+b=0}.
\begin{itemize}
\item
Если $A\ne 0$, то уравнение
\EqRef{xA+B=0}
имеет единственный корень.
\item
Если $A=0$, $B\ne 0$, то уравнение
\EqRef{xA+B=0}
не имеет корней.
\item
Если $A=0$, $B= 0$,
то любое $A$\Hyph число является корнем уравнения
\EqRef{xA+B=0}.
\end{itemize}
Все три варианта противоречат условию теоремы.
Следовательно, преобразование
\FrameEqRef{at=taa+ad}1
не определено в $D$\Hyph алгебре $A$.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{ix-xi=k}
Общее решение линейного уравнения
\DrawEq{ix-xi=k}1
в алгебре кватернионов имеет вид
\DrawEq{x=c12+j}P
\end{\TheoremStyle}

\begin{proof}
Тензор
\ShowEq{1 ox i-i ox 1}
соответствует матрице
\ShowEq{1 ox i-i ox 1 matrix}
\end{proof}

\begin{\TheoremStyle}
Кольцо многочленов $H[x]$
в алгебре кватернионов
не является кольцом Оре.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием теорем
\RefTheorem{ring of polynomials is not Ore ring},
\RefTheorem{ix-xi=k}.
\end{proof}

%\subsection{Левостороний многочлен}

\ShowText{Left-sided Polynomial}

\begin{\ExampleStyle}
Положим
\ShowEq{f=1+ix}
\ShowEq{g=k+jx}
Равенства
\ShowEq{f*g=... 1}
\ShowEq{fg=... 1}
являются следствием равенств
\EqRef{product of left-sided polynomials f and g},
\EqRef{f=1+ix},
\EqRef{g=k+jx}.
Пусть $x=k$.
Равенство
\ShowEq{f(x)= x=k 1}
является следствием равенства
\EqRef{f=1+ix}.
Равенство
\ShowEq{g(x)= x=k 1}
является следствием равенства
\EqRef{g=k+jx}.
Равенство
\ShowEq{f(x)g(x)= x=k 1}
является следствием равенств
\EqRef{f(x)= x=k 1},
\EqRef{g(x)= x=k 1}.
Равенство
\ShowEq{f*g(x)= x=k 1}
является следствием равенства
\EqRef{f*g=... 1}.
Равенство
\ShowEq{fg(x)= x=k 1}
является следствием равенства
\EqRef{fg=... 1}.
Следовательно,
\ShowEq{fg(k) ne f*g(k)}
\end{\ExampleStyle}

\section{Деление в некоммутативной алгебре}

Чтобы ответить на вопрос о делении многочленов
в некоммутативной алгебре, мы должны выйти
за рамки алгебры многочленов.

В алгебре с делением всё просто.
Уравнение $ax=b$ имеет единственное решение,
как только $a\ne 0$.
Но не будем повторяться. Мы рассматривали этот вопрос
в доказательстве теоремы
\RefTheorem{ring of polynomials is not Ore ring}.
Алгебра с делением - это небольшое графство
в обширном королевстве Алгебра.

Рассмотрим произвольную $D$\Hyph алгебру $A$.
Допустим, мы утверждаем, что $A$\Hyph число $b$
делит $A$\Hyph число $a$.
Что значит это утверждение?

Казалось бы, есть простой ответ.

\begin{\DefinitionStyle}
\labelDefinition{left divisor of A number}
Существует $A$\Hyph число $c$ такое, что
\[a=bc\]
В этом случае $A$\Hyph число $b$
называется левым делителем $A$\Hyph числа $a$.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{right divisor of A number}
Существует $A$\Hyph число $c$ такое, что
\[a=cb\]
В этом случае $A$\Hyph число $b$
называется правым делителем $A$\Hyph числа $a$.
\end{\DefinitionStyle}

Но должны ли мы различать левый и правый делители?
Согласно определению,
$D$\Hyph алгебра $A$ - это $D$\Hyph модуль $A$,
в котором определено {\bf билинейное отображение}
\ShowEq{f:A->B}f{A\times A}A
называемое {\bf произведением}.
Но если мы положим, что первый аргумент отображения $f$
является заданным $A$\Hyph числом,
то билинейное отображение превращается
в линейное отображение второго аргумента.

Следовательно, мы будем говорить, что $A$\Hyph число $b$
делит $A$\Hyph число $a$,
если существует линейное отображение
\ShowEq{f:A->B}cAA
такое, что
\[a=c\circ b\]

Например, мы можем переписать определения
\RefDefinition{left divisor of A number},
\RefDefinition{right divisor of A number}
следующим образом:

\begin{\DefinitionStyle}
\labelDefinition{1 ox divisor of A number}
Существует линейное отображение \AoxB 1c такое, что
\ShowEq{c ox d b=a}1c
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{ox 1 divisor of A number}
Существует линейное отображение \AoxB c1 такое, что
\ShowEq{c ox d b=a}c1
\end{\DefinitionStyle}

Мы также будем говорить, что $A$\Hyph число $b$
делит $A$\Hyph число $a$,
если существует линейное отображение
\ShowEq{f:A->B}cAA
и $A$\Hyph число $d$ такие, что
\[a=c\circ b+d\]

Алгоритмы деления, поиска наибольшего общего делителя
или наименьшего общего кратного являются стандартной процедурой.

Решение одного вопроса очень часто порождает новые вопросы.
Среди вопросов, которые надо будет решить - это
разложение $A$\Hyph числа на множители.

Например, какой будет результат деления
$A$\Hyph числа $a$ на $A$\Hyph числа $b_1$ и $b_2$?
Чтобы ответить на этот вопрос, разделим задачу
на несколько шагов.\,\footnote{\,
Чтобы упростить рассуждения,
мы допускаем, что на каждом этапе
мы имеем деление без остатка.
Мы также рассматриваем ассоциативную $D$\Hyph алгебру.
}

Частное от деления $A$\Hyph числа $a$ на $A$\Hyph число $b_1$
имеет вид
\ShowEq{a=c1 o b1}
где линейное отображение $c_1$ имеет вид
\ShowEq{c1=c10s ox c11s}
У нас нет алгоритма деления тензора $c_1$ на $A$\Hyph число $b_2$.
Однако равенство
\ShowEq{a=c10s b1 c11s}
является следствием равенств
\EqRef{a=c1 o b1},
\EqRef{c1=c10s ox c11s}.
Из равенства
\EqRef{a=c10s b1 c11s}
следует, что если мы хотим поделить
$A$\Hyph число $a$ на $A$\Hyph числа $b_1$ и $b_2$,
то мы должны поделить
каждое $A$\Hyph число $c_{10s}$, $c_{11s}$ на $A$\Hyph число $b_2$
и результат подставить в равенство
\EqRef{a=c10s b1 c11s}
\ShowEq{a=c10s b1 c11s 1}
Но выражение в правой части равенства
\EqRef{a=c10s b1 c11s 1}
является билинейным отображением $A$\Hyph чисел $b_1$ и $b_2$ 
\ShowEq{a=c (a1 a2)}

Постепенно увеличивая число множителей,
мы приходим к выводу, что если $A$\Hyph число $a$
является произведением $A$\Hyph чисел $b_1$, ..., $b_n$,
то $A$\Hyph число $a$
является полилинейным отображением $A$\Hyph чисел $b_1$, ..., $b_n$.

Теперь мы можем вернуться к многочленам.
Для того чтобы найти разложение многочлена на неприводимые множители,
мы должны ответить на ряд вопросов.
Как найти множество корней?
Как велико множество разложений, если множество корней бесконечно?
Если многочлен имеет неприводимый делитель, не имеющий корней,
как найти этот делитель?

\DefText{preface rc eigenvalue 1}
{
В этом случае, множество собственных векторов
имеет два эквивалентных определения
\newline
\FrameEqRef{U-*A*U=D \Product-\SideNS}1
\newline
и
\newline
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
}

\section{Обратная матрицы}

Эта тема появилась в процессе написания книги.

В этой книге я рассмотрел определение левых и правых
\RC собственных чисел \nTimes матрицы $a_2$
в случае, когда матрица $a_2$ имеет $\gi n$
различных собственных значений.
\ShowText{preface rc eigenvalue}
Матрицы $u_2$, $a_1$ также являются \nTimes матрицами.
В этом случае, множества левых и правых
\RC собственных чисел совпадают.

Однако профессор Кон обратил внимание, что возможны случаи,
когда множество левых
\RC собственных чисел
отличается от множества правых
\RC собственных чисел.
Чтобы найти такую матрицу, я решил рассмотреть случай,
когда матрица $a_2$ имеет $\gi k$, $\gik<\gin$,
различных собственных значений.
В этом случае я вынужден ограничиться определением,
подобным определению
\ShowEq{def left}
\ShowEq{\DefRow}
\newline
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
В этом случае, матрица $u_2$
является
\ShowEq{gin x gik \SideNS}
матрицей и матрица $a_1$
является \nTimes[k] матрицей.
Пытаясь ответить на вопрос
могу ли я записать определение аналогичное определению
\eqRef{U-*A*U=D \Product-\SideNS}1,
я понял, что мне надо рассмотреть понятие
правой \RC обратной матрицы.

\section{Некоммутативная сумма}

\ShowRemark{Non-commutative Sum}


==> Preface.Eigen.English.tex <==
%auto-ignore
\input{Preface.Eigen.Eq}

\section{Eigenvalue of Matrix}
\labelSection{paper Eigenvalue of Matrix}

\subsection{Eigenvalue in commutative algebra}
\labelSubsection{Eigenvalue in commutative algebra}

I will start from the definition of eigenvalue of matrix
in commutative algebra.\,\footnote{\,
See also the definition on the page
\citeBib{Kurosh: High Algebra}\Hyph 200.
}

Let $a$ be \nTimes matrix whose entries
belong to the field $F$.
The polynomial
\DrawEq{characteristic polynomial}{}
where \aD En is \nTimes unit matrix
is called characteristic polynomial of the matrix $a$.
Roots of characteristic polynomial
are called eigenvalues of matrix $a$.
Therefore, eigenvalues of matrix $a$
satisfy the equation
\ShowEq{characteristic polynomial=0}
and the system of linear equations
\ShowEq{(a-bE)x=0}
has non\Hyph trivial solution
if $b$ is eigenvalue of the matrix $a$.

If matrices $a$ and $a_1$ are similar
\ShowEq{similar matrices}
then the equality
\ShowEq{similar matrices 1}
implies that matricess $a$ and $a_1$
have the same characteristic polynomial,
and, therefore, the same characteristic roots.

Let $V$ be vector space over field $F$.
Let
\ShowEq{basis e e1}
be bases of vector space $V$
and $f$ be coordinate matrix of the basis $\Basis e_1$
with respect to the basis $\Basis e$
\DrawEq{basis e1=fe}1
Let $a$ be the matrix of the endomorphism $\Vector a$
with respect to the basis $\Basis e$.
Then the matrix $a_1$ defined by the equality
\EqRef{similar matrices}
is the matrix of the endomorphism $\Vector a$
with respect to the basis $\Basis e_1$.
If we identify endomorphism
and its matrix with respect to given basis,
then we will say that eigenvalues of endomorphism
are eigenvalues of its matrix with respect to given basis.
Therefore, eigenvalues of endomorphism
do not depend on choice of a basis.

Let
\ShowEq{vx=x e}
Then the equality
\EqRef{(a-bE)x=0}
gets the following form
\DrawEq{va vx=b vx}P
\ShowEq{ax=bx}
with respect to the basis $\Basis e$.
Let $f$ be coordinate matrix of the basis $\Basis e_1$
with respect to the basis $\Basis e$
\FrameEqRef{basis e1=fe}1.
Then coordinate matrix $x_1$ of the vector $\Vector x$ 
with respect to the basis $\Basis e_1$ has the following form
\ShowEq{x1=f- x}
The equality
\ShowEq{f1 x1=b x1}
follows from the equalities
\EqRef{similar matrices},
\EqRef{ax=bx},
\EqRef{x1=f- x}.
Therefore, the equality
\eqRef{va vx=b vx}P
does not depend on choice of a basis,
and we will say that eigenvector of endomorphism
is eigenvector of its matrix with respect to given basis.

The set of eigenvalues of endomorphism $\Vector a$
each eigenvalue being taken with their multiplicity in the characteristic polynomial
is called the spectrum of endomorphism $\Vector a$.

\subsection{Eigenvalue in non-commutative algebra}
\labelSubsection{Eigenvalue in non-commutative algebra}

Let $A$ be
non\Hyph commutative division $D$\Hyph algebra $A$.
If we consider vector space over
$D$\Hyph algebra $A$,
then we want to keep the definition
of eigenvalue and eigenvector
considered in case of
vector space
over commutative algebra.

Let $V$ be left $A$\Hyph vector space of columns.
Since the product is non\Hyph commutative, the question arises.
Should we use the eqaulity
\DrawEq{aox=bx}1
or the eqaulity
\ShowEq{aox=xb}

The equality
\eqRef{aox=bx}1
looks natural
because, on the right side of the equality, we wrote
left\Hyph side product
of vector over scalar.
However, if
\ShowEq{cb ne bc}
then
\ShowEq{a o cx ne b cx}

\begin{Statement}
\labelStatement{set do not generate vector space}
The statement
\EqRef{a o cx ne b cx}
implies that the set of vectors $\Vector x$
which satisfy the equality
\eqRef{aox=bx}1,
do not generate subspace of vector space.
\hfill\(\odot\)
\end{Statement}

If we write down the equality
\eqRef{aox=bx}1
using matrices, then we get the equality
\ShowEq{x cr a=bx}
The equality
\EqRef{x cr a=bx}
is system of linear equations with respect to the set of unknown $x$.
However, we cannot say that this system of linear equations is singular
and has infinitely many solutions.
However this statement is an obvious consequence of the statement
\RefStatement{set do not generate vector space}.

The impression is that the equality
\eqRef{aox=bx}1
not suitable for definition of eigenvalue.
However, we will return to this definition in the section
\RefSection{Left and Right Eigenvalues}.

Consider the equality
\EqRef{aox=xb}.
Let $a$ be matrix of endomorphism $\Vector a$
with respect to the basis $\Basis e$
of left $A$\Hyph vector space of columns.
Let $a$ be matrix of vector $\Vector x$
with respect to the basis $\Basis e$.
The system of linear equations
\ShowEq{x cr a=xb}
follows from the equation
\EqRef{aox=xb}.
The system of linear equations
\EqRef{x cr a=xb}
has non\Hyph trivial solution when the matrix
\ShowEq{a-bEn}
is \CR singular.
In such case, the system of linear equations
\EqRef{x cr a=xb}
has infinitely many solutions.

At first sight,
considered model corresponds to the model
considered in the subsection
\RefSubsection{Eigenvalue in commutative algebra}.
However, if we choose another basis $\Basis e_1$
\ShowEq{e1=g cr e}
then the matrix $a$ will change
\ShowEq{a1=g a g-}
\ShowEq{a=g- a1 g}
and the matrix $x$ will change
\DrawEq[x1x{}g{}{left}{cols}]{v2=v1g-}1
\DrawEq[x{}x1g{}]{v1=v2*a left-cols}{P1}
The equality
\ShowEq{x_1 a_1 g=x_1 g b}
follows from equalities
\EqRef{x cr a=xb},
\EqRef{a=g- a1 g},
\eqRef{v1=v2*a left-cols}{P1}.
From the equality
\EqRef{x_1 a_1 g=x_1 g b},
it follows that column vector $x_1$
is not solution of the system of linear equations
\EqRef{x cr a=xb}.
This contradicts the statement that the equality
\EqRef{aox=xb}
does not depend on choice of basis.

The equality
\EqRef{aox=xb}
requires more careful analysis.
On the right side of the equality
\EqRef{aox=xb}
I wrote down the operation which is not defined
in left $A$\Hyph vector space,
namely, right\Hyph sided product of vector over scalar. 
However we can write the system of linear equations
\EqRef{x cr a=xb}
differently
\ShowEq{x cr a=x cr b E}
where $E$ is unit matrix.
On the right side of the equality
\EqRef{x cr a=x cr b E}
as well as on the left side,
I wrote down \CR product of column vector
over matrix of endomorphism.
Therefore, left and right sides
have the same transformation
when changing the basis.

Similar to vector space over field,
the endomorphism
\ShowEq{left map a En}b{}
which has the matrix $Eb$ with respect to the basis $\Basis e$
is called similarity transformation with respect to the basis $\Basis e$.
Therefore, we should write down the equality
\EqRef{aox=xb}
as
\ShowEq{aox=b e ox}

The equality
\EqRef{aox=b e ox}
is the definition of eigenvalue $b$
and eigenvector $x$ of endomorphism $a$.
If we consider matrix of endomorphism $a$
with respect to the basis $\Basis e$
of left $A$\Hyph vector space of columns,
then the equality
\EqRef{x cr a=xb}
is the definition of \CR eigenvalue $b$
and eigenvector $x$ corresponding
to \CR eigenvalue $b$.

\section{Left and Right Eigenvalues}
\labelSection{Left and Right Eigenvalues}

To better understand essence of eigenvalues,
consider the following theorem.

\ShowEq{def DVector}
\ShowTheorem{n eigenvectors}{field}

\begin{proof}
We will prove the theorem by induction with respect to $\gik$.

Since eigenvector is non\Hyph zero, the theorem is true for $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1}
Let the theorem be true for $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
Let
\ShowEq{di 1n+1}bm{}
be different eigenvalues and
\ShowEq{di 1n+1}vm{}
corresponding eigenvectors
\ShowEq{fovi=di vi}
\ShowEq{di ne dj}
Let the statement
\RefStatement{ai vi=0}
be true.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0}
There exists linear dependence
\ShowEq{ai vi=0}
where
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

The equality
\ShowEq{ai f vi=0}
follows from the equality
\EqRef{ai vi=0}.
The equality
\ShowEq{ai di vi=0}
follows from the equality
\EqRef{fovi=di vi},
\EqRef{ai f vi=0}.
The equality
\ShowEq{ai (di-dm) vi=0}
follows from the equality
\EqRef{ai vi=0},
\EqRef{ai di vi=0}.
Since
\ShowEq{a1(d1-dm) ne 0}
then the equality
\EqRef{ai (di-dm) vi=0}
is linear dependence between vectors
\ShowEq{v1 vm-1}
This statement contradicts the statement
\RefStatement{theorem is true for k=m-1}.
Therefore, the statement
\RefStatement{ai vi=0}
is not true and vectors
\ShowEq{di 1n+1}vm{}
are linearly independent.
\end{proof}

Let dimension of $D$\Hyph vector space $V$ be $\gin$.
From the theorem
\refTheorem{n eigenvectors}{field},
it follows that
if $\gik=\gin$,
then the set of corresponding eigenvectors
is the basis of $D$\Hyph vector space $V$.\,\footnote{\,
If multiplicity of eigenvalue is greater than $1$,
then dimension of $D$\Hyph vector space
generated by corresponding eigenvectors
maybe less than multiplicity of eigenvalue.
}

Let $\Basis e$ be a basis of $D$\Hyph vector space $V$.
Let $a$ be matrix of endomorphism $\Vector a$ with respect to the basis $\Basis e$ and
\ShowEq{matrix of eigenvector k}
be coordinates of eigenvector $x(\gik)$ with respect to the basis $\Basis e$.
Gather a set of coordinates of eigenvectors
\ShowEq{di 1n+1}vn{}
into the matrix
\ShowEq{matrix of eigenvector 1n}
Then we can write down the equality
\newline
\FrameEqRef{va vx=b vx}P
\newline
using product of matrices
\ShowEq{va vx=b vx matrix}
Since the set of vectors
\ShowEq{di 1n+1}vn{}
is basis of $D$\Hyph vector space $V$,
then the matrix $x$ is non\Hyph singular.
Therefore, the equality
\ShowEq{vx- va vx=b matrix}
follows from the equality
\EqRef{va vx=b vx matrix}.
The equality
\EqRef{vx- va vx=b matrix}
implies that the matrix $a$ is similar to diagonal matrix
\ShowEq{D diagonal matrix}bn

Let $V$ be left $A$\Hyph vector space of columns.
Then the equality
\EqRef{va vx=b vx matrix}
gets form
\ShowEq{vx rc va=vx b matrix}
If we select a column $x(\gik)$
in the equality
\EqRef{vx rc va=vx b matrix},
then we get the equality
\ShowEq{vx rc va=vx b k matrix}
The equality
\EqRef{vx rc va=vx b k matrix}
coincides with the equality
\newline
\FrameEqRef{aox=bx}1
\newline
up to notation.

Thus, we get the definition
of left \CR eigenvalue
which is different from \CR eigenvalue
considered in the subsection
\RefSubsection{Eigenvalue in non-commutative algebra}.
If we similarly consider
right $A$\Hyph vector space of rows,
then get the definition
of right \CR eigenvalue.\,\footnote{\,
In the section
\citeBib{Cohn: Skew Fields}\Hyph 8.2,
professor Cohn considers definition
of left and right eigenvalues of \nTimes matrix.
Cohn traditionally considers product of row over column.
Since there exist two products of matrices,
I slightly changed Cohn's definition.

\FrameCiteBib{Cohn: Skew Fields}
}


==> Preface.Eigen.Eq.tex <==
%auto-ignore

\AddEquation{vx rc va=vx b k matrix}
{
\ShowEq{matrix of eigenvector}k
\CRstar
\PMatrix ann
=
b(\gik)
\ShowEq{matrix of eigenvector}k
}

\AddEq{matrix of eigenvector k}
{
\[
x(\gik)=
\ShowEq{matrix of eigenvector}k
\]
}

\AddEq[1]{matrix of eigenvector}
{
\ColMatrix{x(\gi{#1})}n
}

\AddEq{matrix of eigenvector 1n}
{
\[
x=
\begin{pmatrix}
\displaystyle
\ShowEq{matrix of eigenvector}1
&...&
\displaystyle
\ShowEq{matrix of eigenvector}n
\end{pmatrix}
=
\ShowEq{the matrix of eigenvector 1n}
\]
}

\AddEq{the matrix of eigenvector 1n}
{
\begin{pmatrix}
\aU{x(\gi{1})}1&...&\aU{x(\gi{n})}1
\\...&...&...\\
\aU{x(\gi{1})}n&...&\aU{x(\gi{n})}n
\end{pmatrix}
}

\AddEquation{va vx=b vx matrix}
{
\begin{split}
&\,
\PMatrix ann
\ShowEq{the matrix of eigenvector 1n}
\\=&\,
\ShowEq{the matrix of eigenvector 1n}
\begin{pmatrix}
b(\gi 1)&...&0
\\ ...&...&...\\
0&...&b(\gin)
\end{pmatrix}
\end{split}
}

\AddEquation{vx- va vx=b matrix}
{
\begin{split}
&\,
\ShowEq{the matrix of eigenvector 1n}^{-1}
\PMatrix ann
\ShowEq{the matrix of eigenvector 1n}
\\=&\,
\begin{pmatrix}
b(\gi 1)&...&0
\\ ...&...&...\\
0&...&b(\gin)
\end{pmatrix}
\end{split}
}

\AddEquation{vx rc va=vx b matrix}
{
\begin{split}
&\,
\ShowEq{the matrix of eigenvector 1n}
\CRstar
\PMatrix ann
\\=&\,
\begin{pmatrix}
b(\gi 1)&...&0
\\ ...&...&...\\
0&...&b(\gin)
\end{pmatrix}
\CRstar
\ShowEq{the matrix of eigenvector 1n}
\end{split}
}

\AddEq{characteristic polynomial=0}
{
\[
\ShowEq{characteristic polynomial}=0
\]
}

\AddEquation{(a-bE)x=0}
{
(a-b\aD En)x=0
}

\AddEquation{similar matrices}
{
a_1=f^{-1}af
}

\AddEquation{similar matrices 1}
{
a_1-b\aD En=f^{-1}af-b\aD En=f^{-1}af-f^{-1}b\aD Enf=f^{-1}(a-b\aD En)f
}

\AddEq{basis e e1}
{
$\Basis e$, $\Basis e_1$
}

\AddEq{basis e1=fe}
{
\Basis e_1=f\Basis e
}

\AddEquation{vx=x e}
{
\Vector x=\aU xi\aD ei
}

\AddEq{va vx=b vx}
{
\Vector a\Vector x=b\Vector x
}

\AddEquation{ax=bx}
{
ax=bx
}

\AddEquation{x1=f- x}
{
x_1=f^{-1}x
}

\AddEquation{f1 x1=b x1}
{
a_1x_1=f^{-1}aff^{-1}x=f^{-1}ax=f^{-1}bx=bf^{-1}x=bx_1
}

\AddEq{aox=bx}
{
\Vector a\circ\Vector x=b\Vector x
}

\AddEquation{aox=xb}
{
\Vector a\circ\Vector x=\Vector xb
}

\AddEq{cb ne bc}
{
$cb\ne bc$, $b$, $c\in A$,
}

\AddEquation{a o cx ne b cx}
{
\Vector a\circ(c\Vector x)\ne b(c\Vector x)
}

\AddEquation{x cr a=bx}
{
x\CRstar a=bx
}

\AddEquation{x cr a=xb}
{
x\CRstar a=xb
}

\AddEq{a-bEn}
{
$a-b\aD En$
}

\AddEquation{e1=g cr e}
{
\Basis e_1=g\CRstar\Basis e
}

\AddEquation{a1=g a g-}
{
a_1=
g\CRstar a\CRstar g^{\CRInverse}
}

\AddEquation{a=g- a1 g}
{
a=
g^{\CRInverse}\CRstar a_1\CRstar g
}

\AddEquation{x_1 a_1 g=x_1 g b}
{
x_1\CRstar g\CRstar g^{\CRInverse}\CRstar a_1\CRstar g=x_1\CRstar gb
}

\AddEquation{x cr a=x cr b E}
{
x\CRstar a=x\CRstar (Eb)
}

\AddEquation{aox=b e ox}
{
a\circ x=
\ShowEq{left map a En}b{}
\circ x
}

\AddEquation{ai (di-dm) vi=0}
{
\begin{aligned}
&\,a(\gi 1)(b(\gi 1)-b(\gi m))v(\gi 1) + ...
\\ +&\,a(\gi m-\gi 1)(b(\gi m-\gi 1)-b(\gi m))v(\gi m-\gi 1)
=0
\end{aligned}
}

\AddEq{a1(d1-dm) ne 0}
{
\[
a(\gi 1)(b(\gi 1)-b(\gi m))\ne 0
\]
}

\AddEq{v1 vm-1}
{
$v(\gi 1)$, ..., $v(\gi{m}-\gi 1)$.
}


==> Preface.Eigen.Russian.tex <==
%auto-ignore
\input{Preface.Eigen.Eq}

\section{Собственное значение матрицы}
\labelSection{paper Eigenvalue of Matrix}

\subsection{Собственное значение в коммутативной алгебре}
\labelSubsection{Eigenvalue in commutative algebra}

Я начну с определения собственного значения матрицы
в коммутативной алгебре.\,\footnote{\,
Смотри также определение на странице
\citeBib{Kurosh: High Algebra}\Hyph 207.
}

Пусть $a$ - \nTimes матрица, элементы которой
принадлежат полю $F$.
Многочлен
\DrawEq{characteristic polynomial}{}
где \aD En - \nTimes единичная матрица,
называется характерисическим многочленом матрицы $a$.
Корни характеристического многочлена называются
собственными значениями матрицы $a$.
Следовательно, собственные значения матрицы $a$
удовлетворяют уравнению
\ShowEq{characteristic polynomial=0}
и система линейных уравнений
\ShowEq{(a-bE)x=0}
имеет нетривиальное решение,
если $b$ - собственное значение матрицы $a$.

Если матрицы $a$ и $a_1$ подобны
\ShowEq{similar matrices}
то из равенства
\ShowEq{similar matrices 1}
следует, что матрицыs $a$ and $a_1$
имеют одинаковые характеристические многочлены,
и, следовательно, одинаковые характеристические корни.

Пусть $V$ - векторное пространство над полем $F$.
Пусть
\ShowEq{basis e e1}
- базисы векторного пространства $V$
и $f$ - координатная матрица базиса $\Basis e_1$
относительно базиса $\Basis e$
\DrawEq{basis e1=fe}1
Пусть $a$ - матрица эндоморфизма $\Vector a$
относительно базиса $\Basis e$.
Тогда матрица $a_1$, определённая равенством
\EqRef{similar matrices},
является матрицей эндоморфизма $\Vector a$
относительно базиса $\Basis e_1$.
Если мы отождествляем эндоморфизм
и его матрицу относительно заданного базиса,
то мы будем говорить, что собственные значения эндоморфизма
- это собственные значения его матрицы относительно заданного базиса.
Следовательно, собственные значения эндоморфизма
не зависят от выбора базиса.

Если мы положим
\ShowEq{vx=x e}
то равенство
\EqRef{(a-bE)x=0}
принимает вид
\DrawEq{va vx=b vx}P
\ShowEq{ax=bx}
относительно базиса $\Basis e$.
Пусть $f$ - координатная матрица базиса $\Basis e_1$
относительно базиса $\Basis e$
\FrameEqRef{basis e1=fe}1.
Тогда координатная матрица $x_1$ вектора $\Vector x$ 
относительно базиса $\Basis e_1$ имеет вид
\ShowEq{x1=f- x}
Равенство
\ShowEq{f1 x1=b x1}
является следствием равенств
\EqRef{similar matrices},
\EqRef{ax=bx},
\EqRef{x1=f- x}.
Следовательно, равенство
\eqRef{va vx=b vx}P
не зависит от выбора базиса,
и мы будем говорить, что собственный вектор эндоморфизма
- это собственный вектор его матрицы относительно заданного базиса.

Множество собственных значений эндоморфизма $\Vector a$
с учётом их кратности в характеристическом многочлене
называется спектром эндоморфизма $\Vector a$.

\subsection{Собственное значение в некоммутативной алгебре}
\labelSubsection{Eigenvalue in non-commutative algebra}

Пусть $A$ -
некомутативная $D$\Hyph алгебра $A$ с делением.
Если мы рассматриваем векторное пространство над
$D$\Hyph алгеброй $A$,
то мы хотим сохранить определение
собственного числа и собственного вектора,
рассмотренное в случае
векторного пространства
над коммутативной алгеброй.

Пусть $V$ - левое $A$\Hyph векторное пространство столбцов.
Поскольку произведение некоммутативно, возникает вопрос.
Должны мы пользоваться равенством
\DrawEq{aox=bx}1
или равенством
\ShowEq{aox=xb}

Равенство
\eqRef{aox=bx}1
выглядит естественно,
так как в правой части записанно
левостороннее произведение
вектора на скаляр.
Однако, если
\ShowEq{cb ne bc}
то
\ShowEq{a o cx ne b cx}

\begin{Statement}
\labelStatement{set do not generate vector space}
Из утверждения
\EqRef{a o cx ne b cx}
следует, что множество векторов $\Vector x$,
удовлетворяющих равенству
\eqRef{aox=bx}1,
не порождает подпространство векторного пространства.
\hfill\(\odot\)
\end{Statement}

Если мы запишем равенство
\eqRef{aox=bx}1
с помощью матриц, то мы получим равенство
\ShowEq{x cr a=bx}
Равенство
\EqRef{x cr a=bx}
является системой линейных уравнений относительно множества неизвестных $x$.
Однако мы не можем сказать, что эта система линейных уравнений вырождена
и имеет бесконечно много решений.
Но это утверждение является очевидным следствием утверждения
\RefStatement{set do not generate vector space}.

Создаётся впечатление, что равенство
\eqRef{aox=bx}1
не годится для определения собственного значения.
Однако мы вернёмся к этому определению в разделе
\RefSection{Left and Right Eigenvalues}.

Рассмотрим равенство
\EqRef{aox=xb}.
Пусть $a$ - матрица эндоморфизма $\Vector a$
относительно базиса $\Basis e$
левого $A$\Hyph векторного пространства столбцов.
Пусть $a$ - матрица вектора $\Vector x$
относительно базиса $\Basis e$.
Система линейных уравнений
\ShowEq{x cr a=xb}
является следствием уравнения
\EqRef{aox=xb}.
Система линейных уравнений
\EqRef{x cr a=xb}
имеет нетривиальное решение, если матрица
\ShowEq{a-bEn}
\CR вырождена.
В этом случае, система линейных уравнений
\EqRef{x cr a=xb}
имеет бесконечно много решений.

На первый взгляд,
рассмотренная модель соответствует модели,
рассмотренной в разделе
\RefSubsection{Eigenvalue in commutative algebra}.
Однако, если мы выберем другой базис $\Basis e_1$
\ShowEq{e1=g cr e}
то изменятся матрица $a$
\ShowEq{a1=g a g-}
\ShowEq{a=g- a1 g}
и матрица $x$
\DrawEq[x1x{}g{}{left}{cols}]{v2=v1g-}1
\DrawEq[x{}x1g{}]{v1=v2*a left-cols}{P1}
Равенство
\ShowEq{x_1 a_1 g=x_1 g b}
является следствием равенств
\EqRef{x cr a=xb},
\EqRef{a=g- a1 g},
\eqRef{v1=v2*a left-cols}{P1}.
Из равенства
\EqRef{x_1 a_1 g=x_1 g b}
следует, что вектор\Hyph столбец $x_1$
не является решением системы линейных уравнений
\EqRef{x cr a=xb}.
Это противоречит утверждению, что равенство
\EqRef{aox=xb}
не зависит от выбора базиса.

Равенство
\EqRef{aox=xb}
требует более внимательного анализа.
В правой части равенства
\EqRef{aox=xb}
записана операция, которая не определена
в левом $A$\Hyph векторном пространстве,
а именно, правостороннее умножение вектора на скаляр.
Однако мы можем записать систему линейных уравнений
\EqRef{x cr a=xb}
иначе
\ShowEq{x cr a=x cr b E}
где $E$ - единичная матрица.
В правой части равенства
\EqRef{x cr a=x cr b E}
также как и в левой части
записано \CR произведение вектор\Hyph столбца
на матрицу эндоморфизма.
Следовательно, левая и правая части
имеют один и тот же закон преобразования
при замене базиса.

По аналогии с векторным пространством над полем,
эндоморфизм
\ShowEq{left map a En}b,
который имеет матрицу $Eb$ относительно базиса $\Basis e$,
называется преобразованием подобия относительно базиса $\Basis e$.
Следовательно, мы должны записать равенство
\EqRef{aox=xb}
в виде
\ShowEq{aox=b e ox}

Равенство
\EqRef{aox=b e ox}
является определением собственного значения $b$
и собственного вектора $x$ эндоморфизма $a$.
Если мы рассматриваем матрицу эндоморфизма $a$
относительно базиса $\Basis e$
левого $A$\Hyph векторного пространства столбцов,
то равенство
\EqRef{x cr a=xb}
является определением \CR собственного значения $b$
и собственного вектора $x$, соответствующего
\CR собственному значению $b$.

\section{Левые и правые собственные значения}
\labelSection{Left and Right Eigenvalues}

Чтобы лучше разобраться с природой собственных значений,
рассмотрим следующую теорему.

\ShowEq{def DVector}
\ShowTheorem{n eigenvectors}{field}

\begin{proof}
Мы будем доказывать теорему индукцией по $\gik$.

Поскольку собственный вектор отличен от нуля, теорема верна для $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1}
Пусть теорема верна для $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
Пусть
\ShowEq{di 1n+1}bm{}
- различные собственные значения и
\ShowEq{di 1n+1}vm{}
- соответствующие собственные векторы
\ShowEq{fovi=di vi}
\ShowEq{di ne dj}
Пусть утверждение
\RefStatement{ai vi=0}
верно.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0}
Существует линейная зависимость
\ShowEq{ai vi=0}
где
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

Равенство
\ShowEq{ai f vi=0}
является следствием равенства
\EqRef{ai vi=0}.
Равенство
\ShowEq{ai di vi=0}
является следствием равенства
\EqRef{fovi=di vi},
\EqRef{ai f vi=0}.
Равенство
\ShowEq{ai (di-dm) vi=0}
является следствием равенства
\EqRef{ai vi=0},
\EqRef{ai di vi=0}.
Так как
\ShowEq{a1(d1-dm) ne 0}
то равенство
\EqRef{ai (di-dm) vi=0}
является линейной зависимостью между векторами
\ShowEq{v1 vm-1}
Это утверждение противоречит утверждению
\RefStatement{theorem is true for k=m-1}.
Следовательно, утверждение
\RefStatement{ai vi=0}
не верно и векторы
\ShowEq{di 1n+1}vm{}
линейно независимы.
\end{proof}

Пусть $D$\Hyph векторное пространство имеет размерность $\gin$.
Из теоремы
\refTheorem{n eigenvectors}{field}
следует, что
если $\gik=\gin$,
то множество соответствующих собственных векторов
является базисом $D$\Hyph векторного пространства $V$.\,\footnote{\,
Если кратность собственного значения больше чем $1$,
то размерность $D$\Hyph векторного прострвнства,
порождённого соответствующими собственными векторами,
может быть меньше кратности собственного значения.
}

Пусть $\Basis e$ - базис $D$\Hyph векторного пространства $V$.
Пусть $a$ - матрица эндоморфизма $\Vector a$ относительно базиса $\Basis e$ и
\ShowEq{matrix of eigenvector k}
координаты собственного вектора $x(\gik)$ относительно базиса $\Basis e$.
Соберём множество координат собственных векторов
\ShowEq{di 1n+1}vn{}
в матрицу
\ShowEq{matrix of eigenvector 1n}
Тогда мы можем записать равенство
\newline
\FrameEqRef{va vx=b vx}P
\newline
используя произведение матриц
\ShowEq{va vx=b vx matrix}
Так как множество векторов
\ShowEq{di 1n+1}vn{}
является базисом $D$\Hyph векторного пространства $V$,
то матрица $x$ - не вырождена.
Следовательно, равенство
\ShowEq{vx- va vx=b matrix}
является следствием равенства
\EqRef{va vx=b vx matrix}.
Из равенства
\EqRef{vx- va vx=b matrix}
следует, что матрица $a$ подобна диагональной матрице
\ShowEq{D diagonal matrix}bn

Пусть $V$ - левое $A$\Hyph векторное пространство столбцов.
Тогда равенство
\EqRef{va vx=b vx matrix}
приобретает вид
\ShowEq{vx rc va=vx b matrix}
Если мы в равенстве
\EqRef{vx rc va=vx b matrix}
выделим столбец $x(\gik)$,
то мы получим равенство
\ShowEq{vx rc va=vx b k matrix}
Равенство
\EqRef{vx rc va=vx b k matrix}
с точностью до обозначений
совпадает с равенством
\newline
\FrameEqRef{aox=bx}1
%\newline

Таким образом, мы получаем определение
левого \CR собственного значения,
которое отличается от \CR собственного значения,
рассмотренного в разделе
\RefSubsection{Eigenvalue in non-commutative algebra}.
Если мы аналогичным образом рассмотрим
правое $A$\Hyph векторное пространство строк,
то мы получаем определение
правого \CR собственного значения.\,\footnote{\,
В разделе
\citeBib{Cohn: Skew Fields}\Hyph 8.2,
профессор Кон рассматривает определение
левого и правого собственных значений \nTimes матрицы.
Кон по традиции рассматривает произведение строки на столбец.
Поскольку существует две операции произведения матриц,
я слегка изменил определение Кона.

\FrameCiteBib{Cohn: Skew Fields}
}


==> Preliminary.Omega.Russian.tex <==
%auto-ignore
\input{Preliminary.Omega.Eq}

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Chapter{Интеграл Лебега в абелевой \texorpdfstring{$\Omega$}{Omega}-группе}
\fi

\ePrints{5148-4632,2307.09982,5410-9916,4975-6381,1601.03259,309618526,CACAA.06.121}
\Items{8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\Section{\texorpdfstring{$\Omega$}{Omega}-группа}

\begin{ShadedDefinition}
\labelDefinition{additive map}
Пусть в $\Omega$\Hyph алгебре
$A$ определена операция сложения.
Отображение
\ShowEq{f:A->B}fAA
$\Omega_1$\Hyph алгебры $A$
называется
\AddIndex{аддитивным отображением}{additive map},
если
\ShowEq{f(a+b)=}
\end{ShadedDefinition}

\ShowDefinition{polyadditive map}

\ShowDefinition{Omega group}

\ShowTheorem{operation is distributive over addition}
\begin{proof}
Теорема является следствием определений
\RefDefinition{polyadditive map},
\RefDefinition{Omega group}.
\end{proof}

\ShowEq{contents: norm on Omega group}
\fi

\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\Section{Представление мультипликативной \texorpdfstring{$\Omega$}{Omega}-группы}
\fi
\ePrints{5410-9916,4975-6381,1601.03259}
\ifx\Semafor\ValueOff
\ShowDefinition{multiplicative Omega group}
\fi

\ifx\texFuture\Defined
\begin{ShadedDefinition}
\labelDefinition{multiplicative map}
{\it
Пусть $A$, $B$ -
мультипликативные $\Omega$\Hyph группы.
Отображение
\ShowEq{f:A->B}fAB
называется
\AddIndex{мультипликативным}{multiplicative map},
если
\DrawEq{f(ab)=f(a)f(b)}{}
}
\end{ShadedDefinition}
\fi

\ePrints{5148-4632,2307.09982,8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn
\ShowDefinition{Abelian multiplicative Omega group}

\ShowDefinition{Omega ring}

\ShowTheorem{product in Omega ring is distributive over addition}
\ShowProof{product in Omega ring is distributive over addition}

\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOff
\ShowDefinition{matrix over Omega ring}

\ShowConvention{Einstein summation}

\ShowText{matrix operations}

\ShowDefinition{biring matrix}

\ShowTheorem{transpose of identity}
\ShowProof{transpose of identity}

\ShowTheorem{duality principle for biring}

\ShowTheorem{duality principle for biring of matrices}

\ShowEq{remark: reducible biring}
\fi
\fi
\fi

\ePrints{aaa}
\ifx\Semafor\ValueOn
\begin{ShadedDefinition}
\labelDefinition{orbit of left-side representation}
Пусть отображение
\ShowEq{f:A->*B}g{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2{}
мы определим
\AddIndex{орбиту представления}{orbit of representation}
мультипликативной $\Omega$\Hyph группы $A_1$ как множество
\ShowEq{orbit of representation}
}
\end{ShadedDefinition}
\fi

\ePrints{5148-4632,2307.09982,5284-0163,1801.01628,8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\Section{Представление мультипликативной \texorpdfstring{$\Omega$}{Omega}-группы}
\fi

Мы предполагаем, что преобразования представления
\ShowEq{f:A->*B}g{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
могут действовать на $A_2$\Hyph числа либо слева, либо справа.
Мы должны рассматривать эндоморфизм $\Omega_2$\Hyph алгебры $A_2$ как оператор.
При этом должны быть выполнены следующие условия.

\ShowText{representation of group}

\ShowDefinition{Left side covariant representation}
\ShowDefinition{Left side contravariant representation}

\ShowTheorem{left right shift}
\ProofTheorem{\RefRepresentation}{left right shift}

\ShowEq{def left}
\ShowDefinition{orbit of representation}

\ShowEq{def right}
\ShowDefinition{orbit of representation}

\ShowTheorem{proper definition of orbit}
\ProofTheorem{\RefRepresentation}{proper definition of orbit}

\ShowTheorem{duality principle, algebra representation}

\ShowTheorem{single transitive representation of group}
\ProofTheorem{\RefRepresentation}{single transitive representation of group}

\ShowTheorem{shifts on group commuting}
\ShowProof{shifts on group commuting}

\ShowTheorem{two representations of group}
\ShowProof{two representations of group}

\ShowDefinition{twin representations}

\ShowRemark{one representation of group}
\fi

\ePrints{5148-4632,8428-0408,8525-2526,2207.06506}%2307.09982
\ifx\Semafor\ValueOn

\Section{Тензорное произведение представлений}

\ShowDefinition{reduced polymorphism of representations}

\ShowDefinition{tensor product of representations}

\ShowTheorem{tensor product of representations}
\ProofTheorem{\RefRepresentation}{tensor product of representations}

\ShowTheorem{representation, tensor product}
\ProofTheorem{\RefRepresentation}{representation, tensor product}

\ShowTheorem{tensor product and polymorphism}
\ProofTheorem{\RefRepresentation}{tensor product and polymorphism}

\ShowTheorem{B times->B otimes}
\ProofTheorem{\RefRepresentation}{B times->B otimes}
\fi

\ePrints{4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn

\Section{Алгебра множеств}

\ShowEq{contents: Algebra of Sets}

\Section{Интеграл Лебега}

\ShowEq{contents: Lebesgue Integral}

\ShowEq{PreliminaryRefOmegaNormOff}
\ShowEq{PreliminaryRefMeasureOff}
\fi


==> Preliminary.Representation.Russian.tex <==
%auto-ignore
\input{Preliminary.Representation.Eq}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOff
\Chapter{Представление универсальной алгебры}

\ShowText{Preliminary Definitions}
\fi

\ePrints{4975-6381,1506.00061,8428-0408,8525-2526,2207.06506,5148-4632,1908.04418,6860-2955}
\Items{1601.03259,5410-9916,9835-2163,7287-9339,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Отношение эквивалентности}

\begin{\DefinitionStyle}
\labelDefinition{equivalence}
Соответствие
\ShowEq{Phi in AxA}
называется
\AddIndex{отношением эквивалентности}{equivalence},
если\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
соответствие $\Phi$
\AddIndex{рефлексивно}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
соответствие $\Phi$
\AddIndex{симметрично}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
соответствие $\Phi$
\AddIndex{транзитивно}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 27.
}

\begin{\TheoremStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
является отношением эквивалентности и
называется
\AddIndex{ядром отображения}{kernel of map}.\,\footnotemark
\end{\TheoremStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 28.
}
\begin{proof}
\begin{ShadedLemma}
\labelLemma{ker - reflexive correspondence}
{\it
Соответствие
\ShowEq{ker f}
рефлексивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Из равенства
\ShowEq{fa=fa}
и определения
\EqRef{def kernel of map}
следует, что
\DrawEq[aa]{ab in ker}{aa}
Лемма является следствием утверждения
\eqRef{ab in ker}{aa}
и определения
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - symmetric correspondence}
{\it
Соответствие
\ShowEq{ker f}
симметрично.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab symmetric}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ba]{fa=fb}{ba}
является следствием равенства
\eqRef{fa=fb}{ab symmetric}.
Утверждение
\DrawEq[ba]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ba}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab in ker -> ba in ker}
Лемма является следствием утверждения
\EqRef{ab in ker -> ba in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - transitive correspondence}
{\it
Соответствие
\ShowEq{ker f}
транзитивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab transitive}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[bc]{fa=fb}{bc}
является следствием утверждения
\DrawEq[bc]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ac]{fa=fb}{ac}
является следствием равенств
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
Утверждение
\DrawEq[ac]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ac}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab,ac in ker -> ac in ker}
Лемма является следствием утверждения
\EqRef{ab,ac in ker -> ac in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

Утверждение теоремы является следствием лемм
\ShowEq{lemmas for ker}
и определения
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Универсальная алгебра}
\fi

\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{image of map}
\ShowEq{show image of map}
называется
\AddIndex{образом отображения}{image of map}
$f$.
\end{\DefinitionStyle}
\fi

\ePrints{5410-9916,9835-2163,5284-0163,1801.01628,8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOff
\begin{\TheoremStyle}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\,\footnotemark
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnotemark
\end{\TheoremStyle}
\ShowPrevFootnote{
Утверждение теоремы
\RefTheorem{maps and kernel equivalence}
аналогично утверждению на с. \citeBib{Serge Lang}-94.
}
\ShowNextFootnote{
Определение универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.
}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}
\fi

\begin{\DefinitionStyle}
\labelDefinition{Cartesian power}
Для любых множеств\,\footnotemark
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}

\begin{\DefinitionStyle}
\labelDefinition{operation on set}
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnotemark
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\ShowEq{b1n in B}aA,
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
\end{\DefinitionStyle}
\footnotetext{\,
\ePrints{2307.09982,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}

\ePrints{9835-2163,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{\DefinitionStyle}
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnotemark
\ShowEq{operator domain}
вместе с отображением
\ShowEq{f:A->B}a{\Omega}N
Если
\ShowEq{omega in Omega}{},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\begin{\DefinitionStyle}
\labelDefinition{Omega-algebra}
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnotemark
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
\fi
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\ePrints{9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOff
Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\ShowEq{omega n ari}{}{}n{}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\ShowEq{b1n in B}bB,
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{omega in Omega}{}{}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\fi

\ShowFootnote{iso end aut morphism}1

\begin{\DefinitionStyle}
\labelDefinition{homomorphism}
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\ShowEq{omega n ari}{}{}n.
Отображение\,\refFootnote{iso end aut morphism}1
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\ShowEq{b1n in B}aA,
\DrawEq[fa]{afo=aof}{}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{omega in Omega}{}.
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
\end{\DefinitionStyle}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{\TheoremStyle}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955,8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn
\ShowFootnote{iso end aut morphism}2

\begin{\DefinitionStyle}
\labelDefinition{isomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAB
назывется\,\refFootnote{iso end aut morphism}2
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
\end{\DefinitionStyle}
\fi

\begin{\DefinitionStyle}
\labelDefinition{endomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAA
источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{1908.04418,6860-2955}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{1601.03259,2307.09982,5148-4632,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
Изоморфизм
\ShowEq{f:A->B}fAA
называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
\end{\DefinitionStyle}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{1908.04418,6860-2955,2207.06506,8525-2526}%
\ifx\Semafor\ValueOn
\begin{\TheoremStyle}
\labelTheorem{product of homomorphisms}
Пусть отображение
\DrawEq[fAB{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебры $B$.
Пусть отображение
\DrawEq[gBC{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $B$
в $\Omega$\Hyph алгебры $C$.
Тогда отображение\,\footnotemark
\DrawEq[{h=g\circ f}AC{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебры $C$.
\end{\TheoremStyle}
\footnotetext{\,
Я следую предложению
\citeBib{Cohn: Universal Algebra}\Hyph 3.2
на странице
\citeBib{Cohn: Universal Algebra}\Hyph 71.
}
\begin{proof}
Пусть
\ShowEq{omega in Omega}n{}
- n\Hyph арная операция.
Тогда
\DrawEq[fa]{afo=aof}{fa}
для любых
\ShowEq{b1n in B}aA,
и
\DrawEq[gb]{afo=aof}{gb}
для любых
\ShowEq{b1n in B}bB.
Равенство
\ShowEq{agfo=aogf}
является следствием равенств
\eqRef{afo=aof}{fa},
\eqRef{afo=aof}{gb}.
Теорема является следствием равенства
\EqRef{agfo=aogf}
для любой операции $\omega$.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339}%
\Items{8428-0408,1601.03259,2307.09982,5148-4632,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
\begin{\DefinitionStyle}
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
\end{\DefinitionStyle}
\fi
\fi

\ePrints{2307.09982,5148-4632,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowConvention{A number}{\Omega}{алгебры}
\fi

\ePrints{1908.04418,6860-2955,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ePrints{8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{universally attracting object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально притягивающим}{universally attracting},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fRP
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{universally repelling object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально отталкивающим}{universally repelling},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fPR
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{product in category, 2020}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A(Bi)}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
Универсально притягивающий объект категории
\ShowEq{category A(Bi)}
\ShowEq{product in category}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}.\,\footnotemark

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
\end{\DefinitionStyle}
\footnotetext{\,
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 45.
}

\begin{\TheoremStyle}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Произведение множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$
- это объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
такие, что
для любого объекта $R$ и множества морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием определений
\RefDefinition{universally attracting object of category},
\RefDefinition{product in category, 2020}.
\end{proof}
\else
\ShowDefinition{product in category}
\fi

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{\,
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{\TheoremStyle}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
\labelItem{set A is Cartesian product}
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}A{}
\item
\labelItem{homomorphism is projection on factor}
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}A{}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\ShowEq{ref product in category}
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\end{proof}

\begin{\DefinitionStyle}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}A.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}A{}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Ai iI}B.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{\TheoremStyle}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}A{}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}B.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{\DefinitionStyle}
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnotemark
на $A$.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}

\begin{\TheoremStyle}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}

\ePrints{8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{coproduct in category}

\ShowTheorem{coproduct in category}
\ShowProof{coproduct in category}
\fi
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega n ari}{}{}2{}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega n ari}{}{}2.
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega n ari}{}{}2{}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{\DefinitionStyle}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,8428-0408,8525-2526,2207.06506,1601.03259,5148-4632}%
\Items{2307.09982,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOn%
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\ShowDefinition{representation of algebra}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{\DefinitionStyle}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnotemark
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}

\ePrints{2307.09982,5148-4632}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnotemark
\ShowEq{fam ne fbm}
\end{\TheoremStyle}
\footnotetext{\,
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ProofTheorem{\RefRepresentation}{representation is effective}
\fi

\ePrints{1506.00061,7287-9339,5284-0163,1801.01628,8525-2526,2207.06506,8428-0408}%
\ifx\Semafor\ValueOn%
\begin{\DefinitionStyle}
\labelDefinition{free representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что $a=b$.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{\TheoremStyle}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{\DefinitionStyle}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnotemark
если для любых
\ShowEq{ab in A}2{}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}

\ShowTheorem{Representation is single transitive iff}
\ShowProof{Representation is single transitive iff}

\ShowTheorem{single transitive representation generates algebra}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\ShowDefinition{morphism of representations of universal algebra}

\ShowRemark{morphism of representations of universal algebra as map}

\ePrints{5148-4632,2307.09982,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\ShowRemark{notation for morphism of representations}

\ShowTheorem{Tuple of maps is morphism of representations iff}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\ShowRemark{morphism of representations of universal algebra}
\fi

\ShowDefinition{morphism of representation f}

\ePrints{aa}%2307.09982,5148-4632}
\ifx\Semafor\ValueOn

\ShowTheorem{unique morphism of representations of universal algebra}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\ShowDefinition{transformation coordinated with equivalence}

\ShowTheorem{transformation correlated with equivalence}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\ShowTheorem{decompositions of morphism of representations}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}

\ShowTheorem{map is reduced morphism of representations iff}
\ProofTheorem{\RefRepresentation}{map is reduced morphism of representations iff}
\fi

\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn

\ShowDefinition{category of representations A1(mA2)}

\ShowTheorem{product of effective representations}
\ProofTheorem{\RefRepresentation}{product of effective representations}
\fi

\ePrints{5148-4632,2307.09982,5410-9916,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\ShowDefinition{stable set of representation}

\ShowTheorem{subrepresentation of representation}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\ShowTheorem{lattice of subrepresentations}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

\ShowRemark{closure operator, representation}

\ShowDefinition{generating set of representation}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{word of element relative to set, representation}

\ShowTheorem{map of words of representation}
\ProofTheorem{\RefRepresentation}{map of words of representation}

\ShowDefinition{quasibasis of representation}

\ShowTheorem{X is quasibasis of representation}
\ProofTheorem{\RefRepresentation}{X is quasibasis of representation}

\ShowRemark{X is quasibasis of representation}

\ShowRemark{representation in form of Omega2-word is ambiguous}

\ShowRemark{three reasons of ambiguity in Omega2-word}

\ShowDefinition{equivalence on the set of Omega2-words}

\ShowTheorem{equivalence generated by basis}
\ProofTheorem{\RefRepresentation}{equivalence generated by basis}

\ShowDefinition{basis of representation}
\else
\begin{\DefinitionStyle}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}
\fi

\ShowTheorem{automorphism uniquely defined by image of basis}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn

\Section{Диаграмма представлений универсальных алгебр}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Мы можем проиллюстрировать определение
\RefDefinition{diagram of representations}
с помощью теоремы
\RefTheorem{diagram of representations, define map fik}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
\fi

\ePrints{2307.09982,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{\DefinitionStyle}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnotemark
}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\ShowEq{set a1n}{}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\ShowDefinition{parity of permutation}
\fi

\ShowEq{PreliminaryRefOff}


==> Prolog.Cite.Russian.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}

\DefCiteBib{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}

\DefCiteBib{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М.,
Наука, 1974
}

\DefCiteBib{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}

\DefCiteBib{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}

\DefCiteBib{2207.06506}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 1, Алгебра с делением\\
eprint \href{http://arxiv.org/abs/2207.06506}{arXiv:2207.06506} (2022)
}


==> Prolog.Russian.tex <==
%auto-ignore
\ifx\setCACAA\Defined
\maketitle
\input{Prolog.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\DefText{Preliminary Definitions}
{
\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339,309618526,CACAA.06.121,0767-8264}
\ifx\Semafor\ValueOn%
\Chapter{Предварительные определения}

\ShowText{Preliminary Definitions}
\fi


==> Representation.Coproduct.Russian.tex <==
%auto-ignore

\input{Representation.Coproduct.Eq}

%\chapter{Копроизведение представлений}

%\section{Копроизведение универсальных алгебр}

\section{Прямая сумма абелевых групп}

\ShowText{Direct Sum of Abelian Groups}

\begin{\TheoremStyle}
\labelTheorem{A=ker+im}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм абелевых групп.
Если $\im f$ - свободная группа, то
\ShowEq{A=ker+im}
\end{\TheoremStyle}

\begin{proof}
Поскольку
\ShowEq{A/ker=im}
равенство
\EqRef{A=ker+im}
является следствием равенства
\EqRef{B=Ao+B/A}.
\end{proof}

\section{Унитальное расширение кольца}

\ShowText{Unital Extension of Ring}nZdD


==> Similarity.Transformation.Russian.tex <==
%auto-ignore
\input{Similarity.Transformation.Eq}

\chapter{Преобразование подобия}

Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.

\section{Преобразование подобия в левом \texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{def left}
\ShowText{Similarity Transformation}

\section{Преобразование подобия в правом \texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{def right}
\ShowText{Similarity Transformation}

\section{Парные представления \texorpdfstring{$D$}{D}-алгебры с делением}

\ShowText{Twin Representations}

\section{\texorpdfstring{\AoxA A}{AoxA}\hyph модуль}
%\labelSection{A Vector Space}

\ShowEq{theorem, representation Ao2->V}

\begin{proof}
Согласно теоремам
\refTheorem{set of similarity transformations}{right},
\refTheorem{set of similarity transformations}{left},
для заданного $v\in V$,
отображение
\ShowEq{p:ab->}
билинейно.
Согласно теореме
\RefTheorem{tensor product and polylinear map},
для заданного $v\in V$,
существует отображение
\ShowEq{h aoxb=p ab}
\ShowEq{h:aoxb->}
Так как $v\in V$ - произвольно,
то для любых $a$, $b$
\ShowEq{h aoxb}
является отображением
\ShowEq{h aoxb:->}
Согласно теоремам
\refTheorem{similarity transformation}{right-cols},
\refTheorem{similarity transformation}{left-cols},
(а также
\refTheorem{similarity transformation}{right-rows},
\refTheorem{similarity transformation}{left-rows})
\ShowEq{h aoxb in L}

Если в $D$\Hyph модуле \AoxA A
определить произведение
\DrawEq[ab]{product in algebra AA}{}
то $D$\Hyph модуле \AoxA A
является $D$\Hyph алгеброй.
Из равенств
\ShowEq{homomorphism AA}
следует, что отображение
\ShowEq{homomorphism AA 1}
является гомоморфизмом.
Следовательно, отображение $h$ является представлением.
\end{proof}

Согласно теоремам
\RefTheorem{representation Ao2->V left},
\RefTheorem{representation Ao2->V right},
существует три различных представления
$D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Выбор того или иного представления
зависит от рассматриваемой задачи.

Например, множество решений системы линейных уравнений
\ShowEq{system of linear equations}
в алгебре кватернионов является правым $H$\Hyph векторным пространством.
Левая линейная комбинация решений вообще говоря
решением не является.
Однако есть задачи, в которых мы вынуждены отказаться от простой модели
и одновременно рассматривать обе структуры векторного пространства.

Пусть $V$ - левый \AoxA A\Hyph модуль.
Если $v$, $w\in V$, то для любых $a$, $b$, $c$, $d\in A$
\ShowEq{A linear combination}
Выражение
\EqRef{A linear combination}
называется
\AddIndex{линейной комбинацией векторов}{linear combination of vectors}
левого \AoxA A\Hyph модуля $V$.

\ShowEq{def basis, AoxA module}

\section{Собственное значение эндоморфизма}

\ShowText{Eigenvalue of Endomorphism}

\section{Собственное значение матрицы}

\ShowEq{Eigenvalue of Matrix}


==> Statement.Russian.tex <==
%auto-ignore

\def\OneTheorem{теоремы }
\def\ManyTheorems{теорем }

\newenvironment{ProofRef}[2]{%
\def\TheoremList{theorem}
\def\TheoremRef{}

{\sc Доказательство теоремы}
\def\Temp{}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\RefTheorem{#1}.
\else
\refTheorem{#1}{#2}.
\fi
}%
{\qed}

\author{Александр Клейн}
\ifx\setCACAA\undefined
\newtheorem{theorem}{Теорема}[section]
\newtheorem{corollary}[theorem]{Следствие}
\newtheorem{example}[theorem]{Пример}
\newtheorem{definition}[theorem]{Определение}
\newtheorem{remark}[theorem]{Замечание}
\newtheorem{question}[theorem]{Вопрос}
\newtheorem{summary}[theorem]{Сводка результатов}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Лемма}
\else
\theoremstyle{definition}
\theoremstyle{remark}
\fi
\newtheorem{Statement}[theorem]{Утверждение}
\newtheorem{convention}[theorem]{Соглашение}
\newtheorem{xca}[theorem]{Exercise}
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{Список литературы}%
}
\else
\newcommand{\BibTitle}{%
\chapter{Список литературы}%
}
\fi


==> Stmt.2021.11.26.Russian.tex <==
%auto-ignore
\input{Stmt.2021.11.26.Eq}

\DefText{Left-sided Polynomial}
{
В разделе
\citeBib{Cohn: Algebra 1}\Hyph 6.4,
профессор Кон рассмотрел определение левосторонего многочлена,
не опираясь на определение кольца Оре.

Пусть $A$ - ассоциативная алгебра.

На странице
\citeBib{Cohn: Algebra 1}\Hyph 148,
профессор Кон рассмотрел множество
\ShowEq{set of left-sided Polynomials}
левостороних многочленов,
где левостороний многочлен определён
как формальное выражение
\DrawEq[fan]{Left-sided Polynomial}{fan}
\DrawEq[gbm]{Left-sided Polynomial}{gbm}
где
\ShowEq{a1n b1m}
- $A$\Hyph числа
и $x$ - переменная.

Левостороние многочлены $f$ и $g$ равны, если
\ShowEq{a1n=b1m}

Мы также определим на множестве
\ShowEq{set of left-sided Polynomials}
сумму\,\footnote{\,
Если $m<n$, например, то мы положим
\ShowEq{bmn=0}
}
левостороних многочленов $f$ и $g$
\ShowEq{sum of left-sided polynomials f and g}
и произведение
\ShowEq{product of left-sided polynomials f and g}

Нетрудно убедиться, что множество
\ShowEq{set of left-sided Polynomials}
является $D$\Hyph алгеброй.
Очевидно, что левостороний многочлен $f$
является многочленом $f$.
Однако произведение левостороних многочленов $f$ и $g$,
вообще говоря,
не равно произведению многочленов $f$ и $g$.
}

\DefText{Ore introduced the transformation of monomial}
{
В книге
\citeBib{Cohn: Skew Fields}
на странице 48,
профессор Кон писал, что изучать многочлены
над не коммутативным полем - сложная задача.
Поэтому профессор Оре рассмотрел
кольцо правых косых многочленов\,\footnote{\,
Смотри также определение на страницах
\citeBib{Cohn: Skew Fields}\Hyph(48 - 49).
}
где Оре определил преобразование одночлена
\DrawEq{at=taa+ad}1
Отображение
\ShowEq{map a in A}{\alpha}
является эндоморфизмом $D$\Hyph алгебры $A$
и отображение
\ShowEq{map a in A}{\delta}
является $\alpha$\Hyph дифференцированием $D$\Hyph алгебры $A$
\ShowEq{alpha derivation of algebra}
В этом случае
все коэффициенты многочлена могут быть записаны справа.
Подобные многочлены называются правостороними многочленами.

Аналогично мы можем рассматривать
преобразование одночлена
\ShowEq{ta=aat+ad}
В этом случае
все коэффициенты многочлена могут быть записаны слева.
Подобные многочлены называются левостороними многочленами.\,\footnote{\,
Смотри также определение на странице
\citeBib{1702.04935}\Hyph 3.
}

Точка зрения, предложенная Оре,
позволила получить качественную картину теории
полиномов в некоммутативной алгебре.
Однако существуют алгебры где рассматриваемая картина не полна.
}

\DefExample{r=x2-jx-xi-k p=x-i}
{
Пусть
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-jx-xi-k}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 1}
Теперь мы положим
\ShowEq{q0= 1}
Тогда
\ShowEq{s0=s-.p. 1}
Равенство
\ShowEq{r=x2-jx-xi-k 1}
является следствием равенств
\EqRef{s1=r-.p. 1},
\EqRef{s0=s-.p. 1}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-jx-xi-k 1}
\ShowEq{r=x2-jx-xi-k 2}
Мы видим, что представление многочлена $r(x)$ в равенстве
\EqRef{r=x2-jx-xi-k 2}
совпадает с представление многочлена $r(x)$ в равенстве
\eqRef{r=x2-jx-xi-k}1.
}

\AddEq{remark: r=x2-jx-xi-k p=x-i}
{
Ответ
\EqRef{r=x2-jx-xi-k 2}
в примере
\RefExample{r=x2-jx-xi-k p=x-i}
очевиден, так как я намеренно выбрал делитель $p(x)$
равным второму множителю многочлена $r(x)$.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-jx-xi-k}
}

\AddEq{remark: r=x2-ix-xj+k p=x-i}
{
Пример
\RefExample{r=x2-ix-xj+k p=x-i}
более интересен, так как я изменил порядок множителей.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-xj+k p=x-i}
Пусть
\DrawEq{p=x-i Red}{}
\DrawEq{r=x2-ix-xj+k}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 2}
Теперь мы положим
\ShowEq{q0= 2}
Тогда
\ShowEq{s0=s-.p. 2}
Равенство
\ShowEq{r=x2-ix-xj+k 1}
является следствием равенств
\EqRef{s1=r-.p. 2},
\EqRef{s0=s-.p. 2}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-xj+k 1}
\ShowEq{r=x2-ix-xj+k 2}
Мы видим, что представление многочлена $r(x)$ в равенстве
\EqRef{r=x2-ix-xj+k 2}
совпадает с представление многочлена $r(x)$ в равенстве
\eqRef{r=x2-ix-xj+k}1.
\end{\ExampleStyle}

Частное от деления многочлена $r(x)$ на многочлен $p(x)$
в примере
\RefExample{r=x2-ix-xj+k p=x-i}
имеет более сложную структуру чем частное
в примере
\RefExample{r=x2-jx-xi-k p=x-i}.
Это связано с тем, что я пытаюсь записать делитель $p(x)$
справа от частного, хотя изначально многочлен $p(x)$
был левым множителем.
Тем не менее, в результате несложных преобразований
разложение на множители в равенстве
\EqRef{r=x2-ix-xj+k 2}
приняло ожидаемый вид.

\FrameEq{p=x-i Red}
\FrameEq{r=x2-ix-xj+k}
}

\DefExampleNote{polynomial p*r(x)}
{
Пусть
\ShowEq{polynomial p(x)}pin
и
\ShowEq{polynomial p(x)}rjm
левостороние многочлены.
Мы определим произведение многочленов $p$ и $r$ равенством\,\footnotemark
\ShowEq{polynomial p*r(x)}

Рассмотрим многочлены
\DrawEq[Li]{Px=x-i}i
\DrawEq[Rj]{Px=x-i}j
Равенство
\ShowEq{Px=x-i*x-j}
является следствием равенств
\EqRef{polynomial p*r(x)},
\eqRef{Px=x-i}i,
\eqRef{Px=x-i}j.
Пусть
\ShowEq{h=Ri}
\ShowEq{x-=}
\ShowEq{L(x-)=}
Согласно теореме
\citeBib{1702.04935}\Hyph 1, пункт $(ii)$,
многочлен
\ShowEq{P1=L(x-)R(x)}
совпадает с многочленом $P(x)$,
$P_1(x)=P(x)$
\ShowEq{p(x)=L(x-)R(x)}

Однако равенство
\EqRef{p(x)=L(x-)R(x)}
не верно.
Пусть $x=i+j$.
Равенства
\ShowEq{p(i+j)=L(i+j-)R(i+j)}
\ShowEq{p(i+j)=L(i+j-)R(i+j) 1}
являются следствием равенства
\EqRef{p(x)=L(x-)R(x)}.
}
{
Смотри также определение на странице
\citeBib{1702.04935}\Hyph 3.
}

\AddEq{remark: r=x2-ix-jx-k}
{
В примере
\RefExample{r=x2-ix-jx-k}
я рассмотрел деление левосторонего многочлена
\DrawEq{r=x2-ix-jx-k}{}
на многочлен
\ShowEq{p=x-i}i
Я знаю, что многочлен $r(x)$ имеет корень $x=i$,
и хочу найти другой корень.

\begin{\ExampleStyle}
\labelExample{r=x2-ix-jx-k}
%.3.
Пусть
\ShowEq{p=x-i}i
\DrawEq{r=x2-ix-jx-k}{}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 3}
Теперь мы положим
\ShowEq{q0= 3}
Тогда
\ShowEq{s0=s-.p. 3}
Равенство
\ShowEq{r=x2-ix-jx-k 1}
является следствием равенств
\EqRef{s1=r-.p. 3},
\EqRef{s0=s-.p. 3}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-jx-k 1}
\ShowEq{r=x2-ix-jx-k 10}
\end{\ExampleStyle}
}

\DefQuestion{r=x2-ix-jx-k}
{
Имеет ли многочлен
\DrawEq{r=x2-ix-jx-k}{}
корень, отличный от $x=i$?
}

\AddEq{remark: r=x2-ix-jx-k 1}
{
Утверждение, что $x=i$ является корнем многочлена $r(x)$
проверяется непосредственно.
Согласно примеру
\RefExample{r=x2-ix-jx-k},
мы можем представить многочлен $r(x)$ в виде
\DrawEq{r=x2-ix-jx-k 2}2
Следовательно, для того чтобы многочлен $p(x)$
имел корень, отличный от $x=i$,
необходимо чтобы линейное отображение
\DrawEq{r=x2-ix-jx-k map}1
имело нетривиальное ядро
и кватернион $x-i$
принадлежал ядру линейного отображения
\eqRef{r=x2-ix-jx-k map}1.
Линейное отображение
\eqRef{r=x2-ix-jx-k map}1
имеет матрицу
\ShowEq{r=x2-ix-jx-k matrix}
Определить значение $x$, для которого матрица
\EqRef{r=x2-ix-jx-k matrix}
вырождена - задача непростая.
Но я надеюсь провести дополнительное исследование.
}

\AddEq{remark: r=x2-ix-jx-k p=x-j}
{
В примере
\RefExample{r=x2-ix-jx-k p=x-j}
я рассмотрел деление левосторонего многочлена
\ShowEq{r=x2-ix-jx-k  r(j)=}
на многочлен
\ShowEq{p=x-i}j
}

\DefExample{r=x2-ix-jx-k p=x-j}
{
%.3j.
Пусть
\ShowEq{p=x-i}j
\DrawEq{r=x2-ix-jx-k}{}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 3j}
Теперь мы положим
\ShowEq{q0= 3j}
Тогда
\ShowEq{s0=s-.p. 3j}
Равенство
\ShowEq{r=x2-ix-jx-k 3j}
является следствием равенств
\EqRef{s1=r-.p. 3j},
\EqRef{s0=s-.p. 3j}.
Мы можем упростить выражение в равенстве
\EqRef{r=x2-ix-jx-k 3j}
\ShowEq{r=x2-ix-jx-k 3j 1}
}

\AddEq{remark: r=(x-j)(x-k)(x-j-k)}
{
В примере
\RefExample{r=(x-j)(x-k)(x-j-k)}
я рассмотрел многочлен $r(x)$ степени $3$
для того, чтобы найти частное от деления многочлен $r(x)$ на два многочлена.
Сперва я найду частное от деления многочлена
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
на многочлен
\ShowEq{p=x-i}k

\begin{\ExampleStyle}
\labelExample{r=(x-j)(x-k)(x-j-k)}
Пусть
\ShowEq{p=x-i}k
\ShowEq{r=(x-j)(x-k)(x-j-k)}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q2=x2 ox 1}
Тогда
\ShowEq{s2=r-.p. 5}
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=... 5}
Равенство
\ShowEq{s1=s2-.p. 5}
является следствием равенств
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5}.
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q0=... 5}
Равенство
\ShowEq{s0=s1-.p. 5}
является следствием равенств
\EqRef{s1=s2-.p. 5},
\EqRef{q0=... 5}.
Равенство
\ShowEq{r=s0+q1+q2 5}
является следствием равенств
\EqRef{s2=r-.p. 5},
\EqRef{q1=... 5},
\EqRef{q0=... 5},
\EqRef{s0=s1-.p. 5}.
\end{\ExampleStyle}

Частное
\ShowEq{q=q1+q2 5}
от деления многочлена
\ShowEq{r=(x-j)(x-k)(x-j-k) 0}
на многочлен
\ShowEq{p=x-i}k
является тензором зависящим от $x$,
а не многочленом.
Поэтому мы не можем применить теорему
\RefTheorem{r=+q circ (x-a)}.
}

\DefQuestion{how to select factor in the tensor}
{
Нетрудно убедиться, что
\ShowEq{q1+q2 5 x=j}
Поэтому возникает вопрос как выделить в тензоре
\DrawEq{q1+q2 5 x}1
множитель $x-j$.
}

\DefExample{select factor in the tensor}
{
Один из возможных ответов на вопрос
\RefQuestion{how to select factor in the tensor}
состоит в преобразовании
\ShowEq{q1+q2 5 x,1}
Рассмотрим многочлен
\DrawEq{q1+q2 5 x,3}1
Согласно теореме
\RefTheorem{r=+q circ (x-a)},
положим
\ShowEq{q1=x ox 1}
Тогда
\ShowEq{s1=r-.p. 7}
Теперь мы положим
\ShowEq{q0= 7}
Тогда
\ShowEq{s0=s-.p. 7}
Равенство
\ShowEq{r=x2... 7}
является следствием равенств
\EqRef{s1=r-.p. 7},
\EqRef{s0=s-.p. 7}.
Равенство
\ShowEq{q1+q2 5 x,2}
является следствием равенств
\EqRef{q1+q2 5 x,1},
\EqRef{r=x2... 7}.
}

\AddEq{remark: select factor in the tensor}
{
Мы видим, что частное в примере
\RefExample{select factor in the tensor}
является $H^{3\otimes}$\Hyph числом.
}

\DefExample{factorization as bilinear map}
{
Равенство
\ShowEq{r= 8}
является следствием равенств
\EqRef{r=s0+q1+q2 5},
\EqRef{q1+q2 5 x,2}.
}

\DefQuestion{factorization as bilinear map}
{
Равенство
\EqRef{r= 8}
является ответом на вопрос
\RefQuestion{how to select factor in the tensor}.
Мы видим, что разложение многочлена $r(x)$
является билинейным отображением многочленов
$x-j$, $x-k$.
Однако этот ответ не полный.
Согласно замечанию
\RefRemark{monomial of power k},
представление
\EqRef{r=+q circ p}
многочлена не единственно.
Остаётся открытым вопрос о выборе множителей и их порядке.
В то же время существует связь между различными представлениями многочлена
в виде произведения множителей.
}


==> Stmt.Derivative.Russian.tex <==
%auto-ignore
\input{Stmt.Derivative.Eq}

\DefTheorem{bilinear map and differential}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B_1$, $B_2$, $B$ - банаховые $D$\Hyph алгебры.
Пусть
\ShowEq{h:BxB->B}
непрерывное билинейное отображение.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B12}
Отображение
\ShowEq{h(f,g):A->B}
дифференцируемо и
производная удовлетворяет соотношению
\ShowEq{bilinear map and derivative, 3}
\ShowEq{bilinear map and derivative, 5}
}

\AddEq{definition: first integral}
{
\begin{ShadedDefinition}
\labelDefinition{first integral}
Пусть
\ShowEq{dxi/dt=Xi}
система дифференциальных уравнений.
Уравнение
\ShowEq{Ftx1.n}
которое обращается в тождество при некотором значении $c$,
если $x^i(t)$, $i=1$, ..., $n$,
является решением системы дифференциальных уравнений
\EqRef{dxi/dt=Xi},
называется
\AddIndex{первым интегралом}{first integral}\,\footnotemark
системы дифференциальных уравнений
\EqRef{dxi/dt=Xi}.
\end{ShadedDefinition}
\footnotetext{\,
Смотри также определению на странице
\citeBib{Elsgolts: Differential Equations}\Hyph 179.
}
}

\DefTheorem{derivative of product, algebra}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B}
Производная удовлетворяет соотношению
\ShowEq{differential of product, algebra}
\ShowEq{derivative of product, algebra}
}

\DefDefinition{norm of polylinear map}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|x\|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $\|x\|_B$.
Для отображения
\ShowEq{f:An->B}
величина
\ShowEq{norm of polymap}
\ShowEq{norm of map, module}
называется
\AddIndex{нормой отображения}{norm of map} $f$.
}

\DefTheorem{|f(a)|<|f||a| 1n}
{
Для отображения
\ShowEq{f:An->B}
банахового $D$\Hyph модуля $A$ с нормой $\|x\|_A$
в банаховый $D$\Hyph модуль $B$ с нормой $\|x\|_B$
\ShowEq{|f(a)|<|f||a| 1n}
}

\DefProof{|f(a)|<|f||a| 1n}
{
Неравенство
\ShowEq{|f(a)|/|a|<max}
является следствием равенства
\EqRef{norm of map, module}.
Неравенство
\EqRef{|f(a)|<|f||a| 1n}
является следствием неравенства
\EqRef{|f(a)|/|a|<max}.
}

\DefTheorem{|on|->0 ona1p->0}
{
Пусть
\ShowEq{f:A->B}{o_n}{A^p}B
последовательность отображений банахова $D$\Hyph модуля $A$
в банаховый $D$\Hyph модуль $B$ такая, что
\ShowEq{|on|->0}
Тогда для любых $B$\Hyph чисел
\ShowEq{a1n}ap{}
\ShowEq{ona1p->0}
}

\DefProof{|on|->0 ona1p->0}
{
Из теоремы
\RefTheorem{|f(a)|<|f||a| 1n}
следует, что
\ShowEq{|oa1p|<}
Утверждение
\EqRef{ona1p->0}
является следствием утверждений
\EqRef{|on|->0},
\EqRef{|oa1p|<}.
}

\DefTheorem{derivative, standard form, algebra}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля\newline
\ShowEq{L(A->B)}DAB.
Пусть $\Basis e$ - базис $D$\Hyph модуля $B$.
\AddIndex{Стандартное представление производной}
{derivative, standard representation} отображения
\ShowEq{f:A->B}fAB
имеет вид
\ShowEq{standard component of derivative}
\ShowEq{derivative, algebra, standard representation}
Выражение
\ShowEq{standard component of derivative, algebra}
в равенстве
\EqRef{derivative, algebra, standard representation}
называется
\AddIndex{стандартной компонентой производной}
{standard component of derivative} отображения $f$.
}

\AddEq[1]{theorem: Cauchy Riemann equations, complex field}
{
\begin{ShadedTheorem}[Уравнение Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations, complex field}
Производная отображения комплексного переменного удовлетворяет
уравнению Коши\Hyph Римана
\DrawEq[{#1}]{Cauchy Riemann equation, complex field}{theorem}
\end{ShadedTheorem}
}

\AddEq[1]{proof: Cauchy Riemann equations, complex field}
{
\begin{proof}
Равенство
\DrawEq[{#1}]{Cauchy Riemann equations, complex field, 2, 1}{#1}
следует из равенств
\eqRef{Cauchy Riemann equations, complex field, 1}{#1}.
Равенство
\eqRef{Cauchy Riemann equation, complex field}{theorem}
является следствием равенства
\eqRef{Cauchy Riemann equations, complex field, 2, 1}{#1}.
\end{proof}%
}

\DefTheorem{derivative and jacobian, algebra}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля\newline
\ShowEq{L(A->B)}DAB.
Пусть $\Basis e_A$ - базис свободного конечно мерного
$D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $B$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $B$.
Тогда производную отображения
\ShowEq{f:A->B}fAB
можно записать в виде
\ShowEq{derivative and jacobian, algebra}
где $dx\in A$ имеет разложение
\ShowEq{derivative and jacobian, 1, algebra}
относительно базиса $\Basis e_A$ и матрица Якоби отображения $f$ имеет вид
\ShowEq{standard components and Jacobian, algebra A->B}
}

\AddEq{theorem: derivative x2}
{
\begin{ShadedTheorem}
\labelTheorem{derivative x2}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная банаховая $D$\Hyph алгебра.
Тогда\,\footnotemark
\DrawEq{derivative x2, algebra}{theorem}
\ShowEq{derivative x2 differential, algebra}
\ShowEq{derivative x2 component, algebra}
\end{ShadedTheorem}
\footnotetext{\,
Утверждение теоремы аналогично примеру VIII,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\eqRef{derivative x2, algebra}{theorem}
принимает вид
\ShowEq{derivative x2, field}
}
}

\DefProof{derivative x2}
{
Рассмотрим приращение функции $f(x)=x^2$.
\ShowEq{derivative x2, algebra, 1}
Равенство
\eqRef{derivative x2, algebra}{theorem}
является следствием равенства
\EqRef{derivative x2, algebra, 1}
и определения
\refDefinition{differentiable map}{algebra}.
Равенство
\EqRef{derivative x2 differential, algebra}
является следствием равенств
\EqRef{a ox b c=},
\EqRef{derivative x2 differential, algebra},
\eqRef{differential of map =}{Definition}.
Равенство
\EqRef{derivative x2 component, algebra}
является следствием равенства
\eqRef{derivative x2, algebra}{theorem}.
}

\DefExample{differential equation y=xx, real number}
{
Рассмотрим
\AddIndex{метод последовательного дифференцирования}
{method of successive differentiation}
для решения дифференциального уравнения
\ShowEq{differential equation y=xx, real number}
\DrawEq{differential equation, initial}{y=xx, real number}
над полем действительных чисел.
Последовательно дифференцируя уравнение
\EqRef{differential equation y=xx, real number},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, 2...n, real number}
Разложение в ряд Тейлора
\DrawEq{y=x3+C}{}
следует из уравнений
\ShowEq{differential equation y=xx, ref, real number}
}

\DefDefinitionNote{norm on D module}
{
Пусть $D$ - нормированное коммутативное кольцо.\,\footnotemark
\AddIndex{Норма в $D$\Hyph модуле}
{norm on D module} $A$
 - это отображение
\ShowEq{norm on D module}
такое, что
\StartLabelItem
\begin{enumerate}
\ShowEq{norm on D module 1}
\ShowEq{norm on D module 2, 1}
равносильно
\ShowEq{norm on D module 2, 2}
\ShowEq{norm on D module 3}
\end{enumerate}
$D$\Hyph модуль $A$,
наделённый структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированным $D$\Hyph модулем}{normed D module}.
}
{Определение дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3.
Для нормы мы пользуемся обозначением $|a|$ или $\|a\|$.}

\AddEq{definition: equivalent norms}
{
\begin{ShadedDefinition}
\labelDefinition{equivalent norms}
Нормы\,\footnotemark
\ShowEq{|1,|2},
определённые на $D$\Hyph модуле $A$,
называются
\AddIndex{эквивалентными}{equivalent norms},
%если они порождают одну и туже топологию.
если утверждение
\DrawEq{a=lim an}{}
не зависит от выбранной нормы.
\end{ShadedDefinition}
\footnotetext{\,
Смотри также определение
\citeBib{Shilov single 3}\Hyph 12.35.а
на странице 53.
}
}

\DefDefinitionNote{norm on d algebra}
{
Пусть $D$ - нормированное коммутативное кольцо.
Пусть $A$ - $D$\Hyph алгебра.
Норма\,\footnotemark
\ShowEq{norm on d algebra}
в $D$\Hyph модуле $A$ такая, что
\ShowEq{norm on d algebra 3}
называется
\AddIndex{нормой в $D$\Hyph алгебре}
{norm on D algebra} $A$.
$D$\Hyph алгебра $A$,
наделённая структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированной $D$\Hyph алгеброй}{normed D algebra}.
}{
Определение дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3.
Если $D$\Hyph алгебра $A$ является алгеброй с делением,
то норма называется
\AddIndex{абсолютной величиной}{absolute value}
и мы пользуемся записью $|a|$ для нормы $A$\Hyph числа $a$.
Смотри определение из
\citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2.

Неравенство
\EqRef{norm on d algebra 3}
является следствием теоремы
\RefTheorem{there exists equivalent norm |*|=1}.
В противном случае мы должны были бы писать
\ShowEq{norm on d algebra 3 1}
}

\AddEq{theorem: Cauchy Riemann equations, complex field, 1}
{
\begin{ShadedTheorem}[Уравнения Коши\Hyph Римана]
\labelTheorem{Cauchy Riemann equations, complex field, 1}
Если матрица
\DrawEq[y]{Jacobian of map, complex variable}{}
является матрицей Якоби функции комплексного переменного
\ShowEq{map of complex variable}
над полем действительных чисел,
то
\DrawEq[f]{Cauchy Riemann equations, complex field, 1}f
\end{ShadedTheorem}
}

\DefTheorem{df/dx= complex field}
{
Если отображение поля комплексных чисел
\DrawEq[fCC{}]{f: A->B}{}
рассматривать как функцию переменных
\ShowEq{x=x0+ix1}
то
\ShowEq{df/dx= complex field}
}

\DefProof{df/dx= complex field}
{
Производная отображения $f$ - это линейное отображение,
которое имеет матрицу Якоби над полем действительных чисел
\DrawEq[f]{Jacobian of map, complex variable}{}
\TheoremFollows
\RefTheorem{f=.E+.I}.
}

\DefTheorem{df=...dx quaternion}
{
Рассмотрим отображение алгебры кватернионов
\ShowEq{f:A->B}fHH
как функцию переменных
\ShowEq{x=x0+ix1+jx2+kx3}
Если отображение $f$ дифференцируемо,
то существуют частные производные
\ShowEq{H df/dx Jacobi}
и
\DrawEq{df=...dx 03}{theorem}
}

\DefTheorem{Lebesgue Integral along Path}
{
Пусть существует неопределённый интеграл
\DrawEq{f=int g.}{}
Для любого непрерывного спрямляемого пути
\ShowEq{h:[01]->A}
из $a$ в $x$ в $D$\Hyph модуле $A$
\DrawEq{int hn= 2}{path}
}

\DefDefinition{Banach algebra}
{
Нормированная $D$\Hyph алгебра $A$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A$ сходится, т. е.
имеет предел в алгебре $A$.
}

\DefTheorem{there exists equivalent norm |*|=1}
{
Пусть $A$ - $D$\Hyph алгебра.
Если в $D$\Hyph модуле $A$ определена норма $\|x\|_1$ такая, что
норма $\|*\|_1$ произведения в $D$\Hyph алгебре $A$ отлична от $1$,
то в $D$\Hyph модуле $A$ существует эквивалентная норма
\ShowEq{|2=*|1 |1}
такая, что
\ShowEq{|*|2=1}
}

\DefDefinition{Banach module}
{
Нормированный $D$\Hyph модуль $A$ называется 
\AddIndex{банаховым $D$\Hyph модулем}{Banach module}
если любая фундаментальная последовательность элементов
модуля $A$ сходится, т. е.
имеет предел в модуле $A$.
}

\DefTheorem{derivative of the sum}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->B}
Отображение
\ShowEq{derivative of the sum, 2}
дифференцируемо и
производная удовлетворяет соотношению
\ShowEq{derivative of the sum, 3}
}

\DefTheorem{derivative of map of module, IJ}
{
Пусть $V$, $W$ - банаховые $A$\Hyph модули столбцов.
\ShowEq{Let be basis of module}V{}kK{левого }A{}V{}
\ShowEq{Let be basis of module}W{}lL{левого }A{}W{}
Тогда производная отображения
\ShowEq{f:A->B}fVW
имеет представление
\ShowEq{dfk=dfk/dxl dxl}
\ShowEq{df=dfk/dxl dxl ek}
относительно заданных базисов.
\AddIndex{Матрица Якоби отображения}{Jacobi matrix of map}
$f$ имеет вид
\ShowEq{Jacobi matrix of map}
\ShowEq{partial derivative}
\ShowEq{Jacobi matrix of map =}
где
\AddIndex{частная производная}{partial derivative}
\ShowEq{show partial derivative}
- это производная отображения $f^{\gik}$
по переменной $x^{\gil}$
при условии, что остальные переменные заданы.
}

\DefTheorem{chain rule module m x n}
{
Пусть $U$, $V$, $W$ - банаховые $A$\Hyph модули столбцов.
\ShowEq{Let e be basis 1n}Uk{левом}{A}U
\ShowEq{Let e be basis 1n}Vn{левом}{A}V
\ShowEq{Let e be basis 1n}Wm{левом}{A}W
Пусть
\ShowEq{f:A->B}fUV
\ShowEq{f:A->B}gVW
дифференцируемые отображения
\DrawEq[fynk]{df/dx matrix}{}
\DrawEq[gxmn]{df/dx matrix}{}
Тогда отображение
$h=f\circ g$
дифференцируемо и
\ShowEq{dh/dy=df/dx rco dg/dy}
\ShowEq{dh/dy=df/dx o dg/dy}
}

\DefTheorem{derivative of map of module, m x n}
{
Пусть $V$, $W$ - банаховые $A$\Hyph модули столбцов.
\ShowEq{Let e be basis 1n}Vn{левом}{A}V
Представим $V$\Hyph число
\DrawEq [{dx}V]{va=ae1, module (left)(cols)}{}
как вектор столбец
\DrawEq[{dx}n]{a=(a1.n gi)}{dx n}
\ShowEq{Let e be basis 1n}Wm{левом}{A}W
Тогда производная отображения
\ShowEq{f:A->B}fVW
имеет представление
\ShowEq{df=dfk/dxl dxl ek nm}
относительно заданных базисов.
}

\DefExample{derivative of map of module, 2 x 3}
{
Мы можем записать производную отображения
\ShowEq{derivative of map of module, 2 x 3 1}
следующим образом
\ShowEq{derivative of map of module, 2 x 3 2}
Непосредственная оценка приращения имеет вид
\ShowEq{derivative of map of module, 2 x 3 3}
\ShowEq{derivative of map of module, 2 x 3 4}
Нетрудно убедиться, что выражения
\EqRef{derivative of map of module, 2 x 3 3},
\EqRef{derivative of map of module, 2 x 3 4}
и выражения
\EqRef{derivative of map of module, 2 x 3 2}
совпадают.
}

\DefTheorem{differential equation Mdx+Ndy is integrable iff}
{
Дифференциальное уравнение
\DrawEq{Mdx+Ndy xy}1
интегрируемо тогда и только тогда, когда
\ShowEq{dM/dy=dN/dx xx}
\ShowEq{dM/dy=dN/dx yy}
\ShowEq{dM/dy=dN/dx yx}
}

\DefLabeledDefinition [4]{differentiable map}{#4}
{
Пусть $#2$ - банаховый $#1$\Hyph модуль с нормой $\|a\|_#2$.
Пусть $#3$ - банаховый $#1$\Hyph модуль с нормой $\|a\|_#3$.
Отображение
\ShowEq{f:A->B}f{#2}{#3}
называется
\AddIndex{дифференцируемым}{differentiable map}
на множестве $U\subset #2$,
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
если существует дифференциальная $1$\Hyph форма
\ShowEq{x->dnf/dxn in L(A2,B)}DAB{}
такая, что
\else
если в каждой точке $x\in U$
изменение отображения $f$ может быть представлено в виде
\fi
\ShowEq{derivative of map}
\DrawEq{derivative of map, def}{#4}
где
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\ShowEq{df:A->B}{#2}{#3}
линейное отображение $#1$\Hyph модуля $#2$ в $#1$\Hyph модуль $#3$ и
\fi
\ShowEq{f:A->B}o{#2}{#3}
такое непрерывное отображение, что
\DrawEq[{#2}{#3}]{lim |o|/|a|}1
Линейное отображение
\ShowEq{show derivative of map}
называется
\AddIndex{производной отображения}{derivative of map}
$f$ и
\AddIndex{дифференциал $df$ отображения}{differential of map}
$f$ определён равенством
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{Definition}
где $dx$ - дифференциал аргумента.
}

\DefProof{dx/dx=1}
{
Согласно определению
\eqRef{derivative, linear path}1
\ShowEq{dx/dx=}
Равенство
\eqRef{dx/dx=1}1
является следствием
\EqRef{dx/dx=}.
}

\AddEq [4]{remark: derivative as differential form}
{
\begin{remark}
\labelRemark{derivative as differential form, #4}
Согласно определению
\refDefinition{differentiable map}{#4}
при заданном $x$, производная
\ShowEq{df/dx in L(A->B)}{#1}{#2}{#3}
Следовательно, производная отображения $f$ является
дифференциальной $#3$\Hyph значной $1$\Hyph формой
\ShowEq{df/dx:A->L(A->B)}{#1}{#2}{#3}
\qed
\end{remark}
}

\AddEq [4]{remark: differential of map}
{
\begin{remark}
\labelRemark{differential of map, #4}
В математическом анализе, отображение
\ShowEq{differential of independent variable}
\ShowEq{dx=delta}{#1}{#2}
называется
\AddIndex{дифференциалом независимой переменной}
{differential of independent variable}.
Дифференциальная $#3$\Hyph значная $1$\Hyph форма
\ShowEq{df/dx:A->L(A->B)}{#1}{#2}{#3}
записанная в виде
\ShowEq{differential of independent variable}
\ShowEq{differential of map}
\DrawEq{differential of map =}{#4}
называется
\AddIndex{дифференциалом отображения}{differential of map}
$f$.
Впрочем равенство
\eqRef{differential of map =}{#4}
имеет другую интерпретацию.
А именно, мы рассматриваем приращение $df$ отображения $f$
как функцию
\eqRef{differential of map =}{#4}
приращения $dx$ независимой переменной.
\qed
\end{remark}
}

\DefRemark{differential L(A,A)}
{
Согласно определению
\refDefinition{differentiable map}{algebra},
производная отображения $f$ является отображением
\ShowEq{x->dnf/dxn in L(A2,B)}DAB{}
Выражения $d_x f(x)$ и
\ShowEq{df/dx}
являются разными обозначениями одного и того же отображения.
}

\DefTheorem{representation of derivative, algebra A->B}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DAB.
Мы можем представить производную отображения
\ShowEq{f:A->B}fAB
в виде
\ShowEq{coordinates of derivative}
\ShowEq{df/dx=dkf/dx Ik}
}

\DefTheorem{representation of derivative, algebra A->B 2017}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB{}
и
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker df/dx}
Мы можем представить производную отображения
\ShowEq{f:A->B}fAB
в виде
\ShowEq{coordinates of derivative}
\ShowEq{df/dx=dkf/dx Fk G}
}

\DefDefinition{coordinates of derivative, algebra A->B}
{
Выражение
\ShowEq{show coordinates of derivative}
называется
\AddIndex{координатами}{coordinates}
производной
\ShowEq{df/dx}
относительно базиса $\Basis F$.
Выражение
\ShowEq{component of derivative A->B}
\ShowEq{component of derivative A->B =}
называется
\AddIndex{компонентой производной}
{component of derivative} отображения $f(x)$.
}

\DefTheorem{representation of differential, algebra A->B}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DAB.
Мы можем представить дифференциал отображения
\ShowEq{f:A->B}fAB
в виде
\ShowEq{df=sum dsf/dx dx A->B}
}

\DefTheorem{dfa1p/dx=df/dx a1p}
{
Пусть $B$ - банаховый модуль над коммутативным кольцом $D$.
Пусть $U$ - открытое множество банахового $D$\Hyph модуля $A$.
Пусть
\ShowEq{U->L(Ap,B)}
дифференцируемое отображение.
Тогда
\ShowEq{dfa1p/dx=df/dx a1p}
}

\AddEq{proof: dfa1p/dx=df/dx a1p}
{
\begin{proof}
Пусть
\ShowEq{a0 in U}
Согласно определению
\refDefinition{differentiable map}{algebra},
изменение отображения
$f$ может быть представлено в виде
\ShowEq{derivative of map, U->L(B)}
где
\ShowEq{derivative in L(L)}
и
\ShowEq{o:A->LB}
такое непрерывное отображение, что
\ShowEq{o:A->LB, lim o}
Так как
\ShowEq{f(x) in LB}
то для любых
\ShowEq{a1n}ap{}
равенство
\ShowEq{derivative of map, U->B}
является следствием равенства
\EqRef{derivative of map, U->L(B)}.
Согласно теореме
\RefTheorem{|on|->0 ona1p->0},
равенство
\ShowEq{o:A->LB, lim o a1p}
является следствием равенства
\EqRef{o:A->LB, lim o}.
Рассматривая выражение
\ShowEq{f(x) o a1p}
как отображение
\ShowEq{x->f(x) o a1p}
мы получим, что изменение этого отображения
может быть представлено в виде
\ShowEq{derivative of map, U->B 1}
где
\ShowEq{derivative in L}
и
\ShowEq{f:A->B}{o_1}AB
такое непрерывное отображение, что
\ShowEq{o1:A->B, lim o}
Равенство
\ShowEq{derivative of map, U->B = +o}
является следствием равенств
\EqRef{derivative of map, U->B},
\EqRef{derivative of map, U->B 1}.
Равенство
\ShowEq{lim o a1p-o1}
является следствием равенств
\EqRef{o:A->LB, lim o a1p},
\EqRef{o1:A->B, lim o}.
Равенство
\EqRef{dfa1p/dx=df/dx a1p}
является следствием равенств
\EqRef{derivative of map, U->B = +o},
\EqRef{lim o a1p-o1}.
\end{proof}
}

\DefTheorem{derivative, representation in algebra}
{
Определение производной
\eqRef{derivative of map, def}{algebra}
эквивалентно определению
\DrawEq{derivative, linear path}1
}

\DefDefinition{derivative of Second Order, algebra}
{
Полилинейное отображение
\ShowEq{derivative of Second Order}
\ShowEq{derivative of Second Order, algebra}
называется
\AddIndex{производной второго порядка}
{derivative of Second Order} отображения $f$.
}

\DefTheorem{Differential of Second Order, algebra, representation}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть $B$ - свободная ассоциативная банаховая $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DAB.
Мы можем представить
производную второго порядка отображения $f$
в виде
\ShowEq{Differential of Second Order, algebra, representation}
Мы будем
называть выражение
\ShowEq{component of derivative of Second Order}
\DrawEq{component of derivative of Second Order, algebra}{}
\AddIndex{компонентой производной второго порядка}{}
{component of derivative of Second Order} отображения $f(x)$.
}

\DefDefinition{derivative of Order n, algebra}
{
По индукции, предполагая, что определена производная
\ShowEq{dnf/dxn}{n-1}
порядка $n-1$, мы определим
\ShowEq{derivative of Order n}
\ShowEq{derivative of Order n, algebra}
\AddIndex{производную порядка $n$}
{derivative of Order n} отображения $f$.

Мы будем также полагать
\ShowEq{d0f(x)}
}

\DefTheorem{n derivative equal 0, algebra}
{
Если для отображения $f(x)$ выполняется условие
\ShowEq{n derivatives of function, algebra}
то при $t\rightarrow 0$ выражение $f(x+th)$ является бесконечно малой порядка
выше $n$ по сравнению с $t$
\[
f(x_0+th)=o(t^n)
\]
}

\AddEq{Taylor polynomial}
{
Составим многочлен
\ShowEq{Taylor polynomial, f(x), algebra}
Согласно теореме \RefTheorem{n derivative equal 0, algebra}
\ShowEq{Taylor polynomial, f(x)-p(x)}
Следовательно, полином $p(x)$ является хорошей апроксимацией отображения $f(x)$.
}

\AddEq{Taylor series}
{
Если отображение $f(x)$ имеет производную любого порядка,
то переходя к пределу
$n\rightarrow\infty$, мы получим разложение в ряд
\ShowEq{Taylor series, f(x), algebra}
который называется \AddIndex{рядом Тейлора}{Taylor series, algebra}.
}

\DefTheorem{second derivative is symmetric bilinear map}
{
Пусть $A$ - свободный банаховый $D$\Hyph модуль.
Пусть производная второго порядка отображения
\ShowEq{f:A->B}fAB
непрерывна.
Тогда вторая производная является симметричным билинейным отображением
\ShowEq{df/dx2 ab=ba}
}

\DefDefinition{indefinite integral}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$ - банаховая $D$\Hyph алгебра.
Отображение
\ShowEq{g:A->BoxB}gAB
называется
\AddIndex{интегрируемым}{integrable map},
если существует отображение
\ShowEq{f:A->B}fAB
такое, что
\ShowEq{df=g}fg
Тогда мы пользуемся записью
\ShowEq{indefinite integral}g
\DrawEq{f=int g}{}
и отображение $f$ называется
\AddIndex{неопределённым интегралом}{indefinite integral}
отображения $g$.
}

\DefDefinition{indefinite integral 2017}
{
Пусть $A$, $B$ - банаховые $D$\Hyph модули.
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
Отображение
\else
Дифференциальная форма
\fi
\ShowEq{g:A->LBB}gAB
называется
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
\AddIndex{интегрируемым}{integrable map},
\else
\AddIndex{интегрируемой}{integrable differential form},
\fi
если существует отображение
\ShowEq{f:A->B}fAB
такое, что
\ShowEq{df=g}fg
Тогда мы пользуемся записью
\ShowEq{indefinite integral}g
\DrawEq{f=int g}{}
и отображение $f$ называется
\AddIndex{неопределённым интегралом}{indefinite integral}
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOff
отображения
\else
дифференциальной формы
\fi
$g$.
}

\DefDefinition[3]{differential form}
{
Пусть
\ShowEq{U subset A}{#2}
является открытым множеством.
Отображение
\ShowEq{o:U->LAAB}{#1}{#2}{#3}
называется
\AddIndex{дифференциальной формой степени $p$}{differential form of degree p},
определённой на $U$, со значениями в $#3$
или $#3$\Hyph значной
\AddIndex{дифференциальной $p$\Hyph формой}{differential p form},
определённой на $U$.
}

\DefTheorem{exterior differential}
{
Внешний дифференциал удовлетворяет равенству
\ShowEq{do=...sum}
}

\DefProof{exterior differential}
{
Равенство
\EqRef{do=...sum}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior differential def}.
}

\DefTheorem{int x dx=x2}
{
\ShowEq{int x dx=x2}
\ShowEq{int x dx=x2 1}
}

\DefProof{int x dx=x2}
{
Теорема является следствием теоремы
\RefTheorem{derivative x2}
и определения
\RefDefinition{indefinite integral 2017}.
Согласно определению
\ePrints{2021.01.06}%
\ifx\Semafor\ValueOff
\EqRef{a ox b c=}
\else
\EqRef{value of linear map f, basis E}
\fi
мы можем записать интеграл
\EqRef{int x dx=x2}
в виде
\EqRef{int x dx=x2 1}.
}

\AddEq[1]{theorem: int x2 dx=x3}
{
\begin{ShadedTheorem}
\labelTheorem{int x2 dx=x3}
\ShowEq{int x2 dx=x3}
\ShowEq{int x2 dx=x3 1}
где $C$ - произвольное $#1$\Hyph число.
\end{ShadedTheorem}
}

\DefProof{int x2 dx=x3}
{
Теорема является следствием теоремы
\RefTheorem{derivative x3}
и определения
\RefDefinition{indefinite integral 2017}.
Согласно определению
\ePrints{2021.01.06}%
\ifx\Semafor\ValueOff
\EqRef{a ox b c=}
\else
\EqRef{value of linear map f, basis E}
\fi
мы можем записать интеграл
\EqRef{int x2 dx=x3}
в виде
\EqRef{int x2 dx=x3 1}.
}

\DefProof{int x2 dx=x3 successive differentiation}
{
Согласно определению
\RefDefinition{indefinite integral},
отображение $y$ является интегралом
\EqRef{int x dx=x2},
если отображение $y$ удовлетворяет дифференциальному уравнению
\DrawEq{differential equation y=xx, 1, algebra}{integral}
и начальному условию
\DrawEq{differential equation, initial}{y=xx, algebra}
Мы воспользуемся методом последовательного дифференцирования,
чтобы решить дифференциальное уравнение
\eqRef{differential equation y=xx, 1, algebra}{integral}.
Последовательно дифференцируя уравнение
\eqRef{differential equation y=xx, 1, algebra}{integral},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, 2, algebra}
\ShowEq{differential equation y=xx, 3, algebra}
\ShowEq{differential equation y=xx, 4, algebra}
Разложение в ряд Тейлора
\DrawEq{y=x3+C}{algebra}
следует из уравнений
\ShowEq{differential equation y=xx, ref, algebra}
Равенство
\EqRef{int x dx=x2}
является следствием
\eqRef{differential equation y=xx, 1, algebra}{integral},
\eqRef{differential equation, initial}{y=xx, algebra},
\eqRef{y=x3+C}{algebra}.
Согласно определению
\EqRef{a ox b c=},
мы можем записать интеграл
\EqRef{int x2 dx=x3}
в виде
\EqRef{int x2 dx=x3 1}.
}

\DefRemark{notation int=x3 algebra}
{
В доказательстве теоремы
\RefTheorem{int x2 dx=x3}
я пользовался записью вида
\ShowEq{notation theorem int=x3 algebra}
Я записываю  следующие равенства для того,
чтобы показать как работает производная. 
\ShowEq{differential equation y=xx, algebra, 1}
}

\DefRemark{differential equation 3x^2 does not possess a solution}
{
Дифференциальное уравнение
\DrawEq{differential equation y=xx, 1, a, algebra}{integral}
\DrawEq{differential equation, initial}{}
так же приводит к решению $y=x^3$. Очевидно, что
отображение $y=x^3$ не удовлетворяет дифференциальному уравнению
\eqRef{differential equation y=xx, 1, a, algebra}{integral}.
Это говорит о том, что дифференциальное уравнение
\eqRef{differential equation y=xx, 1, a, algebra}{integral}
не имеет решений.

Я советую обратить внимание на то, что
вторая производная не
является симметричным многочленом (смотри разложение Тейлора).
}

\DefDefinition{exterior differential}
{
Пусть $A$, $B$ - банаховы $D$\Hyph алгебры.
Пусть
\ShowEq{U subset A}A
является открытым множеством.
Пусть отображение
\ShowEq{o:U->LAAB}DAB
является дифференциальной $p$\Hyph формой,
класса $C_n$, $n>0$.
Отображение
\ShowEq{exterior differential}
\ShowEq{exterior differential def}
называется
\AddIndex{внешним дифференциалом}{exterior differential}.
}

\DefDefinition{differential form of class Cn}
{
Говорят, что дифференциальная $p$\Hyph форма $\omega$
принадлежит к классу
\ShowEq{class Cn},
если отображение $\omega$ принадлежит к классу $C^n$.
Множество
\ShowEq{set of differential p forms}
$B$\Hyph значных дифференциальных $p$\Hyph форм
класса $C^n$, определённых на $U$
является $D$\Hyph модулем.
}

\DefDefinitionNote{norm on ring}
{
\AddIndex{Норма на кольце}{norm on ring}
$D$ - это отображение\,\footnotemark
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Кольцо $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется
\AddIndex{нормированным кольцом}{normed ring}.
}
{Определение дано согласно определению из
\citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2,
а также согласно определению
\citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.}

\DefDefinition{continuous map, module}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированного $D_1$\Hyph модуля $A_1$ с нормой $\|x\|_1$
в нормированный $D_2$\Hyph модуль $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|fx'-fx|<epsilon}
}

\DefDefinition{map of class Cn}
{
Отображение
\ShowEq{f:A->B}fAB
нормированного $D$\Hyph модуля $A$ в нормированный $D$\Hyph модуль $B$
принадлежит к классу $C^n$,
если отображение имеет непрерывную производную порядка $n$.
Отображение
\ShowEq{f:A->B}fAB
принадлежит к классу $C^{\infty}$,
если отображение имеет непрерывную производную любого порядка.
}

\DefDefinition[2]{starlike set}
{
Подмножество $U$ $#1$\Hyph алгебры $#2$ называется
\AddIndex{звёздным}{starlike set}
относительно $#2$\Hyph числа
\ShowEq{a in U},
если
\ShowEq{t'a+tx in U}{}
для любого $#2$\Hyph числа
\ShowEq{x in U}
и действительного числа
\ShowEq{0<t<1}.
}

\DefDefinition[1]{integral of differential 1 form along path}
{
Пусть
\ShowEq{U subset A}{#1}
- открытое множество.
Пусть
\ShowEq{g:ab->U}
путь класса $C^1$ в $U$.
\AddIndex{Интеграл дифференциальной $1$\Hyph формы $\omega$ вдоль пути}
{integral of differential 1 form along path}
$\gamma$ определён
равенством
\ShowEq{integral of differential 1 form along path}
\DrawEq{integral of differential 1 form along path =}{def}
}

\DefTheorem[2]{for any loop int g o=0}
{
Пусть
\ShowEq{U subset A}{#1}
- открытое связное множество.
Следующие свойства дифференциальной формы
\ShowEq{diff form in U}{\omega}n1{#2}{}
эквивалентны
\StartLabelItem
\begin{enumerate}
\item
$\omega$ интегрируемо в $U$
\labelItem{omega is integrable}
\item
\DrawEq{int g o=0}{-}
для любого кусочно гладкого цикла $\gamma$ в $U$ класса $C^1$
\labelItem{int g o=0}
\end{enumerate}
}

\DefDefinition[2]{definite integral}
{
Пусть
\ShowEq{U subset A}{#1}
- открытое связное множество.
Пусть дифференциальная форма
\ShowEq{diff form in U}{\omega}n1{#2}{}
интегрируема.
Для любых $#1$\Hyph чисел $a$, $b$,
мы определим
\AddIndex{определённый интеграл}{definite integral}
с помощью равенства
\ShowEq{definite integral}
\DrawEq{definite integral ab}{def}
для любого пути $\gamma$ из $a$ в $b$.
}

\DefTheorem[2]{int df=fb-fa}
{
Пусть
\ShowEq{U subset A}{#1}
- открытое множество.
Пусть
\ShowEq{g:ab->U}
путь класса $C^1$ в $U$.
Пусть
\ShowEq{f:A->B}f{#1}{#2}
дифференцируемое отображение.
Тогда
\ShowEq{int df=fb-fa}
}

\DefTheorem[2]{Differential 1 form is integrable iff}
{
Пусть
\ShowEq{U subset A}{#1}
- открытое звёздное множество.
Дифференциальная $1$\Hyph форма
\ShowEq{diff form in U}{\omega}n1{#2}{}
интегрируема тогда и только тогда, когда
\ShowEq{d omega=0}
}

\DefTheorem{derivative of tensor product}
{
Пусть $A$ - банаховый $D$\Hyph модуль.
Пусть $B$, $C$ - банаховые $D$\Hyph алгебры.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{f,g:A->BC}
Производная удовлетворяет соотношению
\ShowEq{differential of tensor product, algebra}
\ShowEq{derivative of tensor product, algebra}
}

\DefTheorem{map is continuous, derivative}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|a\|_A$.
Пусть $B$ - банаховая $D$\Hyph алгебра с нормой $\|b\|_B$.
Если производная
\ShowEq{df/dx}
отображения
\ShowEq{f:A->B}fAB
существует в точке $x$ и имеет конечную норму,
то отображение $f$ непрерывно в точке $x$.
}

\DefConvention{set of permutations SO}
{
Для $n\ge 0$, пусть
\ShowEq{set of permutations SO}
- множество перестановок
\ShowEq{s in SO(kn)}n{\sigma}
таких, что каждая перестановка $\sigma$
сохраняет порядок переменных $x_i$:
если $i<j$, то в кортеже
\ShowEq{s(y1kxn)}{\sigma}k{k+1}
$x_i$
предшествует
$x_j$.
}

\DefLemma{enumerate set of permutations SO(1,n)}
{
Мы можем пронумеровать множество перестановок $SO(1,n)$
индексом
\ShowEq{i 1n}
таким образом, что
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{s1(y)=y}
\item
Если $i>1$, то
\ShowEq{si(xi)=y}
\end{enumerate}
}

\DefProof{enumerate set of permutations SO(1,n)}
{
Так как порядок переменных
\ShowEq{x2...n}
в перестановке
\ShowEq{s in SO1n}
не зависит от перестановки, перестановки
\ShowEq{s in SO1n}
отличаются местом, которое занимает переменная $y$.
Соответственно, мы можем пронумеровать
множество перестановок $SO(1,n)$ индексом,
значение которого соответствует номеру позиции переменной $y$.
}

\AddEq{remark: enumerate set of permutations SO(1,n)}
{
Лемма
\RefLemma{enumerate set of permutations SO(1,n)}
имеет простую интерпретацию.
Предположим, что $n-1$ белых шаров и один чёрный лежат в пенале.
Чёрный шар - самый левый шар, и белые шары
пронумерованы от $2$ до $n$ в том порядке, как они лежат в пенале.
Суть перестановки $\sigma_k$ состоит в том, что мы вынимаем
чёрный шар из пенала и затем мы ложим его в ячейку с номером $k$.
При этом, белые шары с номером, не превышающим $k$, сдвигаются влево.
}

\DefLemma{SO(1,n+1)=SO(1,n)+}
{
Для $n>0$, пусть
\ShowEq{SO+(1,n)=}
Тогда
\ShowEq{SO(1,n+1)=SO(1,n)+}
}

\DefProof{SO(1,n+1)=SO(1,n)+}
{
Пусть
\ShowEq{sigma in SO+}
Согласно определению
\EqRef{SO+(1,n)=},
существует перестановка
\ShowEq{tau in SO1n}
такая, что
\ShowEq{tau x1n n+1}
Согласно соглашению
\RefConvention{set of permutations SO},
из утверждения
\ShowEq{i<j<n+1}
следует, что в кортеже
\ShowEq{tau x1n n+1}
переменная $x_j$ расположена между переменными $x_i$ и $x_{n+1}$.
Согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{sigma in SO1n}
Следовательно
\ShowEq{SO+ subset SO}
Согласно лемме
\RefLemma{enumerate set of permutations SO(1,n)},
множество
\ShowEq{SO+(1,n)}
имеет $n$ перестановок.

Пусть
\ShowEq{sigma=x2n y}
Согласно соглашению
\RefConvention{set of permutations SO},
\ShowEq{sigma in SO}
Согласно определению
\EqRef{SO+(1,n)=},
\ShowEq{sigma not in SO+}

Следовательно, мы перечислили $n+1$ элемент множества $SO(1,n+1)$.
Согласно лемме
\RefLemma{enumerate set of permutations SO(1,n)},
утверждение
\EqRef{SO(1,n+1)=SO(1,n)+}
является следствием утверждений
\EqRef{SO+ subset SO},
\EqRef{sigma in SO}.
}

\DefTheorem{dpn dx=+SO}
{
Для произвольного одночлена
\ShowEq{pn(x)=a xn}
производная имеет вид
\ShowEq{dpn dx=+SO}
}

\DefProof{dpn dx=+SO}
{
Для $n=1$,
отображение
\ShowEq{p1(x)=}
является линейным отображением.
Согласно теореме
\RefTheorem{derivative, fx=axb, algebra}
и соглашению
\RefConvention{set of permutations SO}
\ShowEq{dp1(x)=}

Пусть утверждение справедливо для $n-1$
\ShowEq{dpn-1}
Если
\ShowEq{pn(x)=}
то согласно теореме
\RefTheorem{derivative of product, algebra}
и определению
\EqRef{pn(x)=}
\ShowEq{dpn(x)=}
Равенство
\ShowEq{dpn(x)= 1}
следует из
\eqRef{dx/dx=1}1,
\EqRef{derivative, product over constant, algebra},
\EqRef{dpn-1},
\EqRef{dpn(x)=}.
Равенство
\ShowEq{dpn(x)= 2}
следует из
\EqRef{dpn(x)= 1}
и правила перемножения одночленов
\ePrints{1601.03259,4975-6381}
\ifx\Semafor\ValueOn
(определения
\RefDefinition{otimes -},
\RefDefinition{product of homogeneous polynomials}).
\else
(определение
\RefDefinition{polynomial*polynomial}
и теорема
\RefTheorem{(a*b)x=(ax)(bx)}).
\fi
Согласно лемме
\RefLemma{SO(1,n+1)=SO(1,n)+},
равенство
\EqRef{dpn dx=+SO}
является следствием равенства
\EqRef{dpn(x)= 2}.
}

\AddEq[1]{remark: d/dt sh ch successive differentiation}
{
Мы можем решить систему дифференциальных уравнений
\eqRef{d/dt sh ch #1}{sh ch},
пользуясь методом последовательного дифференцирования.
С этой целью мы рассмотрим степени матрицы $a$
\ShowEq{a**n 0 #1 #1 0}
Равенство
\ShowEq{dx/dt=a rc x, a**n 0 #1 #1 0, Taylor Series}
является следствием равенств
\EqRef{dx/dt=a*x right-cols.Taylor Series},
\EqRef{a**n 0 #1 #1 0}.
Равенство
\ShowEq{sinh t, cosh t, Taylor Series #1}
является следствием равенства
\EqRef{dx/dt=a rc x, a**n 0 #1 #1 0, Taylor Series}.
Из равенств
\EqRef{x=sht y=cht #1},
\EqRef{sinh t, cosh t, Taylor Series #1}
следует, что формула Эйлера
\ShowEq{sht cht Euler t#1}
верна для
\ShowEq{t#1 in}
Равенство
\ShowEq{dsinh/dt dcosh/dt #1}
является следствием равенств
\eqRef{d/dt sh ch #1}{sh ch},
\EqRef{sinh t, cosh t, Taylor Series #1}.
}

\DefLemma{mu,nu=lambda}
{
Пусть
\ShowEq{k<n}
Для любой пары перестановок
\ShowEq{mn in S(k,n)}{}
существует единственная перестановка
\ShowEq{s in SO(k,n)}{\sigma}{k+1}{}
такая, что
\ShowEq{s=nu(mu)}
}

\DefLemma{lambda=mu,nu}
{
Пусть
\ShowEq{k<n}
Для любой перестановки
\ShowEq{s in SO(k,n)}{\sigma}{k+1}{}
существует единственная пара перестановок
\ShowEq{mn in S(k,n)}{}
такая, что
\ShowEq{s=nu(mu)}
}

\DefTheorem{dkpn dx=+SO}
{
Для произвольного одночлена
\ShowEq{pn(x)=a xn}
производная порядка $k$ имеет вид
\ShowEq{dkpn dx=+SO}
}

\DefProof{dkpn dx=+SO}
{
Для $k=1$ утверждение теоремы
является утверждением теоремы
\RefTheorem{dpn dx=+SO}.
Пусть теорема верна для $k-1$. Тогда
\ShowEq{dk-1pn dx=+SO}
Согласно определению
\RefDefinition[\RefCalculus]{derivative of Order n, algebra},
равенство
\ShowEq{dkpn dx=+SO 1}
является следствием равенства
\EqRef{dk-1pn dx=+SO}.
Согласно теореме
\RefTheorem{dpn dx=+SO}
равенство
\ShowEq{dkpn dx=+SO 2}
является следствием равенства
\EqRef{dkpn dx=+SO 1}.
Согласно леммам
\RefLemma{mu,nu=lambda},
\RefLemma{lambda=mu,nu}
равенство
\ShowEq{dkpn dx=+SO 3}
является следствием равенства
\EqRef{dkpn dx=+SO 2}.
Следовательно, теорема верна для $k$.
}

\DefTheorem{e(a+b)=ea*eb}
{
Равенство
\ShowEq{e(a+b)=ea*eb}
справедливо тогда и только тогда, когда
\DrawEq{ab=ba}{exp}
}

\DefProof{e(a+b)=ea*eb}
{
Для доказательства теоремы достаточно рассмотреть ряды Тейлора
\DrawEq[aa]{ea=sum...}{a*}
\DrawEq[bb]{ea=sum...}{b*}
\DrawEq[{a+b}{(a+b)}]{ea=sum...}{a+b*}
Перемножим выражения
\eqRef{ea=sum...}{a*}
и
\eqRef{ea=sum...}{b*}.
Сумма одночленов порядка $3$ имеет вид
\ShowEq{exponent ab 3}
и не совпадает, вообще говоря, с выражением
\ShowEq{exponent a+b 3}
Доказательство утверждения, что
\EqRef{e(a+b)=ea*eb} следует из \eqRef{ab=ba}{exp},
тривиально.
}

\DefCorollary{debxc=ebxc}
{
Если $a=b\otimes c$, то равенство
\EqRef{deax=eax}
имеет вид
\ShowEq{debxc=ebxc}
}

\DefTheorem{deax=eax}
{
Пусть
\ShowEq{a in AA}aA.
\ShowEq{deax=eax}
}

\DefProof{deax=eax}
{
Равенство
\ShowEq{deax/dx=}
является следствием теорем
\RefTheorem{dex=ex},
\RefTheorem[\RefCalculus]{composite map, derivative, D algebra}.
}

\DefDefinition{exponent}
{
Мы назовём отображение
\ShowEq{e**x=Taylor}
экспонентой.
}

\AddEq{theorem: composite map, derivative, D algebra}
{
\begin{ShadedTheorem}
\labelTheorem{composite map, derivative, D algebra}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $\|a\|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $\|b\|_B$.
Пусть $C$ - банаховый $D$\Hyph модуль с нормой $\|c\|_C$.
Пусть отображение
\ShowEq{f:A->B}fAB
дифференцируемо в точке
$x$
и норма производной отображения $f$
конечна
\ShowEq{composite map, norm f, D algebra}
Пусть отображение
\ShowEq{f:A->B}gBC
дифференцируемо в точке
\ShowEq{composite map, y fx, D algebra}
и норма производной отображения $g$
конечна
\ShowEq{composite map, norm g, D algebra}
Отображение\,\footnotemark
\ShowEq{composite map, gfx, D algebra}
дифференцируемо в точке
\labelItem{composite map is differentiable}
$x$
\ShowEq{composite map, derivative, D algebra}
\end{ShadedTheorem}
\footnotetext{\,
Запись
\ShowEq{dg/df}
означает выражение
\ShowEq{dg/df=}
Аналогичное замечание верно для компонент производной.
}
}


==> Stmt.Group.Russian.tex <==
%auto-ignore
\input{Stmt.Group.Eq}

\AddEq{def *}
{
\def\GroupType{мультиплика}%
\def\GroupTypeC{Мультиплика}%
\def\GroupOpNameWNS{произведением}
\def\GroupOpName{произведение }
\def\GroupOpNameC{Произведение }
\def\GroupOpNameNS{умножение}
\def\GroupOpNameS{умножение }
\def\GroupUnit{единичный }
\def\GroupUnitD{единичным }
\def\GroupUnitE{единичному }
\def\GroupUnitC{Единичный }
\def\GroupUnitP{единичные }
\def\OpEnd{о}
\def\OpEndS{о }
\def\ArgsOfOp{сомножители}
}

\AddEq{def +}
{
\def\GroupType{адди}%
\def\GroupTypeC{Адди}%
\def\GroupOpNameWNS{суммой}
\def\GroupOpName{сумма }
\def\GroupOpNameC{Сумма }
\def\GroupOpNameNS{сложение}
\def\GroupOpNameS{сложение }
\def\GroupUnit{нулевой }
\def\GroupUnitD{нулевым }
\def\GroupUnitE{нулевому }
\def\GroupUnitC{Нулевой }
\def\GroupUnitP{нулевые }
\def\OpEnd{а}
\def\OpEndS{а }
\def\ArgsOfOp{слагаемые}
}

\DefFootnote{monoid}
{
Смотри также определения
моноида на странице
\citeBib{Serge Lang}\Hyph 17.
}

\DefLabeledDefinition{monoid}{\GroupLbl}
{
Пусть на множестве $A$ определена
бинарная операция\,\RefFootnote{monoid}
\ShowEq{a,b in A->ab in A (\GroupLbl)}
которую мы называем \GroupOpNameWNS.
Множество $A$ называется \GroupType тивным моноидом, если
\StartLabelItem
\begin{enumerate}
\item
\GroupOpName
{\bf ассоциативн\OpEnd}
\ShowEq{(\GroupLbl) is associative}
\item
\GroupOpName имеет \GroupUnit элемент $\UnitId$
\ShowEq{unit element (\GroupLbl)}
\end{enumerate}
Если \GroupOpName
{\bf коммутативн\OpEnd}
\ShowEq{product is commutative (\GroupLbl)}
то \GroupType тивный моноид $A$ называется
коммутативным или абелевым.
}

\DefFootnote{A=Bo+C}
{
Смотри также замечание в \citeBib{Serge Lang}, страница 56.
}

\DefLabeledTheorem{A=Bo+C}{\GroupLbl}
{
Пусть $B$, $C$ - подгруппы \GroupType вной абелевой группы $A$.
Пусть
\ShowEq{A=B+C}
Тогда\,\RefFootnote{A=Bo+C}
\ShowEq{A=Bo+C}BC
}

\DefProof{A=Bo+C}
{
Отображение
\DrawEq{f:BxC->A}{\GroupLbl}
является гомоморфизмом групп.
Это утверждение следует из равенств
\ShowEq{f x1+x2 =}

Пусть $f(x,y)=\UnitId$.
Из равенства
\eqRef{f:BxC->A}{\GroupLbl}
следует, что
\DrawEq{xB+yC=0}{\GroupLbl}
Из равенства
\eqRef{xB+yC=0}{\GroupLbl}
следует, что
\ShowEq{x=-y in C(\GroupLbl)}
Следовательно,
$x=y=\UnitId$.
Следовательно, отображение $f$ является изоморфизмом групп.

Согласно теореме
\refTheorem{direct sum of Abelian groups}{\GroupLbl}
\DrawEq{BxC=Bo+C}{\GroupLbl}
Теорема является следствием равенства
\eqRef{BxC=Bo+C}{\GroupLbl}.
}

\DefLabeledExample{H o+ G, H in G}{\GroupLbl}
{
Пусть абелевая группа $H$ является подгруппой \GroupType тивной абелевой группы $G$.
Найдём $H\oplus G$.
Мы будем пользоваться теоремой
\refTheorem{direct sum of Abelian groups}{\GroupLbl}.
Положим
\ShowEq{A=HxG}
Мы определим \GroupOpNameS равенством
\ShowEq{sum HxG}
Следовательно, если $a\in H$, то кортежи
$(a,0)$ и $(0,a)$
представляют различные $(H\oplus G)$\Hyph числа.
}

\DefTheorem{A=C o+ D free group}
{
Пусть
\ShowEq{f:A->B}fAB
сюръективный гомоморфизм абелевых групп и
\ShowEq{C=ker f}
Если $B$ - свободная группа,
то существует подгруппа $D$ группы $A$
такая, что ограничение $f$ на $D$
индуцирует изоморфизм $D$ на $B$ и
\ShowEq{A=C o+ D}
}

\DefProof{A=C o+ D free group}
{
\TwoColText
{
\ShowEq{def multiplicative}
\ShowText{A=C o+ D free group}
}
{
\ShowEq{def additive}
\ShowText{A=C o+ D free group}
}
}

\DefText{A=C o+ D free group}
{
Пусть $A$, $B$ - \GroupType тивные абелевые группы.
Пусть
\ShowEq{bi in B}b
- базис группы $B$.
Для каждого \iI, пусть $a_i$ - $A$\Hyph число такое, что
\DrawEq{fai=bi}{\GroupLbl}
Пусть $D$ - подгруппа в $A$, порождённая $A$\Hyph числами
\ShowEq{ai in A}
Пусть
\ShowEq{niai=0(\GroupLbl)}
для целых $n^i$
таких, что множество
\ShowEq{|gi ne 0|}n
конечно.
Равенство
\ShowEq{nifai=0(\GroupLbl)}
следует из равенств
\eqRef{fai=bi}{\GroupLbl},
\EqRef{niai=0(\GroupLbl)}
и теорем
\refTheorem{monoid-homomorphism}{\GroupLbl},
\refTheorem{homomorphism f(na)=nf(a)}{\GroupLbl}.
Так как
\ShowEq{bi in B}b
- базис,
то  согласно определениям
\refDefinition{linearly independent vectors,  Abelian group}{\GroupLbl},
\refDefinition{basis of Abelian group}{\GroupLbl},
утверждение
\ShowEq{ni=0 iI}
следует из равенства
\EqRef{nifai=0(\GroupLbl)}.
Следовательно, множество
\ShowEq{bi in B}a
- базис подгруппы $D$.

Пусть $a\in D$ и $f(a)=\UnitId$.
Так как множество
\ShowEq{bi in B}a
- базис подгруппы $D$,
то существуют целые числа $n^i$ такие, что
\ShowEq{a=nai(\GroupLbl)}
и множество
\ShowEq{|gi ne 0|}n
конечно.
Следовательно, равенство
\ShowEq{0=fa=nbi(\GroupLbl)}
следует из равенства
\EqRef{a=nai(\GroupLbl)}
и теорем
\refTheorem{monoid-homomorphism}{\GroupLbl},
\refTheorem{homomorphism f(na)=nf(a)}{\GroupLbl}.
Так как множество
\ShowEq{bi in B}b
является базисом группы $B$,
$n^i=0$, \iI,
является следствием равенства
\EqRef{0=fa=nbi(\GroupLbl)}.
Следовательно, $a=\UnitId$ и
\ShowEq{D A C=0}

Пусть $a\in A$.
Так как $f(x)\in B$ и множество
\ShowEq{bi in B}b
является базисом группы $B$,
то существуют целые числа $n^i$ такие, что
\ShowEq{fx=nbi(\GroupLbl)}
и множество
\ShowEq{|gi ne 0|}n
конечно.
Равенство
\ShowEq{f(x-niai)=(\GroupLbl)}
является следствием равенств
\eqRef{fai=bi}{\GroupLbl},
\EqRef{fx=nbi(\GroupLbl)}.
Из равенства
\EqRef{f(x-niai)=(\GroupLbl)}
следует, что
\ShowEq{x-niai in ker(\GroupLbl)}
Из утверждения
\EqRef{x-niai in ker(\GroupLbl)}
следует, что
$a\in C+D$.
Согласно теореме
\refTheorem{A=Bo+C}{\GroupLbl},
\ShowEq{A=Bo+C}CD
}

\DefText{B=Ao+B/A}
{
Пусть $B$ - \GroupType тивная абелевая группа.
Согласно примерам
\refExample{0->A->B->C->0}{\GroupLbl},
\refExample{0->A->B->B/A->0}{\GroupLbl},
последовательность гомоморфизмов
\ShowEq{0->A->B->B/A->0 =}
является точной.
Согласно примеру
\refExample{0->A->B->C->0}{\GroupLbl},
гомоморфизм $f$ является мономорфизмом.
Согласно определению
\RefDefinition{exact sequence},
\ShowEq{A=ker g}
Согласно примеру
\refExample{0->A->B->C->0}{\GroupLbl},
гомоморфизм $g$ является эпиморфизмом.
Согласно теореме
\RefTheorem{A=C o+ D free group},
существует подгруппа $D$ группы $B$,
изоморфная группе $B/A$, такая, что
\DrawEq{B=Ao+D}{\GroupLbl}
Если отождествить $D$\Hyph число $d$
и множество $dA$, то равенство
\EqRef{B=Ao+B/A}
является следствием равенства
\eqRef{B=Ao+D}{\GroupLbl}.
}

\DefTheorem{B=Ao+B/A}
{
Пусть $A$ - подгруппа абелевой группы $B$.
Если группа $B/A$ - свободна, то
\ShowEq{B=Ao+B/A}
}

\DefLabeledTheorem{monoid-homomorphism, sum}{\GroupLbl}
{
Пусть отображения
\ShowEq{f:A->B}fAB
\ShowEq{f:A->B}gAB
являются гомоморфизмами
\GroupType тивной абелевой группы $A$ с \GroupUnitD элементом $\UnitId_1$
в \GroupType тивную абелевую группу $B$ с \GroupUnitD элементом $\UnitId_2$.
Тогда отображение
\ShowEq{f:A->B}hAB
определённое равенством
\ShowEq{h(x)=f+g(x)}
является гомоморфизмом
\GroupType тивной абелевой группы $A$
в \GroupType тивный абелевую группу $B$.
}

\DefProof{monoid-homomorphism, sum}
{
Теорема является следствием равенств
\ShowEq{h(x+y)=h(x)+h(y)}
\ShowEq{h(x)=f+g(x) 0}
и теоремы
\refTheorem{monoid-homomorphism}{\GroupLbl}.
}

\DefLabeledExample{0->A->B->C->0}{\GroupLbl}
{
Пусть
\DrawEq{0->A->B->C->0}{\GroupLbl}
точная последовательность гомоморфизмов \GroupType тивных групп.

Согласно равенству
\eqRef{fe1=e2}{(\GroupLbl)}
и определению
\RefDefinition{exact sequence},
\ShowEq{ker f=0}
Согласно теореме
\refTheorem{trivial kernel}{+},
отображение $f$ является мономорфизмом.

Из диаграммы
\eqRef{0->A->B->C->0}{\GroupLbl}
следует, что
\ShowEq{ker h=C}
Согласно определению
\RefDefinition{exact sequence},
\ShowEq{Im g=C}
Согласно определению
\RefDefinition{isomorphism},
гомоморфизм $g$ является эпиморфизмом.
}

\DefLabeledExample{0->A->B->0}{\GroupLbl}
{
Согласно примеру
\refExample{0->A->B->C->0}{\GroupLbl},
если последовательность гомоморфизмов аддитивных групп
\DrawEq{0->A->B->0}{}
точна, то гомоморфизм $f$ является изоморфизмом.
}

\DefLabeledExample{0->A->B->B/A->0}{\GroupLbl}
{
Объединяя примеры
\refExample{0->A->B->C->0}{\GroupLbl},
\refExample{0->A->B->0}{\GroupLbl},
мы получим диаграмму
\ShowEq{0->A->B->B/A->0}
где строки и столбец
являются точными последовательностями гомоморфизмов
и гомоморфизм $f$ является изоморфизмом.
}

\DefLabeledTheorem{Abelian group is free}{\GroupLbl}
{
\GroupTypeC тивная абелевая группа $G$ свободна тогда и только тогда,
когда абелевая группа $G$ имеет базис
\ShowEq{S=si}
и множество $G$\Hyph чисел $S$
линейно независимо.
}

\DefProof{Abelian group is free}
{
Согласно определению
\refDefinition{free Abelian group}{\GroupLbl}
и доказательству теоремы
\refTheorem{free Abelian group}{\GroupLbl},
существует множество $S\subseteq G$ такое, что диаграмма
\DrawEq{AbS ff'g}{}
коммутативна
}

\DefLabeledTheorem{Unit element of monoid is unique}{\GroupLbl}
{
\GroupUnitC элемент \GroupType тивного моноида $A$ определён однозначно.
}

\DefProof{Unit element of monoid is unique}
{
Пусть $\UnitId_1$, $\UnitId_2$ - \GroupUnitP элементы \GroupType тивного моноида $A$.
Равенство
\DrawEq{e1=e2}{\GroupLbl}
следует из утверждения
\RefItem{unit element (\GroupLbl)}.
Теорема следует из равенства
\eqRef{e1=e2}{\GroupLbl}.
}

\DefLabeledRemark{monoid is universal algebra}{\GroupLbl}
{
Согласно определениям
\RefDefinition{Omega-algebra},
\refDefinition{monoid}{\GroupLbl}
и теореме
\refTheorem{Unit element of monoid is unique}{\GroupLbl}
\GroupType тивный моноид - это универсальная алгебра
с одной бинарной операцией (\GroupOpNameNS)
и одной $0$\Hyph арной операцией (\GroupUnit элемент).
}

\DefFootnote{group}
{
Смотри также определение группы на странице
\citeBib{Serge Lang}\Hyph 21.
}

\DefLabeledDefinition{group}{\GroupLbl}
{
\GroupTypeC тивный моноид\,\RefFootnote{group}
$A$ называется \GroupType тивной группой, если
для каждого $A$\Hyph числа $x$
существует $A$\Hyph число $y$
такое, что
\ShowEq{there exists inverse}
$A$\Hyph число $y$ называется обратным к $A$\Hyph числу $x$.
Если \GroupOpName коммутативно,
то \GroupType тивная группа $A$ называется коммутативной или абелевой.
}

\DefLabeledTheorem{monoid-homomorphism}{\GroupLbl}
{
Отображение
\ShowEq{f:A->B}fAB
является гомоморфизмом
\GroupType тивного моноида $A$ с \GroupUnitD элементом $\UnitId_1$
в \GroupType тивный моноид $B$ с \GroupUnitD элементом $\UnitId_2$,
если
\ShowEq{fab=fafb (\GroupLbl)}
\DrawEq{fe1=e2}{(\GroupLbl)}
для любых $A$\Hyph чисел $a$, $b$.
}

\DefProof{monoid-homomorphism}
{
Теорема является следствием определений
\ShowRef{monoid homomorphism}
и замечания
\refRemark{monoid is universal algebra}{\GroupLbl}.
}

\DefFootnote{group-homomorphism}
{
Мы будем также пользоваться термином
гомоморфизм групп
для отображения $f$.
}

\DefLabeledTheorem{group-homomorphism}{\GroupLbl}
{
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм\,\RefFootnote{group-homomorphism}
\GroupType тивной группы $A$ с \GroupUnitD элементом $\UnitId_1$
в \GroupType тивную группу $B$ с \GroupUnitD элементом $\UnitId_2$.
Тогда
\ShowEq{f(a-)=f(a)-(\GroupLbl)}
}

\DefProof{group-homomorphism}
{
Равенство
\ShowEq{f(a-)=f(a)- 1(\GroupLbl)}
является следствием равенств
\ShowRef{f(a-)=f(a)- 2}
Равенство
\EqRef{f(a-)=f(a)-(\GroupLbl)}
является следствием равенства
\EqRef{f(a-)=f(a)- 1(\GroupLbl)}
и теоремы
\refTheorem{inverse in group is unique}{\GroupLbl}.
}

\DefTheorem{Image of group homomorphism}
{
Образ гомоморфизма групп
\ShowEq{f:A->B}fAB
является подгруппой группы $B$.
}

\DefText{Image of group homomorphism}
{
Пусть $A$ и $B$ - \GroupType тивные группы.
Согласно определениям
\ShowRef{group-homomorphism}
и теореме
\refTheorem{monoid-homomorphism}{\GroupLbl},
множество $\im f$ является моноидом.
Согласно теореме
\refTheorem{group-homomorphism}{\GroupLbl},
множество $\im f$ является группой.
}

\DefText{homomorphism addi to multi}
{
Существует гомоморфизм аддитивной группы в мультипликативную.
Например, отображение $y=e^x$ является
гомоморфизмом аддитивной группы действительных чисел
в мультипликативную группу положительных действительных чисел.
}

\DefText{be homomorphism of group}
{
Пусть
\DrawEq[fAB{}{}]{f: A->B}{}
гомоморфизм
\GroupType тивной группы $A$ с \GroupUnitD элементом $\UnitId_1$
в \GroupType тивную группу $B$ с \GroupUnitD элементом $\UnitId_2$.
}

\DefLabeledTheorem{trivial kernel}{\GroupLbl}
{
\ShowText{be homomorphism of group}
Если
\DrawEq{ker f=e}{\GroupLbl}
то ядро гомоморфизма $f$ называется
{\bf тривиальным},
а гомоморфизм $f$ является мономорфизмом.
}

\DefProof{trivial kernel}
{
Пусть существуют $A$\Hyph числа $a$, $b$ такие, что
\DrawEq[ab]{fa=fb}{ab(\GroupLbl)}
Равенство
\ShowEq{f(ab-)=.e(\GroupLbl)}
является следствием равенств
\ShowRef{f(ab-)=.e}
и утверждения
\RefItem{unit element (\GroupLbl)}.
Равенство
\ShowEq{ab-=.e(\GroupLbl)}
является следствием равенств
\ShowRef{ab-=.e}%
Из равенств
\EqRef{-(-a)=a (\GroupLbl)},
\EqRef{ab-=.e(\GroupLbl)}
и теоремы
\refTheorem{inverse in group is unique}{\GroupLbl}
следует, что $a=b$.
}

\DefLabeledTheorem{normal subgroup and homomorphism}{\GroupLbl}
{
Пусть $B$ - нормальная подгруппа \GroupType тивной группы $A$
с \GroupUnitD элементом $\UnitId$.
Существует \GroupType тивная группа $C$
и гомоморфизм
\ShowEq{f:A->B}fAC
такие, что
\DrawEq{ker f=B}{\GroupLbl}
}

\DefProof{normal subgroup and homomorphism}
{
Положим
\ShowEq{fx=xB}
Поскольку множество $\UnitId\GroupLbl B=B$ является
\GroupUnitD элементом \GroupType тивной группы $A/B$, то
\DrawEq{B in ker}{\GroupLbl}
Если $f(x)=B$, то $x\GroupLbl B=B$.
Согласно теореме
\refTheorem{aH A bH ne 0}{\GroupLbl},
$x\in B$.
Следовательно,
\DrawEq{ker in B}{\GroupLbl}
Теорема является следствием утверждений
\eqRef{B in ker}{\GroupLbl},
\eqRef{ker in B}{\GroupLbl}.
}

\DefLabeledDefinition{linear combination of g numbers}{\GroupLbl}
{
Пусть
\ShowEq{S=si}
- множество $G$\Hyph чисел.
\ShowEq{g number linear combination (\GroupLbl)}%
Выражение
\ShowEq{g number linear combination =}
называется
\AddIndex{линейной комбинацией}{linear combination} $G$\Hyph чисел
$\aD si$.
$G$\Hyph число
\ShowEq{g=gi si (\GroupLbl)}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от $G$\Hyph чисел
$\aD si$.
}

\DefText{quasibasis of Abelian group}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{structure of Abelian group}{\GroupLbl}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefLabeledDefinition{quasibasis of Abelian group}{\GroupLbl}
{
Если множество $X\subset G$ является множеством образующих
абелевой группы $G$, то любое множество $Y$, $X\subset Y\subset G$
также является множеством образующих абелевой группы $G$.
Если существует минимальное множество $X$, порождающее
абелевую группу $G$, то такое множество $X$ называется
\AddIndex{квазибазисом}{quasibasis}
абелевой группы $G$.
}

\DefText{generating set of group}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{structure of Abelian group}{\GroupLbl}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefLabeledDefinition{generating set of group}{\GroupLbl}
{
$J(S)$
называется
\AddIndex{подгруппой, порождённой множеством}
{subgroup generated by set} $S$,
а $S$ -
\AddIndex{множеством образующих}{generating set}
подгруппы $J(S)$.
В частности,
\AddIndex{множеством образующих}{generating set}
абелевой группы
будет такое подмножество $X\subset G$, что
\ShowEq{generating set of group}
}

\DefLabeledDefinitionNote{linearly independent vectors, Abelian group}{\GroupLbl}
{
Множество $G$\Hyph чисел\,\footnotemark
\ShowEq{set vi cols}g
%
\AddIndex{линейно независимо}{linearly independent set},
если $w=\UnitId$ следует из уравнения
\ShowEq{group wi vi=0 (\GroupLbl)}
В противном случае, множество $G$\Hyph чисел
\ShowEq{set vi cols}g
\AddIndex{линейно зависимо}{linearly dependent set}.
}
{
Я следую определению в
\citeBib{Serge Lang}, страница 100.
}

\DefLabeledDefinition{basis of Abelian group}{\GroupLbl}
{
Пусть множество $G$\Hyph чисел
\ShowEq{S=si}
является квазибазисом.
Если множество $G$\Hyph чисел $S$
линейно независимо,
то квазибазис $S$ называется
\AddIndex{базисом}{basis}
абелевой группы $G$.
}

\DefLabeledTheorem{ker group-homomorphism}{\GroupLbl}
{
\ShowText{be homomorphism of group}
Множество
\DrawEq{show ker group-homomorphism}{\UnitId}
называется
{\bf ядром гомоморфизма $f$ групп}.
Ядро гомоморфизма групп
является нормальной подгруппой группы $A$.
}

\DefProof{ker group-homomorphism}
{
Пусть $A$ - \GroupType тивная группа.
\StartLabelItem
\begin{enumerate}
\item
Пусть
\ShowEq{ab in ker f}
Равенство
\ShowEq{fab=...e}
является следствием равенств
\ShowRef{fab=...e}
и утверждения
\RefItem{unit element (\GroupLbl)}.
Согласно определению
\eqRef{show ker group-homomorphism}{\UnitId},
$a\GroupLbl b\in\ker f$.
\item
Согласно равенствам
\eqRef{fe1=e2}{(\GroupLbl)},
\eqRef{show ker group-homomorphism}{\UnitId},
\ShowEq{e in ker f}
\item
\labelItem{ker f is monoid (\GroupLbl)}
Из утверждений
\RefItem{a\GroupLbl b in ker f},
\RefItem{\UnitId in ker f}
следует, что множество $\ker f$ является \GroupType тивным моноидом.
\item
Пусть
$a\in\ker f$.
Согласно теореме
\refTheorem{inverse in group is unique}{\GroupLbl},
существует $A$\Hyph число
\ShowEq{a-(\GroupLbl)}
Равенство
\ShowEq{fa-=...\UnitId}
является следствием равенств
\EqRef{e-=e (\GroupLbl)},
\EqRef{f(a-)=f(a)-(\GroupLbl)},
\eqRef{show ker group-homomorphism}{\UnitId}.
Согласно определению
\eqRef{show ker group-homomorphism}{\UnitId},
\ShowEq{a- in ker f(\GroupLbl)}
\end{enumerate}
Согласно утверждениям
\RefItem{ker f is monoid (\GroupLbl)},
\RefItem{a- in ker f(\GroupLbl)},
множество $\ker f$ является \GroupType тивной группой.

Равенство
\ShowEq{fxHx-=e (\GroupLbl)}
является следствием равенств
\ShowRef{fxHx-=e}
Равенство
\ShowEq{xHx-=H (\GroupLbl)}
является следствием равенства
\EqRef{fxHx-=e (\GroupLbl)}.
Следовательно,
\DrawEq{a ker=ker a}{\GroupLbl}
Теорема является следствием равенства
\eqRef{a ker=ker a}{\GroupLbl}
и определения
\refDefinition{normal subgroup}{\GroupLbl}.
}

\DefLabeledTheorem{inverse in group is unique}{\GroupLbl}
{
Пусть $A$ - \GroupType тивная группа.
$A$\Hyph число $y$, обратное к $A$\Hyph числу $a$,
определено однозначно.
Мы пользуемся записью
\ShowEq{y=a- (\GroupLbl)}
\ShowEq{a(a-)=e (\GroupLbl)}
}

\DefProof{inverse in group is unique}
{
Пусть $y_1$, $y_2$ - обратные числа к $A$\Hyph числу $a$.
Равенство
\ShowEq{y1=y2 (\GroupLbl)}
является следствием утверждений
\RefItem{(\GroupLbl) is associative},
\RefItem{unit element (\GroupLbl)}
и определения
\refDefinition{group}{\GroupLbl}.
Теорема является следствием равенства
\EqRef{y1=y2 (\GroupLbl)}.
}

\DefLabeledTheorem{-(-a)=a}{\GroupLbl}
{
Если $A$ - \GroupType тивная группа, то
\ShowEq{-(-a)=a (\GroupLbl)}
}

\DefProof{-(-a)=a}
{
Согласно определению
\EqRef{a(a-)=e (\GroupLbl)},
$A$\Hyph число $y$, обратное к $A$\Hyph числу
\ShowEq{a- (\GroupLbl)}a,
иммет вид
\ShowEq{-(-a) (\GroupLbl)}
\ShowEq{-(-a)= (\GroupLbl)}
равенство
\EqRef{-(-a)=a (\GroupLbl)}
является следствием равенств
\EqRef{a(a-)=e (\GroupLbl)},
\EqRef{-(-a)= (\GroupLbl)}
и теоремы
\refTheorem{inverse in group is unique}{\GroupLbl}.
}

\DefLabeledTheorem{Inverse of unit is unit}{\GroupLbl}
{
Пусть $A$ - \GroupType тивная группа с \GroupUnitD элементом $\UnitId$.
$A$\Hyph число, обратное к \GroupUnitE элементу,
является \GroupUnitD элементом
\ShowEq{e-=e (\GroupLbl)}
}

\DefProof{Inverse of unit is unit}
{
Равенство
\ShowEq{e-=e-e (\GroupLbl)}
является следствием теорем
\refTheorem{Unit element of monoid is unique}{\GroupLbl},
\refTheorem{inverse in group is unique}{\GroupLbl}.
Равенство
\EqRef{e-=e (\GroupLbl)}
является следствием равенства
\EqRef{e-=e-e (\GroupLbl)}.
}

\DefLabeledDefinition{coset in group}{\GroupLbl}
{
Пусть $H$ - подгруппа \GroupType тивной группы $G$.
Множество
\DrawEq{aH=}{\GroupLbl}
называется
{\bf левым смежным классом}.
Множество
\ShowEq{Ha=}
называется
{\bf правым смежным классом}.
}

\DefLabeledTheorem{aH A bH ne 0}{\GroupLbl}
{
Пусть $H$ - подгруппа \GroupType тивной группы $G$.
Если
\DrawEq{aH A bH ne 0}{\GroupLbl}
то
\ShowEq{aH=bH}
}

\DefProof{aH A bH ne 0}
{
Из утверждения
\eqRef{aH A bH ne 0}{\GroupLbl}
и определения
\eqRef{aH=}{\GroupLbl}
следует, что существуют $H$\Hyph числа $c$, $d$ такие, что
\DrawEq{ac=bd}{\GroupLbl}
\StartLabelItem
\begin{enumerate}
\item
Согласно теореме
\refTheorem{inverse in group is unique}{\GroupLbl},
существует $H$\Hyph число
\ShowEq{a- (\GroupLbl)}d.
Следовательно,
\ShowEq{cd-1 in H (\GroupLbl)}
\item
Если $c\in H$, то из определения
\eqRef{aH=}{\GroupLbl}
следует, что
\ShowEq{cH=H}
\item
Из утверждений
\RefItem{cd-1 in H (\GroupLbl)},
\newline
\RefItem{cH=H (\GroupLbl)}
следует, что
\ShowEq{cd-H=H (\GroupLbl)}
\item
Из утверждения
\RefItem{(\GroupLbl) is associative}
и определения
\refDefinition{group}{\GroupLbl}
следует, что
\ShowEq{(ab)H=a(bH)}
\item
\begin{sloppypar}
Равенство
\ShowEq{a(cd-)=b (\GroupLbl)}
является следствием утверждений
\RefItem{(\GroupLbl) is associative},
\RefItem{unit element (\GroupLbl)}
и равенств
\EqRef{a(a-)=e (\GroupLbl)},
\eqRef{ac=bd}{\GroupLbl}.
\end{sloppypar}
\end{enumerate}
Равенство
\ShowEq{bH=.=aH (\GroupLbl)}
является следствием утверждений
\newline
\RefItem{cd-H=H (\GroupLbl)},
\RefItem{a(cd-)=b (\GroupLbl)}.
}

\DefFootnote{normal subgroup}
{
Смотри также определение на странице
\citeBib{Serge Lang}\Hyph 27.
}

\DefLabeledDefinition{normal subgroup}{\GroupLbl}
{
Подгруппа $H$ \GroupType тивной группы $A$ такая, что
\ShowEq{normal subgroup}
для любого $A$\Hyph числа, называется
{\bf нормальной}.\,\RefFootnote{normal subgroup}
}

\DefText{mod H}
{
Согласно теореме
\refTheorem{aH A bH ne 0}{\GroupLbl},
нормальная подгруппа $H$ \GroupType тивной группы $A$
порождает отношение эквивалентности \Mod H на множестве $A$
\DrawEq{a rho b...}{\GroupLbl}
Мы будем обозначать $A/H$ множество классов эквивалентности
отношения эквивалентности \Mod H.
}

\DefLabeledTheorem{aHbH=abH}{\GroupLbl}
{
Пусть $H$ - нормальная подгруппа \GroupType тивной группы $A$.
\GroupOpNameC
\DrawEq{aHbH=abH}{\GroupLbl}
порождает группу на множестве $A/H$.
}

\DefProof{aHbH=abH}
{
Равенство
\DrawEq{aHbH=.abH}{\GroupLbl}
следует из определения
\refDefinition{normal subgroup}{\GroupLbl}
и утверждений
\RefItem{(\GroupLbl) is associative},
\RefItem{(ab)H=a(bH) (\GroupLbl)}.

Равенство
\eqRef{aHbH=abH}{\GroupLbl}
является следствием равенства
\eqRef{aHbH=.abH}{\GroupLbl}.

Пусть
\ShowEq{c in aH, d in bH}
Тогда равенство
\ShowEq{abH=cdH}
следует из определения
\eqRef{aHbH=abH}{\GroupLbl}
и теоремы
\refTheorem{aH A bH ne 0}{\GroupLbl}.
Следовательно, произведение
\eqRef{aHbH=abH}{\GroupLbl}
не зависит от выбора $A$\Hyph чисел
\ShowEq{c in aH, d in bH}

Так как
\ShowEq{eH=H}
то из равенства
\eqRef{aHbH=abH}{\GroupLbl}
следует, что произведение
\eqRef{aHbH=abH}{\GroupLbl}
удовлетворяет определению \GroupType тивной группы.
}

\DefLabeledDefinition{factor group}{\GroupLbl}
{
Пусть $H$ - нормальная подгруппа \GroupType тивной группы $A$.
Группа $A/H$ называется
{\bf факторгруппой}
группы $A$ по $H$ и отображение
\ShowEq{f:A->B}f{a\in A}{a\GroupLbl H\in A/H}
называется
{\bf каноническим отображением}.
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теорем
\refTheorem{action of ring of rational integers in Abelian group}{+},
\refTheorem{Abelian group is free}{+}
и определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
следует, что свободная абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefText[2]{ix-xi-1 roots}
{
многочлен
\DrawEq[1]{ix-xi-1}{#1}
не имеет корней
и многочлен
\DrawEq[k]{ix-xi-1}{#2}
имеет множество корней
\DrawEq{x=c12+j}{#2}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Пусть произведение в алгебре
\AoxA H
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{RH}
Представление
\DrawEq[RH]{h:AoxA->L(A)}H
$R$\Hyph алгебры
\AoxA H
в абелевой группе
\ShowEq{L(A->B)}RHH,
определённое равенством
\DrawEq[RH]{representation AA in LA}{RH}
является левым \BoxB{H}модулем.
Если мы положим $g=E$,
где
\ShowEq{product in algebra AA 3}RHE
- тождественное отображение,
то мы можем отождествить линейное отображение
\DrawEq[fHH{}]{f: A->B}-
алгебры кватернионов и тензор
\DrawEq{linear map f, basis E}1
опираясь на равенство
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
Теорема является следствием утверждения
что отображение
\ShowEq{Eox=x}
порождает любое линейное отображение алгебры кватернионов
}

\DefDefinition{square root}
{
Решение
\ShowEq{square root}
уравнения
\DrawEq{x2=a}{root}
в $D$\Hyph алгебре $A$
называется
\AddIndex{квадратным корнем}{square root}
$A$\Hyph числа $a$.
}

\DefDefinition{polynomial*polynomial}
{
Билинейное отображение
\ShowEq{polynomial*polynomial}
определено равенством
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
Для любых тензоров
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
произведение однородных многочленов
\ShowEq{polynomials a o x,b o x}
определено равенством
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Пусть $H$ - алгебра кватернионов и $a$ - $H$\Hyph число.
\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{Re sqrt a ne 0}
то уравнение
\DrawEq{x2=a}{}
имеет корни
\ShowEq{x=x12}
такие, что
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Если $a=0$, то уравнение
\DrawEq{x2=a}{}
имеет корень $x=0$ кратности $2$.
\labelItem{a=0}
\item
Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней таких, что
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
Полилинейное отображение $D$\Hyph алгебры $A$
\ShowEq{f:A->B}f{A^n}A
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Обозначим
\ShowEq{set polylinear maps An}DAA
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$.
}

\DefRemark{monomial of power k}
{
В теореме
\RefTheorem{monomial of power k}
я рассмотрел рекурсивное представление одночлена в ассоциативной $D$\Hyph алгебре.
Так как скобки в произведении
я могу расставить произвольно,
то в ассоциативной $D$\Hyph алгебре
рекурсивное представление одночлена неоднозначно.
Например, одночлен $ax^2bxcx^3d$
может быть записан в любой из следующих форм
\ShowEq{ax^2bxcx^3d}
Я выбрал равенство
\EqRef{monomial of power k, F=1}
как самое простое для алгоритма деления многочленов.
}

\DefTheorem{monomial of power k}
{
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над ассоциативной $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
где $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
Мы докажем утверждение теоремы индукцией по степени
$n$ одночлена.

Пусть $n=0$.
Так как одночлен $p_0(x)$ является константой,
то мы получаем утверждение
\RefItem{monomial of power 0}.

Пусть $n=k$. Последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.
}

\DefTheorem{r=+q circ p}
{
Пусть
\ShowEq{p=p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
}

\DefText{linear map of A vector space V1->V2}
{
Из определения
\RefDefinition{linear map A module}
следует, что
линейное отображение
$A_1$\Hyph \VectorSetRuB $V_1$
в $A_2$\Hyph \VectorSetRuA $V_2$
- это линейное отображение
$D_1$\Hyph \VectorSetRuB $V_1$
в $D_2$\Hyph \VectorSetRuA $V_2$.
}

\DefLabeledDefinition{linear map of A vector space}{\SideNS}
{
\ShowText{algebra over ring ()}
Пусть $V$, $W$ - \SideRu вые векторные пространства над $D$\Hyph алгеброй $A$.
Линейное отображение
\ShowEq{f:A->B}fVW
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, VW module}
множество линейных отображений
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
}

\DefDefinition{component of linear map, basis E}
{
Выражение
\ShowEq{component of linear map, basis E}
в равенстве
\eqRef{linear map f, basis E}1
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Представление
\DrawEq[DA]{h:AoxA->L(A)}{}
$D$\Hyph алгебры
\AoxA A
в модуле
\ShowEq{L(A->B)}DAA,
определённое равенством
\DrawEq[DA]{representation AA in LA}{}
позволяет отождествить тензор
\ShowEq{d in AxoA}A
с линейным отображением
\ShowEq{product in algebra AA 2}DA{\delta},
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}{\delta}
имеет вид
\ShowEq{a ox b c=}
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Отображения сопряжения
имеют
стандартное представление
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
Согласно равенству
\EqRef{#2x= #1},
отображение сопряжения
\ShowEq{Map of Conjugation}{#2}
имеет матрицу
\ShowEq{#1. matrix I#2}
Равенство
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
является следствием равенств
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of ring and Z}
{
Пусть $D$ - кольцо с единицей \(1_D\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[fnZ{n1_D}D]{f:a in A->b in B}{}
является гомоморфизмом кольца $Z$ в кольцо $D$
и позволяет отождествить \(Z\)\Hyph число \(n\)
и \(D\)\Hyph число \(n\,1_D\).
\labelItem{homomorphism n->n1}
\item
Кольцо \(Z/\ker f\) является подкольцом кольца $D$.
\labelItem{Z is subring of D}
\end{enumerate}
}

\DefProof{unit of ring and Z}
{
Пусть
\ShowEq{d12 in D}nZ
Равенство
\DrawEq[nD]{d1+d2 in A}{nD}
является следствием равенства
\EqRef{(m+n)a=ma+na (+)}.
Равенство
\DrawEq[nD]{d1 d2 in A}{nD}
является следствием равенств
\EqRef{product Z bilinear 1 (+)},
\EqRef{product Z bilinear 2 (+)}.
Утверждение
\RefItem{homomorphism n->n1}
является следствием равенств
\eqRef{d1+d2 in A}{nD},
\eqRef{d1 d2 in A}{nD}.
Утверждение
\RefItem{Z is subring of D}
является следствием утверждения
\RefItem{homomorphism n->n1}.
}

\DefTheorem{ring product Z bilinear}
{
Произведение в кольце $D$ билинейно над
кольцом $Z$
\ShowEq{product Z bilinear 1 (+)}
\ShowEq{product Z bilinear 2 (+)}
}

\DefTheorem{unit of algebra and ring}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с единицей \(1_A\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[fdD{d1_A}A]{f:a in A->b in B}{}
является гомоморфизмом кольца $D$ в центр алгебры $A$
и позволяет отождествить \(D\)\Hyph число \(d\)
и \(A\)\Hyph число \(d\,1_A\).
\labelItem{isomorphism d->d1}
\item
Кольцо \(D\) является подалгеброй алгебры $A$.
\labelItem{D is subalgebra of A}
\item
\ShowEq{D in Z(A)}
\end{enumerate}
}

\DefProof{unit of algebra and ring}
{
Пусть
\ShowEq{d12 in D}dD
Согласно утверждению
\RefItem{distributive law, module},
\DrawEq[dA]{d1+d2 in A}{dA}
Согласно определению
\RefDefinition{algebra over ring},
\DrawEq[dA]{d1 d2 in A}{dA}
Утверждение
\RefItem{isomorphism d->d1}
является следствием равенств
\eqRef{d1+d2 in A}{dA},
\eqRef{d1 d2 in A}{dA}.
Утверждение
\RefItem{D is subalgebra of A}
является следствием утверждения
\RefItem{isomorphism d->d1}.

Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
Утверждение
\RefItem{D in Z(A)}
следует из равенства
\EqRef{ad=da in A}.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
Произведение в алгебре $A$ дистрибутивно по отношению к сложению
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefProof{multiplication in algebra is distributive over addition}
{
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
}

\DefText{multiplication in algebra}
{
Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.
}

\DefTheoremNote{associator of algebra}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.\,\footnotemark
\ShowEq{associator of algebra, 1}
для любых $a$, $b$, $c$, $d\in A$.
}
{
Утверждение
теоремы опирается на равенство
\citeBib{Richard D. Schafer}-(2.4).
}

\DefProof{associator of algebra}
{
Равенство \EqRef{associator of algebra, 1}
следует из цепочки равенств
\ShowEq{associator of algebra, 2}
}

\DefLabeledFootnote{LR ideal}{\VectorSetNS}
{
Смотри также определение на странице
\citeBib{Serge Lang}\Hyph 75.
}

\DefLabeledDefinition{LR ideal}{\SideWS \VectorSetNS}
{
\AddIndex{\SideRuC вый идеал}{\SideWS ideal}\,\refFootnote{LR ideal}{\VectorSetNS}
$\Set_1$ \AlgebraSetRuB $\Set$
- это подгруппа аддитивной группы $\Set$
такая, что
\ShowEq{D1 D in D1}
}

\DefLabeledDefinition{ideal}{\VectorSetNS}
{
\AddIndex{Идеал}{ideal}\,\refFootnote{LR ideal}{\VectorSetNS}
- это подгруппа аддитивной группы $\Set$,
которая одновременно является левым и правым идеалами.
}

\DefText{trivial ideal}
{
Если $\Set$ - \AlgebraSetRuNS,
то множество $\{0\}$ и само $\Set$
являются идеалами,
которые мы называем тривиальными идеалами.
}

\DefLabeledTheorem{LR ideal}{\SideWS \VectorSetNS}
{
Если $\Set_1$ является \SideRu вым идеалом
унитальн\EndB \AlgebraSetRuB $\Set$, то
\ShowEq{D1 D=D1}
}

\DefProof{LR ideal}
{
Теорема является следствием определения
\refDefinition{LR ideal}{\SideWS \VectorSetNS}
и равенства
\ShowEq{D1 1=D1}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{def DModule}
\ShowEq{=DD}
Линейное отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
\ShowEq{D ab in A, d in D}DA
Обозначим
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
множество линейных отображений
%алгебры кватернионов $H$.
$D$\Hyph алгебры $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Копроизведение в категории
\scSide $\Base$\Hyph \CatModule
называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
для прямой суммы \SideRu\TO $\Base$\Hyph \VectorsSetRuB $\Module$ и $\ModuleA$.
}{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\DefText{category of modules}
{
Пусть
\scSide $\Base$\Hyph \CatModule
- категория \SideRu\TO $\Base$\Hyph \VectorsSetRuB,
морфизмы которой - это гомоморфизмы $\Base$\Hyph модуля.
}

\DefLabeledTheoremNote{direct sum of D modules 2024}{\SideWS \Base-\VectorsSetNS}
{
В категории
\scSide $\Base$\Hyph \CatModule
существует прямая сумма
\SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.\,\footnotemark
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph \VectorsSetRuB
\ShowEq{o+Ai}{\Module}
}
{
Смотри также предложение
\citeBib{Serge Lang}\Hyph 1
на странице 98.
}

\DefProof{direct sum of D modules 2024}
{
Пусть
\ShowEq{set Ai}V
- множество \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Пусть
\ShowEq{A=o+Ai}V
прямая сумма абелевых групп.
Пусть
\ShowEq{a=ai in A}
Мы определим действие $\Base$\Hyph числа $a$
на $V$\Hyph число $v$ согласно равенству
\DrawEq{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
\ShowEq{def additive}%

Согласно теореме
\refTheorem{definition of A module, property}{\SideNS},
\ShowEq{direct sum of modules i}
для любых
\ShowEq{p,q in D, v,w in V, i}
Равенства
\ShowEq{direct sum of modules ...}
являются следствием равенств
\ShowEq{module, ..., i}
для любых
\ShowEq{p,q in D, v,w in V, direct sum}

Из равенства
\eqRef{distributive law, direct sum of modules, 1}{\SideWS \Base-\VectorsSetNS}
следует, что отображение
\ShowEq{f:A->B}av{\Multiply av}
определённое равенством
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS},
является эндоморфизмом абелевой группы $V$.
Из равенств
\eqRef{direct sum of modules, associative law}{\SideWS \Base-\VectorsSetNS},
\eqRef{distributive law, direct sum of modules, 2}{\SideWS \Base-\VectorsSetNS}
следует, что отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является гомоморфизмом \ShortAlgebraRuBWS $\Base$ в
множество эндоморфизмов абелевой группы $V$.
Следовательно, отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является представлением \ShortAlgebraRuBWS $\Base$ в абелевой группе $V$.

Пусть $a_1$, $a_2$ - такие $\Base$\Hyph числа, что
\DrawEq{a1(vi)=a2(vi)}{\SideWS \Base-\VectorsSetNS}
для произвольного $V$\Hyph числа
\ShowEq{A=Ai iI}v.
Равенство
\DrawEq{(a1vi)=(a2vi)}{\SideWS \Base-\VectorsSetNS}
является следствием равенства
\eqRef{a1(vi)=a2(vi)}{\SideWS \Base-\VectorsSetNS}.
Из равенства
\eqRef{(a1vi)=(a2vi)}{\SideWS \Base-\VectorsSetNS}
следует, что
\DrawEq{Ai a1vi=a2vi}{\SideWS \Base-\VectorsSetNS}
Поскольку для любого \iI, $V_i$ - $\Base$\Hyph \VectorSetRuANS,
то соответствующее представление эффективно
согласно определению
\ShowRef{module over algebra \Base-\VectorSetNS}
Следовательно, равенство $a_1=a_2$ является следствием утверждения
\eqRef{Ai a1vi=a2vi}{\SideWS \Base-\VectorsSetNS}
и отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является эффективным представлением \ShortAlgebraRuBWS $\Base$ в абелевой группе $V$.
Следовательно, абелевая группе $V$ является \SideRu\What $\Base$\Hyph \VectorSetRuENS.

Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRuTo $\Base$\Hyph \VectorSetRuA $W$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равны $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{+}.
}

\DefLabeledTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph модулей
\ShowEq{o+Ai}{\Module}
}

\DefProof{direct sum of D modules}
{
Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRuTo $\Base$\Hyph модуль $V$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{+}.
}

\DefProof{cr-power, 1}
{
Равенство
\ShowEq{cr-power, 1 1}
является следствием равенств
\eqRef{cr power, 0}1,
\eqRef{cr-power, n}1.
Равенство
\EqRef{cr-power, 1}
является следствием равенства
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
Равенство
\ShowEq{rc-power, 1 1}
является следствием равенств
\eqRef{rc power, 0}1,
\eqRef{rc-power, n}1.
Равенство
\EqRef{rc-power, 1}
является следствием равенства
\EqRef{rc-power, 1 1}.
}

\DefLabeledTheorem[3]{Kernel of Linear Map}{(#1)}
{
Пусть отображение
\newline
\FrameEqRef[fV]{homomorphism D algebra #11}{Vector module, coordinates \Cols}
\newline
является линейным отображением
$D_{#1}$\Hyph модуля $V_1$
в $D_{#2}$\Hyph модуль $V_2$.
Множество
\ShowEq{kernel of linear map}{#3}
\DrawEq[{#3}{}]{ker linear map}{D#3}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
$#3$.
Ядро линейного отображения $#3$
является подмодулем модуля $V_1$.
}

\DefProof[4]{Kernel of Linear Map}
{
Пусть
\ShowEq{vw in V1}
Тогда
\DrawEq{fvw=0 V2}{(#1)}
Равенство
\ShowEq{f v+w=0}
является следствием равенств
\eqRef{homomorphism, f v+w=}{f D module #11},
\eqRef{fvw=0 V2}{(#1)}.
Следовательно, множество
$\ker#3$
является подгруппой аддитивной группы $V_1$.
Равенство
\ShowEq{fpv=0 V2h}{#4}
является следствием равенств
\eqRef{left homomorphism, f av=}{f D module 11},
\eqRef{fvw=0 V2}{(#1)}.
Следовательно, определено представление кольца $D_{#1}$
на множестве
$\ker#3$.
Согласно определению
\refDefinition{submodule}{\SideWS module},
множество
$\ker#3$
является подмодулем $D_{#1}$\Hyph модуля $V_1$.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Если
\ShowEq{c in ZAa}ab,
то
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Пусть
\ShowEq{c in ZAa}ab.
Равенство
\DrawEq{ab=ba}Z
является следствием утверждения
\eqRef{c in S=>bc=cb}{Z(A,b)}.
Теорема является следстием равенства
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Если
\ShowEq{c in ZAa}ab{}
и
\ShowEq{c in ZA}c
то
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
Равенство
\ShowEq{a(bc)=...=(bc)a}
является следствием определений
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Теоремя является следствием равенства
\EqRef{a(bc)=...=(bc)a}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefLemma{pk ck in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}{p,\ c}a,
то
\DrawEq[n]{pcn in Za}n
}

\DefProof{pk ck in Za}
{
Согласно теореме
\RefTheorem{c in S=>bc=cb submodule of A},
\ShowEq{p0 in Za}
Пусть утверждение
\eqRef{pcn in Za}n
верно для $n=k-1$, $k>0$,
\DrawEq[{k-1}{}]{pcn in Za}{k-1}
Тогда утверждение
\ShowEq{pck in Za}
является следсвием утверждения
\eqRef{pcn in Za}{k-1}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Согласно принципу математической индукции,
утверждение
\eqRef{pcn in Za}n
верно для любого $n\ge 0$.
}

\DefTheorem{c in Za=> p(c) in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}ca,
то
\DrawEq[{p(c)}a{}{}]{c in ZAa}1
для любого многочлена
\DrawEq{p(c) p in D}1
}

\DefProof{c in Za=> p(c) in Za}
{
Теорема является следствием леммы
\RefLemma{pk ck in Za}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $b\in A$ существует подалгебра
\ShowEq{center of A number}
$D$\Hyph алгебры $A$ такая, что
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph алгебра
\ShowEq{center Ac}{}
называется
\AddIndex{центром $A$\Hyph числа}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
Подмножество
\ShowEq{center Ac}{}
не пусто так как
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Пусть
\ShowEq{d in D c in S 12}
Тогда
\ShowEq{dcb=bdc}
Откуда следует
\ShowEq{dc in S}
Следовательно, множество
\ShowEq{center Ac}{}
является $D$\Hyph модулем.

Пусть
\ShowEq{c in ZAb}
Тогда
\ShowEq{c1c2 in ZAb}
Из равенства
\EqRef{c1c2 in ZAb}
следует, что
\ShowEq{c1 c2 in ZAb}
Следовательно, $D$\Hyph модуль
\ShowEq{center Ac}{}
является $D$\Hyph алгеброй.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Для любого множества $B$
множество отображений $A^B$ является абелевой группой относительно операции
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
Теорема является следствием определений
\ShowRef{set of maps B->A is Abelian group}
}

\DefTheorem{set of endomorphisms - D module}
{
Множество
\ShowEq{End DV}{}
эндоморфизмов $D$\Hyph модуля $V$
является $D$\Hyph модулем.
}

\DefProof{set of endomorphisms - D module}
{
Теорема является следсвием определения
\RefDefinition{D module, endomorphism}
и следсвия
\RefCorollary{product of linear map over scalar, D module}.
}

\DefDefinition{D module, endomorphism}
{
Линейное отображение
\DrawEq[fVV]{f: A->B}{}
$D$\Hyph модуля $V$
называется
\AddIndex{эндоморфизмом}{endomorphism}
$D$\Hyph модуля $V$.
Обозначим
\ShowEq{set of endomorphisms D module}
множество эндоморфизмов
$D$\Hyph модуля $V$.
}

\DefLabeledDefinition{module over algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRu \DivisionRuNS.
Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefTheorem{quasibasis of so(3) module}
{
Пусть
\ShowEq{V=so3+so3}
- левый $so(3)$\Hyph модуль столбцов.
Множество векторов
\ShowEq{quasibasis of so(3) module}
является квазибазисом левого $so(3)$\Hyph модуля $V$.
}

\DefProof{quasibasis of so(3) module}
{
Согласно теоремам
\ShowRef{so3 quasibasis e}
$V$\Hyph число
\ShowEq{so3 V number}
имеет разложение
\ShowEq{so3 V number expansion}
относительно множества векторов \eV[V][.]
Следовательно, множества векторов \eV[V]
является квазибазисом левого $so(3)$\Hyph модуля $V$.
Из равенства
\ShowEq{so3 V basis dependence}
следует, что квазибазис \eV[V] не является базисом.
}

\DefLabeledTheorem[1]{so3 quasibasis e}{#1}
{
Матрица
\DrawEq[#1]{so3 quasibasis e=}{#1}
является левым квазибазисом
алгебры $so(3)$.
Координаты матрицы
\newline
\FrameEqRef{so3 matrix c}{#1}
\newline
относительно матрицы
\eqRef{so3 quasibasis e=}{#1}
имееют следующий вид
\DrawEq{so3 matrix c coordinates e#1}1
}

\DefProof[1]{so3 quasibasis e}
{
Мы можем представить матрицу
\DrawEq{so3 matrix c}{#1}
в виде
\DrawEq[{#1}]{Jacobson Coordinates of matrix 1}{#1}
Равенство
\DrawEq[{#1}]{Jacobson Coordinates of matrix}{#1}
является следствием равенств
\eqRef{so3 quasibasis e=}{#1},
\eqRef{Jacobson Coordinates of matrix 1}{#1}
Равенство
\ShowEq{Jacobson Coordinates of matrix (#1)}
является следствием равенств
\EqRef{so3 matrix product 2},
\eqRef{Jacobson Coordinates of matrix}{#1}.
Из равенства
\EqRef{Jacobson Coordinates of matrix (#1)}
следует, что координаты матрицы
\newline
\FrameEqRef{so3 matrix c}{#1}
\newline
относительно матрицы
\newline
\FrameEqRef[{#1}]{so3 quasibasis e=}{#1}
\newline
имееют следующий вид
\newline
\FrameEqRef{so3 matrix c coordinates e#1}1
\newline
Из равенства
\eqRef{so3 matrix c coordinates e#1}1
следует, что
матрица $\aD e{#1}$ является не базисом, а левым квазибазисом,
так как значение $q$ произвольно.
}

\DefDefinition{algebra so(3)}
{
Алгебра Ли $so(3)$ - это множество матриц
действительных чисел
\DrawEq[c]{so3 matrix}1
и произведение на множестве $so(3)$ определено равенством
\ShowEq{so3 matrix product 2a}
}

\DefTheorem{algebra so(3)}
{
Произведение в алгебре Ли $so(3)$ определено равенством
\ShowEq{so3 matrix product 2}
}

\DefProof{algebra so(3)}
{
Равенство
\ShowEq{so3 matrix product}
является следствием равенств
\eqRef{so3 matrix}1,
\EqRef{so3 matrix product 2a}.
Равенство
\ShowEq{so3 matrix product 1}
является следствием равенства
\EqRef{so3 matrix product}
Равенство
\EqRef{so3 matrix product 2}
является следствием равенства
\EqRef{so3 matrix product 1}.
}

\DefLabeledDefinition{module over associative algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRu \DivisionRuNS.
Пусть $V$ - $\CBase$\Hyph \VectorSetRuANS.
Пусть в $\CBase$\Hyph \VectorSetRuD
\ShowEq{End DV}{}
определено произведение эндоморфизмов как композиция отображений.
Пусть определён гомоморфизм
\DrawEq[{g_{34}}A{\End(D,V)}{}]{f: A->B}{\SideWS g34}
$\CBase$\Hyph алгебры $A$
в $\CBase$\Hyph алгебру
\ShowEq{End DV}.

Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefText{module over associative algebra}
{
Если $D$\Hyph алгебра $A$ ассоциативна, то мы можем уточнить определение
\refDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - некоммутативная $D$\Hyph алгебра.
Пусть $V$ - $\CBase$\Hyph \VectorSetRuANS.
Пусть в $\CBase$\Hyph \VectorSetRuD
\ShowEq{End DV}{}
определено произведение эндоморфизмов
таким образом, что
существует гомоморфизм
\DrawEq[{g_{34}}A{\End(D,V)}{}]{f: A->B}{}
$\CBase$\Hyph алгебры $A$
в $\CBase$\Hyph алгебру
\ShowEq{End DV}.

Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS nonA \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{nonA \VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{nonA \VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefLabeledTheorem{module over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRuTo $\Base$\Hyph модуль $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
В диаграмме представлений
\eqRef{diagram of representations, \SideWS module}1
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\DrawEq{\SideWS module, a d v}1
}

\DefProof{module over algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\ShowRef{\SideWS module over algebra}
и теоремы
\def\Temp{}
\ifx\SideNS\Temp
\refTheorem{action of ring of rational integers in Abelian group}{+}.
\else
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\eqRef{\SideWS module, a d v}1
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{module over non-associative algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\refDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}
и теоремы
\RefTheorem{Free Algebra over Ring}.
Равенство
\eqRef{\SideWS module, a d v}1
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
\end{ShadedLemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\refDefinition{linear map of D module}1,
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\end{ShadedLemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лемм
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\DefLabeledTheorem{A module -> algebra is associative}{\SideNS}
{
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheorem[1]{action of unital ring}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Для любого $\Base_{\BaseExt}$\Hyph числа
определён эндоморфизм
абелевой группы $V$
\DrawEq[{#1}vV{}]{module, a+d:V->V}{\SideNS,\VectorSetNS}
\DrawEq[{#1}{\Base}]{module, (a+n)v=av+nv}{\SideNS}
Множество преобразований
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}
порождает \SideRu\HSide представление \ShortAlgebraRuBWS $\Base_{(1)}$ в абелевой группе $V$.
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
}

\DefProof{action of unital ring}
{
Согласно теореме
\refTheorem{module over algebra}{\SideNS},
выражения $av$, $\DArg v$ являются $V$\Hyph числами.
Поскольку $V$ является абелевой группой, выражение
\eqRef{module, (a+n)v=av+nv}{\SideNS}
также является $V$\Hyph числом.
}

\DefLabeledTheoremNote{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Для любого множества $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{\SideWS \VectorSetNS}
вектор, порождённый диаграммой представлений
\eqRef{diagram of representations, \SideWS module}1,
имеет следующий вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}{}]{w=sum vi, module=Jv}{\SideWS \Base}
\def\Temp{module}
\ifx\Temp\VectorSetNS
где \algebraa $\Base_{(1)}$
является унитальным расширением
\ShortAlgebraRuBWS $\Base$.
\fi
}
{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}

\DefLabeledTheorem[3]{homomorphism non-associative module}{\SideNS-\Cols(#1#2#3)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRu вый модуль столбцов
над неассоциативной $D$\Hyph алгеброй $A$.
Пусть \eV[i] - квазибазис $A$\Hyph модуль $V_i$.
Гомоморфизм
\DrawEq[f{V_1}{V_2}{}]{f: A->B}{}
$A$\Hyph модуля $V_1$ в $A$\Hyph модуль $V_2$
имеет представление
\DrawEq{v=w(fe2) \SideNS-\Cols}{(#1#2#3)}
где $f$ - матрица $A$\Hyph чисел.
Если квазибазис \eV[2] является базисом,
то матрица $f$ определена однозначно.
}

\DefText[1]{quasibasis module}
{
Пусть $D$\Hyph алгебра $A$
имеет \SideRu вый квазибазис
\DrawEq{eA= iI}{#1}
Пусть \SideRu вый $A$\Hyph модуль $V$
является прямой суммой
\DrawEq{V=+V jJ}{#1}
Тогда квазибазис \eV левого $A$\Hyph модуля $V$ имеет вид
\DrawEq{quasibasis of left module}{#1}
}

\DefLabeledTheorem{quasibasis module}{\SideNS}
{
\ShowText{quasibasis module}1
}

\DefLabeledTheorem{when quasibasis of module is basis}{\SideNS}
{
Если \SideRu вый квазибазис \eV[A]
$D$\Hyph алгебры $A$
является \SideRu вым базисом,
то соответствующий квазибазис \SideRu вого $A$\Hyph модуля $V$
является базисом.
}

\DefLabeledExample{A module over Lie algebra L}{\SideNS}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Пусть $V$ является \SideRu вым $A$\Hyph \VectorSetRuENS.
Пусть
\ShowEq{End DV}{}
- $D$\Hyph алгебра эндоморфизмов \SideRu вого $A$\Hyph \VectorSetRuB $V$,
где произведение эндоморфизмов определено как композиция отображений.
Рассмотрим \SideRu \SidePresentationRuWS представление
\ShowEq{f:A->*B}f{\End(D,V)}V
$D$\Hyph алгебры
\ShowEq{End DV}{}
в $A$\Hyph \VectorSetRuD $V$,
определённое равенством
\ShowEq{av=a o v}
Рассмотрим эффективное \SideRu \SidePresentationRuWS представление
\ShowEq{f:A->*B}gLV
алгебры Ли $L$
в $A$\Hyph \VectorSetRuD $V$,
определённое равенством
\ShowEq{ab=[ab]}
Вообще говоря
\DrawEq{a(bv) ne (ab)v}{Lie}
}

\DefLabeledExample{non-associative A module}{\SideNS}
{
Пусть $A$ - неассоциативная $D$\Hyph алгебра.
Рассмотрим $D$\Hyph модуль
\ShowEq{V=+A iI}
Множество отображений
\ShowEq{a in A, av=}
порождает \SideRu \SidePresentationRuWS представление
$D$\Hyph алгебры $A$ в $D$\Hyph модуле $V$
и, следовательно, порождает структуру
\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuB $V$.
Вообще говоря
\DrawEq{a(bv) ne (ab)v}{nonA}
}

\DefLabeledTheorem{associative law of A module}{\SideNS}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда
\AddIndex{закон ассоциативности}{associative law}
в \SideRu вом $A$\Hyph \VectorSetRuD $V$
принимает вид
\DrawEq{associative law, \SideWS module}1
\ShowEq{p,q in D, v in V}
}

\DefText{unitarity law, module}
{
\DrawEq{unitarity law, module}{\SideWS \Base}
Если \algebrac имеет единицу, то равенство
\eqRef{unitarity law, module}{\SideWS \Base}
имеет вид
\DrawEq{unitarity law, vector space}{\SideWS \Base-\VectorSetNS}
}

\DefText{unitarity law, vector space}
{
\DrawEq{unitarity law, vector space}{\SideWS \Base}
}

\DefLabeledTheorem{definition of A module, property}{\SideNS}
{
Пусть $V$ является \SideRu\What $\Base$\Hyph \VectorSetRuENS.
$V$\Hyph числа удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS vector space}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowText{unitarity law, \VectorSetNS}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
}

\DefLabeledTheorem{definition of A module, property, 2023}{\SideNS}
{
Пусть $V$ является \SideRu вым $A$\Hyph \VectorSetRuENS.
$V$\Hyph числа удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS nonA vector space}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, nonA \SideWS module}
\DrawEq{associative law*, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, nonA \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, nonA \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{m,n in D}
\ShowEq{p,q in D, v,w in V}
}

\DefProof{definition of A module, property}
{
Пусть $v\in V$.

Пусть $\Base_{(1)}$ - множество отображений
\eqRef{module, a+d:V->V}{\SideNS}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
и утверждение
\RefItem{\SideWS representation of D1 in Abelian group}
являются следствием леммы
\refLemma{action of D algebra}{\SideNS}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{\SideWS representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\DrawEq[nmv]{distributive law,, \SideWS module, 2}{\CBase}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\DrawEq[abv]{distributive law,, \SideWS module, 2}{\Base}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \ShortAlgebraRuBWS $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\ShowRef{module, (a+n)+(b+m)=}
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{db(\SideNS)}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{db(\SideNS)}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Опираясь на определение
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{db(\SideNS)}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{db(\SideNS)}.
}

\DefLabeledDefinition{submodule}{\SideWS module}
{
Подпредставление \SideRu\From $\Base$\Hyph \VectorSetRuB $V$ называется
\AddIndex{\VectorSubSetRuD}{\VectorSubSetNS}
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{submodule}{\SideWS module}
{
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если векторы
\ShowEq{set vi cols}v
принадлежат \VectorSubSetRuE $V'$ \SideRu\From $\Base$\Hyph \VectorSetRuB $V$,
то линейная комбинация векторов
\ShowEq{set vi cols}v
принадлежит \VectorSubSetRuE $V'$.
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{submodule}{\SideWS module}.
}

\AddEq{ref in item cvk module}
{
теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A \VectorSetNS}{\SideNS}
}

\AddEq{ref in item cvk vector space}
{
теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
определения
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{set of automorphisms}{\SideNS}
{
Множество $GL(V)$
автоморфизмов
\SideRu вого $A$\Hyph векторного пространства $V$
является группой.
}

\DefLabeledTheorem{active transformations in module}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
Матрицы автоморфизмов \SideRu вого $A$\Hyph векторного пространства \ColsA порождают группу
%\Group nA.
$GL(V_*)$,
изоморфную группе $GL(V)$.
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное представление
\DrawEq[{GL(V_*)}{V_*}{}]{A->*B}{\SideNS-\Cols}
группы $GL(V_*)$
в \SideRu вом $A$\Hyph векторном пространстве $V_*$.
}

\DefLabeledTheoremNote{set of vectors generate set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Существует
множество $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{}
такое, что любое $V$\Hyph число
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}{}]{w=sum vi, module=Jv}{\SideWS \Base}
\ShowEq{linear combination()}%
Множество $v$ называется
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$.
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i)}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\DefText{Let be algebra D}
{
Пусть $D$ - кольцо.
}

\DefText{Let be algebra A}
{
Пусть $A$ - $D$\Hyph алгебра.
}

\DefLabeledLemma[4]{action n of D algebra}{#1#2-\SideNS-\VectorSetNS}
{
Пусть 
\ShowEq{module, d in D}{#1}{#2}.
Отображение
\DrawEq[{#1}{#3}{#4}{\Multiply{#1}{#3}}{#4}{}]{f:a in A->b in B}{#1#2-\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefProof[4]{action n of D algebra}
{
Утверждение
\ShowEq{module, dv in V}{#1}{#3}{#4}%{}
является следствием
\ShowText{#1#3 \VectorSetNS}
Согласно
\ShowText{#1#3 \VectorSetNS,1}
отображение
\eqRef{f:a in A->b in B}{#1#2-\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefLabeledLemma[4]{action of D algebra}{\SideNS-\VectorSetNS}
{
Пусть 
\ShowEq{module, d in D}{#1}{#2},
\ShowEq{module, d in D}a{#4}.
Отображение
\DrawEq[{#1}{#3}{#4}{}]{module, a+d:V->V}{\SideNS-\VectorSetNS}
определённое равенством
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefText{nd module}
{
определения
\ShowRef{nd module}
}

\DefText{nd module,1}
{
теореме
\refTheorem{action of ring of rational integers in Abelian group}{+}
и определению
\RefDefinition{representation of algebra},
}

\DefText{ad module}
{
определения
\ShowRef{ad module}
}

\DefText{ad module,1}
{
утверждению
\RefItem{Product is distributive over sum},
и теоремам
\RefTheorem{0a=0},
\refTheorem{monoid-homomorphism}{+},
}

\DefText{db algebra}
{
определений
\ShowRef{nd algebra}
}

\DefText{db algebra,1}
{
равенству
\eqRef{distributive law, module, 1}1
}

\DefText{ab algebra}
{
определения
\RefDefinition{algebra over ring}.
}

\DefText{ab algebra,1}
{
теореме
\RefTheorem{multiplication in algebra is distributive over addition}
}

\DefProof[4]{action of D algebra}
{
Так как $#4$ является абелевой группой, то утверждение
\ShowEq{module, dv+av in V}{#3}{#4}
является следствием лемм
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}.
Согласно леммам
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}
и теореме
\refTheorem{monoid-homomorphism, sum}{+},
отображение
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $V$.
}

\DefExample{q equation ix-xi=k}
{
Рассмотрим уравнение
\DrawEq{ix-xi=k}1
Умножая уравнение
\eqRef{ix-xi=k}1
на
\ShowEq{ijk}
мы получим уравнения
\ShowEq{ix-xi-k=0 i}
\ShowEq{ix-xi-k=0 j}
\ShowEq{ix-xi-k=0 k}
Положим
\ShowEq{xijk}
Тогда мы получим систему линейных уравнений
\ShowEq{ix-xi-k=0 1ijk}
Решение системы линейных уравнений
\EqRef{ix-xi-k=0 1ijk}
имеет вид
\ShowEq{q equation 3 1ijk j-k x=}
Однако значение $x$ в равенстве
\EqRef{q equation 3 1ijk j-k x=}
не является корнем уравнения
\eqRef{ix-xi=k}1.
Здесь важно обратить внимание, что решение
\DrawEq{x=c12+j}1
уравнения
\eqRef{ix-xi=k}1
зависит от двух действительных произвольных постоянных,
а решение
\EqRef{q equation 3 1ijk j-k x=}
системы линейных уравнений
\EqRef{ix-xi-k=0 1ijk}
зависит от одной кватернион\Hyph значной произвольной постоянной.
}

\DefRef{associative module}
{
равенств
\EqRef{(nm)a=n(ma) (+)},
}

\DefRef{associative algebra}
{
определений
\RefDefinition{algebra over ring},
\RefDefinition{associator of algebra},
равенства
}

\DefRef{associative 1 module}
{
утверждений
\RefItem{() is associative},
\RefItem{A is multiplicative monoid},
теоремы
\refTheorem{homomorphism f(na)=nf(a)}{+},
}

\DefRef{associative 1 algebra}
{
}

\DefText{associative module}
{
}

\DefText{associative algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
}

\DefLabeledTheoremNote[4]{unital extension of D algebra}{\SideNS-\VectorSetNS}
{
\ShowText{associative \VectorSetNS}
Множество отображений
\ShowEq{a o+ b}{#1}
порождает\,\footnotemark
\algebrad $#4_{(1)}$
где сложение определено равенством
\DrawEq[{#1}{}]{(a+n)+(b+m)=}{#1#3(\VectorSetNS)}
и произведение определено равенством
\DrawEq[{#1}{}]{(a+n)(b+m)=}{#1#3(\VectorSetNS)}
\StartLabelItem
\begin{enumerate}
\item
Если \algebrac $#4$ имеет единицу, то
\ShowEq{A1=A unital extension}{#4}
\item
Если \algebrac $#4$ является идеалом $\CBase$, то
\ShowEq{A1=D unital extension}{#4}
\item
В противном случае
\ShowEq{A1=A+D unital extension}{#4}
\item
\algebraa $#4$ является \SideRu\What идеалом \algebrae $#4_{(1)}$.
\labelItem{Algebra is ideal of algebra (1) \SideNS-\VectorSetNS}
\end{enumerate}
\Algebraa $#4_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\algebrae $#4$.
}
{
Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.
}

\DefProof[4]{unital extension of ring}
{
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}

Утверждение
\RefItem{Algebra is ideal of algebra (1) \SideNS-\VectorSetNS}
является следствием леммы
\refLemma{action of D algebra}{\SideNS-\VectorSetNS}.
}

\DefProof[4]{unital extension of D algebra}
{
Выражение для операций на множестве $#4_{(1)}$
не зависит от того, действует ли эндоморфизм
\ShowEq{a o+ b}{#1}
на $#4$\Hyph числа слева или справа.
Однако текст доказательства слегка отличается.
Поэтому мы рассмотрим оба варианта доказательства.

\TwoColText
{
\ShowEq{def left}
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}
}
{
\ShowEq{def right}
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}
}

\ShowEq{def ab=ba}
Утверждение
\RefItem{Algebra is ideal of algebra (1) \SideNS-\VectorSetNS}
является следствием определения
\refDefinition{ideal}{\VectorSetNS}
и лемм
\refLemma{action of D algebra}{left-\VectorSetNS},
\refLemma{action of D algebra}{right-\VectorSetNS}.
}

\DefText[4]{step of proof unital extension}
{
Согласно теореме
\refTheorem{monoid-homomorphism, sum}{+},
равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv +i}{\SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Равенство
\eqRef{(a+n)+(b+m)=}{#1#3(\VectorSetNS)}
является следствием равенства
\eqRef{module, (a+d)v=av+dv +i}{\SideNS-\VectorSetNS}.

Согласно теореме
\RefTheorem{product of homomorphisms},
равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i}{#1#3 \SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i1}{#1#3 \SideNS-\VectorSetNS}
является следствием
\ShowRef{associative \VectorSetNS}
\eqRef{module, (a+d)v=av+dv *i}{#1#3 \SideNS-\VectorSetNS},
\ShowRef{associative 1 \VectorSetNS}
леммы
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i2}{}%{#1#3 \SideNS-\VectorSetNS}
а следовательно и равенство
\eqRef{(a+n)(b+m)=}{#1#3(\VectorSetNS)},
является следствием равенств
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS},
\eqRef{module, (a+d)v=av+dv *i1}{#1#3 \SideNS-\VectorSetNS}
и лемм
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.

Пусть \algebraa $#4$ имеет единицу $e$.
Тогда мы можем отождествить $#1\in #2$ и
$\Multiply{#1}e\in #4$.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv Z in D}{\SideNS-\VectorSetNS}
является следствием равенства
\newline
\FrameEqRef[{#1}{#3}{}]{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}
\newline
Утверждение
\RefItem{A1=A unital extension -\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv Z in D}{\SideNS-\VectorSetNS}.

Пусть \algebraa $#4$ является идеалом $\CBase$.
Тогда
$#4\subseteq\CBase$.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv D in Z}{\SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Утверждение
\RefItem{A1=D unital extension -\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv D in Z}{\SideNS-\VectorSetNS}.
}

\DefText{quasibasis of algebra}
{
Если для любого $a\in A$,
\ShowEq{Aa ne A}
то в $D$\Hyph алгебре $A$ существует \SideRu вый квазибазис,
имеющий более чем одно $A$\Hyph число.
}

\DefLabeledDefinition{quasibasis of algebra}{\SideNS}
{
Пусть $A$ - $D$\Hyph алгебра \ColsNA.
Если множество $A$\Hyph чисел
\DrawEq[aA]{v(i) V}{a \SideNS}
является минимальным множеством таким, что
любое $A$\Hyph число имеет представление
\DrawEq[A{(1)}ab]{w=sum vi, module}{\SideWS D(algebra)}
то множество $a$
называется \SideRu вым квазибазисом $D$\Hyph алгебры $A$.
}

\DefLabeledDefinition{quasibasis of algebra is basis}{\SideNS}
{
Пусть \eV - \SideRu вый квазибазис
$D$\Hyph алгебры $A$ \ColsNA.
Если
\ShowEq{w(i)=0}c
следует из уравнения
\DrawEq[ce]{wi vi=0}{algebra \SideNS}
то \SideRu вый квазибазис \eV называется \SideRu вым базисом
$D$\Hyph алгебры $A$.
}

\DefLemmaProof{w=w12 in Xk-1}
{\leftskip=25pt
Согласно равенству
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12=* \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSet nonA}
конечны.
Так как $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2=* \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSet nonA}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
}

\DefLabeledSummary{Vector Space Type 10-28-2023}{\SideNS-\Cols}
{
Мы представили множество векторов
\ShowEq{\RowN() 1n}vm{}
в виде
\RowA матрицы
\newline
\FrameEqRef[vm]{a=(a1.n \RowN)}{vm \SideNS-\Cols}
\newline
и множество $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{\ColNS() 1n}cm{}
в виде
\ColA матрицы
\newline
\FrameEqRef[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
\newline
Соответствующее представление \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$ мы будем называть
\AddIndex{\SideRu\What $\Base$\Hyph \VectorSetRuE \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
Мы можем записать линейную комбинацию
векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\newline
\FrameEqRef[cvm]{w.e, \SideNS-\Cols}{cv}
\newline
В частности,
если мы запишем векторы базиса $\Basis e$
в виде \RowA матрицы
\newline
\FrameEqRef[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
\newline
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\newline
\FrameEqRef[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
\newline
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\newline
\FrameEqRef[w]{vector w=w*e \SideNS-\Cols}w
}

\DefLabeledSummary{basis of module 10-28-2023}{\SideNS}
{
$X$ является
множеством образующих
\SideRu\From $\Base$\Hyph модуля $V$,
если любое $V$\Hyph число
является линейной комбинацией $V$\Hyph чисел из $X$.
Если существует минимальное множество \eV[][,] порождающее
\SideRuTo $\Base$\Hyph \VectorSetRuA $V$, то такое множество \eV называется
квазибазисом \SideRu\From $D$\Hyph \VectorSetRuB $V$.
Пусть уравнение
\newline
\FrameEqRef[ce]{wi vi=0}{\SideNS}
\newline
имеет единственное решение
\ShowEq{w(i)=0}c
Тогда квазибазис \eV является
базисом \SideRu\From $\Base$\Hyph модуля $V$.

\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRuTo $\Base$\Hyph модуль}{free module},
если \SideRuTo $\Base$\Hyph модуль $V$ имеет базис.
Координаты вектора $v\in V$ относительно базиса $\Basis e$
\SideRu\Which $\Base$\Hyph \VectorSetRuB $V$
определены однозначно.
Из равенства
\newline
\FrameEqRef{e*v=e*w,\SideNS}{\Cols}
\newline
следует, что
\ShowEq{=> v=w}
}

\DefLabeledTheoremNote{set of vectors generated* by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Множество $V$\Hyph чисел, порождённое множеством $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{\SideWS \VectorSetNS}
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}]{w=sum vi, module=Jv*}{\SideWS \Base}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\DefRef{structure of subrepresentations, module}
{
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{action of unital ring}{\SideWS \VectorSetNS},
}

\DefRef{structure of subrepresentations, vector space}
{
и теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
}

\DefLabeledLemma[1]{w=w12 in Xk-1}{\SideWS \VectorSet #1}
{\leftskip=25pt
Пусть
\ShowEq{w=w12 in Xk-1}.
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=aw in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=a*w in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=a*w in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefLemmaProof{w=a*w in Xk-1}
{\leftskip=25pt
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw1 in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}{w_1}
такие, что
\ShowEq{w()=* \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()=* \SideWS module}
следует, что
\ShowEq{aw()=* \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
}

\DefText{set of vectors, step 1, module}
{
Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=0 o+ dik}
Тогда равенство
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i)}{\SideWS \Base}
является следствием равенства
\eqRef{module, (a+n)v=av+nv}{\SideNS}.
Из равенств
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
\eqRef{v(k)=sum v(i)}{\SideWS \Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}
}

\DefText{set of vectors, step 1, vector space}
{
Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i)}{\SideWS \Base}
Из равенств
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
\eqRef{v(k)=sum v(i)}{\SideWS \Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

\ShowText{set of vectors, step 1, \VectorSetNS}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\ShowRef{\SideWS module over algebra}
\ShowRef{structure of subrepresentations, \VectorSetNS}
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=aw in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}A

{\sc Доказательство.}
Согласно равенству
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12= \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
конечны.
Так как $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2= \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
\hfill\(\odot\)

\ShowLemma{w=aw in Xk-1}

{\sc Доказательство.}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw1 in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}w
такие, что
\ShowEq{w()= \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()= \SideWS module}
следует, что
\ShowEq{aw()= \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
\hfill\(\odot\)

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSet A},
\refLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefProof{set of vectors generated* by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i), \SideWS module*}{\Base}
Из равенств
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
\eqRef{v(k)=sum v(i), \SideWS module*}{\Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\refDefinition{module over non-commutative algebra}{left \VectorSetNS}
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=a*w in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}{nonA}
\ShowProof{w=w12 in Xk-1}

\ShowLemma{w=a*w in Xk-1}
\ShowProof{w=a*w in Xk-1}

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSet A},
\refLemma{w=a*w in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefLabeledTheorem{da in DA->da in D1A}{\SideWS module}
{
Отображение
\ShowEq{da in DA->da in D1A}
является гомоморфизмом \SideRu\From $\Base$\Hyph модуля $V$
в \SideRuTo $\Base_{(1)}$\Hyph модуль $V$.
}

\DefProof{da in DA->da in D1A}
{
Равенство
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)+(b+m)=}{nd(\VectorSetNS)}.
Равенство
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)(b+m)=}{nd(\VectorSetNS)}.
Из равенств
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}
следует, что отображение $I_{(1)}$
является гомоморфизмом \ShortAlgebraRuBWS $\Base$
в \ShortAlgebraRuEWS $\Base_{(1)}$.

Равенство
\ShowEq{da in DA->da in D1A 1, \SideWS module}
является следствием равенства
\ShowRef{da in DA->da in D1A}
Теорема является следствием равенства
\EqRef{da in DA->da in D1A 1, \SideWS module}
и определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefLabeledConvention{da in DA->da in D1A}{\SideNS}
{
Согласно теоремам
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\refTheorem{da in DA->da in D1A}{\SideWS module},
множество слов, порождающих
\SideRuTo $\Base$\Hyph модуль $V$,
совпадает с множество слов, порождающих
\SideRuTo $\Base_{(1)}$\Hyph модуль $V$.
Поэтому, не нарушая общности,
мы будем предполагать, что \algebrac $\Base$
имеет единицу.
}

\DefLabeledConvention{linear combination of vectors}{\SideNS}
{
Если необходимо явно указать,
что мы умножаем вектор $v(\gii)$
на $\Base_{\BaseExt}$\Hyph число $c(i)$ с\SideRu ва,
то мы будем называть выражение
\ShowEq{the linear combination()}
\AddIndex{\SideRu вой линейной комбинацией}{\SideWS linear combination}.
Мы будем применять это соглашение к аналогичным терминам.
Например, мы будем говорить, что вектор
\ShowEq{w=c(i)v(i)}
линейно зависит
от векторов
\ShowEq{set vi *}v
с\SideRu ва.
}

\DefLabeledDefinition{linear combination of vectors}{\SideNS}
{
Пусть $\Module$ - \SideRu\HSide \VectorSetRuA.
Пусть
\DrawEq[vV]{v(i) V}{}
- множество векторов.
\ShowEq{linear combination()}%
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i)}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}

\DefLabeledDefinition{generating set of module}{\SideNS}
{
$J(v)$ называется
\AddIndex{подмодулем}{submodule},
порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefLabeledDefinition{generating set of vector space}{\SideNS}
{
$J(v)$
называется
векторным подпространством, порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
векторного подпространства $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu вого $\Base$\Hyph векторного пространства $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefText{generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefText{quasibasis of module}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefDefinition{RCo product of matrices of maps}
{
Пусть
\ShowEq{Let aij rco bij}.
Мы определим \RCo произведение матриц отображений
\ShowEq{aij rco bij}
пользуясь равенством
\DrawEq{a rco b ij}o
}

\DefText{product of maps can be extended}
{
Рассмотренное выше
произведение отображений
\ShowEq{a o b=...}
может быть распространено на произведение матриц отображений
\ShowEq{matrix of maps}a,
\ShowEq{matrix of maps}b.
}

\DefLabeledDefinition{basis of module}{\SideNS}
{
Если множество $X\subset V$ является множеством образующих
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если существует минимальное множество $X$, порождающее
\SideRuTo $\Base$\Hyph \VectorSetRuA $V$, то такое множество $X$ называется
\AddIndex{квазибазисом}{quasibasis} \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{linearly depends on rest of vectors}{\SideWS module}
{
Пусть $\Base$ - \DivAlgebraRu.
Если уравнение
\DrawEq[wv]{wi vi=0}{1 \SideWS \Cols}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0}w,
то вектор
\ARow vj{}
линейно зависит от остальных векторов $v$.
}

\DefProof{linearly depends on rest of vectors}
{
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}vw
и определения
\refDefinition{linear combination of vectors}{\SideNS}.
}

\DefText{0=0vi}
{
Очевидно, что для любого множества векторов
\ARow vi{}
\ShowEq{\SideWS 0=0vi}
}

\DefLabeledDefinitionNote{linearly independent vectors}{\SideNS}
{
Множество векторов\,\footnotemark
\ShowEq{set vi *}v
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$
\AddIndex{линейно независимо}{linearly independent set},
если
\ShowEq{w(i)=0}c
следует из уравнения
\DrawEq[cv]{wi vi=0}{\SideNS}
В противном случае, множество векторов
\ShowEq{set vi *}v
\AddIndex{линейно зависимо}{linearly dependent set}.
}
{Я следую определению на страница
\citeBib{Serge Lang}\Hyph  100.}

\DefLabeledTheorem{quasibasis of module}{\SideNS}
{
Множество векторов
\ShowEq{basis, module}
является квазибазисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e(\gii)$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
}

\DefProof{quasibasis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определению
\refDefinition{linear combination of vectors}{\SideNS},
множество $\Basis e$ порождает \SideRuTo $\Base$\Hyph модуль $V$
(определение
\refDefinition{generating set of module}{\SideNS}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRuTo $\Base$\Hyph модуль $V$.
Согласно определению
\refDefinition{generating set of module}{\SideNS},
множество $\Basis e$ является квазибазисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefLabeledTheorem{basis over division algebra}{\SideNS}
{
Пусть $\Base$ - \AlgebraRu\DivisionRuNS.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы
\ARow ei
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов
\ARow ei.
}

\DefLabeledTheorem{vector space is free module}{\SideNS}
{
\SideRuCTo $\Base$\Hyph векторное пространство
является свободным $\Base$\Hyph модулем.
}

\DefProof{basis over division algebra}
{
Пусть множество векторов
\ShowEq{set vi \Cols}e
линейно зависимо. Тогда в равенстве
\DrawEq[we]{wi vi=0}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}w.
Согласно теореме
\refTheorem{linearly depends on rest of vectors}{\SideWS module},
вектор
\ARow ej{}
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\refDefinition{basis of module}{\SideNS},
множество векторов
\ShowEq{set vi \Cols}e
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{set vi \Cols}e
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{set vi \Cols}e
то множество векторов $v$,
\ShowEq{set vi \Cols}e
не является линейно независимым.
}

\DefLabeledConvention{unit of algebra in basis}{\Cols}
{
Пусть \eV - базис $D$\Hyph алгебры \ColsA $A$.
Если $D$\Hyph алгебра $A$ имеет единицу,
положим \ARow e0 - единица $D$\Hyph алгебры $A$.
}

\DefTheoremNote{algebra A2 representation in LA}
{
Пусть $A_1$ и $A_2$ являются $D$\Hyph алгебрами.
Пусть произведение в алгебре \AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{A2}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnotemark
алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
}
{Определение представления
$\Omega$\Hyph алгебры дано в определении
\ShowEq{ref definition: representation of algebra}.}

\DefLabeledTheorem[4]{matrix generates D module homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers}D{#3}fiIjJ
Отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph модуля \ColsA $V_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $V_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D module homomorphism}
{
Равенство
\ShowEq{fo(v+w) \Cols(#1)}
\begin{sloppypar}
\noindent
является следствием равенств
\ShowRef{homomorphism of D module}{#1}{#2}{#5}
Из равенства
\EqRef{fo(v+w) \Cols(#1)}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\ShowEq{fo(va) \Cols(#1)}
является следствием равенства
\eqRef{left homomorphism, f av=}{f D module #1#2}.
Из равенства
\EqRef{fo(va) \Cols(#1)}
и определений
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{linear map of D module}{#1#2}
следует, что отображение
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
\begin{sloppypar}
\noindent
является гомоморфизмом
$D_{#1}$\Hyph модуля \ColsA $V_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $V_{#4}$.
\end{sloppypar}

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}12{}.%
Равенство
\ShowEq{fov=gov \Cols(#1)}
является следствием теоремы
\refTheorem{linear map of D module}{#1#2}.
Следовательно, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[4]{matrix generates D algebra homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers and C}D{#3}fiIjJ{#1}{#2}
Отображение\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph алгебры \ColsA $A_{#2}$
в $D_{#3}$\Hyph алгебру \ColsA $A_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D algebra homomorphism}
{
Согласно теореме
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
отображение
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
и гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
определён однозначно.

Пусть
\ShowEq{a=ai ei}a1i,
\ShowEq{a=ai ei}b1i.
Равенство
\DrawEq{algebra, homomorphism and product abe #1#2}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)}.
\ShowText{matrix generates D algebra homomorphism (#1)}
Равенство
\DrawEq{algebra, homomorphism and product abe 3(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product abe 4(#1)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
Равенство
\DrawEq{algebra, homomorphism and product abe 5(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 4(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\ShowRef{homomorphism, f vw=}{#1}{#2}
является следствием равенств
\ShowRef{algebra, homomorphism and product 1}{#1}{#2}
Согласно теореме
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2},
отображение
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefText{matrix generates D algebra homomorphism (1)}
{
Так как отображение $h$ является гомоморфизмом
кольца $D_1$ в кольцо $D_2$, то
\DrawEq{algebra, homomorphism and product abe 2}{\Cols}
Равенство
\DrawEq{algebra, homomorphism and product abe 2(1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2}{\Cols}
и равенства
\ShowRef{product in algebra}
}

\DefText{matrix generates D algebra homomorphism ()}
{
Равенство
\DrawEq{algebra, homomorphism and product abe 2()}{\Cols}
является следствием равенства
\ShowRef{product in algebra}
}

\DefLabeledDefinition[1]{exact sequence, D module}{(#1)}
{
Пусть
\ShowEq{Ai, 1n}V
- $D_{#1}$\Hyph модули.
Последовательность гомоморфизмов
\ShowEq{V1->...->Vn (#1)}
называется
\AddIndex{точной}{exact sequence},
если
\ShowEq{Im f=ker hf (#1)}
}

\DefTheorem{submodule is kernel}
{
Пусть $D$\Hyph модуль $V_1$ является свободной аддитивной группой.
Пусть $U$ - подмодуль $D$\Hyph модуля $V_1$.
Существует гомоморфизм
\newline
\FrameEqRef[fV]{homomorphism D algebra 1}{Vector module, coordinates \Cols}
\newline
такой, что
\[\ker f=U\]
}

\DefProof{submodule is kernel}
{
Согласно теореме
\RefTheorem{direct sum of submodules},
существует подмодуль $W$ такой, что
\ShowEq{V=Uo+W}1
Отображение
\ShowEq{u o+ w->w}
является гомоморфизмом и
\[\ker f=U\]
}

\DefTheorem{direct sum of submodules}
{
Пусть $D$\Hyph модуль $V$ является свободной аддитивной группой.
Пусть $U$ - подмодуль $D$\Hyph модуля $V$.
Существует подмодуль $W$ такой, что
\ShowEq{V=Uo+W}{}
}

\DefProof{direct sum of submodules}
{
Согласно определениям
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\refDefinition{submodule}{\SideWS module},
$U$ является подгруппой аддитивной группы $V$.
Согласно теоремам
\RefTheorem{A=C o+ D free group},
\RefTheorem{B=Ao+B/A},
существует подгруппа $W$ аддитивной группы $V$ такая, что
группа $W$ изоморфна группе $V/U$ и
\ShowEq{V=Uo+W}{}

Согласно теореме
\refTheorem{direct sum of D modules 2024}{\SideWS \Base-\VectorsSetNS},
действие $D$\Hyph числа $a$ на произвольное $V$\Hyph число
\ShowEq{v=u0+0w}
имеет вид
\ShowEq{av=u0+0w}
Следовательно, $W$ является подмодулем $D$\Hyph модуля $V$.
}

\DefLabeledFootnote[4]{homomorphism of D module}{\Cols(#1#2)}
{
В теоремах
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefLabeledFootnote[6]{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledFootnote[6]{Coordinates of Linear Map}{\SideNS-\Cols(#1#2#3)}
{
В теореме %ах
\refTheorem{linear map of A module, coordinates}{\SideNS-\Cols(#1#2#3)},
%\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space 2020(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledFootnote[6]{homomorphism of A module 2020}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space 2020(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledDefinition[4]{homomorphism from A1 to A2, D algebra}{#1#2}
{
\ShowText{algebra over ring (#1#2)}
Пусть
\DrawEq[{#1}{1.}{#2}h]{diagram of representations of D algebra}{->1(#1#2)}
диаграмма представлений, описывающая $D_1$\Hyph алгебру $A_1$.
Пусть
\DrawEq[{#3}{2.}{#4}h]{diagram of representations of D algebra}{->2(#1#2)}
диаграмма представлений, описывающая $D_2$\Hyph алгебру $A_2$.
Морфизм
\DrawEq[fA]{homomorphism D algebra #1#2}1
диаграммы представлений
\eqRef{diagram of representations of D algebra}{->1(#1#2)}
в диаграмму представлений
\eqRef{diagram of representations of D algebra}{->2(#1#2)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Обозначим
\ShowEq{set homomorphisms, D algebra #1#2}
множество гомоморфизмов
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefLabeledTheorem[5]{homomorphism from A1 to A2, D algebra}{#1#2}
{
Гомоморфизм
\newline
\FrameEqRef[fA]{homomorphism D algebra #1#2}1
\newline
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$
- это линейное отображение
\eqRef[fA]{homomorphism D algebra #1#2}1
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
такое, что
\DrawEq[fab]{homomorphism, f vw=}{(#1#2)g}
и удовлетворяет следующим равенствам
\ShowEq{define homomorphism of D algebra #1#2}{#1}{#2}{#5}
}

\DefProof[4]{homomorphism from A1 to A2, D algebra}
{
Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение
\eqRef{homomorphism D algebra #1#2}1
явлется морфизмом представления $h_{1.12}$,
описывающего $D_{#1}$\Hyph модуль $A_{#2}$,
в представления $h_{2.12}$,
описывающего $D_{#3}$\Hyph модуль $A_{#4}$.
Следовательно, отображение $f$ является линейным отображением $D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$ и равенства
\ShowEq{ref homomorphism of D algebra(#1)}{#1}{#2}
являются следствием теоремы
\refTheorem{linear map of D module}{#1#2}.

Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение $f$
явлется морфизмом представления $h_{1.23}$
в представления $h_{2.23}$.
Равенство
\DrawEq{morphism of representation, algebra, 23}{#1#2}
следует из равенства
\eqRef{morphism of representations of universal algebra, 2m}{representation}.
Из равенств
\eqRef{diagram of representations of D algebra}{->1(#1#2)},
\eqRef{diagram of representations of D algebra}{->2(#1#2)},
\eqRef{morphism of representation, algebra, 23}{#1#2},
следует
\DrawEq{algebra, morphism of representation 23, 1}{#1#2}
Равенство
\eqRef{homomorphism, f vw=}{(#1#2)g}
следует из равенств
\eqRef{product in D algebra}{definition},
\eqRef{algebra, morphism of representation 23, 1}{#1#2}.
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
Если произведение в $D$\Hyph алгебре $A$ имеет единичный элемент,
то $D$\Hyph алгебра $A$ называется
\AddIndex{унитальной алгеброй}{unital algebra}.\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение унитальной алгебры также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph алгебра \(A\) называется
\AddIndex{алгеброй с делением}{division algebra},
если для любого \(A\)\Hyph числа \(a\ne 0\)
существует \(A\)\Hyph число \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Из утверждения
\ShowEq{ab=ac a ne 0}
следует, что $b=c$.
}

\DefProof{division algebra}
{
Равенство
\ShowEq{ab=ac a ne 0 1}
является следствием утверждения
\EqRef{ab=ac a ne 0 1}.
}

\DefLabeledDefinition[4]{linear map of D module}{#1#2}
{
Морфизм представлений
\DrawEq[fV]{homomorphism D algebra #1#2}{module}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
называется гомоморфизмом или
\AddIndex{линейным отображением}{linear map}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
Обозначим
\ShowEq{set linear maps, module (#1#2)}DV
множество линейных отображений
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
Множество
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Пусть $A$ - нормированный $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - нормированный $D$\Hyph модуль с нормой $|y|_B$.
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}D{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\ShowEq{f()},
\ShowEq{g()}.
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnotemark
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\ShowEq{g()}{}
на $B_1$\Hyph число
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
}

\DefDefinition{symmetric polylinear map}
{
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$a_i=a_{i+1}$
хотя бы для одного\,\footnotemark
\ShowEq{1<=i<n}
}{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}

\DefTheorem[3]{alternation of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\ShowEq{[f]},
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefText[4]{quasibasis of A-module}
{
Пусть
\DrawEq[{#2}{#3}{#4}]{basis e of module cols}-
- квазибазис $A$\Hyph модуля $#1$.
}

\DefLabeledTheorem{a quasibasis of A}{\SideNS}
{
$D$\Hyph алгебра $A$ имеет квазибазис
\ShowEq{e=a in A}
если
\ShowEq{Aa=A}
и $A$\Hyph число $a$ является \OtherSideRu вым делителем нуля.
}

\DefText[2]{quasibasis 1n of A-module}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
квазибазис $A$\Hyph модуля $#1$.
}

\DefTheorem{there exist tensor g=1/f}
{
Пусть
$\aUD Ck{ij}$
- структурные константы $D$\Hyph алгебры $A$.
Пусть
\DrawEq[f]{f=...ei o ek}{}
стандартное представление тензора
\ShowEq{f in AoA}f.
Пусть существует тензор
\ShowEq{g=f-}{}{}
и
\DrawEq[g]{f=...ei o ek}{}
стандартное представление тензора $g$.
Тогда стандартные компоненты тензора $g$
удовлетворяют системе линейных уравнений
\ShowEq{fg=1 e o e}
}

\DefProof{there exist tensor g=1/f}
{
Теорема является следствием равенства
\ShowEq{g o h=1}
и теоремы
\RefTheorem{standard representation of product of tensors}.
}

\DefText{system of linear equations linear map}
{
Пусть
\ShowEq{f:A->B}fVW
линейное отображение $A$\Hyph векторного пространства $V$
в $A$\Hyph векторное пространство $W$.
Отображение координатной матрицы вектора $v\in V$
относительно базиса $\Basis e_V$
в координатную матрицу вектора $f\circ v\in W$
относительно базиса $\Basis e_W$
имеет вид
\DrawEq[vf{(f\circ v)}mn]{system of linear equations linear map}{}
и не зависит от того, рассматриваем мы левое $A$\Hyph векторное пространство
или правое $A$\Hyph векторное пространство.
Чтобы найти координатную матрицу вектора
\ShowEq{v in V, fv=w}
мы должны решить систему линейных уравнений
\DrawEq[vfwmn]{system of linear equations linear map}{preface}
}

\DefLabeledTheorem[2]{direct sum over quasibasis}{\Cols,\SideNS-\VectorSetNS}
{
\def\Temp{#2}%
\def\One{1}%
\ifx\Temp\One%
\ShowText{quasibasis of A-module}V{}iI
\else%
\ShowEq{Let be basis of module}1{}iI{\SideRu\Which}{#1}{}V{}
\fi%
Тогда мы можем представить $#1$\Hyph модуль $V$
как прямую сумму
\DrawEq[{#1}{}]{V=+eiA}{\SideWS \Cols}
}

\DefProof[1]{direct sum over quasibasis}
{
Отображение
\ShowEq{V->+eiA}{#1}
является изоморфизмом.
}

\DefLabeledTheorem{quasibasis and linear map}{\SideWS \Cols}
{
\ShowText{quasibasis of A-module}VViI
\ShowText{quasibasis of A-module}WWjJ
Тогда линейное отображение
\DrawEq[{\Vector f}VW{}]{f: A->B}{fVW \SideWS \Cols}
имеет представление
\DrawEq{quasibasis and linear map}{\SideWS \Cols}
где матрица
\DrawEq{quasibasis and matrix of linear map}{\SideWS \Cols}
называется матрицей линейного отображения $\Vector f$
относительно выбранных базисов.
}

\DefLabeledTheorem{finite quasibasis and product linear map}{}
{
\ShowText{quasibasis 1n of A-module}Uk
\ShowText{quasibasis 1n of A-module}Vn
\ShowText{quasibasis 1n of A-module}Wm
Пусть линейное отображение
\DrawEq[{\Vector f}UV{}]{f: A->B}{}
имеет представление
\DrawEq[funk]{quasibasis nm and linear map}{fu \SideWS \Cols}
относительно выбранных квазибазисов.
Пусть линейное отображение
\DrawEq[{\Vector g}VW{}]{f: A->B}{}
имеет представление
\DrawEq[gvmn]{quasibasis nm and linear map}{gv \SideWS \Cols}
относительно выбранных квазибазисов.
Тогда линейное отображение $f\circ g$
имеет матрицу
\ShowEq{matrix linear f o g}
\ShowEq{matrix linear (f o g)}
относительно выбранных квазибазисов.
}

\DefLabeledTheorem{finite quasibasis and linear map}{}
{
\ShowText{quasibasis 1n of A-module}Vn
\ShowText{quasibasis 1n of A-module}Wm
Тогда линейное отображение
\newline
\FrameEqRef[{\Vector f}VW{}]{f: A->B}{fVW \SideWS \Cols}
\newline
имеет представление
\DrawEq[fvnm]{quasibasis nm and linear map}{\SideWS \Cols}
относительно выбранных квазибазисов.
}

\DefText{linear dependence between vectors of basis}
{
Согласно теореме
\refTheorem{linear dependence between vectors of basis}{\SideWS module},
может существовать линейная зависимость между векторами квазибазиса.
}

\DefLabeledTheorem{linear dependence between vectors of basis}{\SideWS module}
{
Пусть $\Base$ - \Algebra.
Пусть $\Basis e$ - квазибазис \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Пусть
\DrawEq[ce]{wi vi=0}{we \SideWS \Cols}
линейная зависимость векторов квазибазиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{\BaseExt}$\Hyph число
\ShowEq{ci i in I}
не имеет обратного элемента
в \ShortAlgebraRuDWS $\Base_{\BaseExt}$.
\item
Множество $V'$ матриц
\ShowEq{c=ci i in I}
порождает \SideRuTo $\Base$\Hyph модуль $V'$.
\end{enumerate}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{c=ci i in I}
такая, что равенство
\eqRef{wi vi=0}{we \SideWS \Cols}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Если мы положим, что $\Base$\Hyph число
\ACol cj
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}ec
является следствием равенства
\eqRef{wi vi=0}{we \SideWS \Cols}.
Следовательно вектор
\ARow ej{}
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является квазибазисом.
Следовательно, наше предположение неверно,
и $\Base_{\BaseExt}$\Hyph число
\ACol cj
не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[be]{wi vi=0}{}
\DrawEq[ce]{wi vi=0}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[ce]{wi vi=0}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\DefLabeledTheorem{coordinates of vector with linear dependence}{\SideWS module}
{
Пусть \SideRuTo $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что в равенстве
\DrawEq[ce]{wi vi=0}{2 we \SideWS \Cols}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{c=ci i in I}
определяет координаты вектора $0\in V$ относительно квазибазиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно квазибазиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{wi vi=0}{2 we \SideWS \Cols}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно квазибазиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{wi vi=0}{2 we \SideWS \Cols},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{quasibasis of module is basis}{\SideWS \VectorSetNS}
{
Пусть множество векторов квазибазиса \eV
\SideRu\From $\Base$\Hyph модуля $V$
линейно независимо.
Тогда квазибазис \eV является
базисом \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefProof{quasibasis of module is basis}
{
Теорема является следствием определения
\RefDefinition{basis of representation}
и теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}.
}

\DefLabeledDefinitionNote{free module over ring}{\SideNS}
{
\SideRuCTo $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRuTo $\Base$\Hyph модуль}{free module},\,\footnotemark
если \SideRuTo $\Base$\Hyph модуль $V$ имеет базис.
}
{
Я следую
определению в \citeBib{Serge Lang}, страница 103.
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}
и определений
\refDefinition{linearly independent vectors}{\SideNS},
\refDefinition{free module over ring}{\SideNS}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnotemark
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}DAA{}
имеет следующее разложение
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA,
то согласно определению
\refDefinition{free module over ring}{\SideNS},
существует разложение
\DrawEq[A]{expansion of linear map with respect to basis}A
линейного отображения $f$ относительно базиса $\Basis F$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
Равенство
\eqRef{map f generated by basis F}{associative algebra}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A->A, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\ShowEq{A->B}AD.
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefLabeledConvention{sum av() convention}{\SideNS}
{
Мы будем пользоваться соглашением о сумме,
в котором повторяющийся индекс
в линейной комбинации
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av()\SideNS}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefConvention{av=sum av convention}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av convention}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefLabeledTheorem{effective representation of the ring}{\SideWS \Base-\VectorsSetNS}
{
Представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$
в абелевой группе $V$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
}

\DefProof{effective representation of the ring}
{
Если $a$, $b\in \Base$
порождают одно и то же преобразование, то
\DrawEq{representation of ring, 1}{\Base}
для любого $m\in V$.
Из равенств
\eqRef{sum of transformations of Abelian group, 1}{\Base},
\eqRef{representation of ring, 1}{\Base}
следует, что
\DrawEq{representation of ring, 2}{\Base}
Равенство
\ShowEq{f(a-b)=0}
является следствием равенств
\eqRef{0ov=0}{\Base},
\eqRef{representation of ring, 2}{\Base}.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
}

\DefLabeledTheorem{Representation of ring f(0)=v0}{\SideWS \Base-\VectorsSetNS}
{
Представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$
в абелевой группе $V$
удовлетворяет равенству
\DrawEq{f(0)=v0}{\Base}
где
\ShowEq{0:V->V}
отображение такое, что
\DrawEq{0ov=0}{\Base}
}

\DefProof{Representation of ring f(0)=v0}
{
Равенство
\DrawEq{fa=fa+f0}{\Base}
является следствием равенства
\eqRef{sum of transformations of Abelian group, 1}{\Base}.
Равенство
\DrawEq{f0x=0}{\Base}
является следствием равенства
\eqRef{fa=fa+f0}{\Base}.
Равенство
\eqRef{0ov=0}{\Base}
является следствием равенств
\eqRef{f(0)=v0}{\Base},
\eqRef{f0x=0}{\Base}.
}

\DefText{sum of transformations of Abelian group}
{
Согласно теореме
\refTheorem{monoid-homomorphism, sum}{+},
рассматривая представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$ в абелевой группе $V$, мы полагаем
\DrawEq{f(a)+f(b)=}{\Base}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом \algebrae $\Base$.
Следовательно
\DrawEq{f(a+b)=f(a)+f(b)}{\Base}
Равенство
\DrawEq{sum of transformations of Abelian group, 1}{\Base}
является следствием равенств
\eqRef{f(a)+f(b)=}{\Base},
\eqRef{f(a+b)=f(a)+f(b)}{\Base}.
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
Согласно
\citeBib{q-alg-9705026},
\citeBib{math.QA-0208146},
у нас нет определения
детерминанта в случае алгебры с делением.\,\footnote{
В алгебре кватернионов профессор Кирчей
пользуется двойным определителем
(смотри определение в разделе
\citeBib{1812.03397}\Hyph 2.2)
для решения системы линейных уравнений
и для решения задачи о собственных значениях
(смотри раздел
\citeBib{1812.03397}\Hyph 2.5).
Я ограничился рассмотрением квазидетерминантов,
так как меня интересует более широкий класс алгебр.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{1812.03397}
\fi
}
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении
\RefDefinition{RC-quasideterminant},
я следую определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{q-alg-9705026}
\FrameCiteBib{math.QA-0208146}
\fi
}

\DefConvention{basis of algebra as basis of module}
{
Согласно определениям
\refDefinition{free module over ring}{},
\RefDefinition{algebra over ring}
свободная $D$\Hyph алгебра $A$ - это
$D$\Hyph модуль $A$,
который имеет базис \eV[][.]
Однако, вообще говоря, \eV не является
базисом $D$\Hyph алгебры $A$,
так как в $D$\Hyph алгебре $A$ определено произведение.
Например, в алгебре кватернионов произвольный кватернион
\ShowEq{any quaternion}
может быть представлен в виде
\ShowEq{any quaternion i j ij}
Однако при решении большинства задач
использование базиса $D$\Hyph модуля $A$ проще, чем
использование базиса $D$\Hyph алгебры $A$.
Например, легче определить координаты $H$\Hyph числа относительно базиса
$(1,i,j,k)$
$R$\Hyph векторного пространства $H$,
чем определить координаты $H$\Hyph числа относительно базиса
$(1,i,j)$
$R$\Hyph алгебры $H$.
Поэтому фраза "мы рассматриваем базис $D$\Hyph алгебры $A$"
означает, что мы рассматриваем $D$\Hyph алгебру $A$
и базис $D$\Hyph модуля $A$.
}

\DefConvention{we use separate color for index of element}
{
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\DefLabeledTheorem{direct sum of n modules}{\SideWS \Base-\VectorsSetNS}
{
Прямая сумма \SideRu\TO $\Base$\Hyph \VectorsSetRuB
\ShowEq{a1n}{\Module}n{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}{\Module}
}

\DefLabeledTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
Представим $\VNumber$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{}
Представим линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
как вектор строку
\DrawEq[fn]{a=(a1.n row)}{}
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Тогда значение отображения $f$ в $\Module$\Hyph числе $\VNumber$
можно представить как произведение матриц
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
}

\DefProof{foa=fi ai}
{
Теорема является следствием определений
\ShowEq{def left}
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS},
\ShowEq{def right}
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\DefLabeledTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{}
Тогда линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
имеет представление как вектор столбец отображений
\DrawEq[fm]{a=(a1.n col)}{}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
}

\DefProof{foa=fi a}
{
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть \eV[i]
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Выражение
$\ShowSymbol{standard component of tensor}{}$
определено однозначно и называется
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
}

\DefLabeledTheorem{map of direct sum of modules}{\Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\Module$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{v,\SideWS \Base-\VectorsSetNS}
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{w,\SideWS \Base-\VectorsSetNS}
Тогда линейное отображение
\ShowEq{f:A->B}fVW
имеет представление как матрица отображений
\DrawEq[fnm]{a=(a11.nm matrix)}{f,\SideWS \Base-\VectorsSetNS}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[f{\VNumberA}{\VNumber}nm]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
Отображение
\ShowEq{fij:->}{\Module}{\ModuleA}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\DefProof{map of direct sum of modules}
{
Согласно теореме
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
Согласно теореме
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\DefDefinition{Matrix of tensors}
{
Пусть $a$ - матрица и
\ShowEq{a in Aoxn}{\aUD aij}n.
Матрица $a$ называется матрицей тензоров
\ShowEq{Aoxn}n.
Если $n=2$, то матрица $a$ также называется
матрицей отображений.
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{aU A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $\aUD fij$
с помощью \BoxB{\aU Bi}чисел.
}

\DefText{Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\DefText{Coordinates of Linear Map}
{
\section{Общее определение}

\ShowText{def Coordinates of Linear Map}111222{h(p)}{(g\circ a)}

\section{Линейное отображение, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{def Coordinates of Linear Map}{}11{}22p{(g\circ a)}

\section{Линейное отображение, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{def Coordinates of Linear Map}{}{}1{}{}2pa
}

\DefLabeledTheorem[7]{linear map of A module, coordinates}{\SideNS-\Cols(#1#2#3)}
{
Линейное отображение\,\refFootnote{Coordinates of Linear Map}{\SideNS-\Cols(#1#2#3)}
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{linear \SideNS}
\newline
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}{ 0}
\ShowText{f:V1->V2, A module}{#1}{#2}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}{ 0}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
%\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
%\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}{#2_1}{}
\DrawEq [#1{#2_1}]{va=ae1, #8module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS \VectorSetNS}
относительно базиса
\ShowEq{basis e}{#2_2}{}
\DrawEq [#9{#2_2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}{#2_2}.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}{#2_1}{}
и
\ShowEq{basis e}{#2_2}.
}

\DefText[6]{Proof, linear map of A module(1)}
{
Согласно определениям
\ShowRef{Proof, linear map of A module}{#1}{#2}{#3}%
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{\SideNS-\Cols}
\begin{sloppypar}
\noindent
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#4}$\Hyph алгебру $A_{#5}$.
Следовательно, равенства
\ShowRef{Proof, linear map of A module 1}{#1}{#2}{#3}%
следуют из равенств
\ShowRef{Proof, homomorphism of vector space 2}{#1}{#2}{#3}{#4}%
Из теоремы
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
следует что матрица $g$ определена однозначно.
\end{sloppypar}

}

\DefText[6]{Proof, linear map of A module()}
{%
}

\DefProof[6]{linear map of A module, coordinates}
{
\ShowText{Proof, linear map of A module(#2)}{#1}{#2}{#3}{#4}{#5}{#6}%

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map, A module (#2)}{\SideWS \Cols(#1#2)}
является следствием теоремы
\refTheorem{map of direct sum of modules}{\Base-\VectorsSetNS}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\ShowEq{V=o+Ae}#1#2#3
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}DA
алгебры \AOn
в модуле \LAnA,
определённое равенством
\DrawEq[DA]{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[DA]{product in algebra An 2}{DA}
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\DefText[4]{notation for linear map}
{
Если отображение
\eqRef{homomorphism D algebra #1#2}{module}
является линейным отображением $D_{#1}$\Hyph модуля $V_{#2}$ в $D_{#3}$\Hyph модуль $V_{#4}$,
то, согласно определению
\refDefinition[\RefRepresentation]{side representation of group}{left},
я пользуюсь обозначением
\DrawEq{f circ a =}{}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},%, associative algebra},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefProof{representation of composition of linear maps}
{
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
}

\DefDefinition{similar A numbers}
{
$A$\Hyph числа $a$ и $b$ называются подобными,
если существует $A$\Hyph число $c$ такое, что
\ShowEq{similar A numbers}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A->B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет вид
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
Множество линейных отображений
\ShowEq{vI=EI}
является базисом
левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}
и линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
$#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
\ShowEq{vI=... #1}
и $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
кватернионы, представленные строками матрицы $f$.
\ShowEq{fi=fij ej H}
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}O
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map, maps of conjugation, algebra C}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\DrawEq[fCC{}]{f: A->B}{}
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a...= C}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\DefTheorem{sum of polylinear maps, module}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
}

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество \LAB D{A_1}{A_2}
является абелевой группой
относительно суммы отображений.
}

\DefDefinition{linear map A module}
{
\ShowText{algebra over ring (11)}
Пусть
\ShowEq{Ai, i=}V
- $A_i$\Hyph \VectorSetRuANS.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
$A_1$\Hyph \VectorSetRuB $V_1$ в
$A_2$\Hyph \VectorSetRuA $V_2$.
Обозначим
\ShowEq{set linear maps, V12 module}
множество линейных отображений
$A_1$\Hyph \VectorSetRuB $V_1$ в
$A_2$\Hyph \VectorSetRuA $V_2$.
}

\DefText[7]{homomorphism of A module 1}
{
\subsection{Гомоморфизм \SideRu вого \texorpdfstring{$A$}{A}-\VectorSetRuB \ColsNA}
\ShowText{homomorphism of A module 2}{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}

\DefText{homomorphism A module}
{
\section{Общее определение}

\ShowText{def homomorphism A module}111222{h(p)}{(g\circ a)}

\section{Гомоморфизм, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{def homomorphism A module}{}11{}22p{(g\circ a)}

\def\Temp{module}%
\ifx\Temp\VectorSetNS
\ProveTheorem{da in DA->da in D1A}

\ShowConvention{da in DA->da in D1A}
\fi

\section{Гомоморфизм, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{def homomorphism A module}{}{}1{}{}2pa
}

\DefText{algebra over ring (11)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D_i$.%
}

\DefText{algebra over ring (1)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{algebra over ring ()}
{
Пусть $A$
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{module over algebra (11)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRuTo $A_i$\Hyph модуль.
}

\DefText{module over algebra (1)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRuTo $A$\Hyph \VectorSetRuANS.
}

\DefLabeledDefinition[6]{homomorphism A module}{\SideNS(#1#2#3)}
{
Пусть
\DrawEq[{#1}{#2}{#3}{1.}]{diagram of representations, \SideWS module}{->1(#1#2#3)}
диаграмма представлений, описывающая
\SideRuTo $A_{#2}$\Hyph \VectorSetRuA $V_{#3}$.
Пусть
\DrawEq[{#4}{#5}{#6}{2.}]{diagram of representations, \SideWS module}{->2(#4#5#6)}
диаграмма представлений, описывающая
\SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Морфизм
\DrawEq[gf]{homomorphism A module #1#2#3}{\SideNS}
диаграммы представлений
\eqRef{diagram of representations, \SideWS module}{->1(#1#2#3)}
в диаграмму представлений
\eqRef{diagram of representations, \SideWS module}{->2(#4#5#6)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Обозначим
\ShowEq{set homomorphisms, A module #1#2#3 \SideNS}
множество гомоморфизмов
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
%\ShowEq{set homomorphisms, \SideWS A12 module}
%множество гомоморфизмов
%\ShowEq{\SideWS column module}{A_1}
%модуля $V_1$ в
%\ShowEq{\SideWS column module}{A_2}
%модуль $V_2$.
}

\DefText[8]{homomorphism A module 1 111}
{
Отображение
\DrawEq[h{D_1}{D_2}{}{}]{f: A->B}{}
является гомоморфизмом колец и удовлетворяет равенствам
\ShowRef{define homomorphism of A module 111}
\ShowText{homomorphism A module 1 11}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefText[8]{homomorphism A module 1 11}
{
Отображение
\DrawEq[g{A_1}{A_2}{}{}]{f: A->B}{}
является гомоморфизмом $D_{#1}$\Hyph алгебры $A_1$ в $D_{#4}$\Hyph алгебру $A_2$
и удовлетворяет равенствам
\ShowRef{define homomorphism of A module 11}{#1}{#2}{#7}
\ShowText{homomorphism A module 1 1}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefText[8]{homomorphism A module 1 1}
{
Отображение
\DrawEq[f{V_1}{V_2}{}{}]{f: A->B}{}
является гомоморфизмом абелевой группы
\newline
(равенство
\ShowRef{define homomorphism of A module 1}{#1}{#2}
и согласовано с представлением
\newline
(равенство
\ShowRef{define homomorphism of A module 2}{#1}{#2}{#8}
}

\DefLabeledSummary[8]{homomorphism A module}{\SideNS(#1#2#3)}
{
Пусть
\ShowRef{diagram of representations of module}{#1}{#2}{#3}1
диаграмма представлений, описывающая
\SideRuTo $A_{#2}$\Hyph \VectorSetRuA $V_{#3}$.
Пусть
\ShowRef{diagram of representations of module}{#4}{#5}{#6}2
диаграмма представлений, описывающая
\SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Гомомрфизм
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
- это отображение
\ShowRef{homomorphism A module}{#1}{#2}{#3}gf
каждая компонента которого
является гомоморфизмом соответствующей алгебры
и эти гомоморфизмы согласованы.
\ShowText{homomorphism A module 1 #1#2#3}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefLabeledSummary[8]{homomorphism associative A module}{\SideNS(#1#2#3)}
{
\ShowEq{\DefCol}
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowText{matrices of numbers(#2#3)}{#4}{#5}{#1}{#2}
\ShowText{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}{}
Гомоморфизм
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
который имеет%
\ShowText{define homomorphism by given matrix(#2)}%
определён однозначно.

Если $D_2$\Hyph алгебра $A_2$ ассоциативна,
то из равенства
\eqRef{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(111)}
следует равенство
\begin{equation}%
\aU{(\Vector{f}\circ(v\CRstar e_{V_1}))}j=(\Vector g\circ \aU vi)\CRstar \aUD fji
\end{equation}%

Обратное утверждение также верно.
Пусть квазибазис \eV[V_2] является базисом.
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}{#5}
}

\DefLabeledTheorem[8]{define homomorphism A module}{\SideNS(#1#2#3)}
{
Гомоморфизм
\newline
\FrameEqRef[gf]{homomorphism A module #1#2#3}{\SideNS}
\newline
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
удовлетворяет следующим равенствам
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}{}
}

\DefProof[7]{define homomorphism A module}
{
\ShowText{define homomorphism of vector space(#2)}{#1}{#2}{#4}{#5}{#7}
Равенство
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module#7}
является следствием определения
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
так как, согласно определению
\RefDefinition{morphism of representations of universal algebra},
отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module#7}
является следствием равенства
\EqRef{morphism of representations of universal algebra},
так как отображение
\ShowEq{homomorphism A module, 1#7}{#1}{#2}{#3}
является морфизмом представления $g_{1.34}$
в представление $g_{2.34}$.
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefLabeledTheoremNote[5]{linear map of D module}{#1#2}
{
Линейное отображение
\newline
\FrameEqRef[fV]{homomorphism D algebra #1#2}{module}
\newline
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
удовлетворяет равенствам\,\footnotemark
\ShowEq{define homomorphism of D module #1#2}{#1}{#2}{#5}
}
{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of D module}{#1#2}
рассматривается как определение.
}

\DefText{linear map of D module (11)}
{
Согласно определению
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
отображение $h$
явлется гомоморфизмом кольца $D_1$
в кольцо $D_2$.
Равенства
\ShowEq{ref linear map of D module 1}
являются следствием этого утверждения.
}

\DefText{linear map of D module (1)}
{
}

\DefProof[2]{linear map of D module}
{
\ShowText{linear map of D module (#1#2)}
Из определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
следует, что
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{homomorphism, f v+w=}{f D module #1#2}).
Равенство
\eqRef{left homomorphism, f av=}{f D module #1#2}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.

Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\refDefinition{linear map of D module}1,
\RefDefinition{polylinear map of modules}
и теоремы
\refTheorem{linear map of D module}1.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A->B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\DefLabeledTheorem[8]{linear map of A module}{#1#2#3, \SideNS}
{
Линейное отображение
\DrawEq[gf]{homomorphism A module #1#2#3}{linear \SideNS}
\SideRu\From $A_{#5}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
удовлетворяет равенствам
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}{ 0}
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\DefLabeledTheorem[1]{maps of conjugation antilinear}{#1}
{
Отображения сопряжения
\ShowEq{I... #1}
\DoVerb являются антилинейными гомоморфизмами.
}

\DefProof[1]{maps of conjugation antilinear}
{
Произведение $#1$\Hyph чисел
\ShowEq{#1 number Ea}a
и
\ShowEq{#1 number Ea}b
имеет вид
\DrawEq[ab]{#1 product aEx}{ab}
\ShowText{maps of conjugation antilinear #1}
}

\DefText{maps of conjugation antilinear H}
{
\ShowEq{H items maps of conjugation antilinear}
}

\DefText{maps of conjugation antilinear O}
{
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A->B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
%существует разложение
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
Равенство
\eqRef{map f generated by basis F}{expansion}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Пусть $A$ - $D$\Hyph алгебра.
Для любого $A$\Hyph числа $a$, отображение
\ShowEq{f->ao f}
определённое равенством
\ShowEq{ao f=a f o}
является эндоморфизмом $D$\Hyph модуля
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA
является левым $A$\Hyph модулем, порождённым представлением
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A->B)}R{#1}{#1}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\DefText{let i=12}
{
Пусть
\ShowEq{i=1,2}.
}

\DefText[6]{Let be quasibasis of module}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module #5}{#6}
является квазибазисом \SideRu вого $#4$\Hyph \VectorSetRuB $#1_i$.%
}

\DefText[6]{Let be basis of vector space}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module #5}{#6}
является базисом \SideRu вого $#4$\Hyph \VectorSetRuB $#1_i$.%
}

\AddEq [9]{Let be basis of vector space}
{%
Пусть множество векторов
\DrawEq[{#1}{#2}{#3}]{basis e of module #8}{#9}
является базисом \SideRu вого $#4_{#5}$\Hyph \VectorSetRuB $#6_{#7}$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Пусть \eV[#1]
базис \SideRu вого $#2$\Hyph векторного пространства $#3$.%
}%

\AddEq [9]{Let be basis of module}
{%
Пусть
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}-
базис #5 $#6_{#7}$\Hyph \VectorSetRuB \ColsA $#8_{#9}$.
}

\AddEq [9]{Let be basis of algebra}
{%
Пусть множество векторов
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\DefText[5]{Let be basis of algebra and C}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module \Cols}{#5}
является базисом и
\ShowEq{structural constants of algebra}ikij,
\ShowEq{kij in I}{#3}i
- структурные константы $#4$\Hyph алгебры \ColsA $#1_i$.%
}

\AddEq [9]{Let be basis of algebra and C}
{%
Пусть множество векторов
\DrawEq[{#1}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом и
\ShowEq{structural constants of algebra}{#2}kij,
\ShowEq{kij in I}{#4}{}
- структурные константы $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в #3 $#4$\Hyph модуле $#5$.
}

\DefText[5]{coordinates of the linear map 1}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса \eV[#3](\Base)
\def\Temp{D}
\ifx\Temp\Base
\DrawEq [{#1}{#3}{}]{va=ae1, module (#5)(\Cols)}{\SideNS-\VectorSet #1 #4}
\else
\DrawEq [{#1}{#3}]{va=ae1, module (#5)(\Cols)}{}
\fi
}

\DefText[5]{coordinates of the linear map 2(1)}
{
\item
\ShowEq{h(a)=...}{#1}{#2}{#3}{#4}
- матрица $#5$\Hyph чисел.
}

\DefText[5]{coordinates of the linear map 2()}
{
}

\DefText[7]{coordinates of the linear map 3}
{
\item $#6$ - координатная матрица $#2_2$\Hyph числа
\DrawEq[#1#6#4]{vb=f(va)}{}%{#1 #7(\Cols)\SideNS-\VectorSetNS}
относительно базиса \eV[#3]
\def\Temp{D}
\ifx\Temp\Base
\DrawEq [{#6}{#3}]{va=ae1, module (#5)(\Cols)}{#6 #7\SideNS-\VectorSetNS}
\else
\DrawEq [{#6}{#3}]{va=ae1, module (#5)(\Cols)}{}
\fi
}

\DefText[6]{coordinates of the linear map 4}
{
\item $#1$ - координатная матрица множества $#2_2$\Hyph чисел
\ShowEq{Vector f(e1) module}#1{#3}#5#6
относительно базиса \eV[#4][.]
}

\DefText[4]{Let be module of}
{
Пусть  $#1_{#2}$ является \SideRu\What $#3_{#4}$\Hyph \VectorSetRuE \ColsNA.
}

\DefText[2]{we identify linear map and matrix}
{
На основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2cols},
\refTheorem{matrix generates D module homomorphism}{cols(#1#2)},
а также на основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2rows},
\refTheorem{matrix generates D module homomorphism}{rows(#1#2)},
мы идентифицируем линейное отображение
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{}
и матрицу $f$ его представления.
}

\DefLabeledFootnote[4]{homomorphism of d algebra}{#1#2\Cols}
{
В теоремах
\refTheorem{homomorphism of d algebra, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of algebra and C}11iID{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}22jJD{#3}A{#4}-
}

\DefLabeledTheorem[5]{homomorphism of d algebra, coordinates}{#1#2\Cols}
{
Гомоморфизм\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\DrawEq[{\Vector f}A]{homomorphism D algebra #1#2}{}
$D_{#1}$\Hyph алгебры \ColsA $A_{#2}$
в $D_{#3}$\Hyph алгебру \ColsA $A_{#4}$ имеет представление
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{algebra(#1#2)}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\DrawEq[hf12]{f o ea=efa (#1#2)(\Cols)}{algebra}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aA1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aA2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fA{#2}{#4}iI
\ShowText{Morphism of D algebra}{#1}{#2}f{}
\end{itemize}
}

%\DefProofRef[4]{homomorphism of d algebra, coordinates}{#1#2\Cols}
\DefProof[4]{homomorphism of d algebra, coordinates}
{
Равенства
\ShowRef{homomorphism of d algebra, coordinates}{#1}{#2}{#4}
являются следствием теорем
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2}.

Равенство
\DrawEq{algebra, homomorphism and product eiej(#1#2)}{\Cols}
является следствием равенств
\ShowRef{algebra, homomorphism and product eiej}{#1}{#2}{#3}
Равенство
\DrawEq{algebra, homomorphism and product eiej 4(#1#2)}{\Cols}
является следствием равенства
\ShowRef{algebra, homomorphism and product eiej 1}{#1}{#2}
и равенства
\eqRef{algebra, homomorphism and product eiej(#1#2)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}
является следствием равенства
\ShowRef{homomorphism, f vw=}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
и равенства
\eqRef{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
является следствием равенств
\eqRef{algebra, homomorphism and product eiej 4(#1#2)}{\Cols},
\eqRef{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}.
Равенство
\ShowRef{algebra, homomorphism and product}{#1}{#2}f
следует из равенства
\eqRef{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefLabeledTheorem[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Линейное отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
$D_{#1}$\Hyph модуля \ColsA $A_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $A_{#4}$ имеет представление
\DrawEq[hf{#2}{#4}{}]{f o ea=efa (#1#2)(\Cols)}{module}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)module}
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{#1#2}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aV1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aV2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fV{#2}{#4}iI
\end{itemize}
}

\DefProofRef[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Так кaк
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
линейное отображение, то равенство
\ShowEq{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
является следствием равенств
\ShowRef{vb=h(e1)a}{#1}{#2}{#5}
$V_2$\Hyph число
\ShowEq{f(e1)(\Cols)\SideNS}
имеет разложение
\DrawEq{f(e1)=(\Cols)\SideNS}{(#1)(#2)}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
и \eqRef{f(e1)=(\Cols)\SideNS}{(#1)(#2)}, мы получаем
\ShowEq{vb=a f e (#1)(#2)(\Cols)\SideNS}
\eqRef{f:V1->V2, D module \Cols}{#1#2}
следует из сравнения
\newline
\FrameEqRef[b2]{va=ae1, module ()(\Cols)}{b (#1)(#2)\SideNS-\VectorSetNS}
\newline
и \EqRef{vb=a f e (#1)(#2)(\Cols)\SideNS} и
теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefDefinitionNote{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnotemark
в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}
{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.
}

\DefText{algebra inherits type of module}
{
$D$\Hyph алгебра $A$ наследует тип $D$\Hyph модуля $A$.
}

\DefLabeledDefinition{type of algebra}{\Cols}
{
$D$\Hyph алгебра $A$ называется
$D$\Hyph алгеброй \ColsNA,
если $D$\Hyph модуль $A$
является $D$\Hyph модулем \ColsNA.
}

\DefLabeledTheorem{associative product in algebra}{\Cols}
{
Если алгебра $A$ коммутативна, то
\DrawEq{commutative product in algebra, 1}{\Cols}
Если алгебра $A$ ассоциативна, то
\DrawEq{associative product in algebra, 1}{\Cols}
}

\DefProof{associative product in algebra}
{
Для коммутативной алгебры,
равенство
\eqRef{commutative product in algebra, 1}{\Cols}
следует из равенства
\ShowEq{commutative product in algebra}
\begin{sloppypar}
\noindent
Для ассоциативной алгебры,
равенство
\eqRef{associative product in algebra, 1}{\Cols}
следует из равенства
\end{sloppypar}
\ShowEq{associative product in algebra}
}

\DefLabeledTheorem{product in algebra}{\Cols}
{
\ShowEq{Let be basis of algebra}{}{}iID{}A{}-
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\DrawEq{product in algebra}{\Cols}
где
\ShowEq{structural constants of algebra symb}
- \AddIndex{структурные константы}{structural constants}
алгебры $A$ над кольцом $D$.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\DrawEq{product of basis vectors, algebra}{\Cols}
}

\DefProofSloppy{product in algebra}
{
Равенство
\eqRef{product of basis vectors, algebra}{\Cols}
является следствием утверждения, что \eV
является базисом $D$\Hyph алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product in algebra, 1}{\Cols}
Из равенств
\eqRef{product of basis vectors, algebra}{\Cols},
\eqRef{product in algebra, 1}{\Cols},
следует
\DrawEq{product in algebra, 2}{\Cols}
Так как \eV является базисом алгебры $A$, то равенство
\eqRef{product in algebra}{\Cols}
следует из равенства
\eqRef{product in algebra, 2}{\Cols}.
}

\DefText{D-module type}
{
Организацию координат вектора в матрице
мы будем называть типом $D$\Hyph модуля.

В этом разделе мы рассмотрим вектор\Hyph столбец
и вектор\Hyph строку.
Очевидно, что существуют и другие формы представления вектора.
Например, мы можем записать координаты вектора в виде
\nmTimes nm матрицы или в виде треугольной матриц.
Формат представления зависит от рассматриваемой задачи.
}

\DefText{D-module type 1}
{
Если утверждение зависит от формата представления вектора,
мы будем указывать либо тип $D$\Hyph модуля,
либо формат представления базиса.
Оба способа указания типа $D$\Hyph модуля эквивалентны.
}

\DefText{Morphism of D algebra, injection 11}
{
(а следовательно,
\ShowEq{Morphism of D algebra, injection}
}

\DefText{Morphism of D algebra, injection 1}
{
}

\DefText[4]{Morphism of D algebra}
{
\item Матрица гомоморфизма
и структурные константы связаны соотношением
\DrawEq[{#3}{}]{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)#4}
}

\DefText{algebra, homomorphism and product 11}
{
Поскольку отображение $h$ является гомоморфизмом колец,
то равенство
\DrawEq{algebra, homomorphism and product, 4}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product eiej(11)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product, 5 11}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{11\Cols}
и равенства
\eqRef{algebra, homomorphism and product, 4}{\Cols}.
}

\DefText{algebra, homomorphism and product 1}
{
Равенство
\DrawEq{algebra, homomorphism and product, 5 1}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{1\Cols}
и равенства
\eqRef{algebra, homomorphism and product eiej(1)}{\Cols}.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinitionNote{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnotemark
\ShowEq{nucleus of algebra}
}
{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13.}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra = A}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra = A}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnotemark
\ShowEq{center of algebra}
}{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14.
}

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Stmt.Omega.Russian.tex <==
%auto-ignore
\input{Stmt.Omega.Eq}

\DefDefinition{polyadditive map}
{
Отображение
\ShowEq{f:A->B}g{A^n}A
называется
\AddIndex{полиаддитивным отображением}{polyadditive map},
если для любого
\ShowEq{fi(a+b)=}
}

\DefTheorem{shifts on group commuting}
{
Правый и левый сдвиги на мультипликативной $\Omega$\Hyph группе $A_1$ перестановочны.
}

\DefProof{shifts on group commuting}
{
Теорема является следствием ассоциативности произведения в мультипликативной $\Omega$\Hyph группе $A_1$
\ShowEq{L(a)oR(b)=}
}

\DefProof{two representations of group}
{
Мы будем пользоваться групповыми координатами для $A_2$\Hyph чисел $a_2$.
Тогда согласно теореме \RefTheorem{single transitive representation of group}
мы можем записать левый сдвиг $L(a_1)$ вместо преобразования $f(a_1)$.

Пусть
\ShowEq{a b in A}2.
Тогда мы можем найти
одно и только одно
\ShowEq{a in A}1{}
такое, что
\ShowEq{b=aRa}
Мы предположим
\ShowEq{ha=Ra}
Существует
\ShowEq{b in A}1{}
такое, что
\ShowEq{c=Lba}
Согласно теореме \RefTheorem{shifts on group commuting} диаграмма
\ShowEq{Diagram: two representations of group}
коммутативна.

Изменяя $b_1$ мы получим, что $c_2$ - это произвольное $A_2$\Hyph число.

Мы видим из диаграммы, что, если $a_2=b_2$, то $c_2=d_2$ и следовательно $h(e)=\delta$.
С другой стороны, если $a_2\neq b_2$, то $c_2\neq d_2$ потому, что
левостороннее $A_1$\Hyph представление $f$ однотранзитивно.
Следовательно правостороннее $A_1$\Hyph представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $c_2$ мы можем найти $a_1$
такое, что
\ShowEq{d2=c2 h}
Следовательно правостороннее $A_1$\Hyph представление $h$ однотранзитивно.

В общем случае, произведение преобразований левостороннего $A_1$\Hyph представления $f$
не коммутативно и следовательно
правосторонним $A_1$\Hyph представление $h$ отлично от левостороннего $A_1$\Hyph представления $f$.
Таким же образом мы можем создать левостороннее $A_1$\Hyph представление $f$,
пользуясь правосторонним $A_1$\Hyph представлением $h$.
}

\DefDefinition{semiring of sets}
{
Непустая система множеств $\mathcal S$ называется
\AddIndex{полукольцом множеств}{semiring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 43.}
если
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\item
\ShowEq{empty in S}
\item
Если
\ShowEq{A, B in S}
то
\ShowEq{AB in S}
\item
Если
\ShowEq{A, A1 in S},
то множество \(A\) может быть представлено в виде 
\DrawEq{A=+Ai}{def}
где
\ShowEq{Ai*Aj=0}
\labelItem{A=+Ai}
\end{enumerate}
Представление
\eqRef{A=+Ai}{def}
множества \(A\) называется
\AddIndex{конечным разложением множества}{finite expansion of set}
\(A\).
}

\DefDefinition{norm on Omega group}
{
\AddIndex{Норма на $\Omega$\Hyph группе}
{norm on Omega group} $A$\,\footnote{
Определение дано согласно определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\ShowEq{d->|d|}
такое, что
\ifx\setCACAA\undefined
\StartLabelItem
\else
\StartLabelItem[definition]
\fi
\begin{enumerate}
\ShowEq{|a|>=0}
\ShowEq{|a|=0}
равносильно $a=0$
\ShowEq{|a+b|<=|a|+|b|}
\ShowEq{|-a|=|a|}
\end{enumerate}

$\Omega$\Hyph группа $A$,
наделённая структурой, определяемой заданием на $A$ нормы, называется
\AddIndex{нормированной $\Omega$\Hyph группой}{normed Omega group}.
}

\DefTheorem{h=f1...fn omega, converges uniformly}
{
Пусть $A$ - полная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция.
Пусть последовательность отображений
\ShowEq{fim M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f_i$.
Пусть множество значений отображения
$f_i$
компактно.
Тогда последовательность отображений
\ShowEq{hm=f1m...fnm omega}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f1...fn omega}{converges uniformly}
}

\DefTheorem{|int h|<int|omega||f1n|}
{
Пусть
\ShowEq{omega in Omega}{}{}
- $n$\Hyph арная операция в
абелевой \(\Omega\)\Hyph группе \(A\).
Пусть
\ShowEq{fi:X->A}
$\mu$\Hyph измеримое отображение
с компактным множеством значений.
Если отображение \(f_i\), \(i=1\), ..., \(n\),
интегрируемо, то отображение
\DrawEq{h=f1...fn omega}{}
интегрируемо и
\DrawEq{|int h|<int|omega||f1n|}{measurable}
}

\DefTheorem{h=fX g1 g2 representation}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
интегрируемое отображение
с компактным множеством значений.
Тогда отображение
\ShowEq{h=fX g1 g2}
интегрируемо и
\DrawEq{|int h|<int|g1||g2|}{measurable}
}

\DefTheorem{polymorphism of representations}
{
Пусть отображение
\ShowEq{map r1n,R}
является полиморфизмом
представлений $f_1$, ..., $f_n$ в представление $f$.
Для любого
\ShowEq{k,1n}
отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
удовлетворяет равенству
\ShowEq{polymorphism of representation, ak}
Пусть $\omega_1\in\Omega_1(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_{1k}$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega1}
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega2}
}

\DefDefinition{polymorphism of representations}
{
Пусть
\ShowEq{A1n A}
- $\Omega_1$\Hyph алгебры.
Пусть
\ShowEq{B1n}
- $\Omega_2$\Hyph алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}{A_k}{B_k}
представление $\Omega_1$\Hyph алгебры $A_k$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{polymorphism of representation}
называется
\AddIndex{полиморфизмом представлений}
{polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если, для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменных
\ShowEq{ak bk in}
имеют заданное значение, отображение
\ShowEq{map r,R}{r_{1k}}{r_2}{}
является морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение
\ShowEq{map r1n,R}
является полиморфизмом представления $f$.
}

\DefDefinition{Omega group}
{
Пусть в $\Omega_1$\Hyph алгебре
$A$ определена операция сложения,
которая не обязательно коммутативна.
Мы пользуемся символом $+$ для обозначения операции суммы.
Положим
\ShowEq{Omega=...-+}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно операции сложения
и любая операция $\omega\in\Omega$
является полиаддитивным отображением,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph группой}{Omega group}.
Если $\Omega$\Hyph группа $A$ является ассоциативной группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной $\Omega$\Hyph группой}{associative Omega group}.
Если $\Omega$\Hyph группа $A$ является абелевой группой
относительно операции сложения,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{абелевой $\Omega$\Hyph группой}{Abelian Omega group}.
}

\DefTheorem{operation is distributive over addition}
{
Пусть
\ShowEq{omega n ari}{}{}n{}
- полиаддитивное отображение.
Операция $\omega$
\AddIndex{дистрибутивна}{distributive law}
относительно сложения
\ShowEq{omega is distributive over addition}
}

\DefDefinition{multiplicative Omega group}
{
Пусть произведение
\DrawEq{c=ab}{}
является операцией $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o}
Если $\Omega_1$\Hyph алгебра $A$ является группой
относительно произведения
и для любой операции
\ShowEq{omega n ari}{}{}n{}
умножение дистрибутивно относительно операция $\omega$
\DrawEq{a omega=omega a left}{}
\DrawEq{a omega=omega a right}{}
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{мультипликативной $\Omega$\Hyph группой}
{multiplicative Omega group}.
}

\DefDefinition{Abelian multiplicative Omega group}
{
Если
\ShowEq{Abelian multiplicative Omega group}
то мультипликативная $\Omega$\Hyph группа называется
\AddIndex{абелевой}{Abelian multiplicative Omega group}.
}

\DefDefinition{Omega ring}
{
Пусть сложение
\ShowEq{c1=a+b}
\ePrints{8428-0408,8525-2526,2207.06506}%
\ifx\Semafor\ValueOff%
которое не обязательно коммутативно,
\fi%
и произведение
\DrawEq{c=ab}{}
являются операциями $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o+}
Если $\Omega_1$\Hyph алгебра $A$ является
\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn
абелевой
\fi
$\Omega\cup\{*\}$\Hyph группой
и
мультипликативной $\Omega\cup\{+\}$\Hyph группой,
то $\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph кольцом}{Omega ring}.
}

\DefTheorem{product in Omega ring is distributive over addition}
{
Произведение в $\Omega$\Hyph кольце
\AddIndex{дистрибутивно}{distributive law}
относительно сложения
\ShowEq{a*(b1+b2)=}
}

\DefProof{product in Omega ring is distributive over addition}
{
Теорема является следствием определений
\RefDefinition{Omega group},
\RefDefinition{multiplicative Omega group},
\RefDefinition{Omega ring}.
}

\DefDefinition{matrix over Omega ring}
{
Пусть $A$ - $\Omega$\Hyph кольцо.
\AddIndex{Матрица}{matrix}
над $\Omega$\Hyph кольцом $A$ - это таблица $A$\Hyph чисел $a^i_j$,
где индекс $i$ - это номер строки
и индекс $j$ - это номер столбца.
}


==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Кортеж отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefRemark{morphism of representations of universal algebra}
{
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{representation}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}.
}

\DefRemark{morphism of representations of universal algebra as map}
{
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем кортеж отображений
\ShowEq{map r12}r{}
мы будем также называть отображением
и пользоваться записью
\ShowEq{f:A->B}rfg
Пусть
\ShowEq{a=a12}
- кортеж $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{r(a)12}
для образа кортежа $A$\Hyph чисел
при морфизме представлений $r$.
}

\DefTheorem{unique morphism of representations of universal algebra}
{
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа
\ShowEq{n=r2(m)}
заданного элемента $m\in A_2$.
}

\DefLabeledFootnote[1]{iso end aut morphism}{#1}
{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}

\DefConvention[2]{A number}
{
Элемент $#1$\Hyph #2 $A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
}

\DefTheorem{map is reduced morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
является приведенным морфизмом представлений тогда и только тогда, когда
\DrawEq{reduced morphism representation =}{definition}
}

\DefDefinition{morphism of representation f}
{
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
}

\DefRemark{notation for morphism of representations}
{
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B_1$, пользуясь буквой по образцу $b\in B_1$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
}

\DefTheorem{Tuple of maps is morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{representation}
}

\DefDefinition{tower of representations}
{
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1\,2},...,f_{n-1\,n})$.
Множество представлений $f_{k\,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(f,A)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Диаграмма $(f,A)$ представлений универсальных алгебр}
{diagram of representations of algebras}
- это такой ориентированный граф, что
\StartLabelItem
\begin{enumerate}
\item
вершина $A_k$, \Kn1, является $\Omega_k$\Hyph алгеброй;
\item
ребро $f_{kl}$ является представлением
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_l$\Hyph алгебре $A_l$;
\end{enumerate}
Мы будем требовать, чтобы этот граф
был связным и не содержал циклов.
Мы будем полагать, что $A_{[0]}$ - это множество начальных вершин графа.
Мы будем полагать, что $A_{[k]}$ - это множество вершин графа,
для которых максимальный путь от начальных вершин равен $k$.
}

\DefRemark{diagram of representations}
{
Так как в разных вершинах графа
может быть одна и таже алгебра,
то мы обозначим
\ShowEq{A=A1n}A{}
множество универсальных алгебр, которые попарно различны.
Из равенства
\ShowEq{A=A(1n)1n}A
следует, что для любого индекса $(i)$
существует по крайней мере один индекс $i$ такой, что
\ShowEq{A(i)=Ai}i.
Если даны два набора множеств
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
и определено отображение
\ShowEq{hi:Ai->Bi}
для некоторого индекса $(i)$,
то также определено отображение
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
для любого индекса $i$ такого, что
\ShowEq{A(i)=Ai}i{}
и в этом случае $h_i=h_{(i)}$.
}

\DefTheorem{diagram of representations}
{
{\bf(}\AddIndex{Индукция по диаграмме представлений}{induction over diagram of representations}{\bf)}.
Пусть теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[0]}$
диаграммы $(f,A)$ представлений универсальных алгебр.
Пусть из утверждения, что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k]}$
диаграммы $(f,A)$ представлений, следует утверждение,
что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k+1]}$
диаграммы $(f,A)$ представлений.
Тогда теорема $\mathcal T$ верна для множества
универсальных алгебр
диаграммы $(f,A)$ представлений.
}

\DefDefinitionNote{commutative diagram of representations}
{
Диаграмма $(f,A)$ представлений универсальных алгебр
называется
\AddIndex{коммутативной}{commutative diagram of representations},
если выполнено следующее условие.
для каждой пары представлений
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
следующее равенство верно\,\footnotemark
\ShowEq{fik fjk = fjk fik}
}
{
Образно говоря,
представления $f_{ik}$ и $f_{jk}$
прозрачны друг для друга.
}

\DefTheoremNote{diagram of representations, define map fik}
{
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Мы можем описать фрагмент\,\footnotemark
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{f:A->End 2 3}
определено равенством
\ShowEq{define map f13}
где
\ShowEq{a in A}i,
\ShowEq{a in A}j.
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то отображение $f_{ijk}$ является свободным представлением
\ShowEq{f:1->*3}
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре
\ShowEq{End Ak}Ak.
}
{
Теорема
\RefTheorem{diagram of representations, define map fik}
утверждает, что преобразования в башне представлений согласованы.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Пусть
$(f,A)$
- диаграмма представлений, где
\ShowEq{A=A1n}A{}
- множество универсальных алгебр.
Пусть
$(B,g)$
- диаграмма представлений, где
\ShowEq{A=A1n}B{}
- множество универсальных алгебр.
Множество отображений
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
называется \AddIndex{морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$}
{morphism from diagram of representations into diagram of representations},
если для любых индексов $(i)$, $(j)$, $i$, $j$ таких, что
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j,
и для каждого представления
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
пара отображений $(h_j\ \ h_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
Для любого представления $f_{ij}$,
\Kn[i]1, \Kn[j]1,
мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть отображение
\ShowEq{f:A->*B}g{B_1}{B_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений.
Мы будем пользоваться записью
\ShowEq{r2a=r2 o a}
для образа $A_2$\Hyph числа $a_2$
при отображении $r_2$.
Тогда мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{representation}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\DefTheorem{proper definition of orbit}
{
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Если
\ShowEq{orbit, proposition}
то
\ShowEq{A1a2=A1b2}
}

\AddEq{definition: orbit of representation}
{
\begin{ShadedDefinition}
\labelDefinition{orbit of \SideNS-side representation}
Пусть $A_1$ является $\Omega$\Hyph группоидом с произведением
\ShowEq{(ab)->ab}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
$\Omega$\Hyph группоида $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2,
мы определим
\AddIndex{орбиту представления}{orbit of representation}
$\Omega$\Hyph группоида $A_1$ как множество
\ShowEq{orbit of \SideNS-side representation}
\end{ShadedDefinition}
}

\AddEq{Let A->*AB2 be representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\AddEq{Let XY be generating sets}
{
Пусть $X$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $Y$ - множество образующих представления
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\DefDefinitionNote{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnotemark,
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}
{
Определение дано согласно \citeBib{Serge Lang},
страница 45.
}

\DefExample{Cartesian product of sets}
{
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
}

\DefTheorem{product of effective representations}
{
В категории
\ShowEq{A1(mA2)}
существует произведение
эффективных представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным представлением $\Omega_1$\Hyph алгебры $A_1$.
}

\DefTheoremNote{structure of subrepresentations}
{
Пусть\,\footnotemark
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}{
Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.
}

\DefFootnote{direct sum of Abelian groups}
{
Определение дано согласно \citeBib{Serge Lang}, страница 55.
}

\DefLabeledDefinition{direct sum of Abelian groups}{\GroupLbl}
{
Копроизведение в категории \GroupType тивных абелевых групп
\ShowEq{category Ab(\GroupLbl)}
называется
\AddIndex{прямой суммой}{direct sum}.\,\RefFootnote{direct sum of Abelian groups}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}

\DefDefinitionNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A[Bi]}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
Универсально отталкивающий объект категории
\ShowEq{category A[Bi]}
\ShowEq{coproduct in category}
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}.\,\footnotemark

Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
}
{
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 46.
}

\DefFootnote{free Abelian group}
{
Смотри также определение в \citeBib{Serge Lang}, страницы 56, 57.
}

\DefLabeledDefinition{free Abelian group}{\GroupLbl}
{
Пусть $S$ - множество и\,\RefFootnote{free Abelian group}
\ShowEq{category AbS(\GroupLbl)}
- категория, объектами которой являются отображения
\ShowEq{f:A->B}fSG
множества $S$ в \GroupType тивные абелевые группы.
Если
\ShowEq{f:A->B}fSG
\ShowEq{f:A->B}{f'}S{G'}
объекты категории
\ShowEq{category AbS(\GroupLbl)},
то морфизм из $f$ в $f'$
- это гомоморфизм групп
\ShowEq{f:A->B}gG{G'}
такой, что диаграмма
\DrawEq{AbS ff'g}{}
коммутативна.
}

\DefFootnote{theorem free Abelian group}
{
Смотри аналогичное утверждение в \citeBib{Serge Lang}, страница 57.
}

\DefLabeledTheorem{free Abelian group}{\GroupLbl}
{
Универсально отталкивающий объект $G$ категории
\ShowEq{category AbS(\GroupLbl)}
существует.\,\RefFootnote{theorem free Abelian group}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{S in G}
\item
Множество $S$ порождает \GroupType вную абелевую группу $G$.
\labelItem{set generates Abelian group (\GroupLbl)}
\end{enumerate}
Абелевая группа $G$ называется
{\bf free Abelian group},
порождённой множеством $S$.
}

\DefProof{free Abelian group}
{
Пусть $G$
- множество отображений
\ShowEq{f:A->B}hSZ
таких, что множество
\ShowEq{x in -> h(x)}{}
конечно.

\begin{ShadedLemma}
Определим на множестве $G$ операцию
\ShowEq{h1h2=}
Множество $G$ является \GroupType тивной абелевой группой.
\end{ShadedLemma}
{\sc Доказательство.}
Пусть
\ShowEq{h12 in G}
Согласно определению, множества
\ShowEq{x in -> h(x)}1
\ShowEq{x in -> h(x)}2
конечны.
Тогда конечно множество
\ShowEq{H1vH2}
Следовательно,
\ShowEq{h1+h2 in G}
Свойства абелевой группы очевидны.
\hfill\(\odot\)

Пусть $k\in Z$, $x\in S$.
Рассмотрим отображение $h=k*x$, определённое равенством
\ShowEq{k*x=k}
Отображение
\ShowEq{f:S->G}
инъективно и позволяет отождествить $S$ и образ $f(S)\subseteq G$
(утверждение
\RefItem{S in G (\GroupLbl)})
и пользоваться записью
\ShowEq{kx=k*x(\GroupLbl)}
Согласно определению множества $G$,
любое отображение $h\in G$ может быть записано в виде
\ShowEq{h=k*x(\GroupLbl)}
где
\ShowEq{k in Z x in S}
и множество
\ShowEq{|kx ne 0|}
конечно.
Утверждение
\RefItem{set generates Abelian group (\GroupLbl)}
является следствием теоремы
\refTheorem{structure of Abelian group}{\GroupLbl}.

\begin{ShadedLemma}
{\it
Представление
\EqRef{h=k*x(\GroupLbl)}
отображения $h$ единственно.
}
\end{ShadedLemma}
{\sc Доказательство.}
Если отображение $h$ допускает представления
\ShowEq{h=k12*x i(\GroupLbl)}
то равенство
\ShowEq{k1-k2 *x(\GroupLbl)}
является следствием равенства
\EqRef{h=k12*x i(\GroupLbl)}.
\ShowEq{k1=k2 i}
следует из равенства
\EqRef{k1-k2 *x(\GroupLbl)}.
\hfill\(\odot\)

Пусть
\ShowEq{f:A->B}{f'}S{G'}
отображение множества $S$ в абелевую группу $G'$.
Мы определим гомоморфизм
\ShowEq{f:A->B}gG{G'}
таким образом, чтобы диаграмма
\DrawEq{AbS ff'g}{\GroupLbl}
была коммутативной.
Из диаграммы
\eqRef{AbS ff'g}{\GroupLbl}
следует, что
\DrawEq{g(1x)=f'(x)}{\GroupLbl}
Согласно теореме
\refTheorem{homomorphism f(na)=nf(a)}{\GroupLbl},
так как отображение $g$ - гомоморфизм абелевой группы, то равенство
\ShowEq{g(x)=(\GroupLbl)}
для любого отображения $h\in G$
является следствием равенств
\eqRef{g(1x)=f'(x)}{\GroupLbl},
\EqRef{h=k*x(\GroupLbl)}.
Следовательно, гомоморфизм $g$ определён однозначно.
Согласно определениям
\RefDefinition{universally repelling object of category},
\refDefinition{free Abelian group}{\GroupLbl},
абелевая группа $G$ является свободной группой.
}

\DefLabeledTheorem{homomorphism f(na)=nf(a)}{\GroupLbl}
{
Гомоморфизм
\ShowEq{f:A->B}fG{G'}
удовлетворяет равенству
\ShowEq{f(na)=nf(a) (\GroupLbl)}
}

\DefTheoremNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{coproduct in category}
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category},\,\footnotemark
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 46.}

\DefProof{coproduct in category}
{
Теорема является следствием определений
\RefDefinition{universally repelling object of category},
\RefDefinition{coproduct in category}.
}

\DefFootnote{Theorem direct sum of Abelian groups}
{
Смотри также предложение \citeBib{Serge Lang}-10, страница 55.
}

\DefLabeledTheorem{direct sum of Abelian groups}{\GroupLbl}
{
Пусть
\ShowEq{set Bi}A
- семейство \GroupType тивных абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A}
Тогда\,\RefFootnote{Theorem direct sum of Abelian groups}
\ShowEq{A=o+Ai}A
}

\DefProof{direct sum of Abelian groups}
{
Согласно теореме
\RefTheorem[\RefRepresentation]{product exists in category of Omega algebras},
существует абелевая группа $B=\prod A_i$.
Согласно утверждению
\RefItem[\RefRepresentation]{tuple represent A number},
мы можем представить $B$\Hyph число $a$ в виде кортежа
\ShowEq{set Bi}a
$A_i$\Hyph чисел.
Согласно утверждению
\RefItem[\RefRepresentation]{operation is defined componentwise},
\GroupOpName в группе $B$ определен\OpEndS равенством
\DrawEq{(ai)+(bi)=(ai+bi)}{\GroupLbl}

Согласно построению
$A$ является подгруппой абелевой группы $B$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\DrawEq{lj(x)=0x0}{\GroupLbl}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}\GroupLbl
семейство гомоморфизмов в \GroupType тивную абелевую группу $C$.
Мы определим отображение
\ShowEq{f:A->B}fAC
пользуясь равенством
\ShowEq{fxi,i=sum fxi(\GroupLbl)}
\GroupOpNameC в правой части равенства
\EqRef{fxi,i=sum fxi(\GroupLbl)}
конечн\OpEnd, так как все \ArgsOfOp, кроме конечного числа, равны $\UnitId$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\EqRef{fxi,i=sum fxi(\GroupLbl)}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\EqRef{fxi,i=sum fxi(\GroupLbl)}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{\GroupLbl}.
}

\AddEq{remark: Non-commutative Sum}
{
С детства мы знаем, что от перестановки мест слагаемых сумма не меняется.
Поэтому, когда услышал о некоммутативном сложении
(\citeBib{Alain Connes 1994}),
я слегка растерялся.
Однако мне недавно повезло встретить геометрию, где сумма векторов некоммутативна.

В школе я увлекался многими вещами: физикой, химией, черчением.
Математика была немного в стороне.
Я не любил арифметику, но мне нравились алгебра и геометрия.
Я тогда ещё не знал, что все пути ведут в математику.

Черчение было моим любим предметом. Мой учитель,
Габис Сергей Александрович, подарил мне сборник задач по черчению,
и я добросовестно все их перерешал.
А потом придумал свою собственную задачу и решил её.
К моему удивлению, первая теорема, которую мы доказывали на
уроке геометрии на следующий год, была именно решением этой задачи.

Я понимал, что после школы мне будет сложно поступить в институт.
Поэтому после восьмого класса я решил что я буду поступать в техникум.
Бела Марковна предложила позаниматься со мной летом,
посмотреть насколько я готов к экзамену по математике.
Один из уроков остался в моей памяти.
Когда мы рассматривали графики прямой и параболы,
Бела Марковна сказала: нарисовать прямую или параболу легко,
а как быть с кардиограммой?
И я загорелся идеей найти аналитическое выражение 
для кардиограммы.

Мой товарищ предложил мне на протяжении лета
вместе изучать математический анализ.
В нашем доме жили мальчики, которые учились в техникуме,
и они одолжили мне свой учебник по математическому анализу.
К этому времени мой товарищ потерял интерес к своей идее,
и я стал изучать математический анализ самостоятельно.

Первая глава учебника была посвящена аналитической геометрии.
И я понял, что это то что мне нужно для анализа кривых кардиограммы.
Аналитическая геометрия решила моё будущее.
Я понял, что буду готовиться в университет на механико-математический факультет.

Я перечитал много книг по математическому анализу.
Но в какой-то момент у меня сложилось впечатление
что один автор списывает у другого.
Я стал искать другие книги.
Не помню откуда у меня появился первый том Фихтенгольца.
Но эта книга произвела на меня неизгладимое впечатление.
Ближе к весне я почувствовал, что книга становится трудной,
но продолжал читать.
В марте у меня был грипп с необычайно высокой температурой.
Но я сомневаюсь, что это был грипп,
так как после этого первый том Фихтенгольца стал для меня понятен.

Изучение математического анализа отразилось
на моих попытках восстановить функциональную
зависимость с графика. Я тогда ещё не понимал,
что не всякое отображение может быть представлено аналитически.
Я рисовал графики, составлял таблицы приращения функции
в зависимости от приращения аргумента.
Но вскоре эта затея мне надоела,
и я сменил занятие.

Когда мне в руки попала книга по тензорному исчислению,
я обнаружил, что сложные построения аналитической геометрии
по классификации кривых второго порядка
можно заменить простыми теоремами линейной алгебры.
После этого, мой интерес к аналитической геометрии
заметно стал меньше.

Прошло почти полвека.
И неожиданно аналитическая геометрия преподнесла мне
два приятных сюрприза.
Сперва я обнаружил, что аналитическая геометрия
является интересной структурой с точки зрения
теории представлений универсальных алгебр.
Точнее, я отождествляю аналитическую и аффинную геометрии,
но я думаю, что это небольшая ошибка.

Второй сюрприз связан с тем, что я понял,
что я могу построить модель аффинной геометрии
в римановом пространстве.
Так как я очень долго занимался метрико\Hyph аффинными многообразиями,
то оставался один шаг, чтобы увидеть модель аффинной геометрии,
где сумма некоммутативна.
С этого момента некоммутативное сложение перестало быть для меня
абстрактной концепцией.
}

\DefText{side representation of group}
{
Из равенства
\eqRef{* \SideNS-side representation of group}{def}
следует, что
\DrawEq{o \SideNS-side representation of group}{def}
Мы можем рассматривать равенство
\eqRef{o \SideNS-side representation of group}{def}
как
\AddIndex{закон ассоциативности}{associative law},

\begin{sloppypar}
\begin{example}
Пусть
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
эндоморфизмы $\Omega_2$\Hyph алгебры $A_2$.
Пусть произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
является композицией эндоморфизмов.
Так как произведение отображений $f$ и $g$ определено в том же порядке,
как эти отображения действуют на $A_2$\Hyph число,
то мы можем рассматривать равенство
\ShowEq{fga= o \SideNS}
как
закон ассоциативности,
который позволяет записывать равенство
\EqRef{fga= o \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}
а также записать равенство
\eqRef{\SideNS-side representation of group}{def}
в виде
\DrawEq{\SideNS-side 1 representation of group}{def}
\qed
\end{example}
\end{sloppypar}
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{ShadedTheorem}
\labelTheorem{select second basis of representation, #4}
Пусть $#2$ - пассивное преобразование
многообразия базисов #3 $#4$.
Пусть $\Basis e_1$ - базис #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
Пусть для базиса $\Basis e_3$ существует активное преобразование $#1$ такое, что
\ShowEq{e3=R o e1}{#1}31
Положим
\ShowEq{e3=R o e1}{#1}42
Тогда
\ShowEq{e2=e1 o S}{#2}43
\end{ShadedTheorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#3},
активное преобразование координат базиса $\Basis e_3$ имеет вид
\DrawEq{active transformation, 1}{#3}
Пусть
\ShowEq{e2=e1 o S}{#2}53
Из равенства
\eqRef{passive transformation}{#3}
следует, что
\DrawEq{passive transformation, 1}{#3}
Из совпадения выражений в равенствах
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3}
следует, что
\ShowEq{Basis e4=Basis e5}
Следовательно,
коммутативна диаграмма
\ShowEq{passive and active maps}{#1}{#2}
\end{proof}
}

\AddEq[2]{definition: basis manifold}
{
Множество
\ShowEq{basis manifold}
базисов #1 $#2$ называется
\AddIndex{многообразием базисов}{basis manifold}
#1 $#2$.
}

\AddEq{ref active representation, representation}
{
Согласно теоремам
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
Согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
и определению
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{ShadedDefinition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
автоморфизм $#4$ #2 $#3$
порождает преобразование
\DrawEq[{#4}]{active transformation}{#1}
многообразия базисов #2.
Это преобразование называется
\AddIndex{активным}{active transformation of basis}.
Согласно теореме
\RefTheorem{group of automorphisms of #1},
определено левостороннее представление
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $A(f)$ называется
\AddIndex{активным представлением}{active representation in basis manifold}.
Согласно следствию
\RefCorollary{automorphism uniquely defined by image of basis, #1},
это представление однотранзитивно.
\qed
\end{ShadedDefinition}
}

\AddEq[4]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
Согласно замечанию
\RefRemark{X is quasibasis of #1},
могут существовать базисы #2 $#3$,
не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, #4 $#3$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\end{remark}
}

\AddEq[6]{theorem: Coordinate transformation does not depend}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Допустим пассивное преобразование $#2\in GA(f)$ отображает
базис $\Basis e_1\in\mathcal{B}[f]$
в базис $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Допустим #6 $#3$ имеет #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
относительно базиса $\Basis e_1$ и имеет #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
относительно базиса $\Basis e_2$.
Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
не зависит от #4 $#3$ или базиса $\Basis e_1$, а
определенно исключительно координатами #4 $#3$
относительно базиса $\Basis e_1$.
\end{ShadedTheorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
Из \eqRef{passive transformation S}{#1}
и
\eqRef{Omega_2 word, basis e}{2 #1}
следует, что
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Сравнивая \eqRef{Omega_2 word, basis e}{1 #1}
и
\eqRef{Omega word in representation, basis Y, 1}{#1}
получаем, что
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Так как $#2$ - автоморфизм представления, то равенство
\eqRef{coordinate transformation}{#1}
следует из
\eqRef{coordinate transformation in representation, 1}{#1}
и теоремы
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[3]{remark: active and passive transformation}
{
Активное преобразование изменяет базис #1 и
#2 согласовано
и координаты #3 относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат #3 относительно базиса.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Преобразования координат
\eqRef{coordinate transformation}{#1}
порождают эффективное контравариантное
правостороннее представление группы $GA(f)$, называемое
\AddIndex{координатным представлением}{coordinate representation}
в #2.
\end{ShadedTheorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
Согласно следствию
\RefCorollary{map of coordinates of #1},
преобразование
\eqRef{coordinate transformation}{#1}
является эндоморфизмом #4\,\footnote{Это преобразование
не порождает эндоморфизма #4 $#6$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако
#7, координаты которого мы рассматриваем, не меняется.}
#5

Допустим мы имеем два последовательных пассивных преобразования
$#2$ и $#8$. Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
соответствует пассивному преобразованию $#2$.
Преобразование координат
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
соответствует пассивному преобразованию $#8$.
Согласно теореме
\RefTheorem{passive representation in basis manifold, #1},
произведение преобразований координат
\eqRef{coordinate transformation}{#2 #1}
и
\eqRef{coordinate transformation}{#8 #1}
имеет вид
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
Согласно теоремам
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
и определению
\RefDefinition{Left side contravariant representation}
преобразования координат
порождают
правостороннее контравариантное представление группы $GA(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $GA(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Пассивное представление $P(g)$ согласовано
с пассивным представлением $P(f)$,
если существует гомоморфизм $h$ группы $GA(f)$ в группу $GA(g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $GA(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $#2$ многообразии базисов $\mathcal B(f)$
соответствует пассивное преобразование $H(#2)$ многообразия базисов $\mathcal B(g)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Тогда координатное преобразование в #3 $#4$ принимает вид
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{coordinate of geometric object, #1}
Мы будем называть
орбиту
\ShowEq{coordinates of geometric object}{#3}%
\ShowEq{show coordinates of geometric object}{#2}{#3}
\AddIndex{координатами геометрического объекта}{coordinates of geometric object},
определёнными в #4 $#5$.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка
\eqRef{coordinate transformation g}{#1}
орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object}
относительно базиса
\ShowEq{geometric object 2}
\qed
\end{ShadedDefinition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение
\RefDefinition{coordinate of geometric object, #1}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object, #1} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\AddEq[7]{definition: geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
\AddIndex{геометрическим объектом}{geometric object},
определённым в #4 $#5$.
Мы будем также говорить, что $#3$ - это
\AddIndex{геометрический объект типа $H$}{type of geometric object}.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка 
\eqRef{coordinate transformation g}{#1}
орбиты  определяет #6
\ShowEq{geometric object 2, g}{#3}%
#7 мы называем
\AddIndex{представителем геометрического объекта}{representative of geometric object}
в #4 $#5$.
\qed
\end{ShadedDefinition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{ShadedTheorem}[принцип инвариантности]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e_f$.
\end{ShadedTheorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_f$ #2 $#3$,
базис $\Basis e_g$ #2 $#4$
и координаты геометрического объекта
\ShowEq{invariance principle 4}{#5}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}{#5}
Базис $\Basis e_{f1}$ связан с базисом
$\Basis e_f$ пассивным преобразованием
\ShowEq{invariance principle 2 passive}{#6}
Согласно построению это порождает пассивное преобразование
\eqRef{passive transformation of representation g}{#1}
и координатное преобразование
\eqRef{coordinate transformation g}{#1}.
Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3 algebra}{#5}{#6}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{ShadedTheorem}
\labelTheorem{passive representation in basis manifold, #1}
Существует однотранзитивное правостороннее представление
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $P(f)$ называется
\AddIndex{пассивным представлением}{passive representation in basis manifold}.
\end{ShadedTheorem}
}

\DefProof{passive representation in basis manifold}
{
Поскольку $A(f)$ - однотранзитивное левостороннее представление группы $GA(f)$,
то однотранзитивное правостороннее представление $P(f)$
определено однозначно
согласно теореме
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Пассивное преобразование многообразия базисов
является автоморфизмом представления $A(f)$.
\end{ShadedTheorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
Теорема является следствием теоремы
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation, #1}
Преобразование представления $P(f)$
называется
\AddIndex{пассивным преобразованием многообразия базисов}
{passive transformation of basis}
#2.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
для обозначения образа базиса $\Basis e$ при пассивном преобразовании $#3$.
Пассивное преобразование базиса имеет вид
\DrawEq[#3]{passive transformation}{#1}
\end{ShadedTheorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#1},
активное преобразование действует на координаты
базиса слева.
Равенство
\eqRef{passive transformation}{diagram of representations}
следует из теорем
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism},
согласно которым
пассивное преобразование действует на координаты
базиса справа.
\end{proof}
}

\DefLabeledDefinitionNote{side representation of group}{\SideNS}
{
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением\,\footnotemark
\ShowEq{(fg)->fg}
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва.
Мы будем пользоваться записью
\ShowEq{f(a)=o \SideNS}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{(ab)->ab}
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
Мы будем отождествлять
$A_1$\Hyph число $a_1$ с его образом $f(a_1)$
и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{\SideNS-side representation}
В этом случае равенство
\eqRef{\SideNS-side representation of group}{def}
принимает вид
\DrawEq{* \SideNS-side representation of group}{def}
Отображение
\ShowEq{A12->A2 1 \SideNS}
порождённое \SideRu восторонним представлением $f$, называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа $a_2$ на $A_1$\Hyph число $a_1$.
}
{
Очень часто произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
совпадает с суперпозицией эндоморфизмов
\ShowEq{Act=circ}
Однако произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
может отличаться от суперпозиции эндоморфизмов.
}

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefLabeledDefinition{action of rational integers in Abelian group}{\GroupLbl}
{
Мы определим действие кольца целых чисел $Z$
в \GroupType тивной абелевой группе $G$
согласно правилу
\ShowEq{action of rational integers in Abelian group (\GroupLbl)}
}

\DefLabeledTheorem{action of ring of rational integers in Abelian group}{\GroupLbl}
{
Действие кольца целых чисел $Z$
в \GroupType тивной абелевой группе $G$,
рассмотренное в определении
\refDefinition{action of rational integers in Abelian group}{\GroupLbl},
является представлением.
Верны следующие равенства
\ShowEq{representation of Z in G (\GroupLbl)}
}

\DefProof{action of ring of rational integers in Abelian group}
{
Равенство
\EqRef{1a=a (\GroupLbl)}
является следствием равенства
\EqRef{0g=0 (\GroupLbl)}
и равенства
\EqRef{(n+1)g= (\GroupLbl)},
когда $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

Равенство
\ShowEq{(k+n)a-na=ka (\GroupLbl)}
является следствием равенства
\EqRef{(m+n)a=ma+na (\GroupLbl)}.
Равенство
\EqRef{(m-n)a=ma-na (\GroupLbl)}
является следствием равенства
\EqRef{(k+n)a-na=ka (\GroupLbl)},
если мы положим
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

Из равенства
\EqRef{n(a+b)=na+nb (\GroupLbl)}
следует, что отображение
\ShowEq{phi(n):G->G (\GroupLbl)}
является эндоморфизмом абелевой группы $G$.
Из равенств
\EqRef{(m+n)a=ma+na (\GroupLbl)},
\EqRef{(nm)a=n(ma) (\GroupLbl)}
следует, что отображение
\ShowEq{phi:Z->End(G)}
является гомоморфизмом кольца $Z$.
Согласно определению
\RefDefinition[\RefRepresentation]{representation of algebra},
отображение $\varphi$ является представлением
кольца целых чисел $Z$
в абелевой группе $G$.
}

\DefDefinitionNote{tensor product of representations}
{
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.\,\footnotemark
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\ShowEq{a1n}An.
}
{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{ShadedTheorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{ShadedTheorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{ShadedTheorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{ShadedTheorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinitionNote{free representation of algebra}
{
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
}
{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Смотри также теорему
\RefTheorem{free representation of group}.
\fi
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{ShadedDefinition}
}
{definition: norm of operation}
%\DefEq

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\ShowEq{ref definition: left-side representation of algebra}{}
представления универсальной алгебры.
Согласно определению
\xRef[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{ShadedDefinition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\ShowEq{a in U}{}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{ShadedDefinition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{ShadedDefinition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}cA,
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\DefLabeledDefinition{limit of sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
}

\AddEq{theorem: limit of sequence}
{
\begin{ShadedTheorem}
\labelTheorem{limit of sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{ShadedTheorem}
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{limit of sequence}{normed \Algebrac}.
}

\DefLabeledDefinition{fundamental sequence}{normed \Algebrac}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
}

\AddEq{theorem: fundamental sequence}
{
\begin{ShadedTheorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{ShadedTheorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{fundamental sequence}{normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{ShadedDefinition}
}
{definition: complete Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{ShadedDefinition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{ShadedDefinition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefTheorem{sequence converges uniformly, fn-fm}
{
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
}

\DefDefinition{quasibasis of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
и
\ShowEq{Gen f =}
Если для множества $X\subset A_2$ верно
\ShowEq{in Gen}Xf,
то для любого множества $Y$, $X\subset Y\subset A_2$,
также верно
\ShowEq{in Gen}Yf.
Если существует минимальное множество
\ShowEq{in Gen}Xf,
то множество $X$ называется
\AddIndex{квазибазисом}{quasibasis}
представления $f$.
}

\DefTheorem{X is quasibasis of representation}
{
Если множество $X$ является квазибазисом представления $f$,
то для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
}

\DefRemark{X is quasibasis of representation}
{
Доказательство теоремы
\RefTheorem{X is quasibasis of representation}
даёт нам эффективный метод построения квазибазиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить квазибазис этого представления.
}

\AddEq{remark: representation in form of Omega2-word is ambiguous}
{
Мы ввели $\Omega_2$\Hyph слово элемента $x\in A_2$ относительно множества образующих $X$
в определении
\RefDefinition{word of element relative to set, representation}.
Из теоремы
\RefTheorem{X is quasibasis of representation}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_2$ в виде $\Omega_2$\Hyph слова неоднозначно.
}

\DefDefinitionNote{word of element relative to set, representation}
{
Пусть $X\subset A_2$.
Для любого
\ShowEq{x in JX}m{}
существует
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation},
определённое согласно следующему правилам.
\StartLabelItem
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
\ShowEq{a in A1},
то $f(a)(m)$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
Мы будем отождествлять элемент
\ShowEq{x in JX}m{}
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}{}
рассмотрим множество $\Omega_2$\Hyph слов\,\footnotemark
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J[f,X]$}
{word set of representation}.
}{
Выражение $\wXm$
является частным случаем
выражения $\wXm[B]$, а именно
\ShowEq{subset of words of representation, 2}
}

\DefRemark{three reasons of ambiguity in Omega2-word}
{
Существует три источника неоднозначности в записи
$\Omega_2$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_i$\Hyph алгебре $A_i$, $i=1$, $2$,
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_i$,
то верно равенство
\[ae=a\]
для любого $a\in A_i$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_2$\Hyph слова
может быть связана со свойствами представления.
Например, если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и
\ShowEq{a in A1},
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
В тоже время, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A_1$ и операцией
$\Omega_2$\Hyph алгебры $A_2$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $A_2$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
сохраняются при морфизме представления.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_2$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\refTheorem[\RefRepresentation]{linear dependence between vectors of basis}{\SideWS module},
\refTheorem[\RefRepresentation]{coordinates of vector with linear dependence}{\SideWS module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_2$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_2$\Hyph слов, которое
сохраняется при морфизме представления.
}

\DefTheoremNote{equivalence generated by basis}
{
Пусть $X$ - квазибазис представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Для любого множества образующих $X$ представления $f$
существует отношение эквивалентности
\ShowEq{l fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
Если в $\Omega_2$\Hyph алгебре $A_2$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_2$\Hyph алгебры, то
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если в $\Omega_1$\Hyph алгебре $A_1$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_1$\Hyph алгебры, то
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Для любой операции
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Для любой операции
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Пусть
\ShowEq{omega in O1AO2}12.
Если представление $f$ удовлетворяет равенству\,\footnotemark
\ShowEq{f(a1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
}
{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}

\DefDefinition{basis of representation}
{
Квазибазис $\Basis e$ представления $f$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом представления}{basis of representation} $f$.
}

\DefDefinition{equivalence on the set of Omega2-words}
{
Множество образующих $X$ представления $f$
порождает отношение эквивалентности
\ShowEq{rho fX=}
на множестве $\Omega_2$\Hyph слов.
}

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\DefConvention{Einstein summation}
{
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
}

\DefText{in this section G is group}
{
В этом разделе $G$ - \GroupType тивная абелевая группа.
}

\DefLabeledTheorem{structure of Abelian group}{\GroupLbl}
{
Множество $G$\Hyph чисел, порождённое множеством
\ShowEq{S=si},
имеет вид
\ShowEq{J(S)=gi si (\GroupLbl)}
где множество
\ShowEq{|gi ne 0|}g
конечно.
}

\DefProof{structure of Abelian group}
{
Мы докажем теорему по индукции, опираясь на теоремы
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, страница 94, и
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного $\aD sk\in S$,
положим
\ShowEq{gi=dik}
Тогда
\ShowEq{sk=sum si (\GroupLbl)}
\ShowEq{sk in JS}
следует из
\EqRef{J(S)=gi si (\GroupLbl)},
\EqRef{sk=sum si (\GroupLbl)}.

Пусть
\ShowEq{w12 in Jv}gS
Так как $G$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv (\GroupLbl)}gS
Согласно равенству
\EqRef{J(S)=gi si (\GroupLbl)},
существуют $Z$\Hyph числа
\ShowEq{gi12}g
такие, что
\DrawEq[g]{w12= (\GroupLbl)}{group}
где множества
\DrawEq[g]{|ci12 ne 0|}{group(\GroupLbl)}
конечны.
Из равенства
\eqRef{w12= (\GroupLbl)}{group}
следует, что
\DrawEq[g]{w1+w2= (\GroupLbl)}{group}
Равенство
\DrawEq[g]{w1+w2= 1 (\GroupLbl)}{group}
является следствием равенств
\EqRef{(m+n)a=ma+na (\GroupLbl)},
\eqRef{w1+w2= (\GroupLbl)}{group}.
Из равенства
\eqRef{|ci12 ne 0|}{group(\GroupLbl)}
следует, что
множество
\ShowEq{|gi 1+2 ne 0| (\GroupLbl)}g
конечно.
Из равенства
\eqRef{w1+w2= 1 (\GroupLbl)}{group}
следует, что
\ShowEq{w1+w2 in Jv (\GroupLbl)}gS
}

\DefConvention{Einstein summation convention ()}
{
Мы будем пользоваться соглашением о произведении,
в котором повторяющийся индекс (один в основании и один в экспоненте)
подразумевает произведение по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса произведения и знак произведения опускается
\ShowEq{av=prod av}gs
}

\DefConvention{Einstein summation convention (+)}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}gs
}

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0  (\GroupLbl)}
следует, что равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempC{product Z bilinear 1}
\def\TempD{product Z bilinear 2}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k (\GroupLbl)}
Равенство
\ShowEq{#1,n=k+1 (\GroupLbl)}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(m+n)a=ma+na (\GroupLbl)}.
\else
\ifx\TempC\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(a+b)c=distributive}.
\else
\ifx\TempD\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{a(b+c)=distributive}.
\else
равенства
\EqRef{(n+1)g= (\GroupLbl)}.
\fi
\fi
\fi
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na (\GroupLbl)}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k (\GroupLbl)}
Равенство
\ShowEq{#1,n=k-1 (\GroupLbl)}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g= (\GroupLbl)},
\EqRef{(m-n)a=ma-na (\GroupLbl)}.
\else
\ifx\TempC\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(a+b)c=distributive}.
\else
\ifx\TempD\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{a(b+c)=distributive}.
\else
равенства
\EqRef{(n-1)g= (\GroupLbl)}.
\fi
\fi
\fi
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefProofRef{cr transpose}{}
{
Мы можем доказать \eqRef{cr transpose}{Theorem} в случае матриц тем же
образом, что мы
доказали \eqRef{rc transpose}{Theorem}. Тем не менее для нас более
важно показать, что \eqRef{cr transpose}{Theorem}
следует непосредственно из \eqRef{rc transpose}{Theorem}.

Применяя \EqRef{double transpose} к каждому слагаемому в левой части
\eqRef{cr transpose}{Theorem}, мы получим
\ShowEq{cr transpose, 1}
Из \EqRef{cr transpose, 1} и \eqRef{rc transpose}{Theorem}
следует, что
\ShowEq{cr transpose, 2}
\eqRef{cr transpose}{Theorem} следует из \EqRef{cr transpose, 2}
и \EqRef{double transpose}.
}

\DefProofRef{rc transpose}{}
{
Цепочка равенств
\ShowEq{rc transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \eqRef{rc transpose}{Theorem} следует из
\EqRef{rc transpose, 1}.
}

\DefText{matrix operations 1}
{
Согласно традиции произведение
матриц $a$ и $b$ определено как произведение
строк матрицы $a$ и столбцов матрицы $b$.
\ePrints{1908.04418,6860-2955,2020.06.01,2204.06320,2022.01.05}
\Items{8428-0408,8525-2526,2207.06506}%
\ifx\Semafor\ValueOn
В некоммутативной алгебре этой операции умножения
недостаточно для решения некоторых задач.
\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOff
\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

Из примеров
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space}
\else
\TwoColText
{
\ShowEq{def left}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}
{
\ShowEq{def right}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}

Из примеров
\refExample{matrix in vector space}{left},
\refExample{matrix in vector space}{right}
\fi
следует, что
\else
Если произведение в
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
$D$\Hyph алгебре
\else
$\Omega$\Hyph кольце
\fi
некоммутативно,
\fi
мы не можем ограничиться традиционным произведением матриц
и нам нужно определить два вида произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.
}

\DefText{matrix operations 2}
{
Мы так же определим следующие операции на множестве матриц.
}

\DefExample{matrix in left vector space}
{
Мы представим базис $\Basis e$
левого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def left}%
\ShowEq{def AVector}%
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{left basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e left-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{left basis}
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
левого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=vf}
Равенство
\EqRef{v'=vf}
не может быть выражено как традиционное произведение матриц $v$ и $f$.
\fi
}

\AddEq{define basis for example}
{
Мы представим множество векторов
\ShowEq{\RowN() 1n}en{}
базиса $\Basis e$
\SideRu вого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowRef{\SideWS module over algebra}
и теорему
\refTheorem{basis over division algebra}{left})
в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideWS basis}
Мы представим координаты
\ShowEq{\ColNS() 1n}vn{}
вектора
\ShowEq{w=w*e left-cols}v{}
в виде \ColA матрицы
\DrawEq[vn]{a=(a1.n \ColNS)}{vn \SideNS-\Cols}
}

\AddEq{vector as matrix product left}
{
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
}

\AddEq{vector as matrix product right}
{
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
}

\DefLabeledExample{matrix in vector space}{\SideNS}
{
\ShowEq{define basis for example}
\ShowEq{vector as matrix product \SideNS}
}

\DefExample{matrix in right vector space}
{
Мы представим базис $\Basis e$
правого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def right}%
\ShowEq{def AVector}%
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{right})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{right basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e right-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{right basis}
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
правого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=fv}
Равенство
\EqRef{v'=fv}
выражает традиционное произведение матриц $f$ и $v$.
\fi
}

\DefDefinition{row over column product}
{
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC произведение может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.
}

\DefDefinition{column over row product}
{
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR произведение может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.
}

\DefDefinition{transpose of matrix}
{
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
}

\DefDefinition{rc power}
{
Мы определим \AddIndex{\RC степень}{rc power}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$,
пользуясь рекурсивным правилом
\ShowEq{rc power}
\DrawEq{rc power, 0}1
\DrawEq{rc-power, n}1
}

\DefDefinition{cr power}
{
Мы определим \AddIndex{\CR степень}{cr power}
$\mathcal{A}$\Hyph числа $a$,
пользуясь рекурсивным правилом
\ShowEq{cr power}
\DrawEq{cr power, 0}1
\DrawEq{cr-power, n}1
}

\DefDefinitionNote{Hadamard inverse of matrix}
{
Пусть
\DrawEq[ann]{a=(a11.nm matrix)}{}
матрица $A$\Hyph чисел.
Мы называем матрицу\,\footnotemark
\ShowEq{Hadamard inverse of matrix}
\ShowEq{Hadamard inverse of matrix 2}
\ShowEq{Hadamard inverse of matrix 2 entry}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix} $a$
(\citeBib{q-alg-9705026}-\href{https://arxiv.org/pdf/math/9705026.pdf\#Page=4}{page 4}).
}{
Запись в равенстве
\EqRef{Hadamard inverse of matrix 2 entry}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать правую часть равенства
\EqRef{Hadamard inverse of matrix 2 entry}
следующим образом
\ShowEq{Hadamard inverse of matrix 3}
}

\DefDefinition{transformation coordinated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}{}
следует
\ShowEq{fm1 fm2 modS}.
}

\DefTheorem{transformation correlated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование
\ShowEq{f in End A2},
согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве
\ShowEq{End A2/S}S.
}

\DefTheorem{decompositions of morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
}

\DefDefinition{stable set of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
}

\DefTheorem{subrepresentation of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением}{subrepresentation}
представления $f$.
}

\DefTheoremNote{lattice of subrepresentations}
{
Множество\,\footnotemark
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
}{
Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94).
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn%
Вообще говоря, в этой и последующих теоремах 
этой главы необходимо рассмотреть структуру универсальных алгебр
$A_1$ и $A_2$.
Так как основная задача этой главы -
это изучение структуры представления,
я сознательно упростил теоремы, чтобы детали не заслоняли
основные утверждения.
Более подробно эта тема будет раскрыта в главе
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
где теоремы будут сформулированы в общем виде.
\fi
}

\AddEq{remark: closure operator, representation}
{
Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.
}

\DefDefinition{generating set of representation}
{
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением}{subrepresentation},
порождённым множеством $X$,
а $X$ -
множеством образующих
подпредставления $J[f,X]$.
В частности,
\AddIndex{множеством образующих}{generating set}
представления $f$
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
}

\DefTheoremNote{map of words of representation}
{
\ShowEq{Let A->*AB2 be representations}
Пусть $X$ - множество образующих представления $f$.
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления\,\footnotemark
и $X'=R(X)$.
Приведенный морфизм $R$ представления
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
}{
Я рассмотрел морфизм представления в теореме
\RefTheorem[\RefRepresentation]{map of words of diagram of representations}.
}

\DefTheorem{Representation is single transitive iff}
{
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$.
}

\DefProof{Representation is single transitive iff}
{
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
}

\DefTheorem{single transitive representation generates algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
}

\AddEq{theorem: automorphism uniquely defined by image of basis}
{
\begin{ShadedTheorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $\Basis e$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}{\Basis e}
произвольное отображение множества $\Basis e$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}{\Basis e}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}e{\Basis e}
Существует единственный эндоморфизм представлнения $f$\,\footnotemark
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{ShadedTheorem}
\footnotetext{\,
Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.
}
}

\DefDefinition{parity of permutation}
{
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}

\DefText{passive representation of vector space 1}
{
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v3
Тогда
\ShowEq{v=vi ei 123, \SideNS-\Cols}
Пусть пассивное преобразование $g_1$ отображает базис
\ShowEq{Basis e in BVG}1
в базис
\ShowEq{Basis e in BVG}2
\DrawEq[12g1]{e2i=aij e1j \Product-\Cols}{12}
Пусть пассивное преобразование $g_2$ отображает базис
\ShowEq{Basis e in BVG}2
в базис
\ShowEq{Basis e in BVG}3
\DrawEq[23g2]{e2i=aij e1j \Product-\Cols}{23}
}

\DefText{passive representation of vector space 2}
{
Преобразование
\ShowEq{e3=g12 cr e1 \SideNS-\Cols}
является произведением преобразований
\eqRef{e2i=aij e1j \Product-\Cols}{12},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Преобразование координат
\DrawEq[v2v1g1{\SideNS}{\Cols}]{v2=v1g-}{1 \SideNS-\Cols}
соответствует пассивному преобразованию $g_1$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{12}
и теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\DefText{passive representation of vector space 3}
{
Аналогично,
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\fi
преобразование координат
\DrawEq[v3v2g2{\SideNS}{\Cols}]{v2=v1g-}{23 \SideNS-\Cols}
соответствует пассивному преобразованию $g_2$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Произведение преобразований координат
\eqRef{v2=v1g-}{1 left-cols},
\eqRef{v2=v1g-}{23 left-cols}
имеет вид
\ShowEq{v3=v1 cr g1- cr g2- \SideNS-\Cols}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\EqRef{e3=g12 cr e1 \SideNS-\Cols}.
Равенство
\ShowEq{v3=v1 cr g21- \SideNS-\Cols}
является следствием равенств
\EqRef{cr-inverse matrix of product},
\EqRef{v3=v1 cr g1- cr g2- \SideNS-\Cols}.
}

\DefText{passive representation of left vector space}
{
\ShowText{passive representation of vector space 1}
\ShowText{passive representation of vector space 2}
\ShowText{passive representation of vector space 3}
}

\DefDefinition{Left side contravariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{контравариантным}{contravariant representation},
если равенство
\ShowEq{Left side contravariant representation}
верно.
}

\DefDefinition{Left side covariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{ковариантным}{covariant representation},
если равенство
\ShowEq{Left side covariant representation}
верно.
}

\DefDefinition{cr-inverse matrix}
{
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph число
\else
Матрица
\fi
\ShowEq{cr-inverse element}
- это \AddIndex{\CR обратный элемент}{cr-inverse element}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$, если
\DrawEq{cr-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Матрица $a$ называется
\CR невырожденной,
если существует \CR обратная матрица.
\fi
}

\DefDefinition{delta=Matrix}
{
Матрица
\ShowEq{delta=Matrix}
является единицей для обоих произведений.
}

\DefRemark{pronunciation of product}
{
Мы будем пользоваться символом \RC\,\, или \CR\,\,  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символ
$\RCstar$ как
$rc$\hyph произведение (произведение строки на столбец)
и символ $\CRstar$ как
$cr$\hyph произведение (произведение столбца на строку).
Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
Это правило мы распространим на последующую терминологию.
Символ произведения
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \RC произведение
матриц $a$ и $b$ имеет вид
$a\RCcirc b$
и \CR произведение
матриц $a$ и $b$ имеет вид
$a\CRcirc b$.
\fi
}

\DefTheorem{quasideterminant rc cr, matrix 2x2}
{
\ShowEq{quasideterminant matrix 2x2 def}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Тогда
\ShowEq{quasideterminant rc, matrix 2x2}
\ShowEq{quasideterminant cr, matrix 2x2}
\ShowEq{rc inverse matrix 2x2}
}

\DefDefinition{RC-quasideterminant}
{
\AddIndex{$(\aUD{}ji)$\hyph \RC квазидетерминант}{j i RC-quasideterminant}
\nTimes матрицы $a$
- это формальное выражение
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
Мы можем рассматривать $\aUD (ji)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RC-quasideterminant definition}
\ShowEq{RC-quasideterminant definition=}
которую мы будем называть
\AddIndex{\RC квазидетерминантом}{RC-quasideterminant}.
}

\DefDefinition{biring}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\DrawEq{rc transpose}{}
\item транспозиция единицы есть единица
\DrawEq{transpose of identity}E
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
}

\DefTheorem{double transpose is original matrix}
{
Двойная транспозиция есть исходная матрица
\ShowEq{double transpose}
}

\DefProof{double transpose is original matrix}
{
Теорема является следствием определения
\RefDefinition{transpose of matrix}.
}

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца матриц]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{ShadedTheorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$.
\qed
\end{ShadedTheorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
Произведение
\ShowEq{(ab)->ab}
в мультипликативной $\Omega$\Hyph группе $A$
определяет два различных представления.
\begin{itemize}
\EqParm{associative shift}{def left}
\EqParm{associative shift}{def right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
\SideRuC вый сдвиг
\ShowEq{\SideWS shift}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
}

\AddEq{associative shift}
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$
\ShowEq{\SideWS shift, product}
}

\DefDefinition{representation of algebra}
{
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
$A_1$ или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
}

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениями.

\begin{ShadedDefinition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\end{ShadedDefinition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefTheorem{two representations of group}
{
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа.
Пусть левостороннее $A_1$\Hyph представление $f$
на $\Omega_2$\Hyph алгебре $A_2$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное правостороннее $A_1$\Hyph представление $h$
на $\Omega_2$\Hyph алгебре $A_2$
такое, что диаграмма
\ShowEq{two representations of group}
коммутативна для любых $a_1$, $b_1\in A_1$.
}

\AddEq{definition: twin representations}
{
Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями}{twin representations}
мультипликативной $\Omega$\Hyph группы $A_1$.
}

\DefRemark{one representation of group}
{
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если мультипликативная $\Omega$\Hyph группа $A_1$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $A_2$,
то мы можем определить два перестановочных представления на множестве $A_2$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму
\EqRef{Diagram: two representations of group}
и предположить
\ShowEq{haa=Laa}
вместо
\ShowEq{haa=aRa}
и проанализировать, какое выражение $h(a_1)$ имеет в
точке $c_2$. Диаграмма
\ShowEq{Diagram: two representations of group 1}
эквивалентна диаграмме
\ShowEq{Diagram: two representations of group 2}
и мы имеем
\ShowEq{d2=...c2 1}
Следовательно
\ShowEq{d2=...c2}
Мы видим, что представление $h$
зависит от его аргумента.
}

\DefTheorem{single transitive representation of group}
{
Если существует однотранзитивное представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$,
то мы можем однозначно определить координаты на $A_2$, пользуясь $A_1$\Hyph числами.

Если $f$ - левостороннее однотранзитивное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $A_1$.
Если $f$ - правостороннее однотранзитивное представление, то $f(a)$ эквивалентно
правому сдвигу $R(a)$ на группе $A_1$.
}

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратная матрица}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратная матрица}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество однородных многочленов}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис}%
   {Basis}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество \CR собственных значений}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество \RC собственных значений}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {образ отображения}%
   {image of map}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {левое векторное пространство алгебры $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {левое векторное пространство отображений}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {правое векторное пространство алгебры $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {правое векторное пространстао отображений}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {векторное пространство начальных значений системы дифференциальных уравнений}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {векторное пространство решений системы дифференциальных уравнений}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {матрица Вронского}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $A$\Hyph числа}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex


==> Vector.Space.2020.Stmt.Russian.tex <==
%auto-ignore
\input{Vector.Space.2020.Stmt.Eq}

\DefLabeledDefinition{eigenvalue of matrix}{\Product}
{
$A$\Hyph число $b$ называется
{\bf\ProductType собственным значением}
матрицы $f$,
если матрица
$f-b\aD En$
- \ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of matrix}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $f$.
\ColC $v$ называется
{\bf собственн\ColB}
матрицы $f$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols}1
}

\DefLabeledTheorem{0 is eigenvalue of multiplicity}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел и
\ShowEq{\Product-rank a=k<n}
Тогда $0$ является \ProductType собственным значением кратности
$\gin-\gik$.
}

\DefProof{0 is eigenvalue of multiplicity}
{
Теорема является следствием равенства
\[a=a-0E\]
определения
\refDefinition{eigenvalue of matrix}{\Product}
и теоремы
\RefTheorem{star rows system of linear equations, solution}.
}

\DefLabeledTheorem{eigenvalues of pair of matrices}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Пусть $g$ - \ProductType невырожденная $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \ProductType собственные значения пары матриц $(f,g)$
являются корнями любого уравнения
\DrawEq{\Product-det ij f-bg =0}{}
}

\DefProofSloppy{eigenvalues of pair of matrices}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{eigenvalues of pair of matrices}{\Product}.
}

\DefLabeledTheorem{eigenvalues of matrix}{\Product}
{
Пусть $f$ - $\gin\times\gin$ матрица $A$\Hyph чисел.
Тогда ненулевые \RC собственные значения матрицы $f$
являются корнями любого уравнения
\DrawEq{\Product-det ij a=0}{}
}

\DefProofSloppy{eigenvalues of matrix}
{
Теорема является следствием теоремы
\refTheorem{singular matrix and quasideterminant}{\Product}
и определения
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}.
}

\DefLabeledTheorem[6]{product of homomorphisms, A vector space}{\SideNS-\ColN}
{
Пусть $U$, $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}UAU
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fUW{}%
является произведением гомоморфизмов
\ShowEq{vf: A->B}hVW,%
\ShowEq{vf: A->B}gUV{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}UW{}{}
равна \ProductType произведению матрицы $#1$ гомоморфизма $\Vector{#1}$
относительно базисов
\ShowEq{Bases eVW}{#2}{#3}{}{}
на матрицу $#4$ гомоморфизма $\Vector{#4}$
относительно базисов
\ShowEq{Bases eVW}{#5}{#6}{}{}
\DrawEq[f#1{\ProductVal}#4]{f=g*h}{\Product-\Cols}
}

\DefProof[2]{product of homomorphisms, A vector space}
{
Согласно теореме
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}
\DrawEq[ufUW]{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols}
\DrawEq[ugUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols}
\DrawEq[vhVW]{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}
Согласно теореме
\refTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{f o v=g o h o v \SideNS-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g product \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h product \Product-\Cols}.
Равенство
\eqRef{f=g*h}{\Product-\Cols}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f product \Product-\Cols},
\EqRef{f o v=g o h o v \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}.

Пусть
\DrawEq[f#1{\ProductVal}{#2.}]{f=g*h}-
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(gh)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(gh)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является произведением гомоморфизмов $\Vector h$, $\Vector g$.
}

\DefLabeledTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $U$, $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства.
Предположим, что мы имеем
коммутативную диаграмму отображений
\DrawEq{diagram product of homomorphisms, A vector space}{\SideNS}
\newline
\DrawEq{f o u=h o g o u}{\SideNS}
где отображения $g$, $h$ являются
гомоморфизмами \SideRu вого $A$\Hyph векторного пространства.
Отображение
\ShowEq{f=h o g}
является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{произведением гомоморфизмов}{product of homomorphisms}
$h$, $g$.
}

\DefProof{product of homomorphisms is homomorphism, A vector space}
{
Равенство
\eqRef{f o u=h o g o u}{\SideNS}
следует из коммутативности диаграммы
\eqRef{diagram product of homomorphisms, A vector space}{\SideNS}.
Равенство
\DrawEq{(h o g)o(u+v)=}{\SideWS vector space}
является следствием равенства
\ShowRef{homomorphism, f v+w=}
и равенства
\eqRef{f o u=h o g o u}{\SideNS}.
Равенство
\ShowEq{(h o g)o(av)= \SideNS}
является следствием равенства
\ShowRef{homomorphism, f av=}
и равенства
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Теорема является следствием теоремы
\refTheorem{define homomorphism A module}{\SideNS(1)}
и равенств
\eqRef{(h o g)o(u+v)=}{\SideWS vector space},
\EqRef{(h o g)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
{
Пусть $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства
и отображения
\DrawEq[gVW,]{f: A->B}-
\DrawEq[hVW{}]{f: A->B}-
- гомоморфизмы
\SideRu вого $A$\Hyph векторного пространства.
Пусть отображение
\DrawEq[fVW{}]{f: A->B}-
определено равенством
\DrawEq{sum of homomorphisms f o v=}{\SideWS vector space}
Отображение $f$ является гомоморфизмом
\SideRu вого $A$\Hyph векторного пространства
и называется
\AddIndex{суммой
\ShowEq{f=g+h}
гомоморфизмов}{sum of maps}
$g$ and $h$.
}

\DefProof{sum of homomorphisms is homomorphism, A vector space}
{
Согласно теореме
\refTheorem{definition of A module, property}{\SideNS}
(равенство
\eqRef{commutative law}{\SideWS vector space}),
равенство
\newline
\DrawEq{(g+h)o(u+v)=}{\SideWS vector space}
\begin{sloppypar}
\noindent
является следствием равенства
\ShowRef{homomorphism, f v+w=}
и равенства
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.
Согласно теореме
\refTheorem{definition of A module, property}{\SideNS}
(равенство
\eqRef{distributive law, \SideWS module, 1}1),
равенство
\ShowEq{(g+h)o(av)= \SideNS}
\end{sloppypar}
\noindent
является следствием равенства
\ShowRef{homomorphism, f av=}
и равенства
\eqRef{sum of homomorphisms f o v=}{\SideWS vector space}.

Теорема является следствием теоремы
\refTheorem{define homomorphism A module}{\SideNS(1)}
и равенств
\eqRef{(g+h)o(u+v)=}{\SideWS vector space},
\EqRef{(g+h)o(av)= \SideNS}.
}

\DefLabeledTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols}
{
Пусть $V$, $W$ -
\SideRu вые $A$\Hyph векторные пространства \ColsNA.
\ShowEq{Let be Basis of vector space}VAV
\ShowEq{Let be Basis of vector space}WAW
Гомоморфизм
\ShowEq{vf: A->B}fVW{}%
является суммой гомоморфизмов
\ShowEq{vf: A->B}gVW,%
\ShowEq{vf: A->B}hVW{}%
тогда и только тогда, когда
матрица $f$ гомоморфизма $\Vector f$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
равна сумме матрицы $g$ гомоморфизма $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}{}
и матрицы $h$ гомоморфизма $\Vector h$
относительно базисов
\ShowEq{Bases eVW}VW{}.
}

\DefProof{sum of homomorphisms, A vector space}
{
Согласно теореме
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}
\DrawEq[afUV]{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols}
\DrawEq[agUV]{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols}
\DrawEq[ahUV]{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}
Согласно теореме
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS},
равенство
\ShowEq{fov=gov+hov \SideNS-\Cols}
является следствием равенств
\eqRef{a.\Product.(b1+b2)=}1,
\eqRef{(b1+b2).\Product.a=}1,
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{g sum \Product-\Cols},
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{h sum \Product-\Cols}.
Равенство
\ShowEq{f=g+h}
является следствием равенств
\eqRef{f o (ae)=a o f e, vector space \Product-\Cols}{f sum \Product-\Cols},
\EqRef{fov=gov+hov \SideNS-\Cols}
и теоремы
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}.

Пусть
\ShowEq{f=g+h}
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
существуют гомоморфизмы
\ShowEq{vf: A->B}fUV,%
\ShowEq{vf: A->B}gUV,%
\ShowEq{vf: A->B}hUV{}%
такие, что
\ShowEq{fov=(g+h)ov \SideNS-\Cols}
Из равенства
\EqRef{fov=(g+h)ov \SideNS-\Cols}
и теоремы
\refTheorem{sum of homomorphisms is homomorphism, A vector space}{\SideNS}
следует, что
гомоморфизм $\Vector f$
является суммой гомоморфизмов $\Vector g$, $\Vector h$.
}

\AddEq{definition: vector space of maps B->A n}
{
\begin{ShadedDefinition}
\labelDefinition{\SideWS vector space of maps B->A n}
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
и любого целого $n>0$
мы определим \SideRuTo $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of maps B->A n}
используя определение по индукции
\ShowEq{\SideWS vector space of maps B->A k}
\end{ShadedDefinition}
}

\DefLabeledDefinition{vector space of algebra A n}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого целого $n>0$
мы определим \SideRuTo $\Base$\Hyph векторное пространство
\ShowEq{\SideWS vector space of algebra A n}
используя определение по индукции
\ShowEq{\SideWS vector space of algebra A k}
}

\DefTheorem{coordinates of vector of vector space}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
левого $\Base$\Hyph векторного пространства $V$
определены однозначно.
}

\DefLabeledTheorem{coordinates of vector}{\SideNS-\Cols}
{
Координаты вектора $v\in V$ относительно базиса $\Basis e$
\SideRu\Which $\Base$\Hyph \VectorSetRuB $V$
определены однозначно.
Из равенства
\DrawEq{e*v=e*w,\SideNS}{\Cols}
следует, что
\ShowEq{=> v=w}
}

\DefProof{coordinates of vector}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, 0}
линейно зависима и в уравнении
\DrawEq{expansion relative basis, vector space, 1}{\SideNS-\Cols}
по крайней мере $b$ отлично от $0$. Тогда равенство
\DrawEq{expansion relative basis, vector space, 2}{\SideNS-\Cols}
следует из
\eqRef{expansion relative basis, vector space, 1}{\SideNS-\Cols}.
Равенство
\DrawEq{expansion relative basis, vector space}{\SideNS-\Cols}
является следствием из равенства
\eqRef{expansion relative basis, vector space, 2}{\SideNS-\Cols}.

Допустим мы имеем другое разложение
\DrawEq{expansion relative basis, vector space, 3}{\SideNS-\Cols}
Вычтя
\eqRef{expansion relative basis, vector space}{\SideNS-\Cols}
из
\eqRef{expansion relative basis, vector space, 3}{\SideNS-\Cols},
мы получим
\DrawEq{expansion relative basis, vector space, 4}{\SideNS-\Cols}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5}{\SideNS-\Cols}
является следствием равенства
\eqRef{expansion relative basis, vector space, 4}{\SideNS-\Cols}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5}{\SideNS-\Cols}.
}

\DefProof{coordinates of vector 2022}
{
Согласно теореме
\refTheorem{basis over division algebra}{\SideNS},
система векторов
\ShowEq{expansion relative basis, vector space, (0)}
линейно зависима и в уравнении
\ShowEq{expansion relative basis, vector space, 1 \SideNS}
по крайней мере $b$ отлично от $0$. Тогда равенство
\ShowEq{expansion relative basis, vector space, 2 \SideNS}
следует из
\EqRef{expansion relative basis, vector space, 1 \SideNS}.
Равенство
\ShowEq{expansion relative basis, vector space \SideNS}
является следствием из равенства
\EqRef{expansion relative basis, vector space, 2 \SideNS}.

Допустим мы имеем другое разложение
\ShowEq{expansion relative basis, vector space, 3 \SideNS}
Вычтя
\EqRef{expansion relative basis, vector space \SideNS}
из
\EqRef{expansion relative basis, vector space, 3 \SideNS},
мы получим
\ShowEq{expansion relative basis, vector space, 4 \SideNS}
Так как векторы \ARow ei линейно независимы,
то равенство
\DrawEq{expansion relative basis, vector space, 5()}{\SideNS}
является следствием равенства
\EqRef{expansion relative basis, vector space, 4 \SideNS}.
Утверждение теоремы является следствием равенства
\eqRef{expansion relative basis, vector space, 5()}{\SideNS}.
}

\DefProof{coordinates of vector *}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector}{\SideNS-*}.
}

\DefExample{system of linear equations, right vector space of columns}
{
Пусть $V$ - правое $A$\Hyph векторное пространство столбцов и
строка
\ShowEq{rcd linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\aD{\Vector a}i$,
если линейное уравнение
\DrawEq{rcd linear span, 2}f
где
\DrawEq[xn]{a=(a1.n col)}{}
столбец неизвестных коэффициентов разложения,
имеет решение.
Предположим, что
\DrawEq[{}jJ]{basis e of module cols}-
- базис.
Тогда векторы
\ShowEq{rcd linear span, 6}
имеют разложение
\ShowEq{rcd linear span, 7}
Если мы подставим \EqRef{rcd linear span, b}
и \EqRef{rcd linear span, ai}
в
\eqRef{rcd linear span, 2}f,
мы получим
\DrawEq{rcd linear span, 8}f
Применяя теорему \RefTheorem{coordinates of vector of vector space}
к
\eqRef{rcd linear span, 8}f,
мы получим
\AddIndex{систему линейных уравнений}
{system of linear equations}
\DrawEq{system of rcd linear equations}f

Если мы положим
\ShowEq{a1n= b= column}
то мы можем записать систему линейных уравнений
\eqRef{system of rcd linear equations}f
в следующей форме
\ShowEq{star rows system of linear equations 1}
Равенство
\ShowEq{star rows system of linear equations}
является следствием равенств
\ePrints{339295394}%
\ifx\Semafor\ValueOn%
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
и
\else%
\EqRef{rc-product of matrices},
\fi%
\EqRef{star rows system of linear equations 1}.
Записывая сумму
\EqRef{star rows system of linear equations}
в виде строки, мы получим
\DrawEq{star rows system of linear equations 2}2
Мы видим в системе линейных уравнений
\eqRef{star rows system of linear equations 2}2,
что $A$\Hyph столбец $b$ является правой линейной комбинацией $A$\Hyph столбцов
\ShowEq{aD1n}
}

\DefLabeledDefinition{rank of matrix}{\Product}
{
Если подматрица $\aUD aST$ - \ProductType невырожденная матрица,
то мы будем говорить, что
\ProductType ранг матрицы $a$ не меньше, чем $\gik$.
{\bf\ProductType ранг матрицы} $a$,
\ShowEq{\Product-rank of matrix}
- это максимальное значение $\gik$.
Мы будем называть соответствующую подматрицу
{\bf \ProductType главной подматрицей}.
}

\DefLabeledTheorem{vector space of maps B->A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Для любого множества $B$
представление
\ShowEq{representation \SideWS vector space of maps B->A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of maps B->A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of maps B->A}
{
Согласно теореме
\RefTheorem{set of maps B->A is Abelian group},
множество отображений $A^B$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(h+g)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение $f(a)$ является эндоморфизмом абелевой группы $A^B$.
Из равенств
\ShowEq{\SideWS (a1+a2)h=}
\ShowEq{\SideWS a1a2h=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группы $A^B$.
Теорема является следствием определения
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}.
}

\DefText{linear span, vector space}
{
\subsection{\SideRuC вое
\texorpdfstring{$A$}{A}-векторное пространство \ColsNA}
\ShowText{linear span in vector space}
}

\DefLabeledDefinition{coordinates of vector}{\SideWS \VectorSetNS}
{
Пусть $\Basis e$ - квазибазис \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$,
и вектор
\ShowEq{vv in V}vV
имеет разложение
\DrawEq{vv=ve \SideWS module}{Definition}
относительно квазибазиса $\Basis e$.
$\Base_{\BaseExt}$\Hyph числа $\ACol vi$ называются
\AddIndex{координатами}{coordinates}
вектора $\Vector v$ относительно квазибазиса $\Basis e$.
Матрица $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в квазибазисе $\Basis e$.
}

\DefLabeledTheorem{matrix and system of linear equations}{\SideNS-\Cols}
{
Рассмотрим матрицу
\DrawEq{matrix a = set ai \Cols}{\SideNS}
Тогда система линейных уравнений
\eqRef{a*x=b \SideNS}{\Cols}
может быть записана в следующей форме
\ShowEq{a*x=b \SideNS-\Cols}
\DrawEq{a*x=b 1 \SideNS-\Cols}1
}

\DefProof{matrix and system of linear equations}
{
Равенство
\EqRef{a*x=b \SideNS-\Cols}
является следствием равенств
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{a=(a1.n set)}{xm \SideNS-\Cols},
\eqRef{a*x=b \SideNS}{\Cols}
\eqRef{matrix a = set ai \Cols}{\SideNS}
и определения
\RefDefinition{\RowNWS over \ColNWS product}.
}

\DefTheorem{standard representation of product of tensors}
{
Пусть
$\aUD Ck{ij}$
- структурные константы $D$\Hyph алгебры $A$.
Пусть
\DrawEq[f]{f=...ei o ek}f
стандартное представление тензора
\ShowEq{f in AoA}f{}
и
\DrawEq[g]{f=...ei o ek}g
стандартное представление тензора
\ShowEq{f in AoA}g.
Тогда стандартное представление произведения тензоров
\ShowEq{fg=...ei o ek}
удовлетворяет равенству
\ShowEq{fg=CCfg}
}

\DefProof{standard representation of product of tensors}
{
Равенство
\ShowEq{fg=...e o e}
является следствием равенств
\eqRef{f=...ei o ek}f,
\eqRef{f=...ei o ek}g.
Равенство
\ShowEq{fg=...C e o e}
является следствием равенств
\ShowRef{product of basis vectors}
\EqRef{fg=...e o e}.
Равенство
\EqRef{fg=CCfg}
является следствием равенств
\EqRef{fg=...ei o ek},
\EqRef{fg=...C e o e}.
}

\DefLabeledTheoremNote{nonsingular system of linear equations}{\SideNS-\Cols}
{
Решение невырожденной системы линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
определено однозначно и может быть записано в любой
из следующих форм\,\footnotemark
\DrawEq{x=a-*b, matrix \SideNS}{\Cols}
\DrawEq{x=a-*b, quasideterminant \SideNS}{\Cols}
}
{
Мы можем найти решение системы
\eqRef{a*x=b 1 \SideNS-\Cols}1
в теореме
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=19}{1.6.1}.
Я повторяю это утверждение, так как я слегка изменил обозначения.
}

\DefProof{nonsingular system of linear equations}
{
Умножая обе части равенства
\eqRef{a*x=b 1 \SideNS-\Cols}1
слева на $a^{\InverseVal}$, мы получим
\eqRef{x=a-*b, matrix \SideNS}{\Cols}.
Пользуясь определением
\newline
\FrameEqRef{quasideterminant and inverse}{\Product}
\newline
мы получим
\eqRef{x=a-*b, quasideterminant \SideNS}{\Cols}.
Решение системы единственно
в силу теоремы
\RefTheorem{two rc-products equal}.
}

\DefLabeledDefinition{nonsingular system of linear equations}{\SideNS-\Cols}
{
Предположим, что $a$
- \ProductType невырожденная матрица. Мы будем называть соответствующую
систему линейных уравнений
\newline
\FrameEqRef{a*x=b 1 \SideNS-\Cols}1
\newline
\AddIndex{невырожденной системой линейных уравнений}
{nonsingular system of linear equations}.
}

\DefLabeledTheorem{linear span and system of equations}{\SideNS-\Cols}
{
Пусть
\DrawEq[{}jJ]{basis e of module}-
- базис.
Пусть векторы
\ShowEq{linear span, 6}
имеют разложение
\DrawEq[b]{linear span, b \SideNS}{b \Cols}
\DrawEq[{\ARow ai}{}]{linear span, b \SideNS}{a \Cols}
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{xm \SideNS-\Cols}
которые удовлетворяют
\AddIndex{системе линейных уравнений}
{system of linear equations}
\DrawEq{a*x=b \SideNS}{\Cols}
}

\DefProof{linear span and system of equations}
{
Равенство
\DrawEq{e*b=e*a*x \SideNS}{\Cols}
является следствием равенств
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols},
\eqRef{linear span, b \SideNS}{b \Cols},
\eqRef{linear span, b \SideNS}{a \Cols}.
Равенство
\DrawEq{b=a*x \SideNS}{\Cols}
является следствием равенства
\eqRef{e*b=e*a*x \SideNS}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Равенство
\eqRef{a*x=b \SideNS}{\Cols}
является следствием равенства
\eqRef{b=a*x \SideNS}{\Cols}.
}

\DefLabeledTheorem{linear span is vector space}{\SideNS-\Cols}
{
$\spanb$ - подпространство \SideRu вого $A$\Hyph векторного пространства $V$ \ColsNA.
}

\DefProof{linear span is vector space}
{
Предположим, что
\ShowEq{linear span, vector space, 1}
Согласно теореме
\refTheorem{vector in linear span}{\SideNS-\Cols}
\DrawEq[bb]{linear span, 2 \SideNS}{b \SideNS-\Cols}
\DrawEq[cc]{linear span, 2 \SideNS}{c \SideNS-\Cols}
Тогда
\ShowEq{linear span, 3 \SideNS}
Это доказывает утверждение.
}

\DefLabeledDefinition{module type}{\SideNS-\Cols}
{
Мы представили множество векторов
\ShowEq{\RowN() 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{vm \SideNS-\Cols}
и множество $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{\ColNS() 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Соответствующее представление \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$ мы будем называть
\AddIndex{\SideRu\What $\Base$\Hyph \VectorSetRuE \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefLabeledTheorem{linear combination in module type}{\SideNS-\Cols}
{
Мы можем записать линейную комбинацию
\ShowEq{linear combination, \SideNS-\Cols}cvm
векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[cvm]{w.e, \SideNS-\Cols}{cv}
}

\DefProof{linear combination in module type}
{
Теорема является следствием определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{module type}{\SideNS-\Cols}.
}

\DefLabeledTheorem{vector in linear span}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\RowRuWS
\ShowEq{linear span, 0}
задаёт множество векторов.
Вектор $\Vector b$
линейно зависит от векторов $\ARow{\Vector a}i$
\ShowEq{linear span, 1}
если существует \ColWS $A$\Hyph чисел
\DrawEq[xm]{a=(a1.n set)}{}
так\FinA, что верно равенство
\DrawEq[bx]{linear span, 2 \SideNS}{\SideNS-\Cols}
}

\DefProof{vector in linear span}
{
Равенство
\eqRef{linear span, 2 \SideNS}{\SideNS-\Cols}
является следствием определения
\refDefinition{linear span, vector space}{\SideNS-\Cols}
и теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledDefinition{linear span, vector space}{\SideNS-\Cols}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
\ShowEq{linear span, set}
- множество векторов.
\AddIndex{Линейная оболочка}{linear span, vector space}
в \SideRu вом $A$\Hyph векторном пространстве \ColsA - это множество
\ShowEq{linear span, vector space}
векторов, линейно зависимых от векторов
\ARow {\Vector a}i.
}

\DefLabeledTheorem{vector space of algebra A}{\SideNS}
{
Пусть $D$ - коммутативное кольцо с единицей.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Представление, порождённое \SideRu вым сдвигом,
\ShowEq{representation \SideWS vector space of algebra A}
является \SideRu вым векторным пространством
\ShowEq{\SideWS vector space of algebra A}
над $D$\Hyph алгеброй $A$.
}

\DefProof{vector space of algebra A}
{
Согласно определениям
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS},
\RefDefinition{algebra over ring},
$D$\Hyph алгебра $A$ является абелевой группой.
Из равенства
\ShowEq{\SideWS a(b+c)=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}
следует, что отображение
\ShowEq{\SideWS a->ab}
является эндоморфизмом абелевой группы $A$.
Из равенств
\ShowEq{\SideWS (a1+a2)b=}
\ShowEq{\SideWS a1a2b=}
и определений
\RefDefinition{homomorphism},
\RefDefinition{representation of algebra}
следует, что отображение $f$ является
представлением $D$\Hyph алгебры $A$ в абелевой группе $A$.
Теорема является следствием определения
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}.
}

\AddEq{def row text}
{%
\def\ColWS{строка }%
\def\ColC{Cтрока }%
\def\ColA{строки }%
\def\ColB{ой строкой }%
\def\ColBNS{ой строкой}%
\def\ColumnC{ая строка }%
\def\ColumnCNS{ая строка}%
\def\FinA{ая}%
\def\FinB{ей }%
\def\FinC{й }%
\def\endC{ая }%
\def\ColsRu{строки }%
\def\ColsA{строк }%
\def\ColsNA{строк}%
\def\EndA{ых }%
\def\RowRuWS{столбец }%
\def\RowsNSA{столбцов}%
\def\RowA{столбца }%
\def\RowsRWSA{столбцов }%
}

\AddEq{def col text}
{%
\def\ColWS{столбец }%
\def\ColC{Cтолбец }%
\def\ColA{столбца }%
\def\ColB{ым столбцом }%
\def\ColBNS{ым столбцом}%
\def\ColumnC{ый столбец }%
\def\ColumnCNS{ый столбец}%
\def\FinA{ой}%
\def\FinB{им }%
\def\FinC{го }%
\def\endC{ий }%
\def\ColsRu{столбцы }%
\def\ColsA{столбцов }%
\def\ColsNA{столбцов}%
\def\EndA{ых }%
\def\RowsNSA{строк}%
\def\RowA{строки }%
\def\RowsRWSA{строк }%
\def\RowRuWS{строка }%
}

\DefLabeledDefinition{spectrum of matrix}{\Product}
{
Множество
\ShowEq{spectrum of matrix}
всех левых и правых
\ProductType собственных значений называется
\ProductType спектром матрицы a.
}

\DefLabeledTheorem{vector space over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRu вое $A$\Hyph векторное пространство $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
В диаграмме представлений
\eqRef{diagram of representations, \SideWS module}1
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
коммутативного кольца $D$ и $D$\Hyph алгебры $A$
в абелевой группе $V$
\DrawEq{\SideWS module, a d v}1
}

\DefProof{vector space over algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}
и теоремы
\RefTheorem{Free Algebra over Ring}.
Равенство
\eqRef{\SideWS module, a d v}1
является следствием утверждения, что
\SideRu вое преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph векторного пространства $V$.
}

\DefText{Proof unitarity law, module}
{
Согласно теоремам
\refTheorem{module over algebra}{\SideNS},
\refTheorem{action of unital ring}{\SideWS \VectorSetNS},
равенство
\eqRef{unitarity law, module}{\SideWS \Base}
является следствием равенства
\ShowEq{Proof unitarity law 1}
и равенства
\EqRef{1a=a (+)}.
Если \algebrac имеет единицу, то равенство
\eqRef{unitarity law, vector space}{\SideWS \Base-\VectorSetNS}
является следствием теоремы
\RefTheorem{unit of ring and Z}.
}

\DefText{Proof unitarity law, vector space}
{
The equality
\eqRef{unitarity law, vector space}{\SideWS \Base}
является следствием теорем
\RefTheorem{unit of ring and Z},
\refTheorem{vector space over algebra}{\SideNS}
так как представление
$\DRepro$
является \SideRu\SidePresentationRuBWS представлением
мультипликативной группы \ShortAlgebraRuBWS $\Base$.
}

\DefRef{distributive law 1, module}
{
теорем
\refTheorem{monoid-homomorphism}{+},
\refTheorem{action of unital ring}{\SideWS \VectorSetNS}.
}

\DefRef{distributive law 1, vector space}
{
теоремы
\refTheorem{monoid-homomorphism}{+}.
}

\DefProof{definition of A module, property 2020}
{
Равенство
\eqRef{commutative law}{\SideWS vector space}
является следствием определения
\ShowRef{module over algebra \Base}

Равенство
\eqRef{distributive law, \SideWS module, 1}1
является следствием
\ShowRef{distributive law 1, \VectorSetNS}

Равенство
\eqRef{distributive law, \SideWS module, 2}1
является следствием теоремы
\refTheorem{monoid-homomorphism, sum}{+}.

Равенство
\eqRef{associative law, \SideWS module}1
является следствием теоремы
\RefTheorem{product of homomorphisms}.

\ShowText{Proof unitarity law, \VectorSetNS}
}

\DefLabeledTheorem{coordinate matrix of vector}{\SideNS-\Cols}
{
Если мы запишем векторы базиса $\Basis e$
в виде \RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
}

\DefProof{coordinate matrix of vector}
{
Теорема является следствием теоремы
\refTheorem{linear combination in module type}{\SideNS-\Cols}.
}

\DefLabeledExample{Vector Space Type}{\SideNS-\Cols}
{
\ePrints{2022.01.05}
\ifx\Semafor\ValueOff
Мы представили множество векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде
\RowA матрицы
\DrawEq[vm]{a=(a1.n \RowN)}{}
и множество $A$\Hyph чисел
\ShowEq{\ColNWS set 1n}cm{}
в виде
\ColA матрицы
\DrawEq[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
Поэтому мы можем записать линейную комбинацию векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\DrawEq[{\ParmA}{\ParmB}m]{w.e, \SideNS-\Cols}{\ParmA\ParmB}
В частности,
если 
\else
Если 
\fi
мы запишем векторы базиса $\Basis e$ в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideNS-\Cols}
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\DrawEq[wn]{a=(a1.n \ColNS)}{\SideNS-\Cols}
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\DrawEq[w]{vector w=w*e \SideNS-\Cols}w
Соответствующее представление векторного пространства $V$ мы будем называть
\AddIndex{\SideRu вым $A$\Hyph векторным пространством \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
}

\DefRemark{Left and Right Eigenvalues not equal 0}
{
Согласно данному выше определению,
множества левых и правых \ProductType собственных значений совпадают.
Однако мы рассмотрели самый простой случай.
Кон рассматривает определения

\ShowEq{def right}
\ShowEq{\DefCol}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ShowEq{def left}
\ShowEq{\DefRow}
\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
где $a_2$ - \ProductType невырожденная матрица,
как начальную точку для исследования.
}

\AddEq{remark: Left and Right Eigenvalues not equal}
{
Мы предполагаем, что кратность всех \SideRu вых \ProductType собственных значений
\nTimes матрица $a_2$ равна $1$.
Допустим \nTimes матрица $a_2$ не имеет $\gin$
\SideRu вых \ProductType собственных значений,
но имеет
\ShowEq{gik<gin}
\SideRu вых \ProductType собственных значений.
В этом случае, матрица $u_2$ в равенстве

\FrameEqRef[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1

\noindent
является
\ShowEq{gin x gik \SideNS}
матрицей, и матрица $a_1$
является \nTimes[k] матрицей.
Однако из равенства
\eqRef{A \ProductS U=U \ProductS D \SideNS}1
не следует, что
\ShowEq{rank rc u2 =k}

Если
\ShowEq{rank rc u2 =k}
то существует
\ShowEq{gin x gik \OtherSideNS}
матрица
\ShowEq{a in left}w{u_2}{\OtherSideNS}{}
такая, что
\ShowEq{w rc u2=Ek \SideNS}
Равенство
\ShowEq{w rc a2 rc u2=a1 \SideNS}
является следствием равенств
\eqRef{A \ProductS U=U \ProductS D \SideNS}1,
\EqRef{w rc u2=Ek \SideNS}.

Если
\ShowEq{rank rc u2 <k}
то между 
\SideRu выми собственными векторами
существует линейная зависимость.
В этом случае
множества левых и правых \ProductType собственных значений не совпадают.
}

\DefText[5]{define homomorphism of vector space(1)}
{
Согласно определениям
\ShowRef{define homomorphism A module#5}{#1}{#2}
отображение
\DrawEq[gA]{homomorphism D algebra #1#2}{}
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Следовательно, равенства
\ShowRef{homomorphism of A vector space(#1)}{#1}{#2}{#3}{#5}
являются следствием теоремы
\refTheorem{linear map of D module}{#1#2}.
}

\DefText[5]{define homomorphism of vector space()}
{
}

\AddEq{remark: colinear vectors}
{
Векторы $v$ и
\ShowEq{av \SideNS}
называются
\AddIndex{колинеарными}{colinear vectors}
с\OtherSideRu ва.
Из утверждения, что векторы $v$ и $w$
колинеарны с\OtherSideRu ва
не следует, что
векторы $v$ и $w$ линейно зависимы с\SideRu ва.
}

\DefText[7]{be extended basis}
{
Пусть базис
\DrawEq[{#1}{#2}{#3}{#4}{#5}{#6}{#7}]{extended basis}{#7}
является расширением базиса \eV[#1_{#2}][.]
}

\DefLabeledTheorem{Two bases of module}{\SideNS-\Cols}
{
\ShowEq{Let be basis of algebra}A{}kKD{}A{}-
\ShowEq{Let be basis of module}V{}iI{\SideRu\Which}A{}V{}
Тогда множество $V$\Hyph чисел
\DrawEq[V{}A{}ki]{extended basis}{\SideNS-\Cols}
является базисом $D$\Hyph \VectorSetRuB $V$.
Базис \eV[VA] называется расширением базиса
\ShowEq{extension of basis}AV.
}

\DefProofRef{Two bases of module}{\SideNS-\Cols}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector}{-\Cols},
и лемм
\refLemma{Two bases of module 1}{\SideNS-\Cols},
\refLemma{Two bases of module 2}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 1}{\SideNS-\Cols}
{
Множество $V$\Hyph чисел \EBase 2{ik}
порождает $D$\Hyph \VectorSetRuA $V$.
}

\DefLemmaProof{Two bases of module 1}
{
Пусть
\DrawEq{Two bases of module 1 a}{\SideNS-\Cols}
произвольное $V$\Hyph число.
Для любого $A$\Hyph числа \ACol ai,
согласно определению
\RefDefinition{algebra over ring}
и соглашению
\RefConvention{basis of algebra as basis of module},
существуют $D$\Hyph числа \ACol a{ik} такие, что
\DrawEq{Two bases of module 1 ai}{\SideNS-\Cols}
Равенство
\DrawEq{Two bases of module 1 a=ai}{\SideNS-\Cols}
является следствием равенств
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{Two bases of module 1 a}{\SideNS-\Cols},
\eqRef{Two bases of module 1 ai}{\SideNS-\Cols}.
Согласно теореме
\refTheorem{set of vectors generated by set of vectors}{module},
лемма
является следствием равенства
\eqRef{Two bases of module 1 a=ai}{\SideNS-\Cols}.
}

\DefLabeledLemma{Two bases of module 2}{\SideNS-\Cols}
{
Множество $V$\Hyph чисел \EBase 2{ik}
линейно независимо над кольцом $D$.
}

\DefLemmaProof{Two bases of module 2}
{
Пусть
\DrawEq{extended basis 1}{\SideNS-\Cols}
Равенство
\DrawEq{extended basis 2}{\SideNS-\Cols}
является следствием равенств
\eqRef{extended basis}{\SideNS-\Cols},
\eqRef{extended basis 1}{\SideNS-\Cols}.
Согласно теореме
\refTheorem{coordinates of vector}{\SideNS-\Cols},
равенство
\DrawEq{extended basis 3}{\SideNS-\Cols}
является следствием равенства
\eqRef{extended basis 2}{\SideNS-\Cols}.
Согласно теореме
\refTheorem{coordinates of vector}{-\Cols},
равенство
\DrawEq{extended basis 4}{\SideNS-\Cols}
является следствием равенства
\eqRef{extended basis 3}{\SideNS-\Cols}.
Следовательно,
множество $V$\Hyph чисел \EBase 2{ik}
линейно независимо над кольцом $D$.
}

\DefLabeledTheorem{product vector over scalar}{\SideNS}
{
\ShowEq{ab in A,v in V}
\DrawEq{(av)b=a(vb)}{\SideNS}
}

\DefProof{product vector over scalar}
{
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
и определению
\refDefinition{product vector over scalar}{\SideNS},
равенство
\ShowEq{(av)b= \SideNS}
является следствием равенства
\ShowRef{homomorphism, f av=}
Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
является следствием равенства
\EqRef{(av)b= \SideNS}.
}

\DefLabeledDefinition{product vector over scalar}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Билинейное отображение
\DrawEq{\OtherSideWS A*V->V}2
порождённое \OtherSideRu восторонним представлением
\ShowEq{twin to \SideWS product}
называется
\AddIndex{\OtherSideRu восторонним произведением}{\OtherSideNS-side product}
вектора на скаляр.
}

\DefLabeledLemma{rcd dcr basis}{\SideNS}
{
Мы можем отождествить многообразие базисов
\ShowEq{basis manifold of V, \SideNS-cols}{\aD En}{\GL nA}{}
и множество \ProductType невырожденных матриц \GL nA.
}

\AddEq{proof: rcd dcr basis 1}
{
\begin{sloppypar}
{\sc Доказательство.}
Согласно замечанию
\refRemark{identify basis and matrix of coordinates}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$
и матрицу $e$ координат базиса $\Basis e$
относительно базиса $\Basis{\aD En}$
\ShowEq{be=e cr En \SideNS}
\hfill\(\odot\)
\end{sloppypar}
}

\DefLabeledDefinition{dimension of vector space}{\SideNS}
{
Мы будем называть
\AddIndex{размерностью \SideRu вого $A$\Hyph векторного пространства}{dimension of vector space}
число векторов в базисе.
}

\DefLabeledTheorem{coordinate matrix of basis}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Координатная матрица базиса $\Basis{g}$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ является \ProductType невырожденной матрицей.
}

\DefProof{coordinate matrix of basis}
{
Согласно теореме
\refTheorem{rank of matrix}{\Product-\Cols},
\CR ранг координатной матрицы базиса $\Basis{g}$ относительно базиса $\Basis e$
равен размерности левого $A$\Hyph пространства столбцов,
откуда следует утверждение теоремы.
}

\DefLabeledTheorem{automorphism of vector space}{\Product-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Тогда любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
}

\DefProof{automorphism of vector space}
{
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
следует из теоремы
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}.
Так как $\Vector f$ - изоморфизм,
то для каждого вектора $\Vector v'$ существует единственный вектор $\Vector v$ такой, что
\ShowEq{v'=fov}
Следовательно, система линейных уравнений
\eqRef{v1=v2*a \SideNS-\Cols}{automorphism}
имеет единственное решение. Согласно следствию
\RefCorollary{nonsingular rows system of linear equations}
матрица $f$ \ProductType невырожденна.
}

\DefLabeledTheorem{Automorphisms of vector space form a group}{\Product-\Cols}
{
Матрицы автоморфизмов \SideRu вого $A$\Hyph пространства \ColsA порождают группу \Group nA.
}

\DefProof{Automorphisms of vector space form a group}
{
Если даны два автоморфизма $\Vector f$ и $\Vector g$, то мы можем записать
\ShowEq{Automorphisms of vector space, \Product-\Cols}
Следовательно, результирующий автоморфизм имеет матрицу $f\ProductVal g$.
}

\DefLabeledTheorem{av=bv=>a=b}{\SideNS-\Cols}
{
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то из утверждения
\DrawEq{av=bv, v \SideNS}{\Cols}
следует, что $a=b$.
}

\DefProof{av=bv=>a=b}
{
Пусть множество векторов
\DrawEq[{}jJ]{basis e of module cols}-
является базисом левого $A$\Hyph векторного пространство $V$.
Согласно теоремам
\refTheorem{definition of A module, property}{\SideNS},
\refTheorem{coordinates of vector}{\SideNS-\Cols},
равенство
\ShowEq{avi=bvi \SideNS-\Cols}
является следствием равенства
\eqRef{av=bv, v \SideNS}{\Cols}.
Теорема следует из равенства
\EqRef{avi=bvi \SideNS-\Cols},
если мы положим $v=\aD e1$.
}

\DefText[7]{matrix of numbers}
{
Пусть
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
матрица $#1_{#2}$\Hyph чисел.
}

\DefText[9]{matrix of numbers and C}
{
Пусть
\ShowEq{matrix fIJ}{#3}{#4}{#5}{#6}{#7}
матрица $#1_{#2}$\Hyph чисел,
которая удовлетворяют равенству
\ShowRef{algebra, homomorphism and product}{#8}{#9}{#3}
}

\DefText{map be homomorphism of ring (1)}
{%
Пусть отображение
\DrawEq[h{D_1}{D_2}{}]{f: A->B}{}
является гомоморфизмом кольца $D_1$ в кольцо $D_2$.
}

\DefText{map be homomorphism of ring ()}
{%
}

\DefText{equality 11}
{
определённое равенствами
}

\DefText{equality 1}
{
определённое равенством
}

\DefText[7]{matrix generates A module homomorphism}
{
Отображение#7
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\ShowText{equality #2#3}
\ShowText{define homomorphism A module by matrix(#1#2#3)}
является гомоморфизмом
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$.
}

\DefLabeledTheorem[6]{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrices of numbers(#2#3)}{#4}{#5}{#1}{#2}%
\ShowText{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}
{\refFootnote{homomorphism of A module 2020}{\SideNS-\Cols(#1#2#3)}}
Гомоморфизм
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
который имеет%
\ShowText{define homomorphism by given matrix(#2)}%
определён однозначно.
}

\DefText{define homomorphism by given matrix(1)}
{
данное множество матриц $(g,f)$,
}

\DefText{define homomorphism by given matrix()}
{
данную матрицу $f$,
}

\DefText[4]{matrix generates homomorphism (1)}
{
Согласно теореме
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
\begin{sloppypar}
\noindent
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$
и гомоморфизм
\eqRef{homomorphism D algebra #1#2}{(\SideNS-\Cols)algebra}
определён однозначно.
\end{sloppypar}

}

\DefText[4]{matrix generates homomorphism ()}
{
}

\DefProof[7]{matrix generates A module homomorphism}
{
\ShowText{matrix generates homomorphism (#2)}{#1}{#2}{#4}{#5}
Равенство
\DrawEq{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)}
\begin{sloppypar}
\noindent
является следствием равенств
\ShowRef{matrix generates A module homomorphism(#2)}{#2}{#3}{#7}
Из равенства
\eqRef{fo(v+w) (#2)\SideNS-\Cols}{(#1#2)}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\DrawEq{fo(va) (#2)\SideNS-\Cols}{(#1#2)}
является следствием равенств
\ShowRef{fo(va)(#2)}{#2}{#3}{#7}
Из равенства
\eqRef{fo(va) (#2)\SideNS-\Cols}{(#1#2)},
и определений
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)}
следует, что отображение
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{\SideNS}
\newline
\begin{sloppypar}
\noindent
является гомоморфизмом
$A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$.
\end{sloppypar}

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}VW{}.%
Равенство
\ShowEq{fov=gov \SideNS-\Cols}
является следствием теоремы
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}.
Следовательно, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[6]{homomorphism A module}{\SideNS-\Cols(#1#2#3)}
{
Гомоморфизм\refFootnote{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}{}
\ShowText{f o (ae)=a o f e (#2#3)}{#1}{#2}{#3}
относительно выбранных базисов.
Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}{}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
\end{itemize}
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}{#5}
}

\DefLabeledTheorem[6]{homomorphism A module, Two bases of module}{\SideNS-\Cols(#1#2#3)}
{
Пусть отображение\refFootnote{homomorphism of A module 2020}{\SideNS-\Cols(#1#2#3)}
\DrawEq[g{\Vector f}]{homomorphism A module #1#2#3}{\SideNS-\Cols(#1#2#3)}
является гомоморфизмом
левого $A_{#2}$\Hyph модуля $V_{#3}$
в левый $A_{#5}$\Hyph модуль $V_{#6}$.
Пусть
\DrawEq{A homomorphism f}{\SideNS-\Cols(#1#2#3)}
матрица гомоморфизма
\eqRef{homomorphism A module #1#2#3}{\SideNS-\Cols(#1#2#3)}
\ShowText{relative bases #2#3}{#3}{#6}
Пусть отображение
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#3}{\SideNS-\Cols(#1#2#3)}
является гомоморфизмом
$D_{#1}$\Hyph модуля $V_{#3}$
в $D_{#4}$\Hyph модуль $V_{#6}$.
Пусть
\DrawEq{D homomorphism f}{\SideNS-\Cols(#1#2#3)}
матрица гомоморфизма
\eqRef{homomorphism D algebra #1#3}{\SideNS-\Cols(#1#2#3)}
\ShowText{relative extended bases #2#3}{#3}{#6}
Тогда
\DrawEq{f o eVA, Two bases}{\SideNS-\Cols(#1#2#3)}
где $A_{#5}$\Hyph числа
\ShowEq{AD homomorphism f}
удовлетворяют равенству
\DrawEq{f=f o eVA, Two bases}{\SideNS-\Cols(#1#2#3)}
}

\DefLabeledTheorem[6]{homomorphism A module 2020}{\SideNS-\Cols(#1#2#3)}
{
Гомоморфизм\refFootnote{homomorphism of A module 2020}{\SideNS-\Cols(#1#2#3)}
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}{}
\ShowText{f o (ae)=a o f e 2020(#2#3)}{#1}{#2}{#3}
относительно выбранных базисов.
Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}{}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
\end{itemize}
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}{#5}
}

\DefText[4]{matrix of homomorphism relative bases 11}
{
Для заданного гомоморфизма
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
множество матриц $(g,f)$ определено однозначно и называется
{\bf координатами гомоморфизма}
\eqRef{homomorphism A module #1#2#3}{\SideNS}
\ShowText{relative bases 11}{#2}{#4}
}

\DefText[2]{relative bases 11}
{
относительно базисов
\ShowEq{bases eA eV}{#1}1,
\ShowEq{bases eA eV}{#2}2.
}

\DefText[2]{relative extended bases 11}
{
относительно расширения базисов
\ShowEq{bases eA eV}{#1}1,
\ShowEq{bases eA eV}{#2}2.
}

\DefText[4]{matrix of homomorphism relative bases 1}
{
Для заданного гомоморфизма $\Vector f$
матрица $f$ определена однозначно и называется
{\bf матрицей гомоморфизма}
$\Vector f$
относительно базисов \eV[1][,] \eV[2][.]
}

\DefText[2]{relative bases 1}
{
относительно базисов
\ShowEq{bases eA eV}{#1}1,
\ShowEq{bases eA eV}{#2}2.
}

\DefText[2]{relative extended bases 1}
{
относительно расширения базисов
\ShowEq{bases eA eV}{#1}1,
\ShowEq{bases eA eV}{#2}2.
}

\DefText[6]{Proof, homomorphism of vector space(1)}
{
Согласно определениям
\ShowRef{Proof, homomorphism of vector space}{#1}{#2}{#3}%
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{}
\begin{sloppypar}
\noindent
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#4}$\Hyph алгебру $A_{#5}$.
Следовательно, равенства
\ShowRef{Proof, homomorphism of vector space 1}{#1}{#2}{#3}%
следуют из равенств
\ShowRef{Proof, homomorphism of vector space 2}{#1}{#2}{#3}{#4}%
Из теоремы
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
следует что матрица $g$ определена однозначно.
\end{sloppypar}

}

\DefText[6]{Proof, homomorphism of vector space()}
{%
}

\DefProof[6]{homomorphism A module}
{
\ShowText{Proof, homomorphism of vector space(#2)}{#1}{#2}{#3}{#4}{#5}{#6}%
Вектор
\ShowEq{vv in V}v{V_1}
имеет разложение
\DrawEq[v{V_1}]{\SideWS homomorphism \Product, 1}{v#1#2#3}
относительно базиса \eV[V_1][.]
Вектор
\ShowEq{vv in V}w{V_2}
имеет разложение
\DrawEq[w{V_2}]{\SideWS homomorphism \Product, 1}{w#1#2#3}
относительно базиса \eV[V_2][.]
Так кaк $\Vector f$ - гомоморфизм,
то равенство
\DrawEq{vv=v*eV \SideWS \Product(#2)}{(#1)}
является следствием равенств
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module},
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module}.
$V_2$\Hyph число
\ShowEq{Vector f(e) \Cols}
имеет разложение
\DrawEq{f o ei=fij ej \SideWS \Product}{#1#2#3}
относительно базиса \eV[V_2][.]
Равенство
\DrawEq{vb=a cr f cr e \SideWS \Product(#2)}{(#1)}
является следствием равенств
\eqRef{vv=v*eV \SideWS \Product(#2)}{(#1)},
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}.
Равенство
\eqRef{v1=v2*a \SideNS-\Cols}{\SideNS(#1#2#3)}
следует из сравнения
\eqRef{\SideWS homomorphism \Product, 1}{w#1#2#3}
и \eqRef{vb=a cr f cr e \SideWS \Product(#2)}{(#1)} и
теоремы 
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Из равенства
\eqRef{f o ei=fij ej \SideWS \Product}{#1#2#3}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
следует что матрица $f$ определена однозначно.
}

\DefText{notation for homomorphism of module}
{
Мы будем пользоваться записью
\DrawEq{f circ a =}{}
для образа гомоморфизма $f$.
}

\DefText{be division algebra}
{
Пусть $D$\Hyph алгебра $A$ является алгеброй с делением.
}

\DefTheorem{division algebra has unit}
{
\ShowText{be division algebra}
$D$\Hyph алгебра $A$ имеет единицу.
}

\DefProof{division algebra has unit}
{
Теорема является следствием утверждения, что уравнение
\ShowEq{ax=a}
имеет решение для любого $a\in A$.
}

\DefTheorem{division D algebra, ring D is the field}
{
\ShowText{be division algebra}
Кольцо $D$ является полем
и подмножеством центра $D$\Hyph алгебры $A$.
}

\DefProof{division D algebra, ring D is the field}
{
Пусть $e$ - единица $D$\Hyph алгебры $A$.
Так как отображение
\ShowEq{d->d1}
является вложением кольца $D$ в $D$\Hyph алгебру $A$,
то кольцо $D$ является подмножеством центра $D$\Hyph алгебры $A$.
}

\DefText[3]{homomorphism of vector space 2}
{
На основании теорем
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)}
мы идентифицируем гомоморфизм
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA и
координаты его представления
\ShowText{define homomorphism A module by matrix(#1#2#3)}
}

\DefLabeledDefinition{similarity transformation}{\SideNS}
{
Эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
называется
\AddIndex{преобразованием подобия}{similarity transformation}
относительно базиса $\Basis e$.
}

\AddEq{passive transformation for two bases}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
}

\DefLabeledTheorem{covariance of eigenvalue}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.

\begin{Statement}
\labelStatement{covariance of eigenvalue \SideNS-\Cols}
Собственное значение $b$
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}

\begin{Statement}
\labelStatement{covariance of eigenvector \SideNS-\Cols}
Собственный вектор $\Vector v$
эндоморфизма $\Vector f$,
соответствующий собственному значение $b$,
не зависит от выбора базиса $\Basis e_2$.
\hfill\(\odot\)
\end{Statement}
}

\DefProof{covariance of eigenvalue}
{
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Пусть $b$ - собственное значение
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
и
$\Vector v$ собственный вектор
эндоморфизма $\Vector f$,
соответствующее собственному значение $b$.
Пусть
\ShowEq{Ai, i=}v
- матрица вектора $\Vector v$ относительно базиса $\Basis e_i$.

Предположим сперва, что
\ShowEq{basis e1=e2}
Тогда базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $\aD En$
\DrawEq[12{\aD En^{}{}}{}]{e2i=aij e1j \Product-\Cols}{}
Согласно теореме
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}b1
имеет матрицу
\ShowEq{ga*g- \SideNS-En}
относительно базиса $\Basis e_2$.
Следовательно, согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
мы доказали следующие утверждения.

\begin{ShadedLemma}
\labelLemma{matrix f-bEn singular \SideNS-\Cols}
Матрица
\ShowEq{f-bEn \SideNS}1{}
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{ShadedLemma}
\labelLemma{vector v1 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_1$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v \Product-\Cols}
\hfill\(\odot\)
\end{ShadedLemma}

Предположим, что
\ShowEq{basis e1 ne e2}
Согласно теореме
\refTheorem{exists representation, commuting with active}{\SideNS-\Cols},
существует единственное пассивное преобразование
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
и $g$ - \ProductType невырожденая матрица.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{covariance \SideNS-\Cols}
\begin{sloppypar}
\noindent
Согласно теореме
\refTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols},
если $b$ - собственное значение эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{matrix f-ae singular \SideNS-\Cols}.
\end{sloppypar}

\begin{ShadedLemma}
\labelLemma{matrix f-ae singular \SideNS-\Cols}
Матрица
\[\ShowEq{(f-ae)v matrix}f2bg\]
\ProductType вырождена
\hfill\(\odot\)
\end{ShadedLemma}

\begin{sloppypar}
Так как равенство
\ShowEq{f-ae->f-be}
следует из равенства
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{matrix f-ae singular \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvalue \SideNS-\Cols}.
\end{sloppypar}

Согласно теореме
\refTheorem{eigenvector coordinates}{\SideNS-\Cols},
если $\Vector v$ - собственный вектор эндоморфизма $\Vector f$,
то мы должны доказать лемму
\RefLemma{vector v2 f-bEn \SideNS-\Cols}.

\begin{ShadedLemma}
\labelLemma{vector v2 f-bEn \SideNS-\Cols}
Вектор \ColWS $v_2$ удовлетворяет ситеме линейных уравнений
\ShowEq{(f-bEn)v2 \Product-\Cols}
\end{ShadedLemma}

\begin{sloppypar}
{\sc Доказательство.}
Согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{covariance \SideNS-\Cols}
Так как равенство
\ShowEq{f-ae->f-be \SideNS-\Cols}
следует из равенств
\eqRef{f2=a f1 a-}{covariance \SideNS-\Cols},
\eqRef{v2=v1g-}{covariance \SideNS-\Cols},
то лемма
\RefLemma{vector v2 f-bEn \SideNS-\Cols}
следует из леммы
\RefLemma{matrix f-bEn singular \SideNS-\Cols}.
\hfill\(\odot\)
\end{sloppypar}

Следовательно, мы доказали утверждение
\RefStatement{covariance of eigenvector \SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvalue of endomorphism, matrix is singular}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
относительно базиса $\Basis e_2$.
$A$\Hyph число $b$ является собственным значением
эндоморфизма $\Vector f$ тогда и только тогда, когда матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{\SideNS-\Cols}
\ProductType вырождена.
}

\DefProof{eigenvalue of endomorphism, matrix is singular}
{
Теорема является следствием теорем
\RefTheorem{star rows system of linear equations},
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\DefLabeledTheorem{eigenvector coordinates}{\SideNS-\Cols}
{
\ShowEq{passive transformation for two bases}
Пусть $f$ - матрица эндоморфизма $\Vector f$
и $v$ - матрица вектора $\Vector v$
относительно базиса $\Basis e_2$.
Вектор $\Vector v$ является
собственным вектором
эндоморфизма $\Vector f$
относительно базиса $\Basis e_1$
тогда и только тогда, когда
существует $A$\Hyph число $b$ такое, что
система линейных уравнений
\DrawEq[fgbv]{(f-ae)v \Product-\Cols}{fgbv}
имеет нетривиальное решение.
}

\DefProof{eigenvector coordinates}
{
Согласно теоремам
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)},
\refTheorem{similarity transformation, change of basis}{\SideNS-\Cols},
равенство
\ShowEq{e*f*v=e*ae*v \SideNS-\Cols}
является следствием равенства
\eqRef{fov=b e o v}{\SideNS}.
Равенство
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
является следствием равенства
\EqRef{e*f*v=e*ae*v \SideNS-\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
Так как равенство $\Vector v=0$ для нас не интересно,
система линейных уравнений
\eqRef{(f-ae)v \Product-\Cols}{fgbv}
должна иметь нетривиальное решение.
}

\AddEq{remark: eigenvector coordinates}
{
Определение
\refDefinition{Eigenvalue of Endomorphism}{\SideNS}
не зависит от структуры координат
\SideRu вого $A$\Hyph векторного пространства $V$.
Когда мы выбираем базис $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$,
мы видим дополнительную структуру,
которая отражена в теоремах
\refTheorem{eigenvector coordinates}{\SideNS-cols},
\refTheorem{eigenvector coordinates}{\SideNS-rows}.
}

\AddEq{remark: eigenvector of matrix}
{
Одна и таже матрица может соответствовать различным эндоморфизмам
в зависимости рассматриваем ли мы левое или правое
$A$\Hyph векторного пространство.
Поэтому мы должны рассмотреть все определения
собственных векторов, которые могут соответсвовать данной матрице.
Из теорем
\refTheorem{eigenvector coordinates}{left-cols},
\refTheorem{eigenvector coordinates}{right-cols},
\refTheorem{eigenvector coordinates}{left-rows},
\refTheorem{eigenvector coordinates}{right-rows}
следует, что для данной матрицы существует
четыре вида собственных векторов и
четыре вида собственных чисел.
Пара собственный вектор и собственное значение определённого вида
используется в решении задачи,
где возникает соответствующий вид $A$\Hyph векторного пространства.
Это утверждение отражено в названии
собственного вектора и собственного значения.

Собственный вектор эндоморфизма зависит от
выбора двух базисов. Однако когда мы
рассматриваем собственный вектор матрицы,
для нас важен не выбор базисов,
а матрица пассивного преобразования между этими базисами.
}

\DefLabeledDefinition{eigenvalues of pair of matrices}{\Product}
{
$A$\Hyph число $b$ называется
{\bf \ProductType собственным значением}
пары матриц $(f,g)$,
где $g$ - \ProductType невырожденная матрица,
если матрица
\DrawEq[f{}bg]{(f-ae)v matrix}{}
\ProductType вырожденная матрица.
}

\DefLabeledDefinition{eigenvector of pair of matrices}{\Product-\ColN}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
\ColC $v$ называется
{\bf собственн\ColB}
пары матриц $(f,g)$, соответствующ\FinB \ProductType собственному значению $b$,
если верно равенство
\DrawEq{\Product-eigen\Cols(f,g)}{}
}

\AddEq{proof: eigencolumn of matrix}
{
Определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{proof: eigenrow of matrix}
{
Поскольку
\ShowEq{bg.\Product.g-}
то определение
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN}
является следствием определения
\refDefinition{eigenvalues of pair of matrices}{\Product}
и теоремы
\refTheorem{eigenvector coordinates}{\SideNS-\Cols}.
}

\AddEq{theorem: representation Ao2->V}
{
\begin{ShadedTheorem}
\labelTheorem{representation Ao2->V \SideNS}
Пусть $f$, $g(\Basis e)$
парные представления $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Тогда представление
\ShowEq{representation Ao2->V}
$D$\Hyph алгебры \AoxA A в $D$\Hyph модуле $V$
определеное равенством
\ShowEq{representation Ao2->V =}
является левым \AoxA A\Hyph модулем.
\end{ShadedTheorem}
}

\AddEq{theorem: twin representation in vector space}
{
\begin{ShadedTheorem}
\labelTheorem{twin representation in \SideWS vector space}
\ShowEq{Let V be vector space}{}
\ShowEq{f:A->*B}fAV
Эффективное \OtherSideRu востороннее представление
\ShowEq{f:A->*B}{g(\Basis e)}AV
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$
зависит от базиса $\Basis e$ \SideRu вого $A$\Hyph векторного пространства $V$.
Следующая диаграмма
\newline
\DrawEq{twin representations of algebra}{\SideNS}
коммутативна для любых $a$, $b\in A$.
\end{ShadedTheorem}
}

\DefProof{twin representation in vector space}
{
Коммутативность диаграммы
\eqRef{twin representations of algebra}{\SideNS}
является следствием равенства
\eqRef{(av)b=a(vb)}{\SideNS}.
}

\DefLabeledDefinition{twin representation in vector space}{\SideNS}
{
Мы будем называть представления $f$ и $g(\Basis e)$,
рассмотренные в теореме
\RefTheorem{twin representation in \SideWS vector space},
{\bf парными представлениями}
$D$\Hyph алгебры $A$.
Равенство
\eqRef{(av)b=a(vb)}{\SideNS}
представляет
{\bf закон ассоциативности}
для парных представлений.
Это позволяет нам писать подобное выражение не пользуясь скобками.
}

\DefLabeledTheorem{set of similarity transformations}{\SideNS}
{
Пусть $V$ - \SideRu\-вое $A$\Hyph векторное пространство столбцов
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
Множество преобразований подобия
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$
является \OtherSideRu восторонним эффективным представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefProof{set of similarity transformations}
{
Рассмотрим множество матриц
\ShowEq{\SideWS a En}
преобразований подобия
\ShowEq{\SideWS map a En}a{}
относительно базиса $\Basis e$.
Пусть $V^*$ - множество координат $V$\Hyph чисел
относительно базиса $\Basis e$.
Согласно теоремам
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows},
множество $V^*$ является \SideRu вым $A$\Hyph векторным пространством.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
отображение
\ShowEq{\SideWS map a En}a{}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства столбцов.

\ColRowLemma{map a in A->aE in hom is homomorphism}

\ColRowProof{map a in A->aE in hom is homomorphism}

\ColRowProof{set of similarity transformations 1}
}

\AddEq{proof: set of similarity transformations 1}
{
Согласно определению
\refDefinition{side representation of group}{\SideNS}
и лемме
\refLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols},
отображение
\eqRef{a in A->aE hom \SideNS}{\Cols}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V^*$.
Согласно теореме
\RefTheorem{division algebra},
из равенства
\ShowEq{aEn=bEn \SideNS}
следует, что $a=b$.
Согласно определению
\RefDefinition{effective representation of algebra},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
эффективно.

Согласно теоремам
\refTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols},
\RefTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols},
представление
\eqRef{a in A->aE hom \SideNS}{\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
Согласно теореме
\refTheorem{similarity transformation}{\SideNS-\Cols}
множество отображений
\ShowEq{\SideWS map a En}a{}
является \OtherSideRu восторонним представлением
$D$\Hyph алгебры $A$
в \SideRu вом $A$\Hyph векторном пространстве $V$.
}

\DefLabeledLemma{map a in A->aE in hom is homomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Отображение
\DrawEq{a in A->aE hom \SideNS}{\Cols}
является гомоморфизмом $D$\Hyph алгебры $A$.
}

\AddEq{proof: map a in A->aE in hom is homomorphism}
{
{\sc Доказательство.}
Согласно теореме
\refTheorem{homomorphism from A1 to A2, D algebra}1,
лемма является следствием равенств
\ShowEq{(a+b)aE \SideNS}
\ShowEq{(daE)v \SideNS}
\ShowEq{(ab)E \SideNS-\Cols}
\hfill\(\odot\)
}

\DefText{passive transformation and endomorphism}
{
Мы рассмотрим преобразование координат эндоморфизма
\SideRu вого $A$\Hyph векторного пространства \ColsA
в теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.
}

\DefLabeledTheorem{passive transformation and endomorphism}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
$\Basis e_1$, $\Basis e_2$ - базисы в \SideRu вом $A$\Hyph векторном пространстве $V$.
Пусть базисы $\Basis e_1$, $\Basis e_2$ связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}%g
Пусть $f$ - эндоморфизм \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $f$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[fg{\SideNS}{\Cols}]{f2=a f1 a-}{g \SideNS-\Cols}
}

\AddEq[1]{remark: passive transformation and endomorphism}
{
Пусть
\ShowEq{Ai, i=}{#1}
- матрица вектора $#1$ относительно базиса $\Basis e_i$.
Тогда
\DrawEq[{#1}1{#1}2g{}]{v1=v2*a \SideNS-\Cols}{#1}
следует из теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{proof: passive transformation and endomorphism}
{
{\sc Доказательство теоремы
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols}.}
Пусть эндоморфизм $f$ отображает вектор $v$ в вектор $w$
\DrawEq{w=f o v}{\SideNS-\Cols}
\ShowEq{passive transformation and endomorphism}

Согласно теореме
\refTheorem{homomorphism A module 2020}{\SideNS-cols(1)},
равенства
\DrawEq[w1v1f1]{v1=v2*a \SideNS-\Cols}{v1}
\DrawEq[w2v2f2]{v1=v2*a \SideNS-\Cols}{v2}
являются следствием равенства
\eqRef{w=f o v}{\SideNS-\Cols}.
Равенство
\DrawEq[g]{w2=...v2 a f1 \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}v,
\eqRef{v1=v2*a \SideNS-\Cols}{v1},
\eqRef{v1=v2*a \SideNS-\Cols}w.
Так как $g$ - невырожденная матрица,
то равенство
\DrawEq[g]{w2=...v2 a f1 a- \SideNS-\Cols}g
является следствием равенства
\eqRef{w2=...v2 a f1 \SideNS-\Cols}g.
Равенство
\DrawEq[g]{v2 f2=v2 a f1 a- \SideNS-\Cols}g
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v2},
\eqRef{w2=...v2 a f1 a- \SideNS-\Cols}g.
Равенство
\eqRef{f2=a f1 a-}{g \SideNS-\Cols}
является следствием равенства
\eqRef{v2 f2=v2 a f1 a- \SideNS-\Cols}g.
\qed
}

\DefText[2]{coordinates of vector with respect to basis (1,2) cols}
{
Пусть
\DrawEq[{#1_i}n]{a=(a1.n col)}{#2,\SideNS-\Cols}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\DefText[2]{coordinates of vector with respect to basis (1,2) rows}
{
Пусть
\ShowEq{phantom a**b}
\DrawEq[{#1_i^{}{}}n]{a=(a1.n row)}{}
\ShowEq{phantom a**b}
матрица координат вектора $\Vector{#1}$
относительно базиса
\ShowEq{Basis e i=1#2}
}

\AddEq[2]{convention: passive transformation maps the basis 1->2}
{%
Пусть пассивное преобразование $g\in #1$ отображает базис \eV[1]
в базис \eV[2]
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{12 #2}
}

\DefLabeledTheorem{passive transformation of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowConvention{passive transformation maps the basis 1->2}{G(V_*)}1
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v2
Преобразования координат
\DrawEq[v1v2g{}]{v1=v2*a \SideNS-\Cols}{v21g}
\DrawEq[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
не зависят от вектора $\Vector v$ или базиса $\Basis e$, а
определенно исключительно координатами вектора $\Vector v$
относительно базиса $\Basis e$.
}

\DefProof{passive transformation of vector space}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
\ShowEq{v=vi ei 12, \SideNS-\Cols}
Равенство
\ShowEq{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}
является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{12 1},
\EqRef{v=vi ei 12, \SideNS-\Cols}.
Согласно теореме
\refTheorem{coordinates of vector}{\SideNS-\Cols},
преобразование координат
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}
является следствием равенства
\EqRef{v1 cr e1=v2 cr g cr e1, \SideNS-\Cols}.
Так как $g$ - \ProductType невырожденная матрица, то
преобразование координат
\eqRef{v2=v1g-}{12 \SideNS-\Cols}
является следстием равенства
\eqRef{v1=v2*a \SideNS-\Cols}{v21g}.
}

\DefLabeledTheorem{passive transformation and sum of endomorphisms}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$ является суммой эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна сумме матриц $f_1$, $f_2$ эндоморфизмов
$\Vector f_1$, $\Vector f_2$
и это равенство не зависит от выбора базиса.
}

\AddEq{two endomorphisms and two bases}
{
Пусть $\Basis e$, $\Basis e'$ - базисы \SideRu вого $A$\Hyph векторного пространства $V$
и связаны пассивным преобразованием $g$
\ShowEq{\SideWS e'=e*a}{}
Пусть $f$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e$.
Пусть $f'$
- матрица эндоморфизма $\Vector f$ относительно базиса $\Basis e'$.
Пусть
\ShowEq{Ai, i=}f
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e$.
Пусть
\ShowEq{Ai, i=}{f'}
- матрица эндоморфизма $\Vector f_i$ относительно базиса $\Basis e'$.
}

\DefProof{passive transformation and sum of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\refTheorem{sum of homomorphisms, A vector space}{\SideNS-\Cols},
\DrawEq[{}{}]{f=f1+f2 endo}{\SideNS-\Cols}
\DrawEq[{'}{}]{f=f1+f2 endo}{\SideNS-\Cols'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}f
\DrawEq[1]{f'=g f g- \SideNS-\Cols}1
\DrawEq[2]{f'=g f g- \SideNS-\Cols}2
Равенство
\ShowEq{f1+f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1+f2=g.g-}
Из равенств
\eqRef{f=f1+f2 endo}{\SideNS-\Cols'},
\EqRef{f1+f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1+f2 endo}{\SideNS-\Cols}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: passive transformation and product of endomorphisms}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation and product of endomorphisms, vector space, \SideNS-\Cols}
\ShowEq{Let V be vector space of}.
Пусть эндоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства $V$
является произведением эндоморфизмов
$\Vector f_1$, $\Vector f_2$.
Матрица $f$ эндоморфизма $\Vector f$ равна
\ProductType произведению матриц
\ShowEq{f1 f2 \SideNS}
эндоморфизмов
\ShowEq{vf1 vf2 \SideNS}
и это равенство не зависит от выбора базиса.
\end{ShadedTheorem}
}

\DefLabeledDefinition{coordinates of geometric object, vector space}{\SideNS-\Cols}
{
Мы будем называть
орбиту
\ShowEq{def coordinates of geometric object, \SideNS-\Cols}
представления $F_1$
многообразием {\bf координат геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса
\newline
\FrameEqRef[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\newline
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
орбиты  определяет
{\bf координаты геометрического объекта}
в координатном \SideRu вом $A$\Hyph векторном пространстве
относительно базиса \eV[V2].
}

\DefLabeledDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
{
Пусть $a_2$ - \nTimes матрица,
которая \ProductType подобна диагональной матрице $a_1$
\ShowEq{D diagonal matrix}{a_1}n
Следовательно, существует \ProductType невырожденая матрица $u_2$ такая, что
\DrawEq{U-*A*U=D \Product-\SideNS}1
\DrawEq[2{2}{a_1}]{A \ProductS U=U \ProductS D \SideNS}1
\ColC
\ShowEq{ARow u2i \Cols}u2i
матрицы $u_2$ удовлетворяет равенству
\DrawEq[2u]{A*Ui=Ui di \Product-\SideNS}u
$A$\Hyph число $b(\gi i)$ называется \SideRu вым \ProductType {\bf собственным значением}.
Вектор\Hyph\ColWS
\ShowEq{ARow u2i \Cols}u2i
называется
\AddIndex{собственн\ColBNS}{eigen\ColN},
соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$.
}

\DefLabeledTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
{
Собственный вектор
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
не зависит от выбора базиса $\Basis e_2$
\ShowEq{e1i=u2i*e2 \SideNS-\Cols}
}

\AddEq{remark: Eigenvector does not depend on basis}
{
Равенство
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
является следствием равенства
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}.
Однако смысл этих равенств различный.
Равенство
\eqRef{e2i=aij e1j \Product-\Cols}{21u2}
является представлением пассивного преобразования.
Мы видим
в равенстве
\EqRef{e1i=u2i*e2 \SideNS-\Cols}
разложение собственного вектора
для данного \SideRu вого \ProductType собственного значения относительно выбранного базиса.
Задача доказательства теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
- раскрыть смысл равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefProof{Eigenvector does not depend on basis}
{
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)},
мы можем рассматривать матрицу $a_2$ как матрицу автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_2$.
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
матрица $u_2$ является матрицей пассивного преобразования
\DrawEq[21u2]{e2i=aij e1j \Product-\Cols}{21u2}
и матрица $a_1$ является матрицей автоморфизма $a$
\SideRu вого $A$\Hyph векторного пространства относительно базиса $\Basis e_1$.

Матрица координат базиса $\Basis e_1$ относительно базиса $\Basis e_1$
- это единичная матрица $\aD En$.
Следовательно, вектор
\ShowEq{ARow u2i \Cols}e1i
является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b(\gi i)$
\DrawEq[1e]{A*Ui=Ui di \Product-\SideNS}e
Равенство
\ShowEq{U-*A*U*E=E*D \Product-\SideNS}
является следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\eqRef{A*Ui=Ui di \Product-\SideNS}e.
Равенство
\ShowEq{A*U*E=U*E*D \Product-\SideNS}
является следствием равенства
\EqRef{U-*A*U*E=E*D \Product-\SideNS}.
Равенство
\ShowEq{U*Ei=Ui \Product-\SideNS}
является следствием равенств
\eqRef{A*Ui=Ui di \Product-\SideNS}u,
\EqRef{A*U*E=U*E*D \Product-\SideNS}.
Теорема является следствием равенств
\eqRef{e2i=aij e1j \Product-\Cols}{21u2},
\EqRef{U*Ei=Ui \Product-\SideNS}.
}

\DefLabeledTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Любое \SideRu вое \ProductType собственное значение $b(\gi i)$
является \ProductType собственным значением.
Собственн\ColumnC $\ARow ui$,
соответствующ\endC \SideRu вому \ProductType собственному значению $b(\gi i)$,
является собственн\ColBNS,
соответствующ\FinB \ProductType собственному значению $b(\gi i)$.
}

\DefProof{right eigenvalue is eigenvalue}
{
Все элементы строки матрицы
\DrawEq{a1-di En}{\Product-\SideNS}
равны нулю.
Следовательно, матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена
и \SideRu вое \ProductType собственное значение $b(\gii)$
является \ProductType собственным значением.
Поскольку
\DrawEq{e1ij=01 \Cols}{\SideNS}
то собственный вектор
\ShowEq{ARow u2i \Cols}e1i,
соответствующий \SideRu вому \ProductType собственному значению $b(\gii)$,
является собственным вектором, соответствующим \ProductType собственному значению $b(\gii)$.
Равенство
\ShowEq{a1*e1=di e1 \Product-\SideNS}
является следствием определения
\refDefinition{eigenvector of matrix}{\Product-\Cols}.

Из равенства
\eqRef{U-*A*U=D \Product-\SideNS}1
следует, что мы можем записать матрицу
\eqRef{a1-di En}{\Product-\SideNS}
в виде
\ShowEq{U-*A*U-di En \Product-\SideNS}
Так как матрица
\eqRef{a1-di En}{\Product-\SideNS}
\ProductType вырождена,
то матрица
\ShowEq{A-U-*di*U \Product-\SideNS}
также \ProductType вырождена.
Следовательно,
\SideRu вое \ProductType собственное значение $b(\gii)$ матрицы $a_2$
является \ProductType собственным значением
пары матриц $(a_2,u_2)$.

Равенства
\ShowEq{U-*A*U*e1=di e1 \Product-\SideNS}
\ShowEq{A*U*e1=... \Product-\SideNS}
являются следствием равенств
\eqRef{U-*A*U=D \Product-\SideNS}1,
\EqRef{a1*e1=di e1 \Product-\SideNS}.
Из равенств
\EqRef{e1i=u2i*e2 \SideNS-\Cols},
\EqRef{A*U*e1=... \Product-\SideNS}
и из теоремы
\refTheorem{Eigenvector does not depend on basis}{\SideNS-\Cols}
следует, что
собственн\ColumnC
\ShowEq{ARow u2i \Cols}u2i
матрицы $a_2$,
соответствующий \SideRu вому \ProductType собственному значению $b(\gi i)$,
является
собственн\ColB
\ShowEq{ARow u2i \Cols}u2i
пары матриц $(a_2,u_2)$, соответствующ\FinB \ProductType собственному значению $b(\gii)$.
}

\DefLabeledRemark{right eigenvalue is eigenvalue}{\SideNS-\Cols}
{
Равенство
\ShowEq{di*ui=ui*di \Product-\SideNS}
является следствием теоремы
\refTheorem{right eigenvalue is eigenvalue}{\SideNS-\Cols}.
Равенство
\EqRef{di*ui=ui*di \Product-\SideNS}
кажется необычным.
Однако, если мы его слегка изменим
\ShowEq{di*ui=ui*di 1 \Product-\SideNS}
то равенство
\EqRef{di*ui=ui*di 1 \Product-\SideNS}
следует из равенства
\EqRef{e1i=u2i*e2 \SideNS-\Cols}.
}

\DefLabeledTheorem[1]{Eigenvalue a ox a, c in AAA[b]}{\SideNS-\Cols}
{
Пусть вектор\Hyph\ColWS $v$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
Пусть $A$\Hyph число $b$ удовлетворяет условию
\DrawEq[b{}{s#1}]{b in AAA[a]}{bs#1-\Cols}
Тогда
для любого многочлена
\DrawEq{p(c) p in D}{\SideNS-\Cols}
вектор\Hyph\ColWS
\ShowEq{eigenvector cv \SideNS-\Cols}
\ShowEq{c=p(b)}
также является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefProof[2]{Eigenvalue a ox a, c in AAA[b]}
{
Согласно теореме
\RefTheorem{c in Za=> p(c) in Za},
равенство
\ShowEq{as ox as o cv = ..., \SideNS-\Cols}
является следствием условия
\eqRef{b in AAA[a]}{bs#1-\Cols}.
Согласно определению
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols},
из равенства
\EqRef{as ox as o cv = ..., \SideNS-\Cols}
следует, что
вектор\Hyph\ColWS $#2$ является
собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$
матрицы $a$.
}

\DefLabeledDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
{
$A$\Hyph число $b$ называется
\SideRu вым \ProductTypeO {\bf собственным значением}
матрицы $a$,
если существует вектор\Hyph\ColWS $v$ такой, что
\DrawEq[v]{Eigenvalue of Linear Map \SideNS-\Cols}d
Вектор\Hyph\ColWS $v$ называется
{\bf собственн\ColBNS}, соответствующ\FinB \SideRu вому \ProductTypeO собственному значению $b$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \SideRu вым \ProductType собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 1}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{1-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{1-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
и определения
\refDefinition{Left and Right Eigenvalues}{\SideNS-\Cols}
\SideRu вого \ProductType собственного значения
матрицы $a_{#1}$.
}

\DefLabeledTheorem[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Пусть элементы матрицы $a$ удовлетворяют равенству
\DrawEq{as ox as=a1 ox a2, #1}{\SideNS-\Cols}
Тогда \SideRu вое \ProductTypeO собственное значение $b$
является \ProductTypeA собственным значением матрицы $a_{#1}$.
}

\DefProofRef[1]{Eigenvalue of Linear Map a ox a, 2}{\SideNS-\Cols}
{
Равенство
\DrawEq{as ox as o v = v a12, #1, \Cols}{2-\SideNS}
является следствием равенства
\FrameEqRef{as ox as=a1 ox a2, #1}{\SideNS-\Cols}.
\newline
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols}
является следствием равенства
\eqRef{as ox as o v = v a12, #1, \Cols}{2-\SideNS}.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}
является следствием определения
\refDefinition{Eigenvalue of Matrix of Linear Map}{\SideNS-\Cols}
\SideRu вого \ProductTypeO собственного значения
матрицы $a$.
Равенство
\ShowEq{as ox as o v = v a12, matrix, #1 \SideNS-\Cols}
является следствием равенств
\EqRef{as ox as o v = v a12, matrix, #1 1 \SideNS-\Cols},
\EqRef{as ox as o v = v a12, matrix, #1 2 \SideNS-\Cols}.
Теорема является следствием равенства
\EqRef{as ox as o v = v a12, matrix, #1 \SideNS-\Cols},
определения
\refDefinition{eigenvalue of matrix}{\ProductA}
\ProductType собственного значения
матрицы $a_{#1}$
и определения
\refDefinition{eigenvector of matrix}{\ProductA-\Cols}
соответствующего собственного вектора $v$.
}

\DefLabeledTheoremNote[1]{n eigenvectors}{#1}
{
Пусть $\Base$ - \AlgebraRu
и $V$ - $\Base$\Hyph векторное пространство.
Если эндоморфизм имеет $\gik$ различных
собственных значений\,\footnotemark
\ShowEq{di 1n}bk,
то собственные вектора
\ShowEq{di 1n}vk,
относящиеся к различным собственным значениям,
линейно независимы.
}
{
Смотри также теорему на странице
\citeBib{Kurosh: High Algebra}\Hyph 210.
}

\AddEq{remark: n eigenvectors}
{
Однако теорема
\refTheorem{n eigenvectors}{algebra}
не верна.
Мы рассмотрим отдельно доказательства
для левого и правого $A$\Hyph векторного пространств.
}

\DefProof{n eigenvectors}
{
Мы будем доказывать теорему индукцией по $\gik$.

Поскольку собственный вектор отличен от нуля, теорема верна для $\gik=\gi 1$.

\begin{Statement}
\labelStatement{theorem is true for k=m-1 \SideNS}
Пусть теорема верна для $\gik=\gim-\gi 1$.
\hfill\(\odot\)
\end{Statement}

\begin{sloppypar}
Согласно теоремам
\ShowEq{ref 1 for n eigenvectors}
мы можем положить, что
\ShowEq{e2=e1}
Пусть
\ShowEq{di 1n+1}bm{}
- различные собственные значения и
\ShowEq{di 1n+1}vm{}
- соответствующие собственные векторы
\ShowEq{fovi=di vi \SideNS}
\ShowEq{di ne dj}
Пусть утверждение
\RefStatement{ai vi=0 \SideNS}
верно.
\end{sloppypar}

\begin{Statement}
\labelStatement{ai vi=0 \SideNS}
Существует линейная зависимость
\ShowEq{ai vi=0 \SideNS}
где
\ShowEq{a1 ne 0}
\hfill\(\odot\)
\end{Statement}

Равенство
\ShowEq{ai f vi=0 \SideNS}
является следствием равенства
\EqRef{ai vi=0 \SideNS}
и теоремы
\ShowEq{ref 2 for n eigenvectors}
Равенство
\ShowEq{ai di vi=0 \SideNS}
является следствием равенств
\EqRef{fovi=di vi \SideNS},
\EqRef{ai f vi=0 \SideNS}.
Так как произведение не коммутативно,
мы не можем упростить выражение
\EqRef{ai di vi=0 \SideNS}
до линейной зависимости.
}

\AddEq{remark: Eigenvalue and conjugate class}
{
Из теорем
\refTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols},
\refTheorem{Coefficient comutes with matrix}{\SideNS-\Cols}
следует, что множество собственных \ColsNA,
соответствующих данному \SideRu вому \ProductType собственному значению,
не является $A$\Hyph векторным пространством.
}

\DefLabeledTheorem{Eigenvalue and conjugate class}{\SideNS-\Cols}
{
Пусть $A$\Hyph число $b$ - \SideRu вое \ProductType собственное значение матрицы
$a_2$.\refFootnote{Eigenvalue and conjugate class}{\Product}
Тогда любое $A$\Hyph число, $A$\Hyph сопряжённое с $A$\Hyph числом $b$,
является \SideRu вым \ProductType собственным значением матрицы $a_2$.
}

\DefLabeledFootnote{Eigenvalue and conjugate class}{\Product}
{
Смотри аналогичное утверждение и доказательство на странице
\citeBib{Cohn: Skew Fields}\Hyph 375.
}

\DefProof{Eigenvalue and conjugate class}
{
Пусть $v$ -
собственн\ColumnCNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$.
Пусть $c\ne 0$ - $A$\Hyph число.
Утверждение теоремы является следствием равенства
\ShowEq{conjugate eigenvalue \SideNS-\Cols}
}

\DefLabeledTheorem[2]{Coefficient comutes with matrix}{\SideNS-\Cols}
{
Пусть $v$ - собственн\ColumnCNS, соответствующ\endC \SideRu вому \ProductType собственному значению $b$.
Вектор $#1#2$
является собственн\ColB, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefProof[2]{Coefficient comutes with matrix}
{
Вектор $#1#2$
является собственн\ColBNS, соответствующ\FinB \SideRu вому \ProductType собственному значению $b$
тогда и только тогда, когда
верно следующее равенство
\ShowEq{Coefficient comutes with matrix \SideNS-\Cols}
Равенство
\EqRef{Coefficient comutes with matrix \SideNS-\Cols}
верно тогда и только тогда, когда
$A$\Hyph число $c$ коммутирует со всеми элементами матрицы $a_2$.
}

\DefLabeledDefinition{geometric object, vector space}{\SideNS-\Cols}
{
Допустим даны координаты $w_1$ вектора $\Vector w$
относительно базиса  \eV[W1][.]
Мы будем называть
множество векторов
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we}
{\bf геометрическим объектом},
определённым в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA.
Для любого базиса  \eV[W2][,]
соответствующая точка
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
многообразия координат определяет вектор
\DrawEq[w2{w_2}{W2}]{geometric object representative, \SideNS-\Cols}{w=we 1}
который называется
{\bf представителем геометрического объекта}
в \SideRu вом $A$\Hyph векторном пространстве $V$ в базисе \eV[V2][.]
}

\AddEq{remark: geometric object, vector space}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Мы будем также говорить, что $\Vector w$ - это
\AddIndex{геометрический объект типа $F$}{type of geometric object}.

Определения
\refDefinition{coordinates of geometric object, vector space}{\SideNS-cols},
\refDefinition{coordinates of geometric object, vector space}{\SideNS-rows}
строят геометрический объект в координатном пространстве.
Определения
\refDefinition{geometric object, vector space}{\SideNS-cols},
\refDefinition{geometric object, vector space}{\SideNS-rows}
предполагают,
что мы выбрали базис в векторном пространстве $W$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\DefText{Geometric Object of Vector Space}
{
\begin{sloppypar}
Предположим, что $V$, $W$ - \SideRu вые $A$\Hyph векторные пространства \ColsA.
Пусть $G(V_*)$ -  группа симметрий
\SideRu вого $A$\Hyph векторного пространства $V$.
Гомоморфизм
\DrawEq[F{G(V_*)}{GL(W_*)}{}]{f: A->B}{FG \SideNS-\Cols}
отображает пассивное преобразование $g\in G(V_*)$
\DrawEq[{V1}{V2}g{}]{e2i=aij e1j \Product-\Cols}{GOeV}
\SideRu вого $A$\Hyph векторного пространства $V$
в пассивное преобразование
\ShowEq{Fg in GL}
\DrawEq[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\SideRu вого $A$\Hyph векторного пространства $W$.
\end{sloppypar}

Тогда координатное преобразование в
\SideRu вом $A$\Hyph векторном пространстве $W$ принимает вид
\DrawEq{coordinate transformation, vector space W, \SideNS-\Cols}1
Следовательно, отображение
\DrawEq{F1(g)=F(g)**-\Product}{\SideNS}
является \OtherSideRu восторонним представлением
\ShowEq{f:A->*B}{F_1}{G(V_*)}{W_*}
группы $G(V_*)$ на множестве $W_*$.
}

\DefProof{passive transformation and product of endomorphisms}
{
\ShowEq{two endomorphisms and two bases}
Согласно теореме
\refTheorem{product of homomorphisms, A vector space}{\SideNS-\ColN},
\DrawEq[{}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product}
\DrawEq[{'}{}]{f=f1*f2 endo \SideNS-\Cols}{\Product'}
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
\DrawEq[{}{}]{f'=g f g- \SideNS-\Cols}{f*}
\DrawEq[1]{f'=g f g- \SideNS-\Cols}{1*}
\DrawEq[2]{f'=g f g- \SideNS-\Cols}{2*}
Равенство
\ShowEq{f1*f2=g.g- \SideNS-\Cols}
является следствием равенств
\ShowEq{f1*f2=g.g-}
Из равенств
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product'},
\EqRef{f1*f2=g.g- \SideNS-\Cols}
следует, что равенство
\eqRef{f=f1*f2 endo \SideNS-\Cols}{\Product}
ковариантно относительно выбора базиса
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{theorem: finite dimension->representation is free}
{
\begin{ShadedTheorem}
\labelTheorem{finite dimension->representation is free, \SideNS}
Если \SideRu вое $A$\Hyph векторное пространство $V$
имеет конечную размерность,
то соответствующее представление свободно.
\end{ShadedTheorem}
}

\DefProof{finite dimension->representation is free}
{
Теорема является следствием определения
\RefDefinition{free representation of algebra}
и теорем
\refTheorem{av=bv=>a=b}{\SideNS-cols},
\refTheorem{av=bv=>a=b}{\SideNS-rows}.
}

\AddEq[1]{Let V be vector space}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство#1
}

\AddEq[1]{Let V be vector space of}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsNA#1
}

\AddEq{Let V be vector space of and}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство \ColsA и
}

\AddEq{Let V be vector space of and basis}
{
\ShowEq{Let V be vector space of and}
$\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{Let V be vector space and basis}
{
\ShowEq{Let V be vector space}{}
и $\Basis e$ - базис \SideRu вого $A$\Hyph векторного пространства $V$.
}

\AddEq{remark: automorphism of vector space, group}
{
\ShowEq{Let V be vector space of}.
Мы доказали в теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
что если задан базис
\SideRu вого $A$\Hyph векторного пространства $V$,
то любой автоморфизм $\Vector f$
\SideRu вого $A$\Hyph векторного пространства $V$ можно отождествить
с \ProductType невырожденной матрицей $f$.
Соответствующее преобразование координат вектора
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{}
называется
\AddIndex{линейным преобразованием}{linear transformation}.
}

\DefLabeledDefinition{Symmetry Group}{\SideNS-\Cols}
{
Нормальная подгруппа $G(V)$ группы $GL(V)$, которая порождает
автоморфизмы, сохраняющие свойства заданной структуры
называется
{\bf группой симметрии}.

Не нарушая общности, мы будем отождествлять элемент $g$ группы $G(V)$
с соответствующим автоморфизмом
и записывать его действие на вектор $v\in V$ в виде
\ShowEq{v*g, \SideNS-\Cols}
}

\DefText{definition: linear G* representation}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G$ в \SideRu вом $A$\Hyph векторном пространстве
\AddIndex{линейным $G$\Hyph представлением}{linear G* representation}.
}

\DefText{linear G* representation}
{
Если в \SideRu вом $A$\Hyph векторном пространстве $V$ определена дополнительная структура,
не всякий автоморфизм сохраняет свойства заданной структуры.
Например, если мы определим норму в
\SideRu вом $A$\Hyph векторном пространстве $V$,
то для нас интересны автоморфизмы, которые сохраняют норму вектора.
}

\DefLabeledDefinition{active G-representation}{\SideNS}
{
Мы будем называть \OtherSideRu востороннее представление
группы $G(V)$ на множестве базисов \SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным \SideRu восторонним $G$\Hyph представлением}
{active representation, vector space}.
}

\DefText{active G-representation}
{
Если базис \eV задан, то
мы можем отождествить автоморфизм
\SideRu вого $A$\Hyph векторного пространства $V$
и его координаты относительно базиса \eV[][.]
Множество $G(V_*)$ координат автоморфизмов
относительно базиса \eV является группой,
изоморфной группе $G(V)$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G(V)$.
Таким образом, множество базисов
можно представить как объединение орбит группы $G(V)$.
В частности, если базис $\eV\in G(V)$,
то орбита базиса \eV совпадает с группой $G(V)$.
}

\DefLabeledTheorem{representation on basis manifold, vector space}{\SideNS}
{
Активное \OtherSideRu востороннее $G(V)$\Hyph представление на многообразии базисов
однотранзитивно.
}

\DefProof{representation on basis manifold, vector space}
{
Теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
и определений
\refDefinition{basis manifold of vector space}{\SideNS-cols},
а также теорема является следствием теоремы
\refTheorem{active representation is single transitive}{\SideNS-rows}
и определений
\refDefinition{basis manifold of vector space}{\SideNS-rows}.
}

\DefLabeledDefinition{basis manifold of vector space}{\SideNS-\Cols}
{
Мы будем называть орбиту
\ShowEq{basis manifold of vector space, \SideNS-\Cols}
выбранного базиса $\Basis e$
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA.
}

\DefLabeledTheorem{active transformations, vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное \Group nA\Hyph представление.
}

\DefProof{active transformations, vector space}
{
Пусть $a$, $b$ - матрицы автоморфизмов $\Vector a$ и $\Vector b$
относительно базиса $\Basis e$.
Согласно теореме
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(1)}
преобразование координат имеет вид
\DrawEq[{v'}{}v{}a{}]{v1=v2*a \SideNS-\Cols}{v'}
\DrawEq[{v''}{}{v'}{}b{}]{v1=v2*a \SideNS-\Cols}{v''}
Равенство
\ShowEq{a*b, \SideNS-\Cols}
\DrawEq[{v''}{}v{}{\TheProduct}{}]{v1=v2*a \SideNS-\Cols}{}
\begin{sloppypar}
\noindent
является следствием равенств
\eqRef{v1=v2*a \SideNS-\Cols}{v'},
\eqRef{v1=v2*a \SideNS-\Cols}{v''}.
Согласно теореме
\refTheorem{product of homomorphisms, A vector space}{\SideNS-\ColN},
произведение автоморфизмов $\Vector a$ и $\Vector b$
имеет матрицу \TheProduct.
Следовательно, автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
\Group nA\Hyph представление.
\end{sloppypar}

Нам осталось показать,
что ядро неэффективности состоит только
из единичного элемента. Тождественное преобразование
удовлетворяет равенству
\ShowEq{active transformations, vector space, 2, \SideNS-\Cols}
Выбирая значения координат в форме
\ShowEq{ai=delta ik, \Cols},
где $\gik$ задано, мы получим
\ShowEq{identity transformation, vector space, \SideNS-\Cols}
Из \EqRef{identity transformation, vector space, \SideNS-\Cols} следует
\ShowEq{identity transformation, vector space, 1, \Cols}
Поскольку $\gik$ произвольно, мы приходим к заключению $a=\delta$.
}

\DefLabeledTheorem{active transformations, basis, vector space}{\SideNS-\Cols}
{
Автоморфизм $a$, действуя на каждый вектор базиса
в \SideRu вом $A$\Hyph векторном пространстве \ColsA,
отображает базис в другой базис.
}

\DefProof{active transformations, basis, vector space}
{
Пусть $\Basis e$ - базис в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsA.
Согласно теореме
\refTheorem{automorphism of vector space}{\Product-\Cols},
вектор
\ShowEq{vector of basis \Cols}e
отображается в вектор
\ShowEq{vector of basis \Cols}{e'}
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}1
\begin{sloppypar}
\noindent
Если векторы
\ShowEq{vector of basis \Cols}{e'}
линейно зависимы,
то в линейной комбинации
\ShowEq{automorphism, vector space, 2, \SideNS-\Cols}
\end{sloppypar}
\noindent
$\lambda\ne 0$.
Из равенств \eqRef{automorphism, vector space, 1, \SideNS-\Cols}1
и \EqRef{automorphism, vector space, 2, \SideNS-\Cols} следует, что
\ShowEq{automorphism, vector space, 3, \SideNS-\Cols}
и $\lambda\ne 0$. Это
противоречит утверждению, что векторы
\ShowEq{vector of basis \Cols}e
линейно независимы.
Следовательно, векторы
\ShowEq{vector of basis \Cols}{e'}
линейно независимы
и порождают базис.
}

\DefText{extend linear representation to set of bases 1}
{
Таким образом, мы можем распространить
\OtherSideRu востороннее линейное $GL(V_*)$\Hyph представление
в \SideRu вом $A$\Hyph векторном пространстве $V_*$
на множество базисов
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefText{extend linear representation to set of bases 2}
{
Мы будем называть преобразование этого \OtherSideRu востороннего представления
на множестве базисов
\SideRu вого $A$\Hyph векторного пространства $V$
\AddIndex{активным преобразованием}{active transformation, vector space}
потому, что гоморфизм \SideRu вого $A$\Hyph векторного пространства породил это преобразование
(\BlueText{Смотри также определение в разделе
\citeBib{Korn}\Hyph 14.1\Hyph 3,
а также определение на странице
\citeBib{Rashevsky}\Hyph 214}).

\ePrints{2022.01.05,2022.11.26}%
\ifx\Semafor\ValueOn%
\FrameCiteBib{Korn}

\FrameCiteBib{Rashevsky}
\fi
}

\DefText{extend linear representation to set of bases 3}
{
\begin{sloppypar}
Соответственно определению мы будем записывать действие
активного преобразования $a\in GL(V_*)$ на базис $\Basis e$ в форме
\ShowEq{active transformation, vector space, \SideNS-\Cols}.
Рассмотрим равенство
\DrawEq{active transformation ae x=a ex, \SideNS-\Cols}1
Выражение
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
в левой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом базиса \eV при активном преобразовании $a$.
Выражение
\ShowEq{active transformation ae x=a ex 1, \SideNS-\Cols}
в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является разложением вектора $\Vector v$ относительно базиса \eV[][.]
Следовательно,
выражение в правой части равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
является образом вектора $\Vector v$ относительно эндоморфизма $a$
и выражение в левой части равенства
\newline
\FrameEqRef{active transformation ae x=a ex, \SideNS-\Cols}1
\newline
является разложением образа вектора $\Vector v$
относительно образа базиса \eV[][.]
Следовательно, из равенства
\eqRef{active transformation ae x=a ex, \SideNS-\Cols}1
следует, что эндоморфизм $a$ \SideRu вого $A$\Hyph векторного пространства и
соответствующее активное преобразование $a$ действуют синхронно
и координаты $a\circ \Vector v$ образа вектора $\Vector v$ относительно
образа
\ShowEq{active transformation, vector space, \SideNS-\Cols}{}
базиса \eV
совпадают с координатами вектора $\Vector v$ относительно базиса $\Basis e$.
\end{sloppypar}
}

\DefLabeledTheorem{active representation is single transitive}{\SideNS-\Cols}
{
Активное \OtherSideRu востороннее \Group nA\Hyph представление на множестве базисов
однотранзитивно.
Множество базисов, отождествлённое с траекторией
\ShowEq{basis manifold of V, \SideNS-\Cols}e{\Group nA}{}
активного \OtherSideRu востороннего \Group nA\Hyph представления
называется
{\bf многообразием базисов}
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledTheorem{exists representation, commuting with active}{\SideNS-\Cols}
{
На многообразии базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA
существует однотранзитивное
\SideRu востороннее $G(V)$\Hyph представление, перестановочное с активным.
}

\AddEq{proof: exists representation, commuting with active}
{
\begin{sloppypar}
\begin{proof}
Из теоремы
\refTheorem{representation on basis manifold, vector space}{\SideNS}
следует, что многообразие базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
является однородным пространством группы $G$.
Теорема является следствием теоремы
\RefTheorem{two representations of group}.
\end{proof}
\end{sloppypar}
}

\AddEq{remark: passive transformation, vector space}
{
\ePrints{2022.11.26,2306.00880,8764-0830}%
\ifx\Semafor\ValueOn%
Преобразование
\else
Как мы видим из замечания
\RefRemark{one representation of group}
преобразование
\fi
\SideRu востороннего $G(V)$\Hyph представления отличается от активного преобразования
и не может быть сведено к
преобразованию пространства $V$.
}

\DefLabeledDefinition{passive transformation, vector space}{\SideNS-\Cols}
{
Преобразование
\SideRu востороннего $G(V)$\Hyph представления называется
{\bf пассивным преобразованием}
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства \ColsA,
а \SideRu востороннее $G(V)$\Hyph представление называется
{\bf пассивным \SideRu восторонним $G(V)$\Hyph представлением}.
Согласно определению
мы будем записывать пассивное преобразование базиса $\Basis e$,
порождённое элементом $a\in G(V)$, в форме
\ShowEq{passive transformation symbol, \SideNS-\Cols}
}

\AddEq[1]{table: Passive and Active Representations}
{
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefRow}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство строк&&&\\
\hline
\ShowEq{def #1}\SideRu вое $A$\Hyph векторное&\ShowEq{def #1}\ShowEq{\DefCol}\Group nA&
\ShowEq{def #1}\OtherSideRu востороннее&\ShowEq{def #1}\SideRu востороннее\\
пространство столбцов&&&\\
\hline
}

\DefLabeledTheorem{principle of covariance}{\SideNS}%-\Cols}
{
{\bf(Принцип ковариантности).}
Представитель геометрического объекта не зависит от выбора
базиса \eV[V2][.]
}

\DefProof{principle of covariance}
{
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_V$,
базис $\Basis e_W$
и координаты геометрического объекта $w^\alpha$.
Соответствующий представитель геометрического объекта
имеет вид
\DrawEq[w{}wW]{geometric object representative, \SideNS-\Cols}{}
Предположим базис $\Basis e'_V$ связан
с базисом $\Basis e_V$
пассивным преобразованием
\DrawEq[V]{passive transformation e->e', \SideNS-\Cols}{}
Согласно построению это порождает пассивное преобразование
\newline
\FrameEqRef[{W1}{W2}{F(g)}{}]{e2i=aij e1j \Product-\Cols}{GOeW}
\newline
и координатное преобразование
\newline
\FrameEqRef{coordinate transformation, vector space W, \SideNS-\Cols}1
\newline
Соответствующий представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3, \SideNS-\Cols}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
}

\AddEq{definition: sum of geometric objects}
{
\begin{ShadedDefinition}
\labelDefinition{sum of geometric objects, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\ShowEq{sum of geometric objects, 1}
геометрические объекты одного и того же типа,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{sum of geometric objects, 2}
называется \AddIndex{суммой
\ShowEq{sum of geometric objects, 3}
геометрических объектов}{sum of geometric objects}
$\Vector w_1$ и $\Vector w_2$.
\end{ShadedDefinition}
}

\AddEq{definition: product of geometric object and constant}
{
\begin{ShadedDefinition}
\labelDefinition{product of geometric object and constant, \SideNS-\Cols}
\ShowEq{Let V be vector space of and}
\DrawEq[w1{w_1}W]{geometric object representative, \SideNS-\Cols}{}
геометрический объект,
определённый в \SideRu вом $A$\Hyph векторном пространстве $V$.
Геометрический объект
\ShowEq{product of geometric object and constant, 2, \SideNS}
называется \AddIndex{произведением
\ShowEq{product of geometric object and constant, 3, \SideNS}
геометрического объекта $\Vector w_1$ и константы $k\in A$}
{product of geometric object and constant}.
\end{ShadedDefinition}
}

\AddEq{theorem: Geometric objects form A vector space}
{
\begin{ShadedTheorem}
\labelTheorem{Geometric objects form A vector space, \SideNS-\Cols}
Геометрические объекты типа $F$,
определённые в \SideRu вом $A$\Hyph векторном пространстве $V$ \ColsNA,
образуют \SideRu вое $A$\Hyph векторное пространство \ColsNA.
\end{ShadedTheorem}
}

\DefProof{Geometric objects form A vector space}
{
Утверждение теорем
\RefTheorem{Geometric objects form A vector space, \SideNS-cols},
\RefTheorem{Geometric objects form A vector space, \SideNS-rows}
следует из непосредственной проверки
свойств векторного пространства.
}

\DefLabeledTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols}
{
Координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
\SideRu вого $A$\Hyph векторного пространства $V$ \ColsA
совпадает с матрицей пассивного преобразования, отображающего
базис $\Basis e$ в базис $\Basis e'$.
}

\DefProof{coordinate matrix of basis and passive transformation}
{
Согласно теореме
\refTheorem{coordinate matrix of vector}{\SideNS-\Cols},
координатная матрица базиса $\Basis e'$ относительно базиса $\Basis e$
состоит из \ColsNA, являющихся координатными матрицами векторов
$\aD{\Vector e'}i$ относительно базиса $\Basis e$. Следовательно,
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{e'}
В тоже время пассивное преобразование $a$, связывающее два базиса, имеет вид
\ShowEq{coordinate matrix of basis and passive transformation, \SideNS-\Cols}{a}
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols},
\ShowEq{coordinate matrix of basis and passive transformation, \Cols}
для любого $\gii$. Это доказывает теорему.
}

\DefLabeledSloppyRemark{identify basis and matrix of coordinates}{\SideNS-\Cols}
{
Согласно теоремам
\RefTheorem{single transitive representation of group},
\refTheorem{coordinate matrix of basis and passive transformation}{\SideNS-\Cols},
мы можем отождествить базис $\Basis e'$ 
многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG{}
\SideRu вого $A$\Hyph векторного пространства столбцов
и матрицу $g$ координат базиса $\Basis e'$
относительно базиса $\Basis e$
\DrawEq[{}{}]{passive transformation e->e', \SideNS-\Cols}1
Если $\Basis e'=\Basis e$, то равенство
\eqRef{passive transformation e->e', \SideNS-\Cols}1
принимает вид
\ShowEq{passive transformation e->e, \SideNS-\Cols}
Опираясь на равенство
\EqRef{passive transformation e->e, \SideNS-\Cols}
мы будем пользоваться записью
\ShowEq{basis manifold of V, \SideNS-\Cols}{\aD En}G{}
для многообразия базисов
\ShowEq{basis manifold of V, \SideNS-\Cols}eG.
}

\DefText{Passive Transformation}
{
Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к преобразованию
координат вектора относительно базиса.
}

\DefText{transformation of coordinates of vector}
{
Мы рассмотрим преобразование координат вектора в теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\AddEq{remark: active representation is single transitive}
{
Чтобы доказать теоремы
\refTheorem{active representation is single transitive}{\SideNS-cols},
\refTheorem{active representation is single transitive}{\SideNS-rows},
достаточно показать, что для любых двух базисов
определено по крайней мере одно преобразование \OtherSideRu востороннего представления
и это преобразование единственно.
}

\AddEq{left active representation is single transitive}
{
координатной матрицы исходного базиса и матрицы автоморфизма
\ShowEq{left e'=e*a}{}
}

\AddEq{right active representation is single transitive}
{
матрицы автоморфизма и координатной матрицы исходного базиса
\ShowEq{right e'=e*a}{}
}

\DefProofSloppy{active representation is single transitive}
{
Гомоморфизм $a$, действуя на базис $\Basis e$ имеет вид
\DrawEq{automorphism, vector space, 1, \SideNS-\Cols}{}
где
\ShowEq{vector of basis \Cols}{e'}
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e'}
относительно базиса $\Basis h$ и
\ShowEq{vector of basis \Cols}e
- координатная матрица вектора
\ShowEq{vector of basis \Cols}{\Vector e}
относительно базиса $\Basis h$.
Следовательно, координатная матрица образа базиса равна
\ProductType произведению
\ShowEq{\SideWS active representation is single transitive}
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols},
матрицы $g$ и $e$ невырождены. Следовательно, матрица
\ShowEq{homomorphism on A basis, \SideNS-\Cols}
является матрицей автоморфизма, отображающего базис $\Basis e$
в базис $\Basis e'$.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis e$ таковы, что
\ShowEq{two transformations on basis manifold, \SideNS-\Cols}
В силу теорем
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
и
\RefTheorem{two cr-products equal}
справедливо равенство $g_1=g_2$.
Отсюда следует утверждение теоремы.
}

\DefLabeledTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols}
{
Пусть
\ShowEq{Bases e12}V{}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$ столбцов.
Пусть
\ShowEq{Bases e12}W{}
- базисы \SideRu вого $A$\Hyph векторного пространства $W$ столбцов.
Пусть $a_1$ - матрица гомоморфизма
\DrawEq{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и $a_2$ - матрица гомоморфизма
\eqRef{A:V->W}{different bases \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
Если базис $\Basis e_{V1}$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_{V2}$
\DrawEq[Vb]{coordinate matrix, f, g, \SideNS-\Cols}{}
и $\Basis e_{W1}$ имеет координатную матрицу $c$ относительно
базиса $\Basis e_{W2}$
\DrawEq[Wc]{coordinate matrix, f, g, \SideNS-\Cols}C
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[c]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
}

\DefProof{representation of homomorphism relative different bases}
{
Вектор $\Vector v\in V$ имеет разложение
\ShowEq{expansion of vector v, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases e12}V.
Так как $a$ - гомоморфизм, то мы можем записать его в форме
\ShowEq{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW1{}
и
\ShowEq{representation of homomorphism relative different bases, 2, \SideNS-\Cols}
относительно базисов
\ShowEq{Bases eVW}VW2.
В силу теоремы
\refTheorem{coordinate matrix of basis}{\Product-\Cols}
матрица $c$ имеет \ProductType обратную и из равенства
\eqRef{coordinate matrix, f, g, \SideNS-\Cols}C следует
\ShowEq{coordinate matrix, W2, W1, \SideNS-\Cols}
Равенство
\ShowEq{representation of homomorphism relative different bases, 3, \SideNS-\Cols}
\begin{sloppypar}
\noindent
является следствием равенств
\EqRef{representation of homomorphism relative different bases, 2, \SideNS-\Cols},
\EqRef{coordinate matrix, W2, W1, \SideNS-\Cols}.
В силу теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}
сравнение равенств
\EqRef{representation of homomorphism relative different bases, 1, \SideNS-\Cols}
и \EqRef{representation of homomorphism relative different bases, 3, \SideNS-\Cols} даёт
\ShowEq{representation of homomorphism relative different bases, 4, \SideNS-\Cols}
Так как вектор $a$ - произвольный вектор,
утверждение теоремы
является следствием теоремы
\refTheorem{active transformations, vector space}{\SideNS-\Cols}
и равенства
\EqRef{representation of homomorphism relative different bases, 4, \SideNS-\Cols}.
\end{sloppypar}
}

\DefLabeledTheorem{coordinate transformations form representation, vector space}{\SideNS-\Cols}
{
Преобразования координат
\newline
\FrameEqRef[v2v1g{}{\SideNS}{\Cols}]{v2=v1g-}{12 \SideNS-\Cols}
\newline
порождают эффективное линейное
\OtherSideRu востороннее контравариантное $G$\Hyph представление, называемое
{\bf координатным представлением в \SideRu вом $A$\Hyph векторном пространстве}
\ColsNA.
}

\DefProof{coordinate transformations form representation, vector space}
{
\ShowText{passive representation of left vector space}
Согласно определению
\RefDefinition{Left side contravariant representation},
преобразования координат
порождают линейное правостороннее контравариантное $G$\Hyph представление.
Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
}

\AddEq{theorem: representation of automorphism relative different bases}
{
\begin{ShadedTheorem}
\labelTheorem{representation of automorphism relative different bases, \SideNS-\Cols}
Пусть $\Vector a$ - автоморфизм
левого $A$\Hyph векторного пространства $V$ столбцов.
Пусть $a_1$ - матрица этого автоморфизма, заданная
относительно базиса $\Basis e_1$, и
$a_2$ - матрица того же автоморфизма, заданная
относительно базиса $\Basis e_2$.
Если базис $\Basis e_1$ имеет координатную матрицу $b$ относительно
базиса $\Basis e_2$
\DrawEq[{}b]{coordinate matrix, f, g, \SideNS-\Cols}{}
то матрицы $a_1$ и $a_2$ связаны соотношением
\DrawEq[b]{representation of homomorphism relative different bases, \SideNS-\Cols}{}
\end{ShadedTheorem}
}

\DefProof{representation of automorphism relative different bases}
{
Утверждение является следствием теоремы
\refTheorem{representation of homomorphism relative different bases}{\SideNS-\Cols},
так как в данном случае $c=b$.
}

\DefLabeledTheorem[4]{basis of vector space}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of}.
\ShowEq{Let be basis of vector space}{#2}iIA{#1}V{#2}{\Cols}-
\ShowEq{Let be basis of vector space}{#4}jJA{#3}V{#4}{\Cols}-
Если $|\gi I|$ и $|\gi J|$ - конечные числа, то
\ShowEq{|I|=|J|}
}

\DefProof{basis of vector space}
{
Предположим, что
\ShowEq{|I|=m}Im{}
и
\ShowEq{|I|=m}Jn.
Предположим, что
\DrawEq{m<n gi}{1 \SideNS-\Cols}
Так как $\Basis e_1$ - базис, любой вектор
\ShowEq{basis e2 of V \Cols}
имеет разложение
\ShowEq{basis e2 relative e1 \SideNS-\Cols}
Так как $\Basis e_2$ - базис,
\DrawEq{basis e2 of V lambda}{\SideNS-\Cols}
следует из
\ShowEq{basis e2 relative e1, lambda, \SideNS-\Cols}
Так как $\Basis e_1$ - базис, мы получим
\ShowEq{basis e2 relative e1, lambda=0, \SideNS-\Cols}
Согласно
\eqRef{m<n gi}{1 \SideNS-\Cols},
\ShowEq{Rank a<m \Product}
и система линейных уравнений
\EqRef{basis e2 relative e1, lambda=0, \SideNS-\Cols}
имеет больше переменных, чем уравнений. Согласно теореме
\RefTheorem{star rows system of linear equations, solution},
$\lambda\ne 0$, что противоречит
утверждению \eqRef{basis e2 of V lambda}{\SideNS-\Cols}. 
Следовательно, утверждение
\DrawEq{m<n gi}-
неверно.
Таким же образом мы можем доказать, что утверждение
\ShowEq{n<m gi}
неверно.
Это завершает доказательство теоремы.
}

\AddEq{definition: linearly independent, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{linearly independent, AoxA module \Cols}
Пусть $V$ левый \AoxA A\Hyph модуль \ColsNA.
Множество векторов
\ShowEq{Vector A \Cols}
левого \AoxA A\Hyph модуля $V$
{\bf линейно независимо},
если из равенства
\ShowEq{AoxA linearly independent \Cols}
следует
\ShowEq{AoxA linearly independent 1 \Cols}.
В противном случае, множество векторов $\aD ai$
{\bf линейно зависимо}.
\end{ShadedDefinition}
}

\AddEq{definition: basis, AoxA module}
{
\begin{ShadedDefinition}
\labelDefinition{basis, AoxA module \Cols}
Мы называем множество векторов
\ShowEq{basis, AoxA module \Cols}
\AddIndex{базисом}{basis}
\AoxA A\Hyph модуля $V$,
если множество векторов
\ShowEq{basis vector \Cols}
линейно независимо и, добавив к этой системе любой другой вектор,
мы получим новое множество, которое является линейно зависимым.
\end{ShadedDefinition}
}

\DefLabeledDefinition{Eigenvalue of Endomorphism}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Вектор $v\in V$ называется
{\bf собственным вектором}
эндоморфизма
\ShowEq{f:A->B}{\Vector f}VV
относительно базиса $\Basis e$,
если существует $b\in A$ такое, что
\DrawEq[bv]{fov=b e o v}{\SideNS}
$A$\Hyph число $b$ называется
{\bf собственным значением}
эндоморфизма $f$
относительно базиса $\Basis e$.
}

\DefLabeledTheorem{no endomorphism fov=bv}{\SideNS}
{
\ShowEq{Let V be vector space and basis}
Если
\ShowEq{b not in ZA},
то не существует эндоморфизма $\Vector f$ такого, что
\ShowEq{fov=bv \SideNS}
%где $f$ - матрица эндоморфизма $\Vector f$.
}

\DefProofSloppy{no endomorphism fov=bv}
{
Допустим, что существует эндоморфизм $\Vector f$
такой, что равенство
\EqRef{fov=bv \SideNS}
верно.
Равенство
\ShowEq{b(av)=a(bv) \SideNS}
является следствием равенств
\ShowRef{b(av)=a(bv)}
и равенства
\EqRef{fov=bv \SideNS}.
Согласно теореме
\refTheorem{av=bv=>a=b}{\SideNS-\Cols},
равенство
\DrawEq{ab=ba}{\SideNS}
для любого $a\in A$
является следствием равенства
\EqRef{b(av)=a(bv) \SideNS}.
Равенство
\eqRef{ab=ba}{\SideNS}
для любого $a\in A$
противоречит утверждению
\ShowEq{b not in ZA}.
Следовательно, рассматриваемый эндоморфизм $\Vector f$
не существует.
}

\AddEq{remark: Eigenvalue of Endomorphism}
{
\begin{sloppypar}
Согласно теореме
\refTheorem{no endomorphism fov=bv}{\SideNS},
в отличие от \OtherSideRu востороннего произведения
вектора на скаляр
\SideRu востороннее произведение
вектора на скаляр
не является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства.
Из сравнения определения
\refDefinition{similarity transformation}{\SideNS}
и теоремы
\refTheorem{no endomorphism fov=bv}{\SideNS}
следует, что преобразование подобия
играет в некоммутативной алгебре
такую же роль,
что преобразование подобия
играет в коммутативной алгебре.
\end{sloppypar}
}

\DefLabeledTheorem{similarity transformation, change of basis}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and}
\ShowEq{basis e1 e2}
- базисы \SideRu вого $A$\Hyph векторного пространства $V$.
Пусть базисы
\ShowEq{basis e1 e2}
связаны пассивным преобразованием $g$
\DrawEq[12g{}]{e2i=aij e1j \Product-\Cols}{}
Преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\DrawEq[ag]{ga*g- \SideNS-\Cols}a
относительно базиса $\Basis e_2$.
}

\DefProof{similarity transformation, change of basis}
{
Согласно теореме
\refTheorem{passive transformation and endomorphism}{\SideNS-\Cols},
преобразование подобия
\ShowEq{\SideWS map a En}a1
имеет матрицу
\ShowEq{ga*g- 1 \SideNS-\Cols}
относительно базиса $\Basis e_2$.
Теорема является следствием выражения
\EqRef{ga*g- 1 \SideNS-\Cols}.
}

\DefLabeledTheorem{similarity transformation}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Пусть
\ShowEq{dim V=n}
и $\aD En$ - \nTimes единичная матрица.
Для любого $A$\Hyph числа $a$, существует эндоморфизм
\ShowEq{\SideWS map a En}a{}
\SideRu вого $A$\Hyph векторного пространства $V$,
который имеет матрицу
\ShowEq{\SideWS a En}
относительно базиса $\Basis e$.
}

\DefProof{similarity transformation}
{
Пусть $\Basis e$ - базис
\SideRu вого $A$\Hyph векторного пространства столбцов.
Согласно теореме
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(1)}
и определению
\refDefinition{end aut morphism module}{\SideNS},
отображение
\ShowEq{v in V -> av in V \SideNS-\Cols}
является эндоморфизмом
\SideRu вого $A$\Hyph векторного пространства $V$.
}

\DefLabeledDefinition[6]{isomorphism module}{\SideNS(#1#2#3)}
{
Гомоморфизм\,\refFootnote{iso end aut morphism}{\SideNS(#1#2#3)}
\DrawEq[gf]{homomorphism A module #1#2#3}{}
назывется
\AddIndex{изоморфизмом}{isomorphism}
между \SideRu вым $A_{#2}$\Hyph \VectorSetRuE $V_{#3}$
и \SideRu вым $A_{#5}$\Hyph \VectorSetRuE $V_{#6}$,
если существует отображение
\DrawEq[gf]{homomorphism- A module #1#2#3}{}
которое является гомоморфизмом.
}

\DefLabeledDefinition{end aut morphism module}{\SideNS}
{
Гомоморфизм\,\refFootnote{iso end aut morphism}{\SideNS(1)}
\DrawEq[fVV{}]{f: A->B}{}
источником и целью которого является \Same
\SideRuTo $\Base$\Hyph\VectorSetRuANS,
называется
\AddIndex{эндоморфизмом}{endomorphism}.
Эндоморфизм
\DrawEq[fVV{}]{f: A->B}{}
\SideRu\From $\Base$\Hyph\VectorSetRuB $V$
назывется
\AddIndex{автоморфизмом}{automorphism},
если существует отображение $f^{-1}$
которое является эндоморфизмом.
}

\DefLabeledDefinition{iso end aut morphism vector space}{\SideNS}
{
Гомоморфизм
\ShowEq{f:A->B}fVW
назывется\,\refFootnote{iso end aut morphism}1
\AddIndex{изоморфизмом}{isomorphism}
между \SideRu выми $A$\Hyph векторными пространствами $V$ и $W$,
если соответствие $f^{-1}$ является гомоморфизмом.
Гомоморфизм
\ShowEq{f:A->B}fVV
источником и целью которого является одно и тоже
\SideRu вое $A$\Hyph векторное пространство,
называется
\AddIndex{эндоморфизмом}{endomorphism}.
Эндоморфизм
\ShowEq{f:A->B}fVV
\SideRu вого $A$\Hyph векторного пространства $V$
назывется
\AddIndex{автоморфизмом}{automorphism},
если соответствие $f^{-1}$ является эндоморфизмом.
}

\DefText{Basis Manifold}
{
\section{Размерность \SideRu вого \texorpdfstring{$A$}{A}\Hyph векторного пространства}

\ShowText{Dimension of Vector Space}

\section{Многообразие базисов \SideRu вого \texorpdfstring{$A$}{A}-векторного пространства}
%\labelSection{Basis Manifold for Vector Space}

\ShowEq{Basis Manifold for Vector Space}

\section{Пассивное преобразование в \SideRu вом \texorpdfstring{$A$}{A}-векторном пространстве}

\ShowEq{Passive Transformation}
}

\DefLabeledTheorem[3]{rank of matrix}{\Product-\Cols}
{
Предположим, что $a$ - матрица,
\ShowEq{\Product-rank a=k<m}{#1}
и $\SA T$ - \ProductType главная подматрица.
Тогда \ColWS \ARow a{#2} является
\SideRu вой линейной комбинацией \ColsA \ARow a{#3}
\ShowEq{rank of matrix, \Product-\Cols}
\ShowEq{rank of matrix, 1, \Product-\Cols}
\ShowEq{rank of matrix, 2, \Product-\Cols}
}

\DefProof[5]{rank of matrix}
{
Если матрица $a$ имеет $\gik$ \RowsNSA, то, полагая, что \ColWS \ARow a{#2}
- \SideRu вая линейная комбинация
\EqRef{rank of matrix, 1, \Product-\Cols}
\ColsA \ARow a{#3} с коэффициентами $\Coef$,
мы получим систему \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Мы положим, что $\ACol x{#4}=\Coef$ - это неизвестные переменные
в системе \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}.
Согласно теореме
\refTheorem{nonsingular system of linear equations}{\SideNS-\Cols},
система \SideRu вых линейных уравнений
\EqRef{rank of matrix, 2, \Product-\Cols}
имеет единственное решение
и это решение нетривиально потому, что все \ProductType квазидетерминанты
отличны от $0$.

Остаётся доказать утверждение в случае, когда число \RowsRWSA матрицы $a$
больше чем $\gik$.
Пусть нам даны \ColWS \ARow a{#2} и \RowRuWS $\ACol a{#5}$.
Согласно предположению, подматрица
$\SATpr$ - \ProductType вырожденная матрица
и её \ProductType квазидетерминант
\DrawEq{singular matrix and quasideterminant}{\SideNS-\Cols}
Согласно равенству
\eqRef{j i quasideterminant =}{\Product}
равенство
\eqRef{singular matrix and quasideterminant}{\SideNS-\Cols}
имеет вид
\ShowEq{rank of matrix, 4, \Product}
Матрица
\ShowEq{rank of matrix, 5, \Product-\Cols}
не зависит от $\gi{#5}$. Следовательно, для любых
\ShowEq{\rIn}
\ShowEq{rank of matrix, 6, \Product-\Cols}
Чтобы доказать равенство
\EqRef{rank of matrix, 2, \Product-\Cols},
\ \ не\-обходимо доказать равенство
\ShowEq{rank of matrix, 9, \Product-\Cols}
Из равенства
\ShowEq{rank of matrix, 7, \Product-\Cols}
следует, что
\ShowEq{rank of matrix, 8, \Product-\Cols}
Равенство
\EqRef{rank of matrix, 9, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 5, \Product-\Cols},
\EqRef{rank of matrix, 8, \Product-\Cols}.
Равенство
\EqRef{rank of matrix, 2, \Product-\Cols}
является следствием равенств
\EqRef{rank of matrix, 6, \Product-\Cols},
\EqRef{rank of matrix, 9, \Product-\Cols}.
}

\DefLabeledTheorem{set of eigenvectors is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением
матрицы $a$.
Множество собственн\EndA \ColsA
матрицы $a$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors is vector space}
{
Согласно определениям
\refDefinition{eigenvalue of matrix}{\Product},
\refDefinition{eigenvector of matrix}{\Product-\Cols},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0}
с \ProductType вырожденной матрицей \ShowEq{f-bEn \SideNS}{}.
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0}
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefLabeledTheorem{set of eigenvectors fg is vector space}{\Product-\Cols}
{
Пусть $A$\Hyph число $b$ является
\ProductType собственным значением пары матриц
\ShowEq{pair of matrices \Product-\ColN},
где $g$ - \ProductType невырожденная матрица.
Множество собственн\EndA \ColsA
пары матриц $(f,g)$, соответствующих \ProductType собственному значению $b$,
является \SideRu вым $A$\Hyph векторным пространством \ColsNA.
}

\DefProof{set of eigenvectors fg is vector space}
{
Согласно определениям
\refDefinition{eigenvalues of pair of matrices}{\Product},
\refDefinition{eigenvector of pair of matrices}{\Product-\ColN},
координаты собственно\FinC \ColA
являются решением системы линейных уравнений
\ShowEq{\Product-eigen\Cols=0 fg}
с \ProductType вырожденной матрицей
\[f-\ShowEq{ga*g- \SideNS-\Cols}bg\]
Согласно теореме
\RefTheorem{Solutions homogenous system of linear equations},
множество решений системы линейных уравнений
\EqRef{\Product-eigen\Cols=0 fg}
является \SideRu вым пространст\-вом \ColsNA.
}

\DefRemark{simplify definitions of eigenvalue}
{
Пусть
\ShowEq{gij in ZA}
Тогда
\ShowEq{gb rc g-=b}
\ShowEq{gb cr g-=b}
Из равенств
\EqRef{gb rc g-=b},
\EqRef{gb cr g-=b}
следует, что,
если выполнено
условие
\EqRef{gij in ZA},
то мы можем упростить определения
собственного значения и собственного вектора матрицы
и получить определения,
которые будут соответствовать определениям
в коммутативной алгебре.
}

\DefLabeledTheorem{columns of matrix are linearly dependent}{\Product-\Cols}
{
Предположим, что матрица $a$ имеет $\gi{\Lbls}$ \ColsNA.
Если
\ShowEq{\Product-rank a=k<m}{\Lbls}
то \ColsRu матрицы линейно зависимы с\SideRu ва
\DrawEq[{\lambda}a]{columns of matrix are linearly dependent}{}
}

\DefProof[1]{columns of matrix are linearly dependent}
{
Предположим, что \ColWS \ARow a{#1} является \SideRu вой линейной комбинацией \ColsA
\EqRef{rank of matrix, 1, \Product-\Cols}. Мы положим
\ShowEq{\Cols-of-matrix linearly dependent, 1}
и остальные
\ShowEq{\Cols-of-matrix linearly dependent, 2}
}


==> Vector.Space.2022.Russian.tex <==
%auto-ignore
\input{Vector.Space.2022.Eq}

\chapter{Векторное пространство над алгеброй с делением}

\section{Эффективное представление \texorpdfstring{$D$}{D}-алгебры}

\ShowEq{def AModule}
\ShowText{Representation of ring f(0)=v0}

\section{Левое векторное пространство над алгеброй с делением}

\ShowEq{def AVector}
\ShowEq{def left}
\ShowEq{def universal}
\ShowEq{Show Vector Space over Division Algebra}

\section{Базис левого \texorpdfstring{$A$}{A}-векторного пространства}
\labelSection{Basis of Left Vector Space}

\ShowEq{Show Basis of Vector Space}

\begin{ShadedTheorem}
\labelTheorem{division algebra as vector space}
Мы можем рассматривать $D$\Hyph алгебру $A$ с делением как
левое $A$\Hyph векторное пространство с базисом
\ShowEq{basis e=1}
\end{ShadedTheorem}
\begin{proof}
Теорема является следствием равенства
\eqRef{unitarity law, vector space}{\SideWS \Base}.
\end{proof}

\section{Правое векторное пространство над алгеброй с делением}

\ShowEq{def right}
\ShowEq{Show Vector Space over Division Algebra}

\section{Базис правого \texorpdfstring{$A$}{A}-векторного пространства}
%\labelSection{Basis of Left Vector Space}

\ShowEq{Show Basis of Vector Space}


==> Vector.Space.Type.Russian.tex <==
%auto-ignore
\input{Vector.Space.Type.Eq}

\chapter{Тип векторного пространства}

\section{Бикольцо}
\labelSection{Biring}

Мы будем рассматривать матрицы, элементы которых принадлежат
ассоциативной $D$\Hyph алгебре с делением $A$.

\ShowText{matrix operations}

\ShowDefinition{Hadamard inverse of matrix}

Множество \nTimes матриц замкнуто относительно \RC произведения и \CR произведения,
а также относительно суммы.

\ShowDefinition{biring matrix}

\ShowTheorem{transpose of identity}
\ShowProof{transpose of identity}

\ShowEq{power matrix}

Теоремы
\ShowEq{duality between RC nd CR product}
показывают, что существует двойственность
между \RC произведением и \CR произведением.
Мы можем объединить эти утверждения.

\begin{ShadedTheorem}
\AddIndex{Принцип двойственности для бикольца}{duality principle for biring}.
\labelTheorem{duality principle for biring}
Пусть $\mathfrak{A}$ - истинное утверждение о
бикольце $\mathcal{A}$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in\mathcal{A}$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}

\begin{ShadedTheorem}
\AddIndex{Принцип двойственности для бикольца матриц}{duality principle for biring of matrices}.
\labelTheorem{duality principle for biring of matrices}
Пусть $\mathcal{A}$ является бикольцом матриц.
Пусть $\mathfrak{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item столбцы и строки всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}

\begin{remark}
\labelRemark{left and right matrix notation}
В выражении
\ShowEq{a rc b rc c}
мы выполняем операцию умножения слева направо.
Однако мы можем выполнять операцию умножения
справа налево. Тогда выражение
\EqRef{a rc b rc c}
примет вид
\ShowEq{c cr b cr a}
Мы сохраним правило,
что показатель степени и индексы записываются справа от выражения.
Например, если исходное выражение имеет вид
\ShowEq{left and right matrix notation, 1}
то выражение, читаемое справа налево, примет вид
\ShowEq{left and right matrix notation, 2}

Если задать порядок, в котором мы записываем индексы,
то мы можем утверждать, что мы читаем выражение сверху вниз,
читая сперва верхние индексы, потом нижние.
Мы можем прочесть выражение снизу вверх.
При этом мы дополним правило, что символы операции также читаются в том же
направлении, что и индексы. Например, выражение
\ShowEq{left and right matrix notation, 4}
прочтённое снизу вверх, имеет вид
\ShowEq{left and right matrix notation, 5}
Согласно принципу двойственности, если верно одно утверждение,
то верно и другое.
\qed
\end{remark}

\ShowText{matrix product}

\def\SectionTitle{Квазидетерминант}
\ShowEq{def rc}
\ShowText{Quasideterminant}

\ShowEq{def cr}
\ShowText{Quasideterminant}

\begin{ShadedTheorem}
\labelTheorem{two quasideterminants}
\ShowEq{CR and RC quasideterminants}
\end{ShadedTheorem}
\begin{proof}
Согласно
\eqRef{j i quasideterminant =}{rc}
и \EqRef{Hadamard inverse of matrix 2}
\ShowEq{CR and RC quasideterminants, 1}
Пользуясь теоремой
\refTheorem{transpose inverse}{cr},
мы получим
\ShowEq{CR and RC quasideterminants, 2}
Пользуясь \EqRef{transpose of matrix, 1}, мы имеем
\ShowEq{CR and RC quasideterminants, 3}
Пользуясь \EqRef{CR and RC quasideterminants, 3},
\eqRef{j i quasideterminant =}{cr},
мы получим
\EqRef{CR and RC quasideterminants}.
\end{proof}

Теорема \RefTheorem{two quasideterminants} расширяет
принцип двойственности, теорема \RefTheorem{duality principle for biring of matrices},
на утверждения о квазидетерминантах и
утверждает, что одно и тоже выражение является \RC квазидетерминантом
матрицы $a$ и \CR квазидетерминантом матрицы $a^T$.

\begin{ShadedTheorem}{\bf принцип двойственности.}
\labelTheorem{duality principle, quasideterminants}
Пусть $\mathfrak{A}$ - истинное утверждение о бикольце матриц.
Если мы одновременно заменим
\begin{itemize}
\item строку и столбец
\item \RC квазидетерминант и \CR квазидетерминант
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}

\section{Тип векторного пространства}
\labelSection{vector space type}

\subsection{Левое \texorpdfstring{$A$}{A}-векторное пространство столбцов}

\ShowEq{def AVector}
\ShowEq{def left}
\ShowEq{\DefCol}
\ShowText{Vector Space Type}

\subsection{Левое \texorpdfstring{$A$}{A}-векторное пространство строк}

\ShowEq{\DefRow}
\ShowText{Vector Space Type}

\subsection{Правое \texorpdfstring{$A$}{A}-векторное пространство столбцов}

\ShowEq{def right}
\ShowEq{\DefCol}
\ShowText{Vector Space Type}

\subsection{Правое \texorpdfstring{$A$}{A}-векторное пространство строк}

\ShowEq{\DefRow}
\ShowText{Vector Space Type}

